Understanding and Improving the Latency of DRAM-Based Memory Systems

Over the past two decades, the storage capacity and access bandwidth of main memory have improved tremendously, by 128x and 20x, respectively. These improvements are mainly due to the continuous technology scaling of DRAM (dynamic random-access memory), which has been used as the physical substrate for main memory. In stark contrast with capacity and bandwidth, DRAM latency has remained almost constant, reducing by only 1.3x in the same time frame. Therefore, long DRAM latency continues to be a critical performance bottleneck in modern systems. Increasing core counts, and the emergence of increasingly more data-intensive and latency-critical applications further stress the importance of providing low-latency memory access. In this dissertation, we identify three main problems that contribute significantly to long latency of DRAM accesses. To address these problems, we present a series of new techniques. Our new techniques significantly improve both system performance and energy efficiency. We also examine the critical relationship between supply voltage and latency in modern DRAM chips and develop new mechanisms that exploit this voltage-latency trade-off to improve energy efficiency. The key conclusion of this dissertation is that augmenting DRAM architecture with simple and low-cost features, and developing a better understanding of manufactured DRAM chips together lead to significant memory latency reduction as well as energy efficiency improvement. We hope and believe that the proposed architectural techniques and the detailed experimental data and observations on real commodity DRAM chips presented in this dissertation will enable development of other new mechanisms to improve the performance, energy efficiency, or reliability of future memory systems.

==> macros_voltron.tex <==
\usepackage{ifthen}
\usepackage{calc}
\usepackage{pifont}
\usepackage{color}
\usepackage{fancyhdr}
\usepackage{tikz}
%\usepackage{gnuplot-lua-tikz}
%\usepackage[font={small,bf}]{caption}
%\usepackage{subcaption}
\usepackage{anyfontsize}

\newcounter{hours}
\newcounter{minutes}
\newcommand{\printtime}{%
  \setcounter{hours}{\time/60}%
  \setcounter{minutes}{\time-\value{hours}*60}%
  \thehours:\theminutes}

%\DeclareMathSizes{5}{9}{5}{5}
\newcommand{\bl}[0]{{\small{$BL$}}\xspace}
\newcommand{\blbar}[0]{{\small{$\overline{BL}$}}\xspace}
%\newcommand{\vdd}[0]{{\small{$V_{dd}$}}\xspace}
%\newcommand{\vdd}[0]{{$V_{dd}$}\xspace}
%\newcommand{\vddhalf}[0]{$V_{dd}/2$\xspace}

\newcommand{\squishlist} {
    \begin{list}{$\bullet$} {
        \setlength{\itemsep}{-2pt}
            \setlength{\parsep}{2pt}
            \setlength{\topsep}{0pt}
            \setlength{\partopsep}{0pt}
            \setlength{\leftmargin}{1.0em}
            \setlength{\labelwidth}{1em}
            \setlength{\labelsep}{0.5em}
    }
}
\newcommand{\squishend} {
    \end{list}
}


%%%%%%%%%%
% Alias
%%%%%%%%%%
% Set timeofmake to 'true' to print the time the file was compiled
\newboolean{timeofmake}
\setboolean{timeofmake}{false}

\newcommand{\ignore}[1]{}
\newcommand{\unread}[1]{{\color{red}UnreadableComment: \textbf{#1}}\xspace}
\newcommand{\highlight}[1]{{\color{blue}#1}\xspace}
\newcommand{\todo}[1]{{\color{red}TODO: \textbf{#1}}\xspace}
\newcommand{\dhl}[1]{{\color{blue} \textbf{Donghyuk: #1}}\xspace}
%\newcommand{\dhlfix}[1]{{\color{blue}#1}\xspace}
\newcommand{\kevin}[1]{{\color{brown} \textbf{#1}}\xspace}
\newcommand{\sg}[1]{{\color{orange} \textbf{Saugata: #1}}\xspace}
%\newcommand{\changes}[1]{\xspace{\color{blue}#1}\xspace}
\newcommand{\changes}[1]{#1}
\newcommand{\dhlfix}[1]{#1}

\newcommand{\refsec}[1]{\S\ref{sec:#1}}

\newcommand{\voltron}[0]{{Voltron}\xspace}
\newcommand{\memdvfs}[0]{{MemDVFS}\xspace}

\newcommand{\refab}[0]{{\small{$REF_{ab}$}}\xspace}
\newcommand{\refpb}[0]{{\small{$REF_{pb}$}}\xspace}
\newcommand{\trefi}[0]{{\small{$tREFI_{ab}$}}\xspace}
\newcommand{\trefipb}[0]{{\small{$tREFI_{pb}$}}\xspace}
\newcommand{\trfc}[0]{{\small{$tRFC_{ab}$}}\xspace}
\newcommand{\trfcpb}[0]{{\small{$tRFC_{pb}$}}\xspace}
\newcommand{\trc}[0]{{\small{tRC}}\xspace}
\newcommand{\tras}[0]{{{tRAS}}\xspace}
\newcommand{\trp}[0]{{tRP}\xspace}
\newcommand{\trrd}[0]{{\small{tRRD}}\xspace}
\newcommand{\tfaw}[0]{{\small{tFAW}}\xspace}
\newcommand{\fgr}[0]{{\small{FGR}}\xspace}
\newcommand{\trcd}[0]{{{tRCD}}\xspace}
\newcommand{\tcl}[0]{{\small{tCL}}\xspace}
\newcommand{\tcwl}[0]{{\small{tCWL}}\xspace}
\newcommand{\tccd}[0]{{\small{tCCD}}\xspace}
\newcommand{\trtw}[0]{{\small{tRTW}}\xspace}
\newcommand{\twr}[0]{{\small{tWR}}\xspace}
\newcommand{\tbl}[0]{{\small{tBL}}\xspace}

\newcommand{\trcdmin}[0]{$tRCD_{min}$\xspace}
\newcommand{\trpmin}[0]{$tRP_{min}$\xspace}

\newcommand{\src}[0]{\texttt{\small{src}}\xspace}
\newcommand{\dst}[0]{\texttt{\small{dst}}\xspace}
\newcommand{\dsttwo}[0]{\texttt{\small{dst2}}\xspace}
\newcommand{\act}[0]{\texttt{\small{ACTIVATE}}\xspace}
\newcommand{\acts}[0]{\texttt{\small{ACTIVATEs}}\xspace}
\newcommand{\crd}[0]{\texttt{\small{READ}}\xspace}
\newcommand{\cwr}[0]{\texttt{\small{WRITE}}\xspace}
\newcommand{\pre}[0]{\texttt{\small{PRECHARGE}}\xspace}

\newcommand{\putsec}[2]{\vspace{-0.05in}\section{#2}\label{sec:#1}\vspace{-0.075in}}
\newcommand{\putssec}[2]{\vspace{-0.05in}\subsection{#2}\label{ssec:#1}\vspace{-0.075in}}
\newcommand{\putsssec}[2]{\vspace{0.05in}\subsubsection{#2}\label{sssec:#1}\vspace{0.075in}}
\newcommand{\putsssecX}[1]{\vspace{0.0in}\subsubsection*{#1}\vspace{0.0in}}

% Black-background circled text
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.8pt,fill=white,text=black] (char) {#1};}}

\newcommand{\figput}[4][1.0\linewidth]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#3, clip, width=#1]{plots/#2}
\end{center}
\caption{#4 \label{fig:#2}}
\end{minipage}
\end{figure}
}

\newcommand{\figputW}[2]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[clip,width=\linewidth]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputWL}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[clip,width=\linewidth]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#2 \label{fig:#3}}
\end{minipage}
\end{figure*}
}
\newcommand{\figputWS}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputH}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth, height=#2]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHW}[2]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/#1}
\end{center}
%\vspace{-0.15in}
\vspace{-0.2in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHWL}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#3}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHWHeight}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth, height=#3in]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}


\newcommand{\figputGHWHeight}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth,height=#3in]{plots/gnuplots/#1}%
\end{center}
\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGHW}[2]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGTW}[2]{
\begin{figure}[!t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/gnuplots/#1}
\end{center}
\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}


\newcommand{\figputHS}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGHS}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}
\newcommand{\figputGTS}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGTWS}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputTS}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputT}[2]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[clip, width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputTT}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#2, clip, width=1.0\linewidth]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputPlaceHolder}[2]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=0.8, width=1.0\linewidth]{plots/PlaceHolder}
\end{center}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

%\renewcommand{\figurename}{\renewcommand{\baselinestretch}{1.0}\vspace{-0.0in}\footnotesize\sf\bfseries Figure}
%\renewcommand{\tablename}{\renewcommand{\baselinestretch}{1.0}\vspace{-0.0in}\footnotesize\sf\bfseries Table}

\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\eq}[1]{Table~\ref{tab:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\ssecref}[1]{Section~\ref{ssec:#1}}
\newcommand{\sssecref}[1]{Section~\ref{sssec:#1}}
\newcommand{\paratitle}[1]{\textbf{#1.}\xspace}

\newcommand{\module}[3]{{{\textit #1}$_{\mathrm{#2}}^{\mathrm{#3}}$}\xspace}
\newcommand{\moduledate}[3]{{{\hel #1}$_{\mathrm{#2}}^{\mathrm{#3}}$}\xspace}


==> plots/dram_fig.tex <==
\begin{figure*}[t]
    \centering
    \subfloat[DRAM bank organization.]{
        \begin{minipage}{\linewidth/2}
        \begin{center}
        \label{fig:bank}
        \includegraphics[scale=0.90]{plots/bank_org}
        \end{center}
        \end{minipage}
    }
    \subfloat[Open bitline subarray architecture.]{
        \begin{minipage}{\linewidth/2}
        \begin{center}
        \label{fig:subarray}
        \includegraphics[scale=0.90]{plots/open_bitline_sa}
        \end{center}
        \end{minipage}
    }
    \caption{DRAM bank and subarray organization.}
    \label{fig:dram_background}
\end{figure*}


==> plots/main-scurves.tex <==
\begin{figure*}[t]
        \centering
        \subfloat[8Gb.]{
            \begin{minipage}{0.325\textwidth}
            \begin{center}
            \includegraphics[width=\textwidth]{plots/scurve_8gb}
            \vspace{-0.1in}
            \label{fig:8Gb-scurve}
            \end{center}
            \end{minipage}
        }
        %
        \subfloat[16Gb.]{
            \begin{minipage}{0.325\textwidth}
            \begin{center}
            \includegraphics[width=\textwidth]{plots/scurve_16gb}
            \vspace{-0.1in}
            \label{fig:16Gb-scurve}
            \end{center}
            \end{minipage}
        }
        %
        \subfloat[32Gb.]{
            \begin{minipage}{0.325\textwidth}
            \begin{center}
            \includegraphics[width=\textwidth]{plots/scurve_32gb}
            \vspace{-0.1in}
            \label{fig:32Gb-scurve}
            \end{center}
            \end{minipage}
        }
        %

        \caption{Multi-core system performance improvement over baseline
        all-bank refresh using various DRAM density.}\label{fig:scurves}
\end{figure*}

% Vertically stacked
%\begin{figure}[t]
%    \begin{tabular}{c}
%        \subfloat[8Gb.]{
%            \begin{minipage}{\linewidth}
%            \begin{center}
%            \includegraphics[scale=0.8]{plots/scurve_8gb}
%            \label{fig:8Gb-scurve}
%            \end{center}
%            \end{minipage}
%        } \\
%
%        \subfloat[16Gb.]{
%            \begin{minipage}{\linewidth}
%            \begin{center}
%            \includegraphics[scale=0.8]{plots/scurve_16gb}
%            \label{fig:16Gb-scurve}
%            \end{center}
%            \end{minipage}
%        } \\
%
%        \subfloat[32Gb.]{
%            \begin{minipage}{\linewidth}
%            \begin{center}
%            \includegraphics[scale=0.8]{plots/scurve_32gb}
%            \label{fig:32Gb-scurve}
%            \end{center}
%            \end{minipage}
%        } \\
%
%    \end{tabular}
%
%    \caption{Multi-core system performance improvement over baseline
%    all-bank refresh using various DRAM density.}
%    \label{fig:scurves}
%\end{figure}


==> plots/memory-organization.tex <==
%\begin{figure}[h]
%  \centering
%
%  \subfigure[DRAM Memory System Organization.]{
%  \label{fig:dram-organization}
%  \includegraphics[width=\linewidth]{figures/dram-organization}
%  }
%  \subfigure[]{
%  \label{fig:bank-subarray}
%  \includegraphics[width=0.85\linewidth]{figures/bank-organization}
%  }
%
%  \caption{A DRAM bank consists of tiles and subarrays.}
%  \label{fig:bank-organization}
%\end{figure}


==> sec/latvar/abstract_short.tex <==
% !TEX root=../paper.tex

Long DRAM latency is a critical performance bottleneck in current
systems.  DRAM access latency is defined by three fundamental
operations that take place within the DRAM cell array: {\em
(i)}~\emph{activation} of a memory row, which opens the row to perform
accesses; {\em (ii)}~\emph{precharge}, which prepares the cell array
for the next memory access; and {\em (iii)}~\emph{restoration} of the
row, which restores the values of cells in the row that were destroyed
due to activation.  There is significant latency variation for each of
these operations across the cells of a single DRAM chip due to
irregularity in the manufacturing process.  As a result, some cells
are \emph{inherently} faster to access, while others are inherently
slower. Unfortunately, existing systems do not exploit this variation.

The goal of this work is to {\em (i)}~experimentally characterize and
understand the latency variation across cells within a DRAM chip for
these three fundamental DRAM operations, and {\em (ii)}~develop new
mechanisms that exploit our understanding of the latency variation to
reliably improve performance.  To this end, we comprehensively
characterize 240 DRAM chips from three major vendors, and make several
new observations about latency variation within DRAM.  We find that
{\em (i)}~there is large latency variation across the cells for each
of the three operations; {\em (ii)}~variation characteristics exhibit
significant spatial locality: slower cells are clustered in certain
regions of a DRAM chip; and {\em (iii)}~the three fundamental
operations exhibit different reliability characteristics when the
latency of each operation is reduced.

Based on our observations, we propose \mechlong (\mech), a mechanism that
exploits latency variation across DRAM cells within a DRAM chip to improve
system performance.  The key idea of \mech is to exploit the spatial locality of
slower cells within DRAM, and access the faster DRAM regions with reduced
latencies for the fundamental operations. Our evaluations show that \mech
improves the performance of a wide range of applications by 13.3\%, 17.6\%, and
19.5\%, on average, for each of the three different vendors' real DRAM chips, in
a \new{simulated} 8-core system. We conclude that the experimental
characterization and \new{analysis} of latency variation within modern DRAM,
provided by this work, can lead to new techniques that improve DRAM and system
performance.


==> sec/latvar/ack.tex <==
\section*{ACKNOWLEDGMENTS}

We thank our shepherd Christopher Stewart, anonymous reviewers, and
SAFARI group members for feedback. We acknowledge the support of
Google, Intel, Nvidia, and Samsung. This research was supported in
part by the ISTC-CC, SRC, and NSF (grants 1212962 and 1320531). Kevin
Chang is supported in part by the SRCEA/Intel Fellowship.


==> sec/latvar/background.tex <==
\section{Background \& Motivation}

In this section, we first provide necessary background on DRAM organization and
operation to enable a better understanding of the major DRAM timing parameters
we will characterize.  Then, we discuss how we can exploit DRAM variation to
reduce the DRAM access latency.

%modules and their internal organization in order to understand the timing
%parameters.

\subsection{High-Level DRAM System Organization}
\label{sec:dram_sys_back}

A modern DRAM system consists of a hierarchy of channels, modules, ranks, and
chips, as shown in Figure~\ref{dram-organization}. Each \emph{memory channel}
drives DRAM commands, addresses, and data between a memory controller in the
processor and one or more DRAM modules. Each \emph{module} contains multiple
DRAM chips that are divided into one or more ranks. A \emph{rank} refers to a
group of chips that operate in lock step to provide a wide data bus (usually
64 bits), as a single DRAM chip is designed to have a narrow data bus width
(usually 8 bits) to minimize chip cost. Each of the eight chips in the rank
shown in Figure~\ref{dram-organization} transfers 8 bits simultaneously to
supply 64 bits of data.

\input{sec/subplots/memory}

\subsection{Internal DRAM Organization}

Within a DRAM chip, there are multiple banks (e.g., eight in a typical DRAM
chip~\cite{jedec-ddr3}) that can process DRAM commands independently from each
other to increase parallelism. A \emph{bank} consists of a 2D-array of DRAM
cells that are organized into rows and columns, as shown in
Figure~\ref{bank-organization}.  A row typically consists of 8K cells. The
number of rows varies depending on the chip density. Each DRAM cell has {\em
(i)} a \emph{capacitor} that stores binary data in the form of electrical charge
(i.e., fully charged and discharged states represent \texttt{1} and \texttt{0},
respectively), and {\em (ii)} an \emph{access transistor} that serves as a
switch to connect the capacitor to the \emph{bitline}. Each column of cells
share a bitline, which connects them to a \emph{sense amplifier}.  The sense
amplifier senses the charge stored in a cell, converts the charge to digital
binary data, and buffers it. Each row of cells share a wire called the
\emph{wordline}, which controls the cells' access transistors. When a row's
wordline is enabled, the entire row of cells gets connected to the row of sense
amplifiers through the bitlines, enabling the sense amplifiers to sense and
latch that row's data. The row of sense amplifiers is also called the \emph{row
buffer}.

\subsection{Accessing DRAM}
\label{sec:dram_access}

Accessing (i.e., reading from or writing to) a bank consists of three steps:
{\em (i)} {\bf Row Activation \& Sense Amplification}: opening a row to transfer
its data to the row buffer, {\em (ii)} {\bf Read/Write}: accessing the target
\new{column} in the row buffer, and {\em (iii)} {\bf Precharge}: closing the row
and the row buffer. We use Figure~\ref{fig:timing_standard} to explain these
three steps in detail. The top part of the figure shows the phase of the cells
within the row that is being accessed. The bottom part shows both the DRAM
command and data bus timelines, and demonstrates the associated timing
parameters.

%\\ \vspace{-2mm}

\input{sec/subplots/timing_standard}

%\todo{Fix the organization}.

\noindent{\bf Initial State.} Initially, the bank remains in the
\emph{precharged} state (\circled{4} in Figure~\ref{fig:timing_standard}), where
all of the components are ready for activation. All cells are fully charged,
represented with the dark grey color (a darker cell color indicates more
charge). Second, the bitlines are charged to \halfvdd, represented as a thin
line (a thin bitline indicates the initial voltage state of \halfvdd; a thick
bitline means the \new{bitline} is being driven). Third, the wordline is disabled
with \zerov (a thin wordline indicates \zerov; a thick wordline indicates \vdd).
Fourth, the sense amplifier is {\em off} without any data latched in it
(indicated by lighter color in the sense amplifier).\\\vspace{-2mm}

\noindent{\bf Row Activation \& Sense Amplification Phases.} To open a row, the
memory controller sends an \act command to raise the wordline of the
corresponding row, which connects the row to the bitlines (\circled{1}).
%This triggers a phase called \emph{charge sharing} (State \circled{1}).
This triggers an \emph{activation}, where charge starts to flow from the cell to
the bitline (or the other way around, depending on the initial charge level in
the cell) via a process called \emph{charge sharing}. This process perturbs the
voltage level on the corresponding bitline by a small amount. If the cell is
initially charged (which we assume for the rest of this explanation, without
loss of generality), the bitline voltage is perturbed upwards.
%($\delta$) perturbing the bitline's voltage to \halfdelta.
Note that this causes the cell itself to discharge, losing its data temporarily
(hence \new{the lighter color of the accessed row}), but this charge will be
restored as we will describe below. After the activation phase, the sense
amplifier \emph{senses} the voltage perturbation on the bitline, and turns
\emph{on} to further \emph{amplify} the voltage level on the bitline by
injecting more charge into the bitline and the cell (\new{making the activated
    row darker in \circled{2}}). When the bitline is amplified to a certain
    voltage level (e.g., $0.8V_{DD}$), the sense amplifier latches in the cell's
    data, which transforms it into binary data (\circled{2}). At this point in
    time, the data can be read from the sense amplifier. The latency of these
    two phases (activation and sense amplification) is called the
    \emph{activation latency}, and is defined as \textbf{\small tRCD} in the
    standard DDR interface~\cite{jedec-ddr3,jedec-ddr4}. This activation latency
    specifies the latency from the time an \act command is issued to the time
    the data is ready to be accessed in the sense amplifier.\\ \vspace{-2mm}

\noindent{\bf Read/Write \& Restoration Phases.} Once the sense amplifier (row
buffer) latches in the data, the memory controller can send a \crd or \cwr
command to access the corresponding column of data within the row buffer (called
a \emph{column access}). The column access time to read the cache line data is
called \textbf{\small tCL} (\textbf{\small tCWL} for writes). These parameters
define the time between the column command and the appearance of the \emph{first
beat of data} on the data bus, shown at the bottom of
Figure~\ref{fig:timing_standard}. A \emph{data beat} is a 64-bit data transfer
from the DRAM to the processor.
%that combines 8-bit of data read from the same bank of every chip within a rank
%to form 64 bits of data.
In a typical DRAM~\cite{jedec-ddr3}, a column \crd command reads out 8 data
beats (also called an 8-beat burst), thus reading a complete 64-byte cache line.

%A \emph{data beat} is a
%data transfer that combines 8-bit of data read from the same bank of every chip
%within a rank to form 64 bits of data. In a typical DRAM~\cite{jedec-ddr3}, a
%column \crd command reads out 8 data beats (also called an 8-beat burst), thus
%reading a complete 64-byte cache line.

After the bank becomes activated and the sense amplifier latches in the binary
data of a cell, it starts to \emph{restore} the connected cell's charge back to
its original fully-charged state (\circled{3}). This phase is known as
\emph{restoration}, and can happen in parallel with column accesses. The
restoration latency (from issuing an \act command to fully restoring a row of
cells) is defined as \textbf{\small tRAS}, as shown in Figure~\ref{fig:timing_standard}.\\
\vspace{-2mm}

\noindent{\bf Precharge Phase.} In order to access data from a different row,
the bank needs to be re-initialized back to the precharged state (\circled{4}).
To achieve this, the memory controller sends a \cpre command, which {\em (i)}
disables the wordline of the corresponding row, disconnecting the row from the
sense amplifiers, and {\em (ii)} resets the voltage level on the bitline back to
the initialized state, \halfvdd, so that the sense amplifier can sense the
charge from the \new{newly} opened row. The latency of a precharge operation is defined
as \textbf{\small tRP}, which is the latency between a \cpre and a subsequent \act within the
same bank.

\noindent\textbf{Summary.} As shown at the bottom of \figref{timing_standard},
the latency of back-to-back \new{accesses} to different rows in DRAM is decided by
\tras + \trp (restoration latency + precharge latency). The latency of accessing
data from a row is decided by \trcd (activation latency), and is then followed
by \tcl and the data transfer latency (both of which are independent of the
activation/restoration/precharge operations). In this work, we focus on the
three critical timing parameters: \trcd, \trp, and \tras.
%Note that we cannot change \tcl and the data transfer latency using our
%infrastructure.

%less prominent and depend on the data bus
%frequency that is external to DRAM. In this work, we will focus on the
%three critical timing parameters that are internal to DRAM: \trcd,
%\trp, and \tras.


%transfer latency, which are less prominent and depend on the data bus
%frequency that is external to DRAM. In this work, we will focus on the
%three critical timing parameters that are internal to DRAM: \trcd,
%\trp, and \tras.

% After the bitline is fully amplified to \vdd, which happens in parallel while
% the column command is being processed, the sense amplifier starts to
% \emph{restore} the connected cell's charge back to its original fully charged
% state (State \circled{4}). This phase is known as \emph{restoration}. The
% time it takes to restore a row of cells since the \act command is defined as
% \tras, shown in \figref{back_timeline}.

%\input{sec/subplots/timing_reduced}



==> sec/latvar/conclusion.tex <==
\section{Conclusion}

This paper provides the first experimental study that comprehensively
characterizes and analyzes the latency variation within modern DRAM chips for
three fundamental DRAM operations (activation, precharge, and restoration).  We
find that significant latency variation is present across DRAM cells in all 240
of our tested DRAM chips, and that a large fraction of cache lines can be read
reliably even if the activation/restoration/precharge latencies are reduced
significantly. Consequently, exploiting the latency variation in DRAM cells can
greatly reduce the DRAM access latency.
%%We observe that there
%%is a locality in slower cells, clustered in certain regions of a DRAM
%%chip, that can be exploited to develop low-cost mechanisms to
%%reduce latency, where fast regions have lower access latency.
%%
Based on the findings from our experimental characterization, we propose and
evaluate a new mechanism, \mech (\mechlong), which reduces DRAM latency by
exploiting the inherent latency variation in DRAM cells.  \mech reduces DRAM
latency by categorizing the DRAM cells into fast and slow regions, and accessing
the fast regions with a reduced latency.  We demonstrate that \mech can greatly
reduce DRAM latency, leading to significant system performance
\newt{improvements} on a variety of workloads.

We conclude that it is promising to understand and exploit the inherent latency
variation within modern DRAM chips. We hope that the experimental
characterization, analysis, and optimization techniques presented in this paper
will enable the development of other new mechanisms that exploit the latency
variation within DRAM to improve system performance and perhaps reliability.

%
% the
%latency variation in three major DRAM operations
%What
%why
%how
%potential apps
%limitations (couldn't do it on a computer system with memtest)
%Possible avenue for future research
%
%The present study raises the possibility that a link may existing between soft
%errors and timing errors.
%


==> sec/latvar/exp_meth.tex <==
\section{Experimental Methodology}
\label{sec:exp_meth}

To study the effect of using different timing parameters on modern DDR3 DRAM
chips, we developed a DRAM testing platform that allows us to precisely control
the value of timing parameters and the tested DRAM location (i.e., banks, rows,
and columns) within a module. The testing platform, shown in
\figref{dram_fpga_white}, consists of Xilinx FPGA boards~\cite{xilinx-ml605}
and host PCs. We use the RIFFA~\cite{jacobsen-rts2015} framework to communicate
data over the PCIe bus from our customized \emph{testing software} running on
the host PC to our customized \emph{test engine} on the FPGA. Each DRAM module
is tested on an FPGA board, and is located inside a heat chamber that is
connected to a temperature controller. Unless otherwise specified, we test
modules at an ambient temperature of 20$\pm$1\celsius. \new{We examine various
    temperatures in Section~\ref{sec:rcd_temp}.}

%\figputHSTrim{dram_fpga_blue}{0.34}{FPGA-based DRAM testing infrastructure.}{1in 0 0 1}
\figputHS{dram_fpga_white}{0.28}{FPGA-based DRAM testing infrastructure.}
\vspace{-5pt}


\subsection{DRAM Test}

To achieve the goal of controlling timing parameters, our FPGA test engine
supports a list of DRAM commands that get processed directly by the memory
controller on the FPGA. Then, on the host PC, we can write a \emph{test} that
specifies a sequence of DRAM commands along with the delay between the commands
(i.e., timing parameters).  The test sends the commands and delays from the
host PC to the FPGA test engine.

Test~\ref{readcl} shows the pseudocode of a test that reads a cache line from a
particular bank, row, and column with timing parameters that can be specified by
the user. The test first sends an \act to the target row (line 2). After a
\trcd delay that we specify (line 3), it sends a \crd (line 4) to the target
cache line. Our test engine enables us to specify the exact delay between two
DRAM commands, thus allowing us to tune certain timing parameters. The read
delay (\tcl) and data transfer latency (\newthree{\tbl}) are two DRAM internal
timings that cannot be changed using our infrastructure. After our test
waits for the data to be fully transferred (line 5), we precharge the bank (line 6) with our
specified \trp (line 7). We describe the details of the tests that we created
to characterize latency variation of \trcd, \trp, and \tras in the next few
sections.

% Test~\ref{readcl} shows the pseudocode of a test that reads a cache line from a
% particular bank, row, and column with timing parameters that can be specified by
% the user. Our test engine enables us to specify the exact delay between two DRAM
% commands, thus allowing us to tune the timing parameters, such as \trcd and
% \trp. Note that the read delay (\tcl) and data transfer latency cannot be
% changed using our infrastructure.
% %is a DRAM internal timing that we cannot tune using our test.
% Thus, our test needs to properly wait for the data to be fully read and
% transferred with latency defined in the standard before it can perform other
% commands (e.g., \cpre). We will describe the details of our tests that we used
% to characterize latency variation of \trcd, \trp, and \tras in the next few
% Sections.

\input{sec/algos/readcl}

%%
\ignore{
\subsection{Tested Timing Parameters}

Although we have discussed four timing parameters, in this work, we present our
study on the following three timing parameters: 1) \trcd the activation latency,
2) \trp the precharge latency, and 3) \tras the restoration latency. The reason
we didn't examine \tcl is that it is a DRAM internal timing that is not
controlled by the memory controller. It does not define the latency between two
DRAM commands, but the time for the data to be read/written for a column
\crd/\cwr command. As a result, we cannot control \tcl for every memory request
at the memory controller.
}
%%

\subsection{Characterized DRAM Modules}

We \new{characterize} latency variation on a total of 30 DDR3 DRAM modules,
comprising 240 DRAM chips, from the three major DRAM vendors that hold more than
90\% of the market share~\cite{bauer-mckinsey2016}. \tabref{dimm_list_latvar} lists the
\new{relevant} information about the tested DRAM modules. All of these modules are
\emph{dual in-line} (i.e., 64-bit data bus) with a single rank of DRAM chips.
Therefore, we use the terms \emph{DIMM} (dual in-line memory module) and module
interchangeably. In the rest of the paper, we refer to a specific DIMM using the
label \dimm{n}{v}, where $n$ and $v$ stand for the DIMM number and vendor,
respectively. In the table, we group the DIMMs based on their model number,
which provides certain information on the process technology and array design
used in the chips.

% We will later in \secref{scaling} show characterization
% results on chips manufactured in 2010 and 2015 to study the effect of process
% technology scaling.

\input{sec/tables/dimm_table}
%\vspace{-10pt}


==> sec/latvar/exp_results_tras.tex <==
\section{Restoration Latency Analysis} \label{sec:ras_lat_analysis}

In this section, we present \newt{a} methodology and findings on varying the
restoration latency, defined \newt{by} the \tras timing parameter. First, we
elaborate on the impact of reducing \tras on performance and reliability in
\secref{tras_effect}. Then, we explain our FPGA test conducted to characterize
\tras variation, and present our observations.

\subsection{Impact of Reduced tRAS} \label{sec:tras_effect}

As mentioned in Section~\ref{sec:dram_access}, \tras specifies the minimum
amount of time between issuing an \act and a \cpre command to a bank. By
reducing \tras, we can complete an access to one row faster, and quickly switch
to \newt{access} the next row. From the perspective of {\em reliability}, reducing
the restoration latency may potentially induce errors in the cells due to having
insufficient time to restore the lost charge back to the cells. When a row of
cells is activated, the cells temporarily lose their charge to the bitlines, so
that the sense amplifiers can sense the charge. During the restoration phase,
the sense amplifiers restore charge back into the cells, bringing them back
to the fully-charged state. By reducing the restoration latency, the amount of
restored charge reduces, and the cells may not reach the fully-charged state. As
a result, a subsequent access to the same row may not able to sense the correct
value, \newt{thereby leading to} errors.

\subsection{Test Methodology and Results} \label{sec:tras_tests_results}

To characterize the variation in restoration latency (\tras), we consider
another important factor that affects the amount of charge stored in DRAM cells,
which is \emph{leakage}. DRAM cells lose charge over time, thus requiring a
periodic {\em refresh} operation to restore the charge. \newt{Reducing} the
restored charge in the cells can cause them to lose too much charge before the
next refresh, generating an error.

To perform a conservative characterization, we integrate this leakage factor
into our test methodology. We access each row by issuing a pair of commands,
\act and \cpre, with a specific \tras value between these two commands. Then, we
wait for a full refresh period (defined as 64ms in the DRAM
standard~\cite{jedec-ddr3, jedec-ddr4}) before we access the row again to verify
\newt{the correctness of its data}. We test this sequence on a representative
set of DIMMs from all three DRAM vendors and we use four data patterns:
\texttt{0x00}, \texttt{0xff}, \texttt{0xaa}, and \texttt{0xcc}.

In our previously described tests on activation and precharge variation, we test
every time step from the default timing value to a minimum value of 2.5ns, with
a reduction of 2.5ns per step. Instead of reducing \tras all the way down to
2.5ns from its standard value of 35ns, we lower it until \newthree{$t\textsc{ras}_{min}=
\trcd + \tcl + \tbl$}, which is the latency of activating a row and
reading a cache line from it. In a typical situation where the memory controller
reads or writes a piece of data after opening a row, lowering \tras below
$t\textsc{ras}_{min}$ means that the memory controller can issue a \cpre while
the data is still being read or written. Doing so risks terminating \crd or \cwr
operations prematurely, causing unknown behavior.

In order to test \tras with a reasonable range of values, we iterate \tras from
35ns to $t\textsc{ras}_{min}$. Our $t\textsc{ras}_{min}$ is calculated by using
the standard \tcle13.125ns and \newthree{\tble5ns} along with a fast \trcde5ns.
$t\textsc{ras}_{min}$ is rounded up to the nearest multiple of 2.5ns, which
is \emph{22.5ns}.

%After we issue a \cpre command early using a
%reduced \tras, we validate the data in the row until a full refresh period of
%64ms (as specified in the standard~\cite{jedec-ddr3}) has elapsed.

We do not observe errors across the range of \tras values we tested \newt{in any
of our experiments}. This implies that charge restoration in modern DRAMs
completes within the duration of an activation and a read. Therefore, \tras can
be reduced aggressively without affecting data integrity.

% To test the latency variation in restoration time (\tras), we issue a pair of
% commands \act and \cpre to each row, and reduce the latency (i.e., \tras)
% between these two commands.
% %need to \act and \crd from a row, and issue a \cpre command early -- to reduce
% %\tras.
% The impact of reduced \tras is observed by reading and validating the contents
% of the row after waiting for its refresh period (i.e., 64ms in the DRAM
% standards~\cite{jedec-ddr3, jedec-ddr4}). This sequence ensures we are covering
% the worst case scenario as described in Section~\ref{sec:tras_effect}.
%
% We test the above sequence on a representative set of DIMMs from all three DRAM
% vendors and their corresponding models. Four data patterns were used --
% \texttt{0x00, 0xff, 0xaa,} and \texttt{0xcc}. To calculate the range of \tras,
% we use the timing parameters of \tcl=13.125ns and \texttt{tDATA}=5ns based on
% the standards for our DIMMs~\cite{jedec-ddr3}. However, we assume \trcd=5ns to
% accommodate faster reads as described in Section~\ref{sec:trcd_errors}. The
% default \tras value is specified as 35ns (\tabref{dimm_list_latvar}), while the
% minimum \tras computed from these parameters is 23.125ns. Thus we vary \tras
% from 35ns to 22.5ns in steps of 2.5ns. After we issue a \cpre command early
% using a reduced \tras, we validate the data in the row until a full refresh
% period of 64ms (as specified in the standard~\cite{jedec-ddr3}) has elapsed.
%
% In all our experiments, we do not observe errors across the range of \tras
% values we tested. This implies that charge restoration in modern DRAMs happen
% within the read duration, and \tras can be reduced aggressively without
% affecting data integrity.

\obs{Modern DIMMs have sufficient timing margin to complete charge
restoration within the period of an \act and a \crd. Hence, \tras can be
reduced without introducing any errors.}

%	DRAM DIMMs have sufficient timing margins to complete charge restoration
%	within the period of a \crd, and hence \tras can be reduced without
%	introducing any errors.



==> sec/latvar/exp_results_trcd.tex <==
\section{Activation Latency Analysis}
\label{sec:act_lat_analysis}

% Describe what we are going to talk about here.
In this section, we present our methodology and results on varying the
activation latency, which is expressed by the \trcd timing
parameter. We first describe the nature of errors caused by \trcd
reduction in Section~\ref{sec:trcd_errors}. Then, we describe the FPGA
test we conducted on the DRAM modules to characterize \trcd variation in
Section~\ref{sec:trcd_tests}.  The remaining sections describe
different major observations we make based on our results.

\subsection{Behavior of Activation Errors}
\label{sec:trcd_errors}

As we discuss in Section~\ref{sec:dram_access}, \trcd is defined as the minimum
amount of time between the \act and the first column command (\crd/\cwr).
Essentially, \trcd represents the time it takes for a row of sense amplifiers
(i.e., the row buffer) to sense and latch a row of data. By employing a lower
\trcd value, a column \crd command may potentially read data from sense
amplifiers that are still in the \emph{sensing and amplification} phase, during
which the data has not been fully latched into the sense amplifiers. As a
result, reading data with a lowered \trcd can induce timing errors (i.e.,
flipped bits) in the data.

To further understand the nature of activation errors, we perform experiments to
answer two fundamental questions: \romnum{i}~Does lowering \trcd incur errors on
\new{\emph{all}} cache lines read from a sequence of \crd commands on an opened row?
\romnum{ii}~Do the errors propagate back to the DRAM cells, causing
\new{\emph{permanent}} errors for all future accesses?

\subsubsection{Errors Localized to First Column Command}
\label{sec:trcd_errors:first_col}

To answer the first question, we conduct Test~\ref{trcdlocal} that first
activates a row with a specific \trcd value, and then \new{reads} every
cache line in the entire row.
%The test is not shown due to space constraint. For readers who are interested
%in the detail of the test, we provide its pseudocode of this test,
%Test~\ref{trcdlocal}, in Appendix \ref{app_rcd_test}.
By conducting the test on every row in a number of DIMMs from all three vendors,
we make the following observation.

\input{sec/algos/trcdlocal}

\obs{Activation errors are isolated to the cache line from
the first \crd command, and do not appear in subsequently-read cache lines from
the same row.\label{obs:rcd_local}}

There are two reasons why errors do \new{\emph{not}} occur in the subsequent cache line
reads. First, a \crd accesses \new{only} its corresponding sense amplifiers, without
accessing the other columns. Hence, a \newt{\crd's effect is isolated to} its
target cache line. Second, by the time the second \crd is issued, a sufficient
amount of time has passed for the sense amplifiers to properly latch the data.
Note that this observation is independent of DIMMs and vendors as the
fundamental DRAM structure is similar across different DIMMs. We discuss
the number of activation errors due to different \trcd values for each DIMM in
\new{\secref{trcd_ber}.}

\subsubsection{Activation Errors Propagate into DRAM Cells}

To answer our second question, we run two iterations of Test~\ref{trcdlocal}
(i.e., reading a row that is activated with a specified \trcd value) on the same
row. The first iteration reads a row that is activated with a lower \trcd value,
then closes the row. The second iteration re-opens the row using the standard
\trcd value, and reads the data to confirm if the errors remain in the cells.
Our experiments show that if the first iteration observes activation errors
within a cache line, the second iteration observes the same errors. This
demonstrates that activation errors not only happen at the sense amplifiers but
also propagate back into the cells.

We hypothesize this is because reading a cache line early causes the sense
amplifiers to latch the data based on the \emph{current} bitline voltage. If the
bitline voltage has not yet fully developed into \vdd or \zerov, the sense
amplifier latches in unknown data and amplifies this data to the bitline, which
is then restored back into the cell during restoration phase.

\obs{Activation errors occur at the sense amplifiers and propagate back into the
cells. The errors persist until the data is overwritten.}

%This observation raises a few questions on the characteristics of activation
%errors in modern DRAM DIMMs.
\new{After observing that reducing activation latency results in timing errors,
    we now consider \newt{two new questions.}} First, after how much
activation latency reduction do DIMMs start observing timing errors? Second, how
many cells experience activation errors at each latency reduction step?

\subsection{FPGA Test for Activation \newt{Latency}}
\label{sec:trcd_tests}

To characterize activation errors across every cell in DIMMs, we need to perform
an \act and a \crd on one cache line at a time since activation errors only
occur in one cache line per activation. \new{To achieve this}, we use
Test~\ref{trcdtest}, \newt{whose pseudocode is below,} for every cache line within a row.

\input{sec/algos/trcdtest}

The test iterates through each cache line (lines 2-4) and performs the following
steps to test the cache line's reliability under a \new{reduced} \trcd value. First, it opens the
row that contains the target cache line, writes a specified data pattern into
the cache line, and then precharges the bank (line 5). Second, the test \new{re-opens
the row to read the cache line with the standard \trcd (line 6), and verifies if
the value was written properly (line 7).}
Then it precharges the bank again to
prepare for the next \act. Third, it re-activates the row using the reduced
\trcd value ($my\_tRCD$ in Test~\ref{trcdtest}) to read the target cache line
\new{(line 8)}. It records the number of timing errors (i.e., bit flips) out of the
64-byte (512-bit) cache line \new{(line 9)}.

%\vspace{-0.08in}

In total, we have conducted more than 7500 rounds of tests on the DIMMs shown in
\tabref{dimm_list_latvar}, accounting for at least 2500 testing hours. For each round
of tests, we conducted Test~\ref{trcdtest} with a different \trcd value and data
pattern. We tested five different \trcd values: 12.5ns, 10ns, 7.5ns, 5ns, and
2.5ns. Due to the slow clock frequency of the FPGA, we can only adjust timings
at a 2.5ns granularity. We used a set of four different data patterns:
\texttt{0x00}, \texttt{0xaa}, \texttt{0xcc}, and \texttt{0xff}. Each data
pattern represents the value that was written into each byte of the entire cache
line.

%%% Latex black magic: Figs for later sections %%%
%\subsection{Bit Error Rates}
\subsection{Activation Error Distribution}

In this section, we first present the distribution of activation errors
collected from all of the tests conducted on every DIMM. Then, we categorize the
results by DIMM model to investigate variation across models from different
vendors.

\subsubsection{Total Bit Error Rates}
\label{sec:trcd_ber}

\figref{violin} shows the box plots of the \emph{bit error rate} (BER)
observed on every DIMM as \trcd varies. The BER is defined as the fraction of
activation error bits in the total population of tested bits. For each box, the
bottom, middle, and top lines indicate the 25th, 50th, and 75th percentile of
the population. The ends of the whiskers indicate the minimum and maximum BER of
all DIMMs for a given \trcd value. Note that the y-axis is in log scale to
show low BER values. As a result, the bottom whisker at \trcde7.5ns cannot be
seen due to a minimum value of 0. In addition, we show \emph{all}
observation points for each specific \trcd value by overlaying them on top of
their corresponding box. Each point shows a BER collected from one round of
Test~\ref{trcdtest} on one DIMM with a specific data pattern and a \trcd value.
Based on these results, we make several observations.

% trcd violin
%2.5 956 Min 0.000042 Max 0.983907 Med 0.486396
%5.0 966 Min 0.000006 Max 0.520323 Med 0.117577
%7.5 966 Min 0.000000 Max 0.105552 Med 0.000341
%10.0 374 Min 0.000000 Max 0.000000 Med 0.000000
%12.5 374 Min 0.000000 Max 0.000000 Med 0.000000

\figputHW{trcd/ber/all_ber_plots/all_trcd_box_log}{violin}{Bit error
    rate \new{of all DIMMs with reduced \trcd}.}
\vspace{-5pt}
% Old violin plot
%\figputHW{trcd/ber/all_ber_plots/all_violin}{violin}{The bit error rate due to \trcd on all the DIMMs.}

First, we observe that BER exponentially increases as \trcd decreases. With a
lower \trcd, fewer sense amplifiers are expected to have enough strength to
properly sense the bitline's voltage value and latch the correct data. Second,
at \trcd values of 12.5ns and 10ns, we observe no activation errors on any DIMM.
This shows that the \trcd latency of the slowest cells in our tested DIMMs
likely falls between 7.5 and 10ns, which are lower than the standard value
(13.125ns). The manufacturers use the extra latency as \new{a \emph{guardband}} to
provide additional protection against process variation.

Third, the BER variation among DIMMs becomes smaller as \trcd value decreases.
The reliability of DIMMs operating at \trcde7.5ns varies significantly depending
on the DRAM models and vendors, \new{as we} demonstrate in the
\newt{\secref{rcd_model}}.
In fact, some DIMMs have no errors at \trcde7.5ns, which cannot be seen in the
plot due to the log scale. When \trcd reaches 2.5ns, most DIMMs become rife with
errors, with a median BER of 0.48, similar to the probability of a coin toss.

\subsubsection{Bit Error Rates by DIMM Model}
\label{sec:rcd_model}

Since the \new{performance of a DIMM can vary across different models}, vendors,
and fabrication processes, we provide a detailed analysis by breaking down the
\new{BER results by DIMM model} (listed in \tabref{dimm_list_latvar}).
\figref{rcd_ber_20c} presents the distribution of every DIMM's BER grouped by
each \new{vendor and model combination}. Each box shows the quartiles and
median, along with the whiskers indicating the minimum and maximum BERs. Since
all of the DIMMs work reliably at 10ns and above, we show the BERs for
\trcde7.5ns and \trcde5ns.

% Error dots results
%
% \figref{rcd_ber_20c} presents the average BER of DIMMs by their models for
% three different vendors. The error bars denote the 95\% confidence intervals.
% Since all of the DIMMs work reliably at 10ns and above, we show the BERs from
% \trcde7.5ns to 2.5ns.

\figputHW{model_tRCD}{rcd_ber_20c}{\newt{BERs} of DIMMs grouped
by model, when tested with different \trcd \newt{\xspace values}.}

% Old plots
%\input{sec/subplots/rcd_ber_20c}
%\input{sec/subplots/rcd_ber_expand_model_20c}

By comparing the BERs across models and vendors, we observe that BER variation
exists not only across DIMMs from different vendors, but also on DIMMs
manufactured from the same vendor. For example, for DIMMs manufactured by vendor
C, \emph{Model 0} DIMMs have fewer errors than \emph{Model 1} DIMMs. This
result suggests that different DRAM models have different circuit architectures
or process technologies, causing \new{latency variation} between them.

Similar to the observation we made across different DIMM models, we observe
variation across DIMMs that have the same model. Due to space constraints, we
omit figures to demonstrate this variation, but all of our results are available
online~\cite{safari-github}. The variation across DIMMs with the same model can
be attributed to process variation \new{due to} the imperfect manufacturing
process~\cite{nassif-isscc2000,li11,kanad_dram_book, pvt_book}.

% \ignore{
% \subsubsection{Bit Error Rates of Individual DIMMs}
% \figref{rcd_ber_expand_model_20c} shows the average BER of several DIMMs from
% the same model in different vendors. Similarly to the observation we made across
% different DIMM models, we also observe some variation across DIMMs that have the
% same model. For example, even though \dimm{0}{C}, \dimm{2}{C}, and \dimm{4}{C}
% have the same model from the same manufacturing week (i.e., week 11 of 2012),
% they exhibit different BERs at 7.5ns. We hypothesize this is due to process
% variation as no two chips can be precisely fabricated with the same
% characteristics either on the same or different silicon wafers. Nonetheless,
% DIMMs within the same model match more closely with each other than compared to
% DIMMs with different models.
% }

\subsection{Impact of Data Pattern}
\label{sec:rcd_ber_patt}

In this section, we investigate the impact of reading different data patterns
under different \trcd values. \figref{rcd_ber_pattern_20c} shows the average BER
of test rounds for three representative DIMMs, one from each vendor, with four
data patterns. We do not show the BERs at \trcde2.5ns, as rows cannot be
reliably activated at that latency. We observe that pattern \texttt{0x00} is
susceptible to more errors than pattern \texttt{0xff}, while the BERs for
\new{patterns} \texttt{0xaa} and \texttt{0xcc} lie in between.\footnote{In a
    cache line, we write the 8-bit pattern to every byte.} This can be clearly
    seen on \dimm{0}{C}, where we observe that \texttt{0xff} incurs 4 orders of
    magnitude fewer errors than \patt{0x00} on average at \trcde7.5ns. We make a
    similar observation for the rest of the 12 DIMMs from vendor C.

With patterns \texttt{0xaa} and \texttt{0xcc}, we observe that bit \texttt{0} is
more likely to be misread than bit \texttt{1}. In particular, we examined the
flipped bits on three DIMMs that share the same model as \dimm{0}{C}, and
observed that \emph{all of the flipped bits} are due to bit \texttt{0} flipping
to \texttt{1}. From this observation, we can infer that there is a bias towards
bit \texttt{1}, which can be more reliably read under a shorter activation
latency than bit \texttt{0}.

\figputHW{pattern_tRCD}{rcd_ber_pattern_20c}{BERs due to four different data
patterns on three different DIMMs as \trcd varies.}
%\input{sec/subplots/rcd_ber_pattern_20c}

We believe this bias is due to the sense amplifier design. One major DRAM vendor
presents a circuit design for a contemporary sense amplifier, and observes that
it senses the \vdd value on the bitline faster than
\zerov~\cite{kyunam-isscc2012}. Hence, the sense amplifier is able to sense and
latch bit \texttt{1} faster than \texttt{0}. Due to this pattern dependence, we
believe that it is promising to investigate asymmetric data encoding or error
correction mechanisms that favor \texttt{1}s over \texttt{0}s.

%\obs{DRAM has a strong pattern biasness towards bit \texttt{1}, and can read bit
%\texttt{1} significantly more reliably than bit \texttt{0} at fast activation
%latencies.}

%\obs{\new{Data pattern dependence exists--reading bit \texttt{1} is significantly
%more reliable than bit \texttt{0} at fast activation latencies.}}

\obs{\newt{Errors caused by reduced activation latency are dependent on the
stored data pattern. Reading bit \texttt{1} is significantly more reliable than
bit \texttt{0} at reduced activation latencies.}}

\subsection{Effect of Temperature}
\label{sec:rcd_temp}

Temperature is an important external factor that may affect the reliability of
DIMMs~\cite{schroeder-sigmetrics2009,el-sayed-sigmetrics2012,
liu-isca2013,khan-sigmetrics2014}. In particular, Schroeder et
al.~\cite{schroeder-sigmetrics2009} and El-Sayed et
al.~\cite{el-sayed-sigmetrics2012} do not observe clear evidence for increasing
DRAM error rates with increased temperature in data centers. \new{Other works
    find that data retention time strongly depends on
    temperature~\cite{khan-sigmetrics2014,liu-isca2013,qureshi-dsn2015}}. However, none
    of these works have studied the effect of temperature on DIMMs when
    they are operating with a lower activation latency.

To investigate the impact of temperature on DIMMs operating with an activation
latency lower than the standard value, we perform experiments that adjust the
\emph{ambient temperature} using a closed-loop temperature controller (shown in
\figref{dram_fpga_white}). \figref{rcd_ber_temp} shows the average BER of
\new{three example} DIMMs under three temperatures: 20\celsius, 50\celsius,
and 70\celsius~for \trcde7.5/5ns. We include error bars, which are computed
using 95\% confidence intervals.

%\vspace{-0.1in}
\input{sec/subplots/rcd_ber_temp_vert}
%\input{sec/subplots/rcd_ber_temp}
%\vspace{-0.05in}

We make two observations. First, at \trcde7.5ns (\figref{temp_rcd75}), every
DIMM shows a different BER trend as temperature increases. By calculating the
\emph{p-value} between the BERs of different temperatures, we find that the
change in BERs is not statistically significant from one temperature to another
for \new{two out of the three tested} DIMMs, meaning that we cannot conclude
that BER \new{increases at} higher temperatures. For instance, the p-values
between the BERs at 20\celsius~and 50\celsius~for \dimm{0}{A}, \dimm{0}{B}, and
\dimm{0}{C} are 0.084, 0.087, and 0.006, respectively. Two of the three DIMMs
have p-values greater than an $\alpha$ of 0.05, meaning that the BER change is
statistically insignificant. Second, at lower \trcd values~(5ns), the difference
between the BERs due to \new{temperature} becomes even smaller.

\obs{Our study does not show enough evidence
to conclude that activation errors increase with higher temperatures.}

%\begin{observation}
    %We do not observe evidence for increasing activation errors due to higher
    %temperatures.
%\end{observation}
%\obs
%    \textit{The study does not show enough evidence
%    to conclude that activation errors increase with higher temperatures.}



==> sec/latvar/exp_results_trp.tex <==
\section{Precharge Latency Analysis}
\label{sec:pre_lat_analysis}

In this section, we present the methodology and results on varying the precharge
latency, represented by the \trp timing parameter. We first describe the nature
of timing errors caused by reducing the precharge latency in
Section~\ref{sec:trp_errors}. Then, we describe the FPGA test we conducted to
characterize \trp variation in Section~\ref{sec:trp_tests}. In the remaining
sections, we describe four major observations from our result analysis.

\subsection{Behavior of Precharge Errors}
\label{sec:trp_errors}

In order to access a new DRAM row, a memory controller issues a \cpre command,
which performs the following two functions in sequence: {\em (i)}~it closes the
currently-activated row in the array (i.e., it disables the \newt{activated} row's
wordline); and {\em (ii)}~it reinitializes the voltage value of every bitline
inside the array back to \halfvdd, to prepare for a new activation.

\newt{Reducing the precharge latency by a small amount} affects only the
reinitialization process of the bitlines \newt{without interrupting the process
of closing the row}. The latency of this process is determined by the
\emph{precharge unit} that is placed \newt{by} each bitline, next to the sense
amplifier. By using a \trp value lower than the standard specification, the
precharge unit may not have \newt{sufficient time} to reset the bitline voltage
from either \vdd (\texttt{bit 1}) or \zerov (\texttt{bit 0}) to \halfvdd,
thereby causing the bitline to float at some other intermediate voltage value.
As a result, in the \emph{subsequent} activation, the sense amplifier can
incorrectly sense the wrong value \newt{from the DRAM cell} due to the extra
charge left on the bitline. \newt{We define precharge errors to be timing errors
due to reduced precharge latency.}
%We define precharge errors to be these timing errors induced by reducing
%precharge latency.

To further understand the nature of precharge errors, we use a test similar to
the one for reduced activation latency in \secref{trcd_errors}. The
test reduces only the precharge latency, while keeping the activation latency at
the standard value, to isolate the effects that occur due to a reduced precharge
latency. We attempt to answer two fundamental questions: \romnum{i} Does
lowering the precharge latency incur errors on multiple cache lines in the row
activated \emph{after} the precharge? \romnum{ii} Do these errors propagate back
to the DRAM cells, causing permanent errors for all future accesses?

\subsubsection{Precharge Errors \newt{Are} Spread Across a Row}

Throughout repeated test runs on DIMMs from all three vendors, we observe that
\newt{reducing} the precharge latency induces errors that are spread across
multiple cache lines in the row activated after the precharge. This is because
reducing the \trp value affects the latency between two \emph{row-level} DRAM
commands, \cpre and \act. As a result, having an insufficient amount of
precharge time for the array's bitlines affects the entire row.

\obs{\newt{Timing} errors occur in multiple cache lines in the row activated after a
    precharge with \newt{reduced} latency.}

Furthermore, these precharge errors are due to the sense amplifiers sensing the
wrong voltage on the bitlines, causing them to latch incorrect data. Therefore,
as the restoration operation reuses the data latched in the sense amplifiers,
the wrong data is written back into the cells.

\subsection{FPGA Test for Precharge \newt{Latency}}
\label{sec:trp_tests}

In contrast to activation errors, precharge errors are spread across an
\emph{entire} row. As a result, we use a test that varies \trp at the row level.
The pseudocode of the test, Test~\ref{trptest}, is shown below.

\input{sec/algos/trptest}

% For readers interested in the test (Test~\ref{trptest}), its
% pseudocode is in Appendix~\ref{app_rp_test}.

In total, we have conducted more than 4000 rounds of tests on the DIMMs shown in
\tabref{dimm_list_latvar}, which accounts for at least 1300 testing hours. We use three
groups of different data patterns: (\texttt{0x00}, \texttt{0xff}),
(\texttt{0xaa}, \texttt{0x33}), and (\texttt{0xcc}, \texttt{0x55}). Each group
specifies two different data patterns, which are the inverse of each other,
placed in consecutive rows in the same array. This ensures that as we iterate
through the rows in order, the partially-precharged state of the bitlines will
not favor the data pattern in the \newt{adjacent row to be activated}.

\subsection{\newt{Precharge Error Distribution}}

\newt{In this section, we first show the distribution of precharge errors collected
from all of the tests conducted on every DIMM. Then, we categorize the results
by DIMM model to investigate variation across models from different vendors.}

\subsubsection{\newt{Total Bit Error Rates}}

\figref{trp_violin} shows the box plots of the BER observed for every DIMM as
\trp is varied from 12.5ns down to 2.5ns. Based on these results, we make
several observations.
% Old violin
%\figputHW{trcd/ber/all_ber_plots/all_trp_violin}{trp_violin}{The bit error rate
%due to reducing precharge latency (\trp) for all DIMMs.}
\figputHW{trp/ber/all_ber_plots/all_trp_box_log}{trp_violin}{Bit error rate
    \newt{of all DIMMs with reduced \trp}.}
%\vspace{-8pt}
First, similar to the observation made for activation latency, we do not observe
errors when the precharge latency is reduced to 12.5 and 10ns, as the \newt{reduced
latencies} are still within the guardband provided. Second, the precharge BER is
significantly higher than the activation BER when errors start appearing at
7.5ns -- the median of the precharge BER is 587x higher than that of the
activation BER \newt{(shown in \figref{violin})}. This is partially due to the
fact that reducing the precharge latency causes the errors to span across
multiple cache lines in an \newt{\emph{entire row}}, whereas reducing the
activation latency affects \newt{\emph{only the first cache line}} read from the
row. Third, once \trp is set to 5ns, the BER exceeds the tolerable range,
resulting in a median BER of 0.43. In contrast, the activation BER does not
reach this high an error rate until the activation latency is lowered down to
2.5ns.

%Number of total tests:4018
%2.5 476 Min 0.215954 Max 0.867957 Med 0.433574
%5.0 772 Min 0.211182 Max 0.868078 Med 0.433603
%7.5 777 Min 0.000000 Max 0.866598 Med 0.200455
%10.0 690 Min 0.000000 Max 0.000000 Med 0.000000
%12.5 287 Min 0.000000 Max 0.000000 Med 0.000000

\obs{With the same amount of latency reduction, the number of precharge errors
is significantly higher than the number of activation errors.}

\subsubsection{Bit Error Rates by DIMM Model}

To examine the precharge error trend for individual DIMM models, we show the BER
distribution of every DIMM categorized by DRAM model in \figref{rp_ber_20c}.
Similar to the observation we made \newt{for} activation errors in \secref{trcd_errors},
variation exists across different DIMM models. These results provide further
support for the existence \newt{and prevalence} of latency variation in modern DRAM chips.

%\input{sec/subplots/rp_ber_20c}
\figputHW{model_tRP}{rp_ber_20c}{\newt{BERs of DIMMs grouped by
model, when tested with different \trp values.}}

\subsection{Spatial Locality of Precharge Errors}
\label{sec:trp_spatial}

In this section, we investigate the location and distribution of precharge
errors. Due to the large amount of available data, we show representative
results from two DIMMs, \dimm{0}{C} and \dimm{1}{C} from model C-M0. Our results
for some DIMMs are available publicly~\cite{safari-github}. \figref{trp_err_loc}
and \figref{trp_err_loc_2} show the probability of each cache line seeing at
least a one-bit precharge error in all banks of \dimm{0}{C} and \dimm{1}{C},
respectively, when we set \trp to 7.5ns. The x-axis indicates the cache line
number, and the y-axis indicates the row number (in thousands). The results are
gathered from 12 iterations of tests. We make several observations based on our
results.

\input{sec/subplots/trp_err_loc}

%\figputTWS{scaling_tRCD}{1}{BER trends across four different generations of
%DIMMs under three \trcd values.}

First, some banks do not have any precharge errors throughout the experiments,
such as Bank~0 (\figref{rp_col_err_b0}, hence \newt{the plot is all white}).
Similar to the activation errors, precharge errors are \newt{\emph{not}} distributed uniformly
across locations within DIMMs. Second, \figref{rp_col_err_b7} shows that
the errors concentrate on a certain region of rows, \newt{while} the other regions
experience much fewer or no errors. This demonstrates that certain sense
amplifiers, or cells at certain locations are more robust than others, allowing
them to work reliably under a reduced precharge latency.

\obs{Precharge errors do not occur uniformly within DIMMs, but exhibit strong
spatial concentration at certain regions.}

Overall, we observe that 71.1\%, 13.6\%, and 84.7\% of cache lines contain no
precharge errors when they are read from \mbox{A-M1}, B-M1, and C-M0 model
DIMMs, respectively, \newt{with \trpe7.5ns}. Similar to the trend discussed in
\secref{rcd_ecc}, C-M0 DIMMs have the highest fraction of reliable cache lines
among the DIMMs tested, while B-M1 DIMMs experience the largest amount of
errors. Even though the number of error-free cache lines at \trpe7.5ns is lower
than that at \trcde7.5ns, the portion is still significant enough to show the
\newt{prevalence} of precharge latency variation in modern DIMMs.

\obs{When precharge latency is reduced, a majority of cache lines can be read without any timing errors in some
of our tested DIMMs. However, other DIMMs are largely susceptible to
precharge errors, resulting in a small fraction of error-free cache lines.}



==> sec/latvar/intro.tex <==
% !TEX root=../paper.tex

\section{Introduction}

Over the past few decades, the long latency of memory has been a
critical bottleneck in system performance. Increasing core counts,
emergence of more data-intensive and latency-critical applications,
and increasingly limited bandwidth in the memory system are together
leading to higher memory latency.  Thus, low-latency memory operation
is now even more important to improving overall system
performance\new{~\cite{wilkes-sigarch2001, mckee-cf2004, lee-hpca2013,
son-isca2013, dean-cacm2013, kanev-isca2015, lee-hpca2015,
superfri,chang-hpca2016,hassan-hpca2016,shin-hpca2014,
o-isca2014,lu-micro2015,lee-tech2010,seshadri-micro2013,mutlu-imw2013}}.

The latency of a memory request is predominantly defined by the
timings of two fundamental operations: \emph{activation} and
\emph{precharge}.  These operations take place on the two-dimensional
arrays of memory \emph{cells} that store data.  Activation is the
process of ``opening'' a row of cells, in order to allow data within
that row to be accessed.  Once a row is \emph{activated}, the memory
controller can read from or write to it one cache line at a time.
Precharge is the process of ``closing'' the activated row, and
preparing the cell array for the next memory access.  Once the array
is \emph{precharged}, another row can be activated.  Specifically for
DRAM, we also need to consider the latency of a third operation, known
as \emph{restoration}.  A DRAM cell uses a capacitor, whose charge
level represents the stored data value.  The activation process of a
row affects the charge level in the capacitor, which can destroy the
data value stored within the cell.  To prevent data loss, DRAM must
\emph{restore} the charge level of each DRAM cell in the row to
reflect the cell's data value before activation, which takes time.


The latencies of these three DRAM operations, as defined by vendor
specifications, have \emph{not} improved significantly in the past decade, as
depicted in Figure~\ref{fig:latency_trend}. This is especially true
when we compare \new{latency improvements}
%compared
to the capacity (64$\times$=$\frac{8Gb}{128Mb}$) and bandwidth
%\fontdimen2\font=0.68ex
improvements (16$\times$$\approx\frac{2133MT/s}{133MT/s}$)~\cite{jedec-ddr3,
jedec-ddr4, lee-hpca2013, son-isca2013, lee-hpca2015} commodity DRAM chips
\fontdimen2\font=\origiwspc
experienced in the past decade. In fact, the activation and precharge latencies
\emph{increased} from 2013 to 2015, when DDR \new{DRAM} transitioned from the
third generation (12.5ns for DDR3-1600J~\cite{jedec-ddr3}) to the fourth
generation (14.06ns for DDR4-2133P~\cite{jedec-ddr4}). As the latencies
specified by vendors have not reduced over time, the system performance
bottleneck caused by raw main memory latency remains largely unaddressed in
modern systems.

%\fontdimen2\font=\origiwspc

\figputHW{latency_trend/an_lat_trend_1999}{latency_trend}{DRAM latency trends
  over time~\cite{micronSDR_128Mb,jedec-ddr2,jedec-ddr3,jedec-ddr4}.}
%\vspace{-10in}

% \figputHSL{latency_trend/latency_trend}{1}{\color{blue}DRAM latency trend over
% time~\cite{jedec-ddr2,jedec-ddr3,jedec-ddr4}.\vspace{-0pt}}{latency_trend}

In this work, we observe that \new{the three fundamental DRAM} operations can
\emph{actually} complete with a much lower latency for many DRAM cells than the
specification, because \emph{there is inherent latency variation present across
the DRAM cells within a DRAM chip}.  This is a result of manufacturing process
variation, which causes the \emph{sizes} and \emph{strengths} of cells to be
different, thus making some cells faster and other cells slower to be accessed
reliably~\cite{li11,hamamoto98,kim09}.  The speed gap between the fastest and
slowest DRAM cells is getting worse~\cite{kanad_dram_book, pvt_book}, as the
technology node continues to scale down to sub-20nm feature sizes.
Unfortunately, instead of optimizing the latency specifications for the common
case, DRAM vendors use a single set of standard access latencies, which provide
reliable operation guarantees for the \emph{worst case} (i.e., slowest cells),
to maximize manufacturing yield.

We find that the (widening) speed gap among DRAM cells presents an opportunity
to reduce DRAM access latency.  If we can understand and characterize the
inherent variation in cell latencies, we can use the resulting understanding to
reduce the access latency for those rows that contain faster cells.
\textbf{The goal of this work} is to {\em (i)}~experimentally characterize and
understand the impact of latency variation in the three fundamental DRAM
operations for cell access (activation, precharge, and restoration), and
{\em(ii)}~develop new mechanisms that take advantage of this variation to
improve system performance.

To this end, we build an FPGA-based DRAM testing infrastructure and characterize
240 DRAM chips from three major vendors. We analyze the variations in the
latency of the three fundamental DRAM operations by operating DRAM at multiple
reduced latencies.  Faster cells do not get affected by the reduced timings, and
can be accessed reliably without changing their stored value; however, slower
cells {\em cannot} be reliably read with reduced latencies for the three
operations, leading to bit flips. In this work, we define a {\em
timing error} as a bit flip in a cell that occurs due to a reduced-latency
access, and characterize timing errors incurred by the three DRAM operations. Our
experimental characterization yields six new \textbf{key observations}.

%%% ONUR: We characterize these timing errors to understand how they
%%% can be mitigated.  --> Do we really examine how these can be
%%% mitigated?

%%% ONUR: The new material above is a bit rough, Italics for the full
%%% sentece was not needed. Also, why did you switch to the ``timing
%%% error'' terminology?


%any failure; however, slower cells {\em cannot} be
%reliably read with reduced latencies in cell operations, leading to
%failures.

First, we find that significant variation is present in modern DRAM
chips for the latencies of all three fundamental DRAM operations. For
example, we observe that 68\%, 100\%, and 36\% of cache lines can be
read reliably when activation/restoration/precharge latencies are
reduced by 43\%/36\%/43\%, respectively, across all 240 of our tested
DRAM chips. We conclude that exploiting latency variation in DRAM
cells has the potential to greatly reduce the access latency.

Second, we find that when we reduce the latency for different DRAM
operations, there is \new{spatial} locality in inherently slower cells: such cells
are clustered in certain \new{\emph{regions}} of a DRAM chip, as opposed to being
randomly distributed. We conclude that such spatial locality can be
exploited to develop low-cost mechanisms to reduce latency, where fast
regions are accessed with lower latency, and slow regions are accessed
with the standard high latency.

\new{Third, when we reduce the three latencies, we observe that each latency
exhibits a different level of impact on the inherently-slower cells.}
% we observe different impacts on the inherently slower cells when we
% reduce each of the three latencies.}
Lowering the activation latency affects
\emph{only} the cells read in the first accessed cache line. In contrast,
lowering the restoration or precharge latencies affects \emph{all} cells in the
row. We explain in detail why this is the case.  We also find that the number of
timing errors introduced is very sensitive to reductions in activation and
precharge latencies, but not that sensitive to reduction in restoration latency.
We conclude that different levels of mitigation are required to address the
timing errors that result from lowering each of the different DRAM operation
latencies, and that reducing restoration latency does not introduce timing
errors in our experiments.

%%% ONUR: Isn't the last conclusion about ``no impact on reliability''
%%% too strong? It can be taken wrongly. Have we studied all worst
%%% case effects like temperature, data pattern etc? Can we rephrase
%%% this to be more ceraful?

%%% ONUR: On a related note: do we have temperature experiments?

Fourth, we analyze the number of timing errors that occur when DRAM access
latencies are reduced, and experimentally demonstrate that most of the erroneous
cache lines have a single-bit error, with only a small fraction of cache lines
experiencing more than one bit flip. We conclude, therefore, that using simple
error-correcting codes (ECC) can correct most of these errors, thereby enabling
lower latency for many inherently slower cells.

Fifth, we find no clear correlation between temperature and variation in cell
access latency. We believe that it is not essential for latency reduction
techniques that exploit such variation to be aware of the operating temperature.

%%% ONUR: The last sentence above seems wrong... AL-DRAM is a latency
%%% reduction technique and it clearly needs to be aware of
%%% temperature. Please rephrase. We do not want to say wrong things.
%%% See how I fixed it. I still think it is strong. ``Conclude'' and
%%% ``do not need to be aware'' can be replaced with less strong
%%% words.

Sixth, we find that the stored data pattern in cells affects access latency
variation. Certain patterns lead to more timing errors than others. For example,
the bit value \texttt{1} can be read significantly more reliably at a reduced
access latency than the bit value \texttt{0}.  We conclude that it is promising
to investigate asymmetric data encoding or error correction mechanisms that
favor \texttt{1}s over \texttt{0}s.

%%% ONUR: The above paragraph. Does the data pattern affect the magnitude of variation?
%%% The provided observation of 1 and 0 bias seems unrelated to variation. Comments?

%examine asymmetric error correction codes that protect \texttt{0}s better.

Based on these major conclusions from our comprehensive analysis and
characterization of 240 DRAM chips from three major DRAM
manufacturers, we propose and evaluate a new mechanism, called \mech
(\mechlong). \mech's key idea is to {\em (i)} categorize the DRAM
cells into fast and slow regions, {\em (ii)} expose this information
to the memory controller, and {\em (iii)} reduce overall DRAM latency
by accessing the fast regions with a lower latency. Our
simulation-based analysis shows that \mech improves the performance of
a wide range of applications in an 8-core system. Based on our
experimental observations, we also discuss a page allocator design
that exploits the latency variation in DRAM to improve system
performance.

We hope that our extensive \new{analysis} leads to other new mechanisms to
improve DRAM performance and reliability. To facilitate this, we will make our
characterization results for all tested \new{DRAM chips} and the \new{\mech
simulator} publicly available~\cite{safari-github}.

To our knowledge, this is the first work to make the following major
contributions:

\squishlist

\item It experimentally demonstrates and characterizes the significant
  variation in latency of three fundamental DRAM operations
  (activation, restoration, and precharge) across different cells
  within a DRAM chip.

\item It experimentally demonstrates that reducing the latency of each
  of these three fundamental DRAM operations has a different effect on
  slower cells.  It shows that {\em (i)} while the memory controller
  can introduce timing errors in slower cells by reducing the
  activation and precharge latencies, it can reduce the restoration
  latency without impacting these cells, thus providing greater
  opportunities to improve performance without causing timing errors;
  %while reducing the activation and precharge latencies can introduce several
  %timing errors in slower cells, reducing the restoration latency has no impact
  %on these cells, thus providing greater opportunities to improve performance
  %without causing errors;
  and {\em (ii)} errors due to reducing the activation latency appear only in
  the first cache line accessed in a row, limiting the scope of impact.

%Reducing Activation
%latency only impacts the first read, making it very effective in reducing latency
%without introducing failures in the slower cells.  Reduction in Restoration
%has the most robustness against slower cells, where reduction in Precharge
%has the least.
\item It experimentally demonstrates that access latency variation
  exhibits spatial locality within DRAM, and that the error rate with
  reduced latencies is correlated with the stored data pattern in
  cells, but not with temperature.

\item It proposes a new mechanism, \mech, which exploits the lower
  latencies of DRAM regions with faster cells by introducing
  heterogeneous timing parameters into the memory controller.  We find that
  \mech improves performance in an 8-core system by 13.3\%, 17.6\%,
  and 19.5\%, on average, for each of the three different vendors'
  real DRAM chips, across a wide range of applications.

\squishend



==> sec/latvar/long_abstract.tex <==
% !TEX root=../paper.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract is in abstract_short.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Long DRAM latency is a critical performance bottleneck in current systems.  DRAM
% access latency is defined by three fundamental operations that take place within
% the DRAM cell array: {\em (i)}~\emph{activation} of a memory row, which opens
% the row to perform accesses; {\em (ii)}~\emph{precharge}, which prepares the
% cell array for the next memory access, and {\em (iii)}~\emph{restoration} of the
% row, which restores the values of cells in the row that were destroyed due to
% activation.  There is significant latency variation for each of these operations
% across the cells of a single DRAM chip due to irregularities in the
% manufacturing process.  As a result, some cells are \emph{inherently} faster to
% access, while others are inherently slower. \new{Based on this fact, accessing cells
% using their inherent latency is imperative for achieving low memory
% latency. However, DRAM manufacturers define fixed latencies within their
% standards for each of these operations based on the worst-case (i.e.,
% slowest) cells to maximize manufacturing yield, artificially increasing the
% overall memory latency.}
%
% % Previous version of the ending sentence
% % Instead of catering to the speed of
% % the majority of cells, DRAM manufacturers define fixed latencies within their
% % standards for each of these operations based on the \emph{worst-case} (i.e.,
% % slowest) cells.
%
%
% The goal of this work is to {\em (i)}~experimentally characterize and understand
% the latency variation across cells within a DRAM chip for these three
% fundamental DRAM operations, and {\em (ii)}~develop new mechanisms that exploit
% our understanding of the latency variation to reliably improve performance.  To
% this end, we comprehensively characterize 240 DRAM chips from three major
% vendors, and make several new observations about latency variation within DRAM.
% We find that (1)~there is large latency variation across the cells:
% \new{68\%/100\%/36\% of cache lines can operate with 43\%/36\%/43\% lower
% activation/restoration/precharge latency, respectively, than the remainder of
% cache lines in all of our tested DRAM chips;}
% % 68\%/100\%/36\% of cache lines can be read reliably when the
% % activation/restoration/precharge latency is reduced by 43\%/36\%/43\%,
% % respectively, across all of our tested DRAM chips;
% (2)~variation characteristics exhibit significant spatial locality: slower cells
% are clustered in certain regions of a DRAM chip; and (3)~the three fundamental
% operations have different variation and reliability characteristics when the
% latency of each operation is reduced.
%
% Based on our observations, we propose \new{\mechlong (\mech)}, a mechanism that
% exploits latency variation across DRAM cells within a DRAM chip to improve
% system performance.  The key idea of \mech is to exploit the spatial locality of
% slower cells within DRAM, and access the faster DRAM regions with reduced
% latencies for the three fundamental operations.  Our evaluations show that \mech
% improves the performance of a wide range of applications by 13.3\%, 17.6\%, and
% 19.5\%, on average, using three different vendors' real DRAM chips, in an 8-core
% system.  We conclude that experimentally characterizing and understanding
% latency variation within modern DRAM can lead to new techniques that improve
% DRAM and system performance.


==> sec/latvar/mechanism.tex <==
% !TEX root=../paper.tex

\section{Exploiting Latency Variation}

Based on our extensive experimental characterization, we propose two new
mechanisms to reduce DRAM latency for better system performance. Our mechanisms
exploit the key observation that different DIMMs have different \newt{amounts of
tolerance} for lower DRAM latency, and there is a strong correlation between the
location of the cells and the lowest latency that the cells can tolerate. The
first mechanism (Section~\ref{sec:var_latency_mc}) is a pure hardware approach
to reducing DRAM latency. The second mechanism
(Section~\ref{sec:dram_aware_page_alloc}) leverages OS support to maximize the
benefits of the first mechanism.

\subsection{Flexible-Latency DRAM}
%\subsection{\mechlong (\mech)}
\label{sec:var_latency_mc}

As we discussed in Sections~\ref{sec:trcd_loc} and~\ref{sec:trp_spatial}, the
timing errors caused by reducing the latency of the activation/precharge
operations are concentrated on certain DRAM regions, which implies that the
latency heterogeneity among DRAM cells exhibits strong locality. Based on this
observation, we propose \emph{\mechlong (\mech)}, a software-transparent design
that exploits this heterogeneity in cells to reduce the overall DRAM latency.
The key idea of \mech is to determine the shortest reliable access latency of
each DRAM region, and to use the memory controller to apply that latency to the
corresponding DRAM region at runtime. There are two key design challenges of
\mech, as we discuss below.

The first challenge is determining the shortest access latency.  This can be
done using a \emph{latency profiling} procedure, which \romnum{i}~runs
Test~\ref{trcdtest} (Section~\ref{sec:trcd_tests}) with different timing values
and data patterns, and \romnum{ii}~records the smallest \newt{latency that
enables reliable access to} each region.  This procedure can be performed at one
of two times. First, the system can run the procedure the very first time the
DRAM is initialized, and store the profiling results to non-volatile memory
(e.g., \newt{disk} or flash memory) for future reference. Second, DRAM vendors
can run the procedure at manufacturing time, and embed the results in the Serial
Presence Detect (SPD) circuitry (a ROM present in each DIMM)~\cite{jedec-spd}.
The memory controller can read the profiling results from the SPD circuitry
during DRAM initialization, and apply the correct latency for each DRAM region.
While the second approach involves a slight modification \newt{to the DIMM}, it
can provide better latency information, as DRAM vendors have detailed knowledge
on DRAM cell variation, and can use this information to run more thorough tests
to determine a lower bound on the latency of each DRAM region.

The second design challenge is limiting the storage overhead of the latency
profiling results. Recording the shortest latency for each cache line can incur
a large storage overhead. For example, supporting four different \trcd and \trp
timings requires 4~bits per 512-bit cache line, which is almost 0.8\% of the
entire DRAM storage. Fortunately, the storage overhead can be reduced based on
\newt{a new} observation of ours. As shown in Figures~\ref{fig:rcd_col_err} and
\ref{fig:rcd_err_region}, timing errors typically concentrate on certain DRAM
\emph{columns}. Therefore, \mech records the shortest latency \emph{at the
granularity of DRAM columns}. Assuming we still need 4~bits per DRAM cache line,
we need only 512~bits per DRAM bank, or an insignificant \newt{0.00019\%}
storage overhead for the DIMMs we evaluated. One can imagine using more
sophisticated structures, such as Bloom Filters~\cite{bloom-cacm70}, to provide
finer-grained latency information within a reasonable storage overhead, as shown
in prior work on variable DRAM refresh time~\cite{liu-isca2012,qureshi-dsn2015}.
We leave this for future work.

\newt{The} \mech memory controller \romnum{i} loads the latency profiling results
%(collected by either the system user or the DRAM manufacturer)
into on-chip SRAMs at system boot time, \romnum{ii} looks up the profiled latency for
each memory \newt{request} based on its memory address, and \romnum{iii} applies the
\newt{corresponding latency to the request}. By reducing the latency values of
\trcd, \tras, and \trp for some memory requests, \mech improves overall system
performance, which we quantitatively demonstrate in the next two sections.

% Evaluation results
\input{sec/vldram_eval}

\subsection{Discussion: DRAM-Aware Page Allocator}
\label{sec:dram_aware_page_alloc}

While \mech significantly improves system performance in a software-transparent
manner, we can take better advantage of it if we expose the \newt{different
latency regions of \mech to} the software stack.
%As we observed in Sections~\ref{sec:trcd_loc} and \ref{sec:trp_spatial}, there
%is a spatial concentration of errors that occur when we lower the activation
%and precharge latencies. This means that when DRAM operation latencies are
%reduced, there are some rows that are more prone to errors, and other rows that
%remain error-free. Based on this observation, we
\newt{We} propose the idea of a DRAM-aware page allocator in the OS, whose goal is to
better take advantage of \mech by intelligently mapping application pages to
different-latency DRAM regions in order to improve performance.

Within an application, there is heterogeneity in the access frequency of
different pages, where some pages are accessed much more frequently than other
pages~\cite{verghese-asplos1996, bhattacharjee-isca2009,ramos-ics2011,
son-isca2013,sudan-asplos2010,yoon-iccd2012}. Our DRAM-aware page allocator
places more frequently-accessed pages into lower-latency regions in DRAM. This
\emph{access frequency aware placement} allows a greater number of DRAM accesses
to \newt{experience} a reduced latency than a page allocator that is oblivious
to DRAM latency variation, thereby likely increasing system performance.

%Our allocator places
%the least frequently accessed pages into DRAM regions that are more likely to
%experience errors when the access latency is lowered. For these pages, \mech
%maintains the standard higher access latency to maintain reliable operation.
%Since these pages are accessed less often, the amount of performance improvement
%lost by not lowering the access latency is minimized.
%compared to a DRAM-oblivious allocator.

For our page allocator to work effectively, it must know which pages are
expected to be accessed frequently.  In order to do this, we extend the OS
system calls for memory allocation to take in a Boolean value, which states
whether the memory being allocated is expected to be accessed frequently.  This
information either can be annotated by the programmer, or can be estimated by
various dynamic profiling techniques~\cite{jiang-hpca2010, sudan-asplos2010,
    verghese-asplos1996, marathe-ppopp2006, ramos-ics2011, agarwal-asplos2015,
chandra-asplos1994,yoon-iccd2012}. The page allocator uses this information to
find a free physical page in DRAM that suits \newt{the expected access frequency
of the} application page that is being allocated.

We expect that by using our proposed page allocator, \mech can perform close to
the upper-bound performance reported in
Section~\ref{sec:var_latency_mc:results}, even for DIMMs that have a smaller
fraction of fast regions.

%%%%%
% Old stuff
\ignore{
\subsection{Column Command Re-Ordering}
\label{sec:col_comm_reorder}

As we observed in Section~\ref{sec:trcd_errors:first_col}, when the activation
latency is lowered aggressively, errors can appear when reading from DRAM, but
\emph{only} within the first cache line that is read out.  We also observed in
Section~\ref{sec:trcd_loc} that these errors do not occur uniformly across a
DIMM, and that errors tend to cluster within only certain columns of a row.
Based on these observations, we develop a scheduling mechanism whose
goal is to reduce the probability of errors due to shortened activation latency,
by reordering requests such that the first column accessed is the most robust.

When a row is activated, there is often more than one request to access that
row, due to spatial locality.  Several memory scheduling algorithms, such as
the widely-used FR-FCFS~\cite{rixner-isca2000}, work to exploit \emph{row buffer
locality}, where multiple pending requests to an activated row are sent
back-to-back in order to avoid activating the row multiple times (and incurring
additional activation and precharge latencies).  To do this, memory schedulers
reorder the pending requests to DRAM by adding a set of prioritization
rules (e.g.,~\cite{rixner-isca2000,mutlu-isca2008,kim-micro2010,subramanian-iccd2014}).

We propose a memory scheduler where we expose the reliability of each column
within a row.  Similar to our approach in Section~\ref{sec:var_latency_mc}, we
perform profiling to classify the expected number of errors for each cache line
within a row, and store this within a table in the memory controller.  We then
feed this information into a modified version of the FR-FCFS scheduler, which
prioritizes pending requests to activated rows.  Our modified scheduler adds
another layer of prioritization amongst all of the pending requests to activated
rows, choosing the request whose desired cache line has the lowest expected
number of errors first.  When a requests first arrives into the memory
controller, the profiling data is looked up from the table, and then stored
alongside the other request data in the transaction queue.  The scheduler uses
the data in the transaction queue to make its decisions.

By reordering the requests, we expect that our scheduler can often find column
commands with no or very few errors, as we see many of these in
Section~\ref{sec:density_err}. Therefore, we conclude that a memory scheduler
that is aware of the distribution of errors across the cache lines within a row
can mitigate a large percentage of the errors that take place due to reduced
activation latency.
}

%\subsection{Pattern Inversion on Writes}
%1. Perform an actual pattern inversion when writing data. Different from DBI
%that only works on the bus!




==> sec/latvar/motivation.tex <==
%\section{Motivation}
\subsection{Opportunities for Reducing Latency}
\label{sec:motivation}

% In the previous section, we have described three major DRAM operations
% (activation, restoration, and precharge) that are required to access a cache
% line in a bank. The latencies of these operations are defined in the DRAM standard
% using specific timing parameters (\trcd, \tras, and \trp). For example, the
% timing parameter \trcd specifies the latency of the activation operation. A
% \crd command following an \act command has to wait at least for the time
% specified by \trcd before it can be issued.

DRAM standards define fixed values that are used for each of the timing
parameters that we have described (e.g., DDR3 DRAM~\cite{jedec-ddr3,
jedec-lpddr3}).  Unfortunately, these latencies do \emph{not} reflect the
\emph{actual} time the DRAM operations take for each cell.
%true latency of the corresponding DRAM operations to each cell.
This is because the true access latency varies for each cell, as every cell is
different in size and strength due to manufacturing process variation effects.
For simplicity, and to ensure that DRAM yield remains high, DRAM manufacturers
define a single set of latencies that guarantees reliable operation, based on
the \emph{slowest} cell in {\em any} DRAM chip across \emph{all} DRAM vendors.
As a result, there is a significant opportunity to reduce DRAM latency if,
instead of always using worst-case latencies, we employ the true latency for
each cell \newt{that enables the three operations reliably}.
%that reliably performs the corresponding operations.

\new{\textbf{Our goal} in this work is to {\em (i)}~understand the
impact of cell variation in the three fundamental DRAM operations for cell
access (activation, precharge, and restoration); {\em (ii)}~experimentally
characterize the latency variation in these operations; and {\em (iii)}~develop
new mechanisms that take advantage of this variation to reduce the latency of
these three operations.}

%In this work, we reduce \new{the} latency of \new{three} DRAM operations by
%leveraging the variation in cells. However, this requires a comprehensive
%analysis and characterization of the latency variation in cells and their
%behavior when reduced latencies are used for the fundamental DRAM operations.
%
%\textbf{Our goal}, \new{therefore}, in this work is to {\em (i)} understand the impact
%of cell variation in the three fundamental DRAM operations for cell
%access (activation, precharge, and restoration); {\em (ii)}~experimentally
%characterize the latency variation in these operations; and {\em (iii)}
%develop new mechanisms that take advantage of this variation to
%improve performance.

To achieve this goal, we discuss the impact of reducing activation
(Section~\ref{sec:act_lat_analysis}), precharge
(Section~\ref{sec:pre_lat_analysis}), and restoration
(Section~\ref{sec:ras_lat_analysis}) latencies on DRAM cells by
\new{experimentally analyzing and characterizing the latency} variation in cells
in 240 real DRAM chips.


==> sec/latvar/related.tex <==
% !TEX root=../paper.tex

\section{Related Work}

To our knowledge, this is the first work to {\em (i)}~provide a detailed
experimental characterization and analysis of latency variation for three
\newt{major} DRAM operations (\trcd, \trp, and \tras) \emph{across different
cells within a DRAM chip}, {\em (ii)}~demonstrate that a reduction in latency
for each of these fundamental operations has a different impact on slower cells,
{\em (iii)}~show that access latency variation exhibits spatial locality, {\em
(iv)}~demonstrate that the error rate \newt{due to reduced latencies} is
correlated with the \newt{stored} data pattern but not \newthree{conclusively correlated} with temperature, and {\em
(v)}~propose mechanisms that take advantage of variation \emph{within a DRAM
chip} to improve system performance.

\noindent\textbf{DRAM Latency Variation.} Adaptive-Latency DRAM (AL-DRAM) also
characterizes and exploits DRAM latency variation, but does so at a much coarser
granularity~\cite{lee-hpca2015}. This work experimentally characterizes latency
variation across different DRAM chips under different operating temperatures.
AL-DRAM sets a uniform operation latency for the \emph{entire} DIMM. In
contrast, our work characterizes latency variation \emph{within each chip}, at
the granularity of individual DRAM cells. Our mechanism, \mech, can be combined
with AL-DRAM to further improve performance.

Chandrasekar et al.\ study the potential of reducing some DRAM timing
parameters~\cite{chandrasekar-date2014}. Similar to AL-DRAM, this work observes
and characterizes latency variation \emph{across} DIMMs, whereas our work
studies variation \newt{across} cells \emph{within a DRAM chip}.

\noindent\textbf{DRAM Error Studies.} There are several studies that
characterize various errors in DRAM. Many of these works observe how specific
factors affect DRAM errors, analyzing the impact of
temperature~\cite{el-sayed-sigmetrics2012,lee-hpca2015} and hard
errors~\cite{hwang-asplos2012}. Other works have conducted studies of DRAM error
rates in the field, studying failures across a large sample
size~\cite{schroeder-sigmetrics2009, meza-dsn2015, li-usenixatc2010,
sridharan-sc2012, sridharan-asplos2015}. There are also works that have studied
errors through controlled experiments, investigating errors due to
retention~\newt{\cite{liu-isca2013, khan-sigmetrics2014, khan-dsn2016,
qureshi-dsn2015}}, disturbance from neighboring DRAM cells~\cite{kim-isca2014},
and latency variation \emph{across DRAM chips}~\cite{chandrasekar-date2014,
lee-hpca2015}. None of these works study errors due to latency variation across
the cells within a DRAM chip, which we extensively characterize in our work.

\noindent\textbf{DRAM Latency Reduction.} Several types of commodity
DRAM (Micron's RLDRAM~\cite{micron-rldram3} and Fujitsu's
FCRAM~\cite{sato-vlsic1998}) provide low latency at the cost of high
area overhead~\cite{kim-isca2012, lee-hpca2013}. Many prior works
\newt{(e.g.,~\cite{chang-hpca2014,kim-isca2012,
    lee-hpca2013,o-isca2014,chang-hpca2016,hidaka-ieeemicro90,
    seshadri-micro2013, seshadri-cal2015,
    zhang-isca2014,lu-micro2015,son-isca2013})} propose various
architectural changes \emph{within} DRAM chips to reduce latency. In
contrast, \mech does not require any changes to a DRAM chip. Other
works~\newt{\cite{shin-hpca2014,lee-tech2010,hassan-hpca2016,seshadri-isca2014,seshadri-micro2015}}
reduce DRAM latency by changing the memory controller, and \mech is
complementary to them.

\newthree{
\noindent\textbf{ECC DRAM.} Many memory systems incorporate ECC
DIMMs, which store information used to correct data during a read operation.
Prior work (e.g.,~\cite{vecc, yoon.isca12.boom, udipi2012lot, kim2015bamboo,
    li2012mage, khan-sigmetrics2014, wilkerson-isca2010, gongclean,
jian2013low}) proposes more flexible or more powerful ECC schemes for DRAM. While
these ECC mechanisms are designed to protect against faults using standard DRAM
timings, we show that they also have the potential to correct timing errors that
occur due to reduced DRAM latencies.
% Although these ECC mechanisms are mainly used to protect against hardware
% faults in DRAM, in this work, we show that ECC DIMM has the potential to
% provide low latency and reliability.
}


==> sec/latvar/subplots/b1_rcd3_dimm_heatmap_20c.tex <==
\begin{figure*}[h]
    \centering

    \subcaptionbox{Bank0}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc0.pdf} }
    \subcaptionbox{Bank1}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank1_ecc0.pdf} }
    \subcaptionbox{Bank2}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank2_ecc0.pdf} }
    \subcaptionbox{Bank3}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank3_ecc0.pdf} }

    \subcaptionbox{Bank4}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank4_ecc0.pdf} }
    \subcaptionbox{Bank5}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank5_ecc0.pdf} }
    \subcaptionbox{Bank6}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank6_ecc0.pdf} }
    \subcaptionbox{Bank7}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/whole_dimm/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank7_ecc0.pdf} }
    \caption{Error coverage overlapped from 12 experimental runs on DIMM A0 at \trcd=7.5ns at 20\celsius.}
    \label{fig:dimm_va_b1_rcd_20c}
\end{figure*}


==> sec/latvar/subplots/b1_rcd_ecc_heatmap_20c.tex <==
\begin{figure*}[h]
    \centering

    \subcaptionbox{No EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc0.pdf} }
    \subcaptionbox{1EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc1.pdf} }
    \subcaptionbox{2EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc2.pdf} }
    \subcaptionbox{3EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_6_hist_128x16384_b1_rcd3_pattff00_20c_bank0_ecc3.pdf} }

    \caption{Effect of ECC on DIMM A0 at \trcd=7.5ns at 20\celsius.}
    \label{fig:b1_rcd_ecc_heatmap_20c}
\end{figure*}


==> sec/latvar/subplots/burst_rcd2_20c.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    %\subcaptionbox{Two DIMMs (A-M1).}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_cr_m1_dimms_burst_rcd2.pdf}
    %}
    %%
    %\subcaptionbox{One DIMMs (B-M1).}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_hy_m1_dimms_burst_rcd2.pdf}

    %}
    %%
    %\subcaptionbox{Six DIMMs (C-M0).}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.3\linewidth]{plots/trcd/bursts/all_y_dimms_burst_rcd2.pdf}
    %}

    \subcaptionbox{A-M1}%[\linewidth]
    {
        \includegraphics[width=0.46\linewidth]{plots/trcd/bursts/all_cr_m1_dimms_burst_rcd2.pdf}
        \vspace{-5pt}
    }
    \subcaptionbox{B-M1}%[\linewidth]
    {
        \includegraphics[width=0.46\linewidth]{plots/trcd/bursts/all_hy_m1_dimms_burst_rcd2.pdf}
        \vspace{-5pt}
    }
    %
    \subcaptionbox{C-M0}[\linewidth]
    {
        %\includegraphics[scale=0.6]{plots/trcd/bursts/all_y_dimms_burst_rcd2.pdf}
        \includegraphics[width=0.46\linewidth]{plots/trcd/bursts/all_y_dimms_burst_rcd2.pdf}
        \vspace{-5pt}
    }

    \caption{Breakdown of the number of error bits observed in each data
    beat of erroneous cache lines at \trcde5ns.}
    \label{fig:burst_rcd2_20c}
\end{figure}

%all_cr_m1_dimms_burst_rcd2.pdf
%all_hy_m1_dimms_burst_rcd2.pdf
%all_y_dimms_burst_rcd2.pdf

%\begin{figure*}[h]
%    \centering
%    \captionsetup[subfigure]{justification=centering}
%    \subcaptionbox{DIMM A0.}[0.225\textwidth]
%    {
%        \includegraphics[width=0.225\linewidth]{plots/trcd/bursts/b1_all_patt_rcd2_20c.pdf}
%    }
%    %
%    \subcaptionbox{DIMM B0.}[0.225\textwidth]
%    {
%        \includegraphics[width=0.225\linewidth]{plots/trcd/bursts/burst_dist_p6_all_att_rcd2.pdf}
%    }
%    %
%    \subcaptionbox{DIMM C0.}[0.225\textwidth]
%    {
%        \includegraphics[width=0.225\linewidth]{plots/trcd/bursts/burst_dist_y22_all_patt_rcd2_20c.pdf}
%    }
%    %
%    \subcaptionbox{DIMM C5.}[0.225\textwidth]
%    {
%        \includegraphics[width=0.225\linewidth]{plots/trcd/bursts/burst_dist_g1_all_patt_rcd2_20c.pdf}
%    }
%
%    \caption{Breakdown on the number of error bits observed in data
%    bursts, which form a cache line, due to \trcd=5ns at 20\celsius.}
%    \label{fig:burst_rcd2_20c}
%\end{figure*}


==> sec/latvar/subplots/p6_rcd_ecc_heatmap_20c.tex <==
\begin{figure*}[h]
    \centering

    \subcaptionbox{No EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_12_hist_128x16384_p6_rcd2_pattff00_20c_bank0_ecc0.pdf} }
    \subcaptionbox{1EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_12_hist_128x16384_p6_rcd2_pattff00_20c_bank0_ecc1.pdf} }
    \subcaptionbox{2EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_12_hist_128x16384_p6_rcd2_pattff00_20c_bank0_ecc2.pdf} }
    \subcaptionbox{3EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{plots/trcd/heatmap/ecc/filecnt_12_hist_128x16384_p6_rcd2_pattff00_20c_bank0_ecc3.pdf} }

    \caption{Effect of ECC on DIMM B0 at \trcd=5ns at 20\celsius.}
    \label{fig:p6_rcd_ecc_heatmap_20c}
\end{figure*}


==> sec/latvar/subplots/rcd_ber_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A.}[0.3\textwidth]
    {
        %\includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_plots/crucial_ber_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/model_ber_plots/crucial_model_patt0x0_ber.pdf}
    }
    %
    \subcaptionbox{Vendor B.}[0.3\textwidth]
    {
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/model_ber_plots/hynix_model_patt0x0_ber.pdf}
    }
    %
    \subcaptionbox{Vendor C.}[0.3\textwidth]
    {
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/model_ber_plots/samsung_model_patt0x0_ber.pdf}
    }
    %
    %\subcaptionbox{Vendor C-Batch2.}[0.225\textwidth]
    %{
    %    \includegraphics[width=0.225\linewidth]{plots/trcd/ber/ber_plots/samsung_g_ber_20c.pdf}
    %}

    %\caption{Bit error rates (BERs) of various DRAM DIMMs running at different \trcd parameters at 20\celsius.}
    \caption{Bit error rates (BERs) of DRAM DIMMs by their models running at different \trcd parameters.}
    \label{fig:rcd_ber_20c}
\end{figure*}


==> sec/latvar/subplots/rcd_ber_expand_model_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A and model A-M0.}[0.3\textwidth]
    {
        \includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_plots/crucial_ber_20c_model0.pdf}
    }
    %
    \subcaptionbox{Vendor B and model B-M0.}[0.3\textwidth]
    {
        \includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_plots/hynix_ber_20c_model0.pdf}
    }
    %
    \subcaptionbox{Vendor C and model C-M0.}[0.3\textwidth]
    {
        \includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_plots/samsung_ber_20c_model0.pdf}
    }

    \caption{Bit error rates (BERs) of various DIMMs with the same model running at different \trcd parameters.}
    \label{fig:rcd_ber_expand_model_20c}
\end{figure*}


==> sec/latvar/subplots/rcd_ber_pattern_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{\dimm{0}{A}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/crucial_ber_pattern_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/crucial_b1_ber_pattern_20c.pdf}
    }
    %
    \subcaptionbox{\dimm{0}{B}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/hynix_ber_pattern_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/hynix_p1_ber_pattern_20c.pdf}
    }
    %
    \subcaptionbox{\dimm{0}{C}.\label{fig:pattern_vc}}[0.3\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/samsung_y_ber_pattern_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/samsung_y17_ber_pattern_20c.pdf}
    }
    %
    %\subcaptionbox{Vendor C-Batch2.}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.28\linewidth]{plots/trcd/ber/ber_pattern_plots/samsung_g_ber_pattern_20c.pdf}
    %}
    \caption{BERs due to four different data patterns as \trcd varies.}
    \label{fig:rcd_ber_pattern_20c}
\end{figure*}


==> sec/latvar/subplots/rcd_ber_temp.tex <==
\begin{figure*}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{\dimm{0}{A}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/crucial_b1_rcd7.5_temp_violin}.pdf}
        \includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/crucialb1_temp_bars}.pdf}
    }
    %
    \subcaptionbox{\dimm{0}{B}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/hynix_p1_rcd7.5_temp_violin}.pdf}
        \includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/hynixp1_temp_bars}.pdf}
    }
    %
    \subcaptionbox{\dimm{0}{C}.}[0.3\textwidth]
    {
        %\includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/samsung_y17_rcd7.5_temp_violin}.pdf}
        \includegraphics[width=0.3\linewidth]{{plots/trcd/ber/ber_temp_plots/samsungy17_temp_bars}.pdf}
    }
    %
    %\subcaptionbox{Vendor C, DIMM g1.}[0.3\textwidth]
    %{
    %    \includegraphics[width=0.25\linewidth]{plots/trcd/ber/ber_temp_plots/samsung_g1.pdf}
    %}

    \caption{BERs of various DRAM DIMMs operating under different temperatures.}
        %(average with 95\% confidence intervals).}
    \label{fig:rcd_ber_temp}
\end{figure*}


==> sec/latvar/subplots/rcd_error_breakdown_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A.}[0.24\textwidth]
    {
        \includegraphics[width=0.23\linewidth]{plots/trcd/bargraph/crucial_rcd_err_b1_3_18.pdf}
    }
    %
    \subcaptionbox{Vendor B.}[0.24\textwidth]
    {
        \includegraphics[width=0.23\linewidth]{plots/trcd/bargraph/hynix_rcd_err_25C_p1_3_6.pdf}
    }
    %
    \subcaptionbox{Vendor C-Batch1.}[0.24\textwidth]
    {
        \includegraphics[width=0.23\linewidth]{plots/trcd/bargraph/samsung_rcd_err_25C_y17_19_22.pdf}
    }
    %
    \subcaptionbox{Vendor C-Batch2.}[0.24\textwidth]
    {
        \includegraphics[width=0.23\linewidth]{plots/trcd/bargraph/samsung_rcd_err_25C_g1_5_15.pdf}
    }

    \caption{Breakdown on the fraction of cache lines containing 0, 1, or $\ge$2
    erroneous bits in different DIMMs with varying tRCD values (ns) at 20\celsius.}
    \label{fig:rcd_error_breakdown_20c}
\end{figure*}


==> sec/latvar/subplots/rcd_error_breakdown_pattern_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A, DIMM b1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/crucial_rcd_err_b1_ff_00_cc_aa.pdf}
    }
    %
    \subcaptionbox{Vendor B, DIMM p1.\label{fig:vb-p1-errbar-pattern-20c}}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/hynix_rcd_err_p1_ff_00_cc_aa.pdf}
    }
    %
    \subcaptionbox{Vendor C-Batch1, DIMM g1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/samsung_rcd_err_g1_ff_00_cc_aa.pdf}
    }
    %
    \subcaptionbox{Vendor C-Batch2, DIMM y17.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/samsung_rcd_err_y17_ff_00_cc_aa.pdf}
    }

    \caption{Different data patterns running at different
        tRCD parameters at 20\celsius.}
    \label{fig:rcd_error_breakdown_pattern_20c}
\end{figure*}


==> sec/latvar/subplots/rcd_error_breakdown_temp.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A, DIMM b1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/crucial_rcd_err_b1_26_35_50_70C.pdf}
    }
    %
    \subcaptionbox{Vendor B, DIMM p1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/hynix_rcd_err_p1_26_35_50_70C.pdf}
    }
    %
    \subcaptionbox{Vendor C, DIMM g1.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/samsung_rcd_err_g1_26_35_50_70C.pdf}
    }
    %
    \subcaptionbox{Vendor C, DIMM y17.}[0.225\textwidth]
    {
        \includegraphics[width=0.225\linewidth]{plots/trcd/bargraph/samsung_rcd_err_y17_26_35_50_70C.pdf}
    }

    \caption{Breakdown on the fraction of cache lines containing 0, 1, or $\ge$2
        erroneous bits in different DIMMs with varying tRCD parameters operating
        under different temperatures.}
    \label{fig:rcd_error_breakdown_temp}
\end{figure*}


==> sec/latvar/subplots/rp_ber_20c.tex <==
\begin{figure*}[h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    \subcaptionbox{Vendor A.}[0.28\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trp/ber/crucial_ber_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trp/ber/trp_model_ber_plots/crucial_trp_model_ber.pdf}
    }
    %
    \subcaptionbox{Vendor B.}[0.28\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trp/ber/hynix_ber_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trp/ber/trp_model_ber_plots/hynix_trp_model_ber.pdf}
    }
    %
    \subcaptionbox{Vendor C.}[0.28\textwidth]
    {
        %\includegraphics[width=0.28\linewidth]{plots/trp/ber/samsung_y_ber_20c.pdf}
        \includegraphics[width=0.28\linewidth]{plots/trp/ber/trp_model_ber_plots/samsung_trp_model_ber.pdf}
    }
    %
    %\subcaptionbox{Vendor C-Batch2.}[0.28\textwidth]
    %{
    %    \includegraphics[width=0.28\linewidth]{plots/trp/ber/samsung_g_ber_20c.pdf}
    %}

    \caption{Bit error rates (BERs) of various DRAM DIMMs by their models running at different \trp parameters.}
    \vspace{5pt}
    \label{fig:rp_ber_20c}
\end{figure*}


==> sec/latvar/subplots/scaling.tex <==
\begin{figure*}[!h]
    \centering
    %\captionsetup[subfigure]{justification=centering}
    \captionsetup[subfigure]{justification=justified}

    \subcaptionbox{\trcd xx.\vspace{0.1in}\label{fig:scaling_trcd}}%[\linewidth]
    {
        \includegraphics[scale=1]{plots/scaling_tRCD}
    }

    \subcaptionbox{\trp xx.\label{fig:scaling_trp}}%[\linewidth]
    {
        \includegraphics[scale=1]{plots/scaling_tRP}

    }

    \caption{xxxx.}
    \label{fig:scaling}
\end{figure*}


==> sec/latvar/subplots/timing_reduced.tex <==
\begin{figure}[h]
    \centering
    \captionsetup[figure]{justification=centering}
    \includegraphics[width=1.0\linewidth]{plots/timing_reduced}
    \caption{DRAM Operation with Reduced Timings}
    \label{fig:timing_reduced}
\end{figure}


==> sec/latvar/subplots/y17_rcd3_dimm_heatmap_20c.tex <==
\begin{figure}[!h]
    \centering

    \subcaptionbox{Bank0}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank0_ecc0}.pdf} }
    \subcaptionbox{Bank1}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank1_ecc0}.pdf} }

    \subcaptionbox{Bank2}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank2_ecc0}.pdf} }
    \subcaptionbox{Bank3}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank3_ecc0}.pdf} }

    \subcaptionbox{Bank4}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank4_ecc0}.pdf} }
    \subcaptionbox{Bank5}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank5_ecc0}.pdf} }

    \subcaptionbox{Bank6}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank6_ecc0}.pdf} }
    \subcaptionbox{Bank7}[0.48\linewidth] {
    \includegraphics[width=0.48\linewidth]{plots/trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank7_ecc0}.pdf} }
    \caption{Probability of errors in \dimm{0}{C} at \trcd=7.5ns.}
    \label{fig:dimm_y17_rcd3}
\end{figure}


==> sec/latvar/subplots/y19_rp_ecc_heatmap_20c.tex <==
\begin{figure*}[h]
    \centering

    \subcaptionbox{No EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{{plots/trp/heatmap/samsung_heatmap_trp/samsungy19/ecc0/filecnt_36_hist_128x16384_samsungy19_rp7.5ns_allpatts_20c_bank1_ecc0}.pdf}
    }
    \subcaptionbox{1EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{{plots/trp/heatmap/samsung_heatmap_trp/samsungy19/ecc1/filecnt_36_hist_128x16384_samsungy19_rp7.5ns_allpatts_20c_bank1_ecc1}.pdf}
    }
    \subcaptionbox{2EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{{plots/trp/heatmap/samsung_heatmap_trp/samsungy19/ecc2/filecnt_36_hist_128x16384_samsungy19_rp7.5ns_allpatts_20c_bank1_ecc2}.pdf}
    }
    \subcaptionbox{3EC}[0.22\linewidth] {
        \includegraphics[width=0.22\linewidth]{{plots/trp/heatmap/samsung_heatmap_trp/samsungy19/ecc3/filecnt_36_hist_128x16384_samsungy19_rp7.5ns_allpatts_20c_bank1_ecc3}.pdf}
    }

        \caption{Effect of ECC on \dimm{2}{C} at \trp=7.5ns at 20\celsius.}
    \label{fig:y19_rp_ecc_heatmap_20c}
\end{figure*}


==> sec/latvar/trcd_err_location.tex <==
\subsection{Spatial Locality of Activation Errors}
\label{sec:trcd_loc}

To understand the locations of activation errors within a DIMM, we show the
probability of experiencing at least one bit error in each cache line
over a large number of
experimental runs. Due to limited space, we present the results of two
representative DIMMs from our experiments.

Figure~\ref{fig:err_loc} shows the locations of activation errors in the first
bank of two DIMMs using \trcde7.5ns. Additional results \new{showing} the error
locations in every bank for \new{some DIMMs} are available
online~\cite{safari-github}. The x-axis and y-axis indicate the cache line
number and row number (in thousands), respectively. In our tested DIMMs, a row
size is 8KB, \new{comprising} 128 cache lines (64 bytes). \new{Results} are
gathered from 40 and 52 iterations of tests for \dimm{0}{C} and \dimm{3}{A},
respectively.

\input{sec/subplots/err_loc}
\input{sec/subplots/burst_rcd3_20c}

The main observation on \dimm{0}{C} (\figref{rcd_col_err}) is that errors tend
to cluster at certain \emph{columns of cache lines}. For the majority of the
remaining cache lines in the bank, we observe no errors throughout the
experiments. We observe similar characteristics in other DIMMs from the same
model. In addition, we observe clusters of errors at certain regions.
\new{For example}, \dimm{3}{A} (\figref{rcd_err_region}) shows that the activation
errors repeatedly occur within the first half of the majority of rows.

%\figputHW{trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank0_ecc0}.pdf}{rcd_col_err}{Bank 0 of \dimm{0}{C} under \trcde7.5ns at 20\celsius.}
%\figputHSL{trcd/heatmap/samsungy17_1124/ecc0/{filecnt_40_hist_128x16384_samsungy17_rcd7.5ns_allpatts_20c_bank0_ecc0}.pdf}{0.8}{Bank 0 of \dimm{0}{C} under \trcde7.5ns at 20\celsius.}{rcd_col_err}

%\figputHW{trcd/heatmap/y7_1125/ecc0/{filecnt_52_hist_128x16384_y7_rcd7.5ns_allpatts_20c_bank0_ecc0}.pdf}{rcd_err_region}{Bank 0 of \dimm{3}{A} under \trcde7.5ns at 20\celsius.}
%\figputHSL{trcd/heatmap/y7_1125/ecc0/{filecnt_52_hist_128x16384_y7_rcd7.5ns_allpatts_20c_bank0_ecc0}.pdf}{0.8}{Bank 0 of \dimm{3}{A} under \trcde7.5ns at 20\celsius.}{rcd_err_region}

We hypothesize that the cause of \new{such spatial locality of errors is due to
the locality of} variation in the fabrication process during manufacturing:
certain cache line locations can end up with less robust components, such as
weaker sense amplifiers, weaker cells, or higher resistance bitlines.

\obs{Activation errors do not occur uniformly within \new{DRAM. They instead}
exhibit strong spatial concentration at certain regions.}

\subsection{Density of Activation Errors}
\label{sec:density_err}

In this section, we investigate how errors are distributed within the erroneous
cache lines. We present the distribution of error bits at the granularity of
\emph{data beats}\new{, as conventional error-correcting codes (ECC)
work at the same granularity. We discuss the effectiveness of employing
ECC in Section~\ref{sec:rcd_ecc}}. Recall from \secref{dram_access} that a cache line
transfer consists of eight 64-bit data beats.

%A data beat is a 64-bit data chunk that a DIMM transfers
%through the 64-bit data bus connected between the processor and DRAM module.
%In total, reading a 64-byte cache line results in a burst of 8 data beats.

\figref{burst_rcd3_20c} shows the distribution of error bits observed in each
data beat of all erroneous cache lines when using \trcde7.5ns. We show
experiments from 9 DIMMs, categorized into three DIMM models (one per vendor).
We select the model that observes the lowest average BER from each vendor, and
show the frequency of observing 1, 2, 3, and $\ge$4 error bits in each data
beat. The results are aggregated from all DIMMs of the selected models. We make
two observations.

First, most data beats experience only fewer than 3 error bits at \trcde 7.5ns. We
observe that more than 84\%, 53\%, and 91\% of all the recorded activation
errors are just 1-bit errors for DIMMs in A-M1, B-M1, and C-M0, respectively.
\new{Across all of the cache lines that contain at least one error bit, 82\%,
41\%, and 85\% of the data beats that make up each cache line have no errors for
A-M1, B-M1, and C-M0, respectively.} Second, when \trcd is reduced to 5ns, the
number of errors increases. The distribution of activation errors in data beats
when using \trcde5ns is \newt{available online~\cite{safari-github}}, and it
shows that 68\% and 49\% of data beats in A-M1 and C-M0 still have no more than
one error bit.

%\trcde5ns is available in Appendix~\ref{app_err_bursts}, and it shows that 68\%
%and 49\% of data beats in A-M1 and C-M0 still have no more than one error bit.

\obs{\newt{For cache lines that experience activation errors, the majority of
their constituent data beats contain either no errors or just a 1-bit error.}}

%%%%%%% High ber results %%%%%%%%%
%\subsubsection{Error Distribution under High BER}
%\figputHW{trcd/heatmap/high_ber/filecnt_12_hist_128x16384_p1_rcd3_pattff00_20c_bank0_ecc0.pdf}{rcd_high_err}{Bank
%0 of DIMM B2 under \trcde7.5ns at 20\celsius.}
%\figref{rcd_high_err} -- results are gathered from 12 experimental runs.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Effect of Error Correction Codes}
\label{sec:rcd_ecc}

As shown in the previous section, a majority of data beats in erroneous cache
lines contain only a few error bits. In contemporary DRAM, ECC is used to detect
and correct errors at the granularity of data beats. Therefore, this creates an
opportunity for applying error correction codes (ECC) to correct \new{activation
errors}. To study of the \new{effect of ECC}, we perform an analysis that
uses various strengths of ECC to correct activation errors.

\figref{err_free_rcd3_new} shows the percentage of cache lines that do
\new{\emph{not}} observe any activation errors when using \trcde 7.5ns at
various ECC strengths, ranging from single to triple error bit correction. These
results are gathered from the same 9 DIMMs used in
Section~\ref{sec:density_err}. The first bar of each group is the percentage of
cache lines that do not exhibit any activation errors in our experiments. The
following data bars show the fraction of error-free cache lines after applying
single, double, and triple error correction codes.

%\figputGHS{err_free_rcd3_new}{1}{Percentage of error free cache lines due to various
%strengths of error correction (EC) with \trcde7.5ns.}
\figputGHW{err_free_rcd3_new}{Percentage of error-free cache lines with various
strengths of error correction (EC), with \trcde7.5ns.}
%\vspace{-5pt}

We make two observations. First, without any ECC support, a large fraction of
cache lines can be read reliably without any errors in many of the DIMMs we
study. Overall, 92\% and 99\% of cache lines can be read without any activation
errors from A-M1 and C-M0 DIMMs, respectively. On the other hand, B-M1 DIMMs are
\new{more} susceptible to reduced activation latency\new{: only 12\% of their
cache lines can be read without any activation errors.}

\obs{A majority of cache lines can be read without any activation errors in most
    of our tested DIMMs. However, some \newt{DIMMs} are very susceptible to
activation errors, resulting in a small fraction of error-free cache lines.}

Second, ECC is very effective in correcting the activation errors.  For example,
with a single error correction code (1EC), which is widely deployed in many
server systems, the fraction of reliable cache lines improves from 92\% to 99\%
for A-M1 DIMMs. Even for B-M1 DIMMs, which exhibit activation errors in a large
fraction of cache lines, \new{the} triple error correcting code is able to
improve the percentage of \new{error-free} cache lines from 12\% to 62\%.

\obs{ECC is an effective mechanism to correct activation errors, even in
modules with a large fraction of erroneous cache lines.}

%\input{sec/subplots/b1_rcd_ecc_heatmap_20c}
%\figref{b1_rcd_ecc_heatmap_20c} -- results are gathered from 6 experimental runs using pattern \pattff and \pattzero.
%\input{sec/subplots/p6_rcd_ecc_heatmap_20c}
%\figref{p6_rcd_ecc_heatmap_20c} -- results are gathered from 12 experimental runs using pattern \pattff and \pattzero.


==> sec/lisa/abstract.tex <==
% !TEX root = ../paper.tex

This paper introduces a new DRAM design that enables fast and energy-efficient
bulk data movement across subarrays in a DRAM chip.  While bulk data movement is
a key operation in many applications and operating systems, contemporary systems
perform this movement inefficiently, by transferring data from DRAM to the
processor, and then back to DRAM, across a narrow off-chip channel. The use of
this narrow channel for bulk data movement results in high latency and energy
consumption.  Prior work proposed to avoid these high costs by exploiting the
\emph{existing} wide internal DRAM bandwidth for bulk data movement, but the
limited connectivity of wires within DRAM allows fast data movement
within only a single DRAM subarray. Each subarray is only a few megabytes in
size, greatly restricting the range over which fast bulk data movement can
happen within DRAM.% a DRAM chip.

% Bulk data movement has been demonstrated to be an essential operation in a wide
% range of applications and operating system functions. However, performing this
% movement in contemporary systems can be slow and can consume significant
% energy, as the movement requires data to go through the processor, forcing it
% to traverse a pin-limited off-chip channel (typically 64 bits wide) between the
% processor and DRAM.  There has been prior work to enable hardware support for
% bulk data movement wholly within DRAM, by exploiting the wide bandwidth
% available within the DRAM chip and avoiding the pin-limited channel.  While the
% wide bandwidth can improve movement latency and energy efficiency, the limited
% internal connectivity in existing DRAM architectures  provides such bandwidth
% for transfers \emph{only within one DRAM subarray}.  Unfortunately, each
% subarray, the smallest building block in today's DRAM chips, contains only a few
% megabytes of data, greatly restraining the opportunities for efficient
% movement.

We propose a new DRAM substrate, \capfullname (\lisa), whose goal is to enable
fast and efficient data movement across a large range of memory at low cost.
\lisa adds low-cost connections \emph{between} adjacent subarrays.  By using
these connections to interconnect the existing internal wires (\emph{bitlines})
of adjacent subarrays, \lisa enables wide-bandwidth data transfer across
multiple subarrays with little (only 0.8\%) DRAM area overhead.  As a DRAM
substrate, \lisa is versatile, enabling an array of new applications.  We
describe and evaluate three such applications in detail: (1)~fast inter-subarray
bulk data copy, (2)~in-DRAM caching using a DRAM architecture whose rows have
heterogeneous access latencies, and (3)~accelerated bitline precharging by
linking multiple precharge units together. Our extensive evaluations show that
each of LISA's three applications significantly improves performance and memory
energy efficiency, and their combined benefit is higher than the benefit of
each alone, on a variety of workloads and system configurations.

% The goal of this work is to enable fast and efficient data movement across a
% large range of memory at low cost.  We propose a new DRAM substrate,
% \lisafullname (\lisa), that adds low-cost connections \emph{between} subarrays
% to provide a wide bandwidth data transfer across multiple subarrays.  We take
% advantage of the vertical wires within existing subarrays, called
% \emph{bitlines}, each of which connects a column of cells together. While
% bitlines are not currently connected across two different subarrays, we observe
% that the bitlines of adjacent subarrays lie very close to each other. We propose
% to use low-cost isolation transistors to \emph{interconnect} these bitlines,
% forming a wide-bandwidth datapath between adjacent subarrays. Through this wide
% connection, we can move data in one subarray to another subarray at low latency
% and energy.

% \lisa is a versatile substrate, which can enable a large array of DRAM
% architecture optimizations.  We describe and evaluate three such optimizations
% in detail: (1)~fast inter-subarray bulk data copy, (2)~in-DRAM caching using a
% heterogeneous-latency DRAM architecture, and (3)~accelerated bitline precharging
% by linking multiple precharge units together. Our evaluation shows that, with an
% area overhead of just 0.8\% of a DRAM chip, these three optimizations
% (individually and in combination) significantly improve system performance and
% memory energy efficiency.

%%%%%%%%%%%%%%%%%%%%%% IGNORE %%%%%%%%%%%%%%%%%%%%%%%%%%

\ignore{We evaluate three such optimizations in detail: (1)~fast inter-subarray bulk
copy, which reduces the latency and memory energy of a bulk copy operation by
9.2x and 48.1x over prior work, respectively. This results in 59.6\%
performance improvement and 53.6 DRAM energy reduction over a range of copy
workloads; (2)~in-DRAM caching using a heterogeneous-latency DRAM architecture,
which improves multi-core system performance by 5.1\% (up to 16.1\%); and
(3)~accelerated bitline precharging by linking multiple precharge units
together, which improves system performance by 8.1\%. \lisa requires an area
overhead of just 0.8\% of a DRAM chip.}


==> sec/lisa/abstract_hpca_v1.tex <==
With ever increasing data demand from applications and growing compute power,
the performance and energy efficiency of DRAM-based memory systems have become
more important in today's systems. Unfortunately, commodity DRAM merely serves
as a data storage that is controlled by the processor to move the data in and
out of DRAM at the cache line granularity (i.e., 64B). This paper identifies a
low-cost DRAM design that can rapidly move a large amount of data (e.g., 8KB)
across subarrays within individual banks. This design enables five memory
architectural techniques to improve system performance and memory energy
efficiency.

This paper proposes \fullname (\lisa), the first DRAM substrate to enable such
fast data movement support across subarrays in a bank without moving data out of
DRAM. The key idea is to insert isolation transistors to interconnect bitlines
of subarrays that are in close proximity. This substrate is versatile, and we
quantitatively evaluate three out of the five architectural optimizations. The
first optimization reduces the latency of an inter-subarray bulk-copy operation
within a bank by 88.9\% over prior work. Second, \lisa enables a heterogeneous
in-DRAM caching scheme to improve system performance by up to 16.1\% on a 4-core
system. Lastly, \lisa leverages multiple precharge units to reduce the precharge
latency by 63.6\%. When combined, these optimizations deliver 94.8\% performance
improvement and 49\% energy savings at 0.8\% DRAM chip area overhead.

\ignore{
Existing approaches to move data are bottlenecked by memory channels between the
memory and processor, and DRAM-internal data bus. These two mediums provide
narrow data bandwidth at the cache line level. However, expanding these buses
requires significant modification to the modification and area overhead.
The insight in this work is that within each subarray, bitlines serve a row-wide
bus that connects DRAM cells to sense amplifiers. However, these bitlines are
disconnected across subarrays. We observe that subarrays are symmetrical and in
close proximity in each bank. Therefore, the key idea is to insert ...}


==> sec/lisa/abstract_old.tex <==
% ISCA
\ignore{
Contemporary DRAM has been architected using subarray structures to support
high-density memory devices. Unfortunately, there is no support in DRAM today
for quickly transferring data between subarrays within the same bank.  This
shortcoming actually limits or prevents many performance- and energy-oriented
optimizations within DRAM, such as high-speed bulk data copy across subarrays,
low-latency DRAM operations, and efficient in-DRAM caching.

This paper proposes \fullname (\lisa), the first DRAM substrate to enable such
support for inter-subarray \isos within a bank.  The key idea is to use
isolation transistors to interconnect bitlines of subarrays that are in close
proximity. This substrate is versatile, and we show that it can enable at least
five architectural optimizations, three of which we evaluate exhaustively. The
first optimization reduces the latency of an inter-subarray bulk-copy operation
within a bank by 88.9\% over prior work. The second reduces the precharge
latency by 74.5\%. Lastly, \lisa enables an in-DRAM caching scheme to improve
system performance by up to 7.9\% on a 4-core system. When combined, these
optimizations can deliver significant performance improvements and energy
savings at 0.8\% DRAM chip area overhead.
}

\ignore{
This paper proposes \fullname (\lisa), the first DRAM substrate to enable such
support for inter-subarray \isos within a bank.  The key idea is to use
isolation transistors to interconnect bitlines of subarrays that are in close
proximity.  This substrate is versatile, and we show that it can enable at
least five architectural optimizations, three of which we evaluate
exhaustively.  Over a wide spectrum of applications and microkernels, each of
these optimizations can deliver performance improvements.  When all three are
combined, \lisa can improve performance by 2.61x, while reducing DRAM energy
consumption by 79.1\%, over using existing DDR3 DRAM for a variety of quad-core
workloads that consist of copy- and memory-intensive benchmarks.
}

\ignore{
The main memory channel represents a critical bottleneck in modern
systems, as data must travel off-chip between the processor and DRAM,
incurring a long latency with a constrained bandwidth.  For operations
that move or copy data between two memory locations, this off-chip
movement is wasteful, incurring not only long latencies but consuming
additional energy.  Typically, the only reason this data needs to go
to the processor chip is due to limitations in current DRAM design,
where the datapath design prevents direct communications between rows
without using the memory channel.

We propose a new DRAM substrate, \fullname (\lisa), that provides simple
modifications to improve the interconnectivity of DRAM. The implementation of
\lisa is simple -- it uses isolation
transistors to connect bitlines of subarrays that are in close proximity. Using \lisa, we can
provide an in-DRAM means of transferring data across different subarrays, which
was not possible previously. Our substrate is versatile, and it enables several
architectural optimizations.

First, we support fast inter-subarray bulk data copies without the need to use
the memory channel, resulting in performance improvements and energy savings
over a number of applications. Second, we show how our substrate can
significantly reduce the precharge latency by connecting two precharge units.
Third, our substrate enables an efficient implementation of an in-DRAM caching
scheme on heterogeneous DRAM with fast subarrays in every bank. By enabling all
three optimizations, \lisa improves performance by 2.61x and reduces energy
consumption by 79.1\% compared to \\baseline. In all, we provide details on
how to implement five different optimizations using our new substrate.
}

%%
\ignore{
We propose a new DRAM substrate, \fullname, that provides simple
modifications that improve the interconnectivity of DRAM. By taking
advantage of the subarrays in the open bitline architecture, we can
provide an in-DRAM means of transferring data across different
subarrays, which was not possible previously.  Our substrate is
versatile, and can enable several architectural and system-level
optimizations.  In particular, we can support inter-subarray transfers
and copies without the need to use the memory channel, resulting in
performance improvements and energy savings over a number of
applications.  We also show how our substrate can reduce the precharge
latency.  In all, we provide details on how to implement five
different optimizations using our new substrate.
}


==> sec/lisa/ack.tex <==
\vspace{-0.06in}
\section*{Acknowledgments}
\vspace{-0.05in}
%\textbf{Acknowledgments.}

We thank the anonymous reviewers and SAFARI group members for their helpful
feedback. We acknowledge the support of Google, Intel, Nvidia, Samsung, and
VMware. This research was supported in part by the ISTC-CC, SRC, CFAR, and NSF
(grants 1212962, 1319587, and 1320531). Kevin Chang is supported in part by the
SRCEA/Intel Fellowship.


==> sec/lisa/background_short.tex <==
% !TEX root = ../paper.tex

\section{Background: DRAM Organization}
\label{sec:background}

A modern DRAM system consists of a hierarchy of components: channels, ranks,
banks, and subarrays. A memory channel drives DRAM commands, addresses, and data
between a memory controller and a group of DRAM ranks. Within a
rank, there are multiple banks that can serve memory requests (i.e., reads or
writes) concurrently, independent of one another.\footnote{Physically, a rank
consists of multiple DRAM chips. Every chip in a rank operates in lockstep
to serve fragments of data for the same request. Many prior
works provide further details on DRAM rank
organization~\cite{udipi-isca2010, zhang-isca2014}.}

\subsection{DRAM Subarrays}
\label{sec:background:dram}

In this work, we focus on operations across subarrays within the \emph{same}
bank. Typically, a bank is subdivided into multiple
\emph{subarrays}~\cite{chang-hpca2014, kim-isca2012, seshadri-micro2013,
vogelsang-micro2010}, as shown in \figref{background_bank_sa_detail}.
%\footnote{Note that we are illustrating a logical view of the bank.  Throughout
%this section, we abstract away the multiple chips that physically exist within
%a rank for the sake of clarity.} Note that we are illustrating the bank
%structure at a logical level that covers all eight chips in a \texttt{x8} rank
%to abstract away the physical-level detail for clarity.}
Each subarray consists of a 2D-array of DRAM cells that are connected to sense
amplifiers through \emph{bitlines}. Because the size of a sense amplifier is
more than 100x the size of a cell~\cite{lee-hpca2013}, modern DRAM designs
    fit in only enough sense amplifiers in a row to sense \emph{half a row of
cells}. To sense the \emph{entire} row of cells, each subarray has bitlines that
connect to \emph{two rows} of sense amplifiers --- one above and one below the
cell array (\circled{1} and \circled{2} in \figref{background_bank_sa_detail},
for Subarray 1).
This DRAM design is known as the \emph{open bitline architecture}, and is
commonly used to achieve high-density DRAM~\cite{lim-isscc2012,
takahashi-jsscc2001}. For the rest of the paper, we refer to a single
row of sense amplifiers, which holds the data from \emph{half} a row of
activated cells, as a \emph{row buffer}.

%\figputHS{lisa_back_hpca}{1.0}{DRAM bank and subarray Organization.}
%\figputHS{background_bank_sa_detail}{1.0}{DRAM bank and subarray Organization.}
\figputHW{background_bank_sa_detail}{Bank and subarray organization in a
DRAM chip.}
%\figputHS{lisa_back_hpca_times}{1.0}{DRAM bank and subarray Organization.}


\subsection{DRAM Subarray Operation}
\label{sec:background:access}

Accessing data in a subarray requires two steps. The DRAM row (typically 8KB
across a rank of eight x8 chips) must first be \emph{activated}. Only
after activation completes, a column command (i.e., a \crd/\cwr)
can operate on a piece of data (typically 64B across a rank; the
size of a single cache line) from that row.

When an \act command with a row address is issued, the data stored within a row
in a subarray is read by \emph{two} row buffers (i.e., the row buffer at the
top of the subarray \circled{1} and the one at the bottom \circled{2}). First,
a wordline corresponding to the row address is selected by the subarray's row
decoder. Then, the top row buffer and the bottom row buffer
each sense the charge stored in half of the row's cells through the bitlines,
and amplify the charge to full digital logic values (0 or 1) to latch in the
cells' data.

After an \act finishes latching a row of cells into the row buffers, a
\crd or a \cwr can be issued. Because a typical read/write memory request is
made at the granularity of a single cache line, only a subset of bits are
selected from a subarray's row buffer by the column decoder.
%, typically 64B out of 8KB.
On a \crd, the selected column bits are sent to the global sense
amplifiers through the \emph{internal data bus} (also known as the global data
lines) \circled{3}, which has a narrow width of 64B across a rank of eight
chips. The global sense amplifiers \circled{4} then drive the data to the bank
I/O logic \circled{5}, which sends the data out of the DRAM chip to the memory
controller.

While the row is activated, a consecutive column command to the same row can
access the data from the row buffer without performing an additional \act. This
is called a \emph{row buffer hit}. In order to access a different row, a \cpre
command is required to reinitialize the bitlines' values for another \act. This
re-initialization process is completed by a set of \emph{precharge units}
\circled{6} in the row buffer. For more detail on DRAM commands and internal
DRAM operation, we refer the reader to prior works~\cite{kim-isca2012,
lee-hpca2015, lee-hpca2013, liu-isca2012, seshadri-micro2013, son-isca2013}.


==> sec/lisa/conclusion.tex <==
% !TEX root = ../paper.tex

\section{Conclusion} \label{sec:conclusion}

We present a new DRAM substrate, \emph{\fullname (\lisa)}, that expedites bulk
data movement across subarrays in DRAM. \lisa achieves this by creating a new
high-bandwidth datapath at low cost between subarrays, via the insertion of a
small number of isolation transistors. We describe and evaluate three
applications that are enabled by \lisa. First, \lisa significantly reduces the
latency and memory energy consumption of bulk copy operations between subarrays
over two state-of-the-art mechanisms~\cite{seshadri-micro2013}. Second, \lisa
enables an effective in-DRAM caching scheme on a new heterogeneous DRAM
organization, which uses fast subarrays for caching hot data in every bank.
Third, we reduce precharge latency by connecting two precharge units of
adjacent subarrays together using \lisa. We experimentally show that the three
applications of LISA greatly improve system performance and memory energy
efficiency when used individually or together, across a variety of workloads
and system configurations.

We conclude that \lisa is an effective substrate that enables several effective
applications. We believe that this substrate, which enables low-cost
interconnections between DRAM subarrays, can pave the way for other applications
that can further improve system performance and energy efficiency through fast
data movement in DRAM.


==> sec/lisa/eval.tex <==
% !TEX root = ../paper.tex

\section{Evaluation} \label{sec:eval}

We quantitatively evaluate our proposed applications of \lisa: (1)~rapid bulk
copying (\lisarc), (2)~in-DRAM caching with heterogeneous subarrays
(\lisavilla), and (3)~reduced precharge time (\lisapre).

\subsection{Bulk Memory Copy}
\label{sec:eval_lisaclone}

\subsubsection{Single-Core Workloads} \figref{1c_perf} shows the performance of
three copy benchmarks on a single-core system with one memory channel and 1MB
of last-level cache (LLC). We evaluate the following bulk copy mechanisms:
(1)~\baseline, which copies data over the memory channel; (2)
\rc~\cite{seshadri-micro2013}; and (3) \lisarc. We use two different hop counts
between the source and destination subarray for \mbox{\lisarc}: 15 (longest)
and 1 (shortest). They are labeled as \lisarc-15 and \lisarc-1, respectively,
in the figure. We make four major observations.

\input{plots/1c_copy_results}

First, \lisarc achieves significant improvement over \mbox{\rcirsa} for all three
benchmarks in terms of both IPC and memory energy consumption, shown in
\figref{1c_ipc} and \figref{1c_e}, respectively. This shows that the LISA
substrate is effective at performing fast inter-subarray copies.

Second, both \lisarc-1 and \lisarc-15 significantly reduce the memory energy
consumption over \baseline. This is due to (1)~reduced memory traffic over the
channel by keeping the data within DRAM, and (2)~higher performance.

%by
%58.0\%, 94.7\%, and 77.1\% for \texttt{bootup}, \texttt{forkbench}, and
%\texttt{shell}, respectively.

Third, \lisarc-1/-15 provides 12.6\%/10.6\%, 4.9x/4.3x, and 1.8\%/0.7\% speedup
for \texttt{bootup}, \texttt{forkbench}, and \texttt{shell}, respectively, over
\baseline. The performance gains are smaller for \texttt{bootup} and
\texttt{shell}. Both of these benchmarks invoke fewer copy operations (i.e.,
2171 and 2682, respectively) than \texttt{forkbench}, which invokes a large
number (40952) of copies. As a result, \texttt{forkbench} is more sensitive to
the memory latency of copy commands. Furthermore, the large LLC capacity (1MB)
helps absorb the majority of memory writes resulting from \baseline for
\texttt{bootup} and \texttt{shell}, thereby reducing the effective latency of
\baseline.

Fourth, \rcirsa performs \emph{worse} than \baseline for \texttt{bootup} and
\texttt{shell} due to its long \emph{blocking} copy operations. Although, it
attains a 19.4\% improvement on \texttt{forkbench} because \baseline causes
severe \emph{cache pollution} by installing a large amount of copied data into
the LLC. Compared to the 20\% cache hit rate for \baseline, \rcirsa has a much
higher hit rate of 67.2\% for \texttt{forkbench}. The copy performance of
\baseline is strongly correlated with the LLC management policy and size.

To understand performance sensitivity to LLC size, \figref{1c_cache_sweep} shows
the speedup of \lisarc-1 over \baseline for different LLC capacities. We make
two observations, which are also similar for \lisarc-15 (not shown). First, for
\texttt{bootup} and \texttt{shell}, the speedup of LISA over \baseline reduces
as the LLC size increases because the destination locations of \baseline
operations are more likely to hit in the larger cache.
%Thus, this negative effect of \baseline is likely to become exacerbated as the
%effective cache capacity decreases. cache interference increases with more
%cores or threads.

Second, for \texttt{forkbench}, LISA-RISC's performance gain over \baseline
decreases as cache size reduces from 1MB to 256KB. This is because the LLC hit
rate reduces much more significantly for \lisarc, from 67\% (1MB) to 10\%
(256KB), than for \baseline (from 20\% at 1MB, to 19\% at 256KB). When
\texttt{forkbench} uses \lisarc for copying data, its working set mainly
consists of non-copy data, which has good locality. As the LLC size reduces by
4x, the working set no longer fits in the smaller cache, thus causing a
significant hit rate reduction. On the other hand, when \baseline is used as the
copy mechanism, the working set of \texttt{forkbench} is mainly from bulk copy
data, and is less susceptible to cache size reduction. Nonetheless,
\mbox{\lisarc} still provides an improvement of 4.2x even with a 256KB cache.

We conclude that \lisarc significantly improves performance and memory energy
efficiency in single-core workloads that invoke bulk copies.

%The reason
%why \baseline's hit rate is much lower than \lisarc for larger LLC (1MB) is that
%\lisarc avoids \emph{cache pollution} from copied data by performing
%\emph{in-memory copies}. Therefore, the copy performance of \baseline is
%strongly correlated with the LLC management policy and size.

\subsubsection{Multi-Core Workloads}

\figref{4c_copy_perf} shows the system performance and energy efficiency (i.e.,
memory energy per instruction) of different copy mechanisms across 50 workloads,
on a quad-core system with two channels and 4MB of LLC. The error bars in this
figure (and other figures) indicate the 25th and 75th percentile values across
all 50 workloads. Similar to the performance trends seen in the single-core
system, \lisarc consistently outperforms other mechanisms at copying data
between subarrays. \lisarc-1 attains a high average system performance
improvement of 66.2\% and 2.2x over \baseline and \rcirsa, respectively.
Although Mix~5 has the smallest number of copy operations out of the five
presented workload mixes, \lisarc still improves its performance by 6.7\% over
\baseline. By moving copied data only within DRAM, \lisarc significantly reduces
memory energy consumption (55.4\% on average) over \baseline. In summary,
\lisarc provides both high performance and high memory energy efficiency for
bulk data copying for a wide variety of single- and multi-core workloads.

\input{plots/4c_copy_results}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{In-DRAM Caching with \lisavilla}
\label{sec:eval_lisavilla}

\figref{villa_multic_errbar} shows the system performance improvement of
\lisavilla over a baseline without any fast subarrays in a four-core system. It
also shows the hit rate in \villa, i.e., the fraction of accesses that hit in
the fast subarrays. We make two main observations. First, by exploiting \lisarc
to quickly cache data in \villa, \lisavilla improves system performance for a
wide variety of workloads --- by up to 16.1\%, with a geometric mean of 5.1\%.
This is mainly due to reduced DRAM latency of accesses that hit in the fast
subarrays (which comprise 16MB of total storage across two memory channels).
The performance improvement heavily correlates with the VILLA cache hit rate.
Our work does not focus on optimizing the caching scheme, but the hit rate may
be increased by an enhanced caching policy
(e.g.,~\cite{qureshi-isca2007,seshadri-pact2012}), which can further improve
system performance.

\figputGHWHeight{villa_multic_errbar}{Performance improvement and hit rate with \lisavilla, and
performance comparison to using \rcirsa with \villa.}{1}

Second, the \villa design, which consists of heterogeneous subarrays, is not
practical without \lisa. \figref{villa_multic_errbar} shows that using
\rcirsa to move data into the cache \emph{reduces} performance by 52.3\% due to
slow data movement, which overshadows the benefits of caching. The results indicate
that \lisa is an important substrate to enable not only fast bulk data
copy, but also a fast in-DRAM caching scheme.

%villa rc base
%2.724 1.238 2.593 % 5.1% improvement, -52.3% for rc
%avg hit rate = lisa:0.317 rc:0.183


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Accelerated Precharge with \lisapre}
\label{sec:eval_lisapre}

\figref{pre_norm_ws_4c_multic} shows the system performance improvement of
\lisapre over a baseline that uses the standard DRAM precharge latency, as well
as \lisapre's row-buffer hit rate, on a four-core system across 50
workloads. \lisapre attains a maximum gain of 13.2\%, with a mean improvement of
8.1\%. The performance gain becomes higher as the row-buffer hit rate decreases,
which leads to more precharge commands. These results show that \lisa is a
versatile substrate that effectively reduces precharge latency in addition to
accelerating data movement.

\figputGHWHeight{pre_norm_ws_4c_multic}{Speedup and row buffer (RB) hit rate of
\lisapre.}{0.85}

We also evaluate the effectiveness of combining \lisavilla and \lisapre (not
shown, but available in our technical report~\cite{chang-tr2016}). The combined
mechanism, which is transparent to software, improves system performance by
12.2\% on average and up to 23.8\% across the same set of 50 workloads without
bulk copies. Thus, LISA is an effective substrate that can enable mechanisms to
fundamentally reduce memory latency.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Putting Everything Together}
\label{sec:everything_results}

As all of the three proposed applications are complementary to each other, we
evaluate the effect of putting them together on a four-core system.
\figref{all_norm_ws_4c} shows the system performance improvement of adding
\lisavilla to \lisarc (15 hops), as well as combining all three optimizations,
compared to our baseline using \baseline and standard DDR3-1600 memory. We draw
several key conclusions. First, the performance benefits from each scheme are
additive. On average, adding \lisavilla improves performance by 16.5\% over
\lisarc alone, and adding \lisapre further provides an 8.8\% gain over
\lisarcvilla. Second, although \lisarc alone provides a majority of the
performance improvement over the baseline (59.6\% on average), the use of
both \mbox{\lisavilla} and \mbox{\lisapre} further improves performance,
resulting in an average performance gain of 94.8\% and memory energy reduction
(not plotted) of 49.0\%. Taken together, these results indicate that \lisa is
an effective substrate that enables a wide range of high-performance and
energy-efficient applications in the DRAM system.

%\figputGHW{all_norm_ws_4c}{Combined WS improvement of \lisa applications.}
\figputGHWHeight{all_norm_ws_4c}{Combined WS improvement of \lisa
applications.}{0.97}
\vspace{-2pt}

\subsection{Sensitivity to System Configuration}

\figref{4c_sensitivity_errbar} shows the weighted speedup for \baseline and
\mbox{\lisa-All} (i.e., all three applications) on a 4-core system using varying
memory channel counts and LLC sizes. The results show that performance
improvement increases with fewer memory channels, as memory contention
increases.  On the other hand, adding more memory channels increases
memory-level parallelism, allowing more of the copy latency to be hidden.
Similar trends are observed with the LLC capacity. As LLC size decreases,
the working set becomes less likely to fit with \baseline,
worsening its performance. \lisa-All provides significant performance
benefits for all configurations.

\figputGHWHeight{4c_sensitivity_errbar}{Performance sensitivity to channels and LLC
size.}{0.85}
\vspace{-2pt}

\subsection{Effect of Copy Distance on \lisarc}

\tabref{4c_lisa_sweep} shows that the performance gain and memory energy savings
of \lisarc over \baseline increases as the copy distance reduces. This is
because with fewer subarrays between the source and destination subarrays, the
number of \xfer commands invoked by \lisarc reduces accordingly, which decreases
the latency and memory energy consumption of bulk data copy.

\input{sec/tables/4c_lisa_sweep}


==> sec/lisa/eval_isca.tex <==
\section{Evaluation} \label{sec:eval}

In this section, we quantitatively evaluate three
optimizations enabled by \lisa: (1) rapid in-DRAM copy, called \lisarc
(Section~\ref{sec:lisaclone}), (2) reduced
precharge time, called \lisapre (Section~\ref{sec:lisapre}), and (3) in-DRAM caching with heterogeneous
subarrays, called \lisavilla (Section~\ref{sec:villa}).

\subsection{In-DRAM Copy Mechanisms}
 \label{sec:eval_lisaclone}

\newcommand{\rcintersa}[0]{{RC Inter-SA}\xspace}
\newcommand{\rcintrasa}[0]{{RC Intra-SA}\xspace}
\newcommand{\rcinterb}[0]{{RC Inter-Bank}\xspace}

\subsubsection{Single-Core Performance} \figref{1c_copy_ipc} shows the
performance of the copy-intensive benchmarks on a single-core system. We
evaluate the following copy mechanisms: (1) \\baseline, which transfers one
cache line at a time through the memory channel (\emph{Baseline}), (2) the three
RowClone methods, \emph{RC Inter-SA (subarray), RC Inter-Bank, and RC Intra-SA},
that copy data within different DRAM components, and (3) our proposed copy
mechanism that uses the \lisa substrate (\lisarc). For \lisarc, we use two
configurations for the subarray distance (hop counts) between the source and
destination subarrays: (1) the shortest distance with 1 hop count and (2) the
longest distance with 15 hop counts within each bank that has 16 subarrays. We
make several major observations.

\figputGHS{1c_copy_ipc}{1.0}{Single-core performance for various copy methods.}

First, \rcintersa performs similarly to \\baseline mechanism because it also
copies one cache line at a time serially within DRAM. Second, by pipelining
reads and writes across banks to transfer data, \rcinterb achieves
higher performance than \rcintersa by 25.4\% on average. Third, \rcintrasa
improves performance significantly, by
47.5\% and 85.0\% on average over \rcinterb and \rcintersa, respectively. This is because
\rcintrasa has a much smaller copy latency than the other two mechanisms, while
allowing the rank to continue serving requests. Because \rcinterb moves data
across the internal data bus shared by all banks, it prevents the entire rank
from serving requests, despite the data only moving between two banks.

Fourth, \lisarc achieves significant performance gains over the \rcintersa by
77.4\% and 70.0\% on average with hop counts of 1 and 15, respectively. The main
reason is that \lisarc exploits the large data bandwidth provided by \lisa to
transmit data between subarrays without using the small-bandwidth global data
lines. Fifth, the system performance only degrades by 4.2\% when the copy
distance between two subarrays increases from 1 subarray to 15 subarrays.
\tabref{1c_lisa_sweep} shows the system performance sensitivity of \lisarc as
the subarray hop count increases. As shown, the performance degradation is
minimal with higher hop counts because the transfer latency between subarrays is
very small (8ns for every transfer across two subarrays). Lastly, \lisarc
performs within 4.0\% of \rcintrasa, while being able to provide much higher
copy range and granularity control over the amount of data to copied.

\input{sec/tables/1c_lisa_sweep}

\figputGTS{1c_copy_e}{1.0}{Single-core energy efficiency for various copy methods.}

\subsubsection{Single-Core Energy Consumption} \figref{1c_copy_e} shows the
energy consumption of these copy mechanisms on the same single-core system. We
draw two major conclusions. First, similar to the observations on system
performance, \rcintrasa provides a significant reduction on the energy
consumption of 89.1\%, and \lisarc reduces the energy consumption by
approximately the same amount (6.5\% worse than \rcintrasa). Second, copy
energy becomes dominant in the copy-intensive forkbench, taking up 85.7\% of
total energy for \\baseline. Third, although \rcintersa attains similar system
performance as \\baseline, it consumes 24.2\% less energy than \\baseline by
transferring data without using the external memory channel.

\subsubsection{Combining \lisarc and RowClone} To demonstrate the efficacy of
\lisarc with \rc, we replace the \rcintersa mechanism with \lisarc in the \rc
framework. \figref{1c_copy_frac} compares the performance of the \rc framework
to \rc combined with \lisarc as the ratio of the number of intra-subarray copy
command to the inter-subarray copy command changes. In addition, we also show
the performance of \\baseline method and inter-subarray-only \lisarc
as reference points. We observe that the combination of
\lisarc and \rc provides much higher performance than just using \rc. For
instance, when the fraction of intra-subarray copies is 50\%, the combination
provides 41.1\% higher performance than \rc alone. In summary, \lisarc not only
provides high performance, but also high energy efficiency. By using \lisa as a
substrate for in-DRAM copying, the in-DRAM copy framework becomes more complete
and energy efficient.

\figputGTS{1c_copy_frac}{1.0}{Single-core performance due to different amounts of
intra-subarray copies.}
\figputGTS{4c_copy_norm_lisa}{1.0}{Performance improvement due to \lisa over \\baseline for 50 workloads.}

\subsubsection{Multi-Core Results}

\tabref{4c_copy_norm_ws} shows the average system performance of different copy
mechanisms for a 4-core system across 50 workloads. We also evaluate an ideal
scheme that takes zero cycle to copy data. We draw the following
conclusions. First, the performance benefits of copy mechanisms with shorter
copy latency become higher in a multi-core system than in a single-core system. On
average, \lisarc and \rcintrasa improve system performance by 2.13x and 2.26x
over \\baseline, respectively. This is because the memory system becomes more contended in a
multi-core system, as each memory copy command blocks the service of memory
requests from multiple applications. Therefore, faster service times for the memory
copy command allow the memory to serve more memory requests from multiple
cores. Second, similar to the single-core system, \lisarc consistently improves
system performance over \rcinterb and \rcintersa, and it performs very
closely to the \rcintrasa and ideal mechanisms.

\input{sec/tables/4c_copy_norm_ws}

\figputGTWS{1c_pre_ipc}{1.0}{Performance impact of \lisa on single-core benchmarks.}

\figref{4c_copy_norm_lisa} compares the system performance of \lisarc to the
\baseline system. The numbers are sorted based on \lisarc's performance. In
addition, it also shows the number of copy operations performed for each
workload. There are two key takeaways. First, \lisarc consistently improves
system performance across a wide range of workloads. The benefit increases as
the workloads become more copy-intensive with more copy calls. Second, the
performance improvement significantly increases for certain workloads because of
higher memory copy operations. Based on our results, we conclude that \lisa is
an effective substrate to enable a fast copy mechanism with improved performance
and energy for systems running a variety of workloads.

%%%%%%%%%%%%%%%%%%%%%%

\subsection{Dual Precharge with \lisapre}
\label{sec:eval_lisapre}

\subsubsection{Single-Core Performance} \figref{1c_pre_ipc} shows the
performance and read latency improvement due to \lisapre on all of our
benchmarks. The percentage values on top of the bars indicates the minimum,
median, maximum, and average performance gains. The main takeaway from our
results is that \lisapre improves performance for most of the
benchmarks compared to \\baseline. On average, \lisapre attains an 8.3\%
improvement, with a maximum gain of 20.1\%. The performance benefits are the
highest for those benchmarks that have a higher memory latency.

% norm scurve
%\figputGHS{pre_norm_ws_4c}{1.0}{Performance improvement of \lisa-PRE on a 4-core system.}

\subsubsection{Multi-Core Performance} \figref{multic_pre_ws+e} shows the
system performance and energy consumption for 2-core (1 channel) and 4-core (2
channels) systems. In addition to \\baseline and \lisapre, we show an ideal
zero-cycle precharge scheme. The percentage numbers show the
improvement due to \lisapre. First, as the
memory contention increases with higher core counts, the benefits of \lisapre
increase, resulting in 13.5\% and 14.7\% average performance improvement
for 2-core and 4-core systems, respectively. Second, as expected, a similar
trend is observed for energy consumption, because \lisapre is able to reduce the
execution time of these workloads with its faster precharge time. Lastly, \lisapre
performs within 3.2\% and 3.8\% to the ideal scheme for 2-core and 4-core
systems. As a result, exploiting the \lisa substrate to perform double precharge
operations provides significant improvement in system performance and energy
efficiency.

\figputGHS{multic_pre_ws+e}{1.0}{Performance improvement as the core count varies.}

\subsection{In-DRAM Caching with \lisavilla}
\label{sec:eval_lisavilla}

\figref{villa_norm_ws_4c} shows the performance improvement due to \lisavilla
over a \baseline without any fast subarrays in a 4-core system. By exploiting
\lisa to quickly cache data in \villa, \lisavilla improves system performance by
3.2\% on average, and up to 7.9\%. The average hit rate in the fast subarray is
50.3\% and the average migration count is 27970. Because our work does not focus
on optimizing the caching scheme, the hit rate may be further increased by an
enhanced caching policy. Nonetheless, this software-transparent caching scheme
would not be able to improve performance without \lisa. In fact, using either
\\baseline or \rc to cache data reduces system performance due to the high
cost of data movement. Therefore, we conclude that \lisa also enables a fast
in-DRAM cache scheme with low overhead.

%\figputGHS{villa_norm_ws_4c}{1.0}{Performance improvement due to \lisavilla.}
\figputGTS{villa_norm_ws_4c}{1.0}{Performance improvement due to \lisavilla.}
\figputGTS{all_norm_ws_4c}{1.0}{Performance improvement of different
optimizations.}

\subsection{Putting Everything Together}

Because all the proposed optimizations are orthogonal to each other, we evaluate
the effect of putting them together on a 4-core system. \figref{all_norm_ws_4c}
shows the system performance improvement of adding just \lisavilla to \lisarc,
as well as combining all three optimizations. We draw several key conclusions.
First, the performance benefits from each scheme are additive. On average,
adding \lisavilla improves performance by 6.7\% over \lisarc alone, and adding
\lisapre further provides an 11.5\% gain over \lisarcvilla. Second, although
\lisarc alone provides a majority of performance improvement over \\baseline
(2.19x on average), the addition of both \lisavilla and \lisapre further
improves the performance, resulting in a significant performance benefit of
2.61x, and an energy reduction of 79.1\%, over \\baseline. We conclude that
\lisa is an effective substrate that enables a wide range of high-performance
and energy-efficient applications in DRAM systems.

%% E base = 748.15
%% E all = 156.0153

%\figputGHS{all_norm_ws_4c}{1.0}{Performance improvement as the core count varies.}


==> sec/lisa/impl.tex <==
% !TEX root = ../paper.tex

%\vspace{-0.05in}
\section{Hardware Cost}
%\vspace{-0.05in}

%\subsection{Die Area Overhead}

\subsection{Die Area Overhead}
\label{sec:hwarea}
 To evaluate the area overhead of adding isolation
transistors, we use area values from prior work, which adds isolation
transistors to disconnect bitlines from sense amplifiers~\cite{o-isca2014}. That
work shows that adding an isolation transistor to every bitline incurs a total of
0.8\% die area overhead in a 28nm DRAM process technology. Similar to prior work
that adds isolation transistors to DRAM~\cite{lee-hpca2013,o-isca2014}, our
\lisa substrate also requires additional control logic outside the DRAM banks to
control the isolation transistors, which incurs a small amount of area and is
non-intrusive to the cell arrays. For \lisavilla, we use 1024 six-bit saturating
counters to track the access frequency of rows in every bank; this
requires an additional 6KB storage within a memory controller connected to one rank.

%\subsection{Handling Repaired Rows}

\subsection{Handling Repaired Rows} To improve yield, DRAM manufacturers often
employ post-manufacturing repair techniques that can remap faulty rows to
spare rows provisioned in every subarray~\cite{keeth-dram-tutorial}.
Therefore, consecutive row addresses as observed by the memory controller may
physically reside in \emph{different} subarrays. To handle this issue for
techniques that require the controller to know the subarray a row resides in
(e.g., RowClone~\cite{seshadri-micro2013}, \lisarc), a simple approach can be
used to expose the repaired row information to the memory controller. Since
DRAM already stores faulty rows' remapping information inside the chip, this
information can be exposed to the controller through the serial presence
detect (SPD)~\cite{jedec-spd}, which is an EEPROM that stores DRAM information
such as timing parameters. The memory controller can read this stored
information at system boot time so that it can correctly determine a repaired
row's location in DRAM. Note that similar techniques may be necessary for
other mechanisms that require information about physical location of rows in
DRAM (e.g.,~\cite{chang-hpca2014, kang14, kim-isca2014, kim-isca2012,
lee-hpca2013, liu-isca2013}).

\ignore{
\subsection{ISA Support for \rc and \lisarc} To enable applications to use the \rc
framework, Seshadri et al.~\cite{seshadri-micro2013} introduce a new ISA
instruction for bulk data copy, which has similar semantics to the existing bulk
instructions in x86 processors (e.g., \texttt{rep movsw}). If the system uses a
DRAM with the \lisa substrate, \lisarc can be added into the \rc framework, and
the memory controller can choose which bulk copy commands to use based on the
operands of \texttt{memcopy}.
}

%Some changes to the DRAM interface?
%\textbf{Clone Implementation.} Subarray exposure and other issues?
%\textbf{Precharge Implementation.} \todo{The internal precharge command would raise the
%isolation transistors.}

%%%%%%%%%%%%%%%%%
% based on tl-dram numbers
%%%%%%%%%%%%%%%%%

%\subsection{Die Area Overhead}
%
%To evaluate the area overhead of isolation transistors that connect two
%subarrays, we use the area values from a prior work that adds isolation
%transistors in the subarray between cells~\cite{lee-hpca2013}. We conservatively
%assume that adding an isolation transistor increases the height of a subarray
%even though it is added around a sense amplifier instead of in the array itself,
%which may potentially have spare area. The area of a sense amplifier and an
%isolation transistor are respectively 115.2x and 11.5x taller than an individual
%DRAM cell. By adding two isolation transistors around each sense amplifier, the
%area overhead is $\frac{11.5\times2}{115.2+512}=3.66\%$. Prior
%work~\cite{lee-hpca2013} shows that with the additional area of the peripheral
%and I/O circuitry in DRAM, the area overhead results in approximately 3.15\%.


==> sec/lisa/intro.tex <==
% !TEX root=../paper.tex

\section{Introduction} \label{sec:intro}

Bulk data movement, the movement of thousands or millions of bytes between two
memory locations, is a common operation performed by an increasing number of
real-world applications (e.g.,~\cite{kanev-isca2015, lee-hpca2013,
    ousterhout-usenix1990, rosenblum-sosp1995, seshadri-cal2015,
    seshadri-micro2013, son-isca2013, sudan-asplos2010,zhao-iccd2005}).
    Therefore, it has been the target of several architectural optimizations
    (e.g.,~\cite{blagodurov-usenix2011, jiang-pact2009, seshadri-micro2013,
    wong-fpt2006, zhao-iccd2005}). In fact, bulk data movement is important
    enough that modern commercial processors are adding specialized support to
    improve its performance, such as the ERMSB instruction recently added to the
    x86 ISA~\cite{intel-optmanual2012}.

In today's systems, to perform a bulk data movement between two locations in
memory, the data needs to go through the processor \emph{even though both the
source and destination are within memory}. To perform the movement, the data is
first read out one cache line at a time from the source location in
memory into the processor caches, over a pin-limited off-chip channel (typically
64~bits wide). Then, the data is written back to memory, again one cache line at
a time over the pin-limited channel, into the destination location. By going
through the processor, this data movement incurs a significant penalty in terms
of latency and energy consumption.

%\input{sec/tables/migration_opt}
%\input{sec/tables/migration_opt_short}

While it is clear that fast \emph{inter-subarray} data movement can have several
applications that improve system performance and memory energy
efficiency~\cite{kanev-isca2015, ousterhout-usenix1990,
rosenblum-sosp1995,seshadri-cal2015,seshadri-micro2013,zhao-iccd2005}, there is
currently no mechanism that performs such data movement quickly and
efficiently.  This is because \emph{no wide datapath exists today between
subarrays} within the same bank (i.e., the connectivity of subarrays is low
    in modern DRAM). \textbf{Our goal} is to design a low-cost
    DRAM substrate that enables fast and energy-efficient data movement
\emph{across subarrays}.

% To this end, we aim to improve the connectivity of subarrays within each bank.
%moving data across subarrays within the same bank is bottlenecked by the narrow
%internal data bus.

%The rows \emph{within} a subarray are interconnected by \emph{bitlines}, which
%allow the contents of an \emph{entire row} to be moved between the DRAM cells
%and the \emph{row buffer}.

We make two key observations that allow us to improve the connectivity of
subarrays within each bank in modern DRAM. First, accessing data in DRAM causes
the transfer of an entire row of DRAM cells to a buffer (i.e., the \emph{row
buffer}, where the row data temporarily resides while it is read or written)
via the subarray's \emph{bitlines}. Each bitline connects a column of cells
to the row buffer, interconnecting every row within the same subarray
(\figref{intro_baseline}). Therefore, the bitlines essentially serve as a very
wide bus that transfers a \emph{row's worth of data} (e.g., 8K~bits) at once.
Second, subarrays within the same bank are placed in close proximity to each
other. Thus, the bitlines of a subarray are very close to (but are not currently
connected to) the bitlines of neighboring subarrays (as shown in
\figref{intro_baseline}).

\vspace{5pt}
\noindent\textbf{Key Idea.} Based on these two observations, we introduce a new
DRAM substrate, called \emph{\lisafullname} (\emph{\lisa}). \lisa enables
\emph{low-latency, high-bandwidth inter-subarray connectivity} by linking
neighboring subarrays' bitlines together with \emph{isolation transistors}, as
illustrated in \figref{intro_lisa}. We use the new inter-subarray connection in
\lisa to develop a new DRAM operation, \emph{\xferfull (\xfer)}, which moves
data that is latched in an activated row buffer in one subarray into an inactive
row buffer in another subarray, without having to send data through the narrow
internal data bus in DRAM. \xfer exploits the fact that
the activated row buffer has enough drive strength to induce charge perturbation
within the idle (i.e., \emph{precharged}) bitlines of neighboring subarrays,
allowing the destination row buffer to sense and latch this data when the
isolation transistors are enabled.

By using a rigorous DRAM circuit model that conforms to the JEDEC
standards~\cite{jedec-ddr3} and ITRS
specifications~\cite{itrs-fep-2013,itrs-interconnect-2013}, we show that \xfer
performs inter-subarray data movement at 26x the bandwidth of a modern 64-bit
DDR4-2400 memory channel (500~GB/s vs.\ 19.2~GB/s; see~\refsec{trans_lat}), even
after we conservatively add a large (60\%) timing margin to account for process
and temperature variation.

%reduces the transfer time of a row by 26x compared to a modern DRAM.
%\todo{26x, thereby greatly reduces the transfer time}

\vspace{5pt}
\noindent\textbf{Applications of \lisa.} We exploit LISA's \emph{fast
inter-subarray movement} to enable many applications that can improve system
performance and energy efficiency. We implement and evaluate the following three
applications of \lisa:
%\tabref{migration_opt_short} lists several example
%applications of LISA, from which we evaluate the first three:

\begin{itemize}

    \item \textbf{Bulk data copying.} Fast inter-subarray data movement can eliminate
     long data movement latencies for copies between two locations in the same
     DRAM chip. Prior work showed that such copy operations are widely used in
     today's operating systems~\cite{ousterhout-usenix1990,rosenblum-sosp1995}
     and datacenters~\cite{kanev-isca2015}. We propose \underline{R}apid
     \underline{I}nter-\underline{S}ubarray \underline{C}opy
     (\emph{\lisarcnol}), a new bulk data copying mechanism based on LISA's \xfer
     operation, to reduce the latency and DRAM energy of an inter-subarray copy
     by 9.2x and 48.1x, respectively, over the best previous mechanism,
     \rc~\cite{seshadri-micro2013} (\refsec{lisaclone}).

    \item \textbf{Enabling access latency heterogeneity within DRAM.} Prior
        works~\cite{lee-hpca2013, son-isca2013} introduced non-uniform access
        latencies within DRAM, and harnessed this heterogeneity to provide a
        data caching mechanism within DRAM for hot (i.e., frequently-accessed)
        pages. However, these works do not achieve either one of the following
        goals: (1)~low area overhead, and (2)~fast data movement from the slow
        portion of DRAM to the fast portion. By exploiting the \lisa substrate,
        we propose a new DRAM design,
        \underline{V}ar\underline{I}ab\underline{L}e \underline{LA}tency
        (\emph{\lisavillanol}) DRAM, with asymmetric subarrays that reduce the
        access latency to hot rows by up to 63\%, delivering high system
        performance and achieving both goals of low overhead and fast data
        movement (\refsec{villa}).

    \item \textbf{Reducing precharge latency.} Precharge is the process of
        preparing the subarray for the next memory access~\cite{jedec-ddr3,
        kim-isca2012, lee-hpca2015, lee-hpca2013}. It incurs latency that is on
        the critical path of a bank-conflict memory access. The precharge
        latency of a subarray is limited by the drive strength of the precharge
        unit attached to its row buffer. We demonstrate that \lisa enables a new
        mechanism, \underline{LI}nked \underline{P}recharge
        (\emph{\lisaprenol}), which connects a subarray's precharge unit with
        the idle precharge units in the neighboring subarrays, thereby
        accelerating precharge and reducing its latency by 2.6x (\refsec{lisapre}).

     %We discuss the background on a precharge operation in
     %Section~\ref{sec:background}, and explain our mechanism in
     %Section~\ref{sec:lisapre}.

\end{itemize}
These three mechanisms are complementary to each other, and we show that when
combined, they provide additive system performance and energy efficiency
improvements (\refsec{everything_results}). LISA is a versatile DRAM substrate, capable of supporting several
other applications beyond these three, such as performing efficient data
remapping to avoid conflicts in systems that support subarray-level
parallelism~\cite{kim-isca2012}, and improving the efficiency of bulk bitwise
operations in DRAM~\cite{seshadri-cal2015} (see \refsec{other_apps}).

% \tabref{migration_opt_short} summarizes two other examples of
% applications that can be efficiently implemented on top of \lisa (see
% \secref{other_apps} for detailed descriptions).

%\todo{Due to
%lack of space, we defer detailed explanations and evaluations to future
%work.}

%%% Original paragraph %%%
\ignore{
As discussed earlier, fast inter-subarray migration has several applications. We
use \lisa, and our new row buffer migration operation, to implement and
quantitatively evaluate two of them: (1)~rapid inter-subarray copy, and (2)~hot
data caching in fast subarrays within a heterogeneous DRAM design. In addition,
we demonstrate that our substrate enables a mechanism to reduce memory
latency by accelerating precharge operations. (We discuss background on the
precharge operation in Section~\ref{sec:background}, and explain our mechanism
in Section~\ref{sec:lisapre}.) These three mechanisms are complementary to
each other, and we show that they significantly improve system performance
and energy efficiency when combined.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

This paper makes the following major contributions:
\begin{itemize}%[leftmargin=0.75cm]

\item We propose a new DRAM substrate, \emph{\lisafullname} (\emph{\lisa}),
     which provides high-bandwidth connectivity between subarrays within the same
     bank to support bulk data movement at low latency, energy, and cost (\refsec{lisa}).

 %\item We demonstrate, using a SPICE model that conforms to JEDEC and ITRS
 %    specifications, that \lisa performs inter-subarray data movement at 26x the
 %    bandwidth of a modern 64-bit DDR4-2400 memory channel (500~GB/s vs.\
 %    19.2~GB/s; see~\refsec{trans_lat}) even after we conservatively
 %    add a large timing margin of 60\% to account for process variation.

 \item We propose and evaluate three new applications that take
     advantage of \lisa: (1)~Rapid Inter-Subarray Copy (\emph{\lisarcnol}), which
     copies data across subarrays at low latency and low DRAM energy;
     (2)~Variable Latency (\emph{\lisavillanol}) DRAM, which reduces the access
     latency of hot data by caching it in fast subarrays; and (3)~Linked
     Precharge (\emph{\lisaprenol}), which reduces the precharge latency for a
     subarray by linking its precharge units with neighboring idle precharge
     units.

 \item We extensively evaluate LISA's applications individually and combined
     together. Our evaluation shows that (1)~RISC improves average system
     performance by 66\% over workloads that perform intensive bulk data movement and
     (2)~VILLA/LIP improve performance by 5\%/8\% over a wide variety of
     workloads. Combining all three applications improves system performance by
     94\% and reduces memory energy by 49\% on a 4-core system running workloads
     with intensive bulk data movement (\refsec{everything_results}).

 % \item We comprehensively evaluate the performance and energy benefits of the
  %   three optimizations \lisa enables. \tabref{migration_opt} shows the key
  %   benefits of these optimizations. Because they are complementary to each
  %   other, our results show that combining them significantly improves system
  %   performance by 94.8\% and reduces memory energy by 49\% on a 4-core system
  %   (Section~\ref{sec:eval}).

\end{itemize}


==> sec/lisa/intro_hpca_v1.tex <==
% !TEX root=../paper.tex

\section{Introduction} \label{sec:intro}

% Over the past few decades, DRAM-based main memory has become an important system
% performance limiter, as the performance gap between processors and main memory
% continues to increase.  The two constraints limiting memory performance are the
% long memory access latencies and narrow memory bandwidth, which are collectively
% referred to as the \emph{memory wall}~\cite{wulf-can95, mckee-cf2004}.  In
% particular, the narrow bandwidth between the processor and main memory can be
% especially problematic when performing larger-scale memory operations.  For
% example, in a commodity system, duplicating data within main memory requires
% the data to be transmitted, one cache line at a time, from the memory to the
% processor and back, creating a significant bottleneck and consuming unnecessary
% energy for off-chip transfers.

In this work, we observe that enabling \emph{fast bulk-data movement} within
DRAM can alleviate this bottleneck.  There are several use cases that benefit from
a fast data movement connection.  First, as we already mentioned, data copying between two
DRAM locations benefits significantly from avoiding costly off-chip transfers,
and such copy operations are widely used~\cite{zhao-iccd2005, vaidyanathan-cc2007, jiang-pact2009,
seshadri-micro2013}.  A second application is rapid data migration, where two
frequently accessed DRAM rows lie within the same DRAM structure (i.e., bank,
subarray)~\cite{sudan-asplos2010, jeong-hpca2012, kim-isca2012}.  Rapid data
movement makes it practical to perform migration when such conflicts occur, as
the overhead for migration can be reduced significantly.  In-memory computation
also benefits from a fast data movement connection, such as prior work that has
proposed to perform bulk bitwise Boolean logic within
DRAM~\cite{seshadri-cal2015}.  If these applications are forced to transfer
data over the pin-limited connection between the processor and DRAM, the
performance and energy overhead will be so high that many of these applications
no longer become viable.


% SAUGATA: *new* paragraph 2 below

In-DRAM data migration is limited by the amount of wire connectivity that exists
within a DRAM chip. A modern DRAM chip, as shown in
Figure~\ref{fig:dram-overview}, is divided into several levels of hierarchy. A
single chip consists of multiple \emph{banks}. Each bank can only service a
single DRAM command at a time.  Each bank is further decomposed into several
\emph{subarrays}~\cite{kim-isca2012, seshadri-micro2013, vogelsang-micro2010},
each containing a subset of rows of DRAM cells. The rows \emph{within} a
subarray are interconnected by \emph{bitlines}, which allow the contents of an
\emph{entire row} to be moved between the DRAM cells and the \emph{row buffer},
which contains a series of \emph{sense amplifiers} that can drive the contents
of a selected DRAM row.

Unfortunately, there is no such row-width connectivity
that exists outside of the subarray: inter-subarray and inter-bank
communications must be performed across the internal DRAM bus, which has the
same narrow width (typically 64~bits) as the external DRAM channel.

The prior state-of-the-art in data migration,
RowClone~\cite{seshadri-micro2013}, takes advantage of the \emph{existing}
in-DRAM connectivity at three different granularities, as illustrated in
Figure~\ref{fig:dram-overview}:
\begin{enumerate}
    \item RowClone can use the bitlines within the subarray to perform
        \emph{fast intra-subarray migration}, as the existing bitlines allow an
        entire row of data to be migrated to another row in the same subarray
        in a single operation.

    \item RowClone introduces a new DRAM command that enables data
        \emph{inter-bank migration} (i.e., between two \emph{different} banks.
        This requires the data to be transferred in a pipelined fashion, as
        it must move across the narrow internal DRAM bus. This limitation
        makes inter-bank migration much slower than intra-subarray migration.

    \item RowClone also leverages the pipelined data transfer mechanism from
        inter-bank migration to perform \emph{inter-subarray migration} (i.e.,
        between two different subarrays \emph{in the same bank}). To achieve
        this, RowClone performs inter-bank migration to temporarily copy the
        data into a different bank, and then performs a \emph{second} inter-bank
        migration to save the data back into the original bank. This operation
        is very slow, and because it ties up the internal DRAM bus for a long
        duration, it can block read or write commands \emph{going to other
        banks} from executing.
        % TODO: should we add a pointer to \ref{sec:lisaclone:shortcomings}?
\end{enumerate}
While RowClone can deliver very fast intra-subarray migration, it has two major
shortcomings. First, it is difficult for a system to exploit fast migration at
such a small granularity, as the OS must consciously allocate a destination
memory page for migration within the same subarray as the source page. Today,
the OS has no knowledge of the subarray-level partitioning within DRAM, making
the probability quite low that a source and destination page will be in the same
subarray. Second, for inter-subarray migration, RowClone actually performs worse
than today's mechanism that moves data out of the DRAM due to its long blocking
operation. Our evaluation results indicate that RowClone degrades system
performance by 24.0\% compared to today's system when copying data across
subarrays on a quad-core system (Section~\ref{sec:lisaclone}). Overall, it is
difficult for the benefits of RowClone to be exploited, and it delivers
especially poor performance for inter-subarray migration.


% In this work, we observe that enabling \emph{fast bulk-data movement} across
% subarrays within a bank is important for improving DRAM performance because it
% can enable multiple applications to alleviate the memory wall problem. The first
% application is bulk data copying between DRAM rows across
% subarrays~\cite{zhao-iccd2005, vaidyanathan-cc2007, jiang-pact2009,
% seshadri-micro2013}. This can significantly save the channel bandwidth and
% reduce the bulk-copy latency (Section~\ref{sec:lisaclone}). Second, to reduce
% memory access latency, we can design asymmetric subarrays that provide
% non-uniform access latency and cache the hot data in the fast subarray. The
% efficacy of this optimization is dependent on the latency of data movement
% between slow and fast subarrays (Section~\ref{sec:villa}). Third, when multiple
% frequently accessed DRAM rows are within the same DRAM structure (i.e., bank or
% subarray), the access latency increases due to frequent row buffer misses
% (e.g.,~\cite{sudan-asplos2010, jeong-hpca2012, kim-isca2012}). With fast data
% movement across subarrays, a mechanism can address this problem by
% \emph{migrating} hot rows to different subarrays at low cost to reduce conflicts
% and latency (Section~\ref{sec:opt_qual}). Fourth, fast data movement is critical
% for in-memory computations that rely on efficient data transfers across
% subarrays to improve performance. For instance, prior work has proposed bulk
% bitwise AND and OR and it requires fast data movement without nullifying the
% benefits~\cite{seshadri-cal2015}. Therefore, it's clear that providing fast data
% movement across subarrays is an important problem.

% Unfortunately, existing memory system does not provide efficient bulk inter-subarray
% data movement because data cannot directly transfer between subarrays. The main
% bottleneck is that data have to first transfer across the pin-limited memory
% channels from the memory to the processor before they get written back into
% memory, resulting in a long latency operation. This bottleneck imposes
% fundamental limits on memory-bound operations, and has a significant impact on
% system performance and energy.

%\todo{
%The state-of-the-art work that we know of,
%RowClone~\cite{seshadri-micro2013}, is insufficient in providing fast
%inter-subarray data movement either as its main benefit comes from
%\emph{intra-subarray} cloning. In contrast to the existing system that moves
%data one cache line at a time with individual memory requests, RowClone
%inter-subarray data movement is a \emph{long blocking operation}. This actually
%results in degraded system performance by incurring long queueing latency on
%other memory requests even though the RowClone operation consumes less energy
%without transferring data over the channel. Our evaluation results indicate that
%RowClone degrades system performance by 24.0\%, but improves energy efficiency
%by 5.1\% compared to today's system when copying data across subarrays on a
%quad-core system (Section~\ref{sec:eval_lisaclone}). Therefore, our goal is to
%propose a new design that outperforms both mechanisms in terms of latency and
%energy efficiency for inter-subarray data movement.
% ** But rc is not really a data movement mechanism? is it? **}

% Prior work has examined some of the benefits of performing bulk data movement
% directly within DRAM~\cite{seshadri-micro2013}. This work, RowClone, exploits
% the bulk data movement capability within individual subarrays to copy two DRAM
% rows \emph{within the same subarray} with low latency. Unfortunately, the
% limited size of a subarray greatly restricts the copy range of RowClone--- a row
% of data can only be copied to one of only 511 other rows within a subarray in
% the DRAM we evaluate (for comparison, there are 64K total rows in the DRAM).
% While RowClone also copies data across subarrays, it can only do so using a
% \emph{long blocking operation}.  In fact, as we will show, using RowClone to
% transfer data across subarrays can \emph{degrade} system performance by 24.0\%,
% though it does improve energy efficiency by 5.1\%, when compared to copying data
% on a commodity quad-core system (see Section~\ref{sec:eval_lisaclone} for
% experiment details). Our goal is to design a DRAM substrate that can enable
% fast and energy-efficient data transfer \emph{across subarrays}.

The main source of slowdown for bulk data movement in memory systems is that data
must go through a narrow-bandwidth DRAM-internal bus, serially transferring data
one cache line at a time, as illustrated in \figref{intro_baseline}. The key idea
of our new DRAM substrate is to improve the connectivity between subarrays
within the same bank at low design cost (0.8\% die-area overhead), as
illustrated in \figref{intro_lisa}. Our design, called \emph{\lisafullname}
(\emph{\lisa}), enables high-bandwidth data transfers by linking subarrays through
isolation transistors in the row buffer, leveraging two key characteristics of
today's DRAM: (1) accessing data in DRAM causes the entire row of DRAM cells to
transfer to the corresponding row buffer through their bitlines. The bitlines
essentially serve as a bus to transfer row-wise data, and (2) subarrays within
the same bank are placed in close proximity with each other, thus each
subarray's bitlines are very close to its neighbor subarrays' bitlines, although
they are disconnected. \lisa exploits this proximity by connecting these
subarrays' bitlines using a set of isolation transistors.

\input{plots/intro_motiv}

\input{sec/tables/intro_opt_wide}

With the large-bandwidth connection between subarrays in the same bank, we can
transmit a row of data from one row buffer to another row buffer through the
connected bitlines \emph{without} going through the memory channel. This is
achieved by exploiting the activated row buffer to drive the data. When the
destination row buffer is disabled with its bitlines in the initialization
(i.e., precharged) state, the activated source row buffer is strong enough to
drive these initialized bitlines. Therefore, the destination row buffer can sense
the changes on its own bitlines and help drive the bitlines with the source row
buffer's values, thus latching in the source data.

As a result of using the \lisa substrate, the latency and energy consumption
reduce significantly for fast inter-subarray data movement. This not only enables
multiple optimizations that rely on efficient data movement, as we discussed
before, but it also reduces the DRAM precharge latency, by linking precharge units
from different idle subarrays to accelerate the process. In all, we describe
five architectural optimizations that \lisa enables. A brief description of each
optimization is listed in \tabref{intro_opt_wide}. We qualitatively describe all
of these optimizations in this work, and quantitatively evaluate the benefits of
the first three optimizations.

In this paper, we make the following main contributions:
\begin{itemize}[leftmargin=0.75cm]

  \item We propose a new DRAM substrate, \fullname (\lisa), that provides
    high-bandwidth connections between subarrays within the same bank to support
    bulk data movement at low cost, latency, and energy (Section~\ref{sec:lisa}).

  \item We propose and evaluate three architectural optimizations that build on
      top of \lisa: (1) \lisa-\underline{R}apid
      \underline{I}nter-\underline{S}ubarray \underline{C}opy
      (\emph{\lisarcnol}) copies data across subarrays at low latency and low
      energy consumption (Section~\ref{sec:lisaclone}), (2)
      \lisa-\underline{V}ar\underline{I}ab\underline{L}e \underline{LA}tency
      (\emph{\lisavillanol}) reduces the access latency of hot data by caching it
      in fast subarrays (Section~\ref{sec:villa}), and (3)
      \lisa-\underline{LI}nked \underline{P}recharge (\emph{\lisaprenol})
      reduces precharge latency by linking the about-to-be-precharged subarray's
      precharge units with the nearby idle precharge units
      (Section~\ref{sec:lisapre}).

  \item We comprehensively evaluate the performance and energy benefits of the
    three optimizations \lisa enables. \tabref{intro_opt_wide} shows the key
    benefits of these optimizations. Because they are complementary to each
    other, our results show that combining them significantly improves system
    performance by 94.8\% and reduces memory energy by 49\% on a 4-core system
    (Section~\ref{sec:eval}).

\end{itemize}


==> sec/lisa/intro_isca.tex <==
\section{Introduction} \label{sec:intro}

Modern computer systems continue to experience the \emph{von Neumann bottleneck},
described by Backus as the narrow tube that connects the CPU to its data
store~\cite{backus-cacm1978}. Today, the von Neumann bottleneck exists between
the processor and DRAM, which are connected by pin-limited memory channels.
This bottleneck imposes fundamental limits on memory-bound operations, and often
has a significant impact on system performance, especially when combined with
restrictions in data movement within current DRAM devices.

Contemporary DRAM chips use a subarray-based organization to deliver higher chip
densities. Within each chip, each DRAM \emph{bank} is partitioned into smaller
chunks known as \emph{subarrays} that contain a portion of the total number of
rows within a bank. The connections (i.e., bitlines) \emph{within a subarray}
allow two rows in the same subarray to communicate quickly with each other.
Such connections can enable a number of architectural optimizations within DRAM,
many of which can reduce pressure on Backus' von Neumann bottleneck.

As an example, prior work has leveraged these connections to enable the
\emph{intra-subarray} copying of bulk data (multiple memory pages) between two
rows~\cite{seshadri-micro2013}. Such bulk data copies can be requested by both
user space applications (e.g., \texttt{memcopy}) and operating systems (e.g.,
\texttt{copy\_mm}). However, since wide \emph{inter-subarray} connections do not
exist within DRAM, even within the same bank, this
proposal~\cite{seshadri-micro2013} only works for a limited number of
source-destination pairs. \emph{Inter-subarray} transfers must instead go
through a narrow-bandwidth DRAM-internal data bus even though both source and
destination reside in the same bank (\figref{intro_\baseline}),
incurring \texttildelow11.6x longer latency than intra-subarray
copies~\cite{seshadri-micro2013}. Many such optimizations are restricted in
effectiveness by the lack of a better-interconnected DRAM architecture.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ignore{This bottleneck is particularly detrimental when large amounts of data are
being transferred between two different physical locations within memory.
Currently, the processor must act as a facilitator for such operations---the
data being transferred is first brought into the processor chip, and then is
sent back to the DRAM to its destination location. This procedure forces the
data to travel across the bandwidth-limited memory channel \emph{twice}, quite
inefficient for an operation whose source and destination were both in DRAM.
Alongside the performance disadvantages of forcing two off-chip data transfers,
a significant amount of energy is wasted by unnecessarily sending so much
information across the memory channel.

Allowing data to quickly transfer between two DRAM locations without going
through memory channels enables several optimizations that can significantly
improve the system performance and energy efficiency. One particular prior
work~\cite{seshadri-micro2013} addresses this problem for \emph{only} copying
bulk data (often one or more pages of memory) between two physical locations in
DRAM. Such bulk-data copy operation are typically requested by either user space applications (e.g.,
\texttt{memcopy}) or operating systems (e.g., \texttt{copy\_mm}). The proposal
takes advantage of DRAM \emph{subarray structures} to enable fast copying
between two addresses inside the same subarray (\emph{intra-subarray}). Modern
DRAM chips use the concept of a subarray in order to deliver high chip
densities, partitioning each DRAM \emph{bank} within the chip into smaller
chunks.\footnote{Section~\ref{sec:background} provides a detailed description of
this modern DRAM organization.} However, \emph{inter-subarray} transfers must
still go through a narrow-bandwidth DRAM-internal data bus despite residing in
the same bank, thus incurring \texttildelow11.6x longer latency than
intra-subarray copies~\cite{seshadri-micro2013}, as illustrated in
\figref{intro_\baseline}.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\input{plots/intro_motiv}

\input{sec/tables/intro_opt_wide}

Our goal is to design a new, more flexible DRAM substrate that introduces
improved connectivity between subarrays within the same bank at low design cost
(0.8\% die-area overhead), as illustrated in \figref{intro_lisa}. Our design,
called \emph{\lisafullname} (\lisa), enables high-bandwidth data transfers by
linking subarrays through isolation transistors in the row buffer, leveraging
two key characteristics of today's DRAM: (1) accessing data in DRAM causes the
entire row of DRAM cells to transfer to the corresponding row buffer through
their bitlines, which connect the cells to the row buffer, and (2) subarrays
within the same bank are placed in close proximity with each other, thus each
subarray's bitlines are very close to its neighbor subarrays' bitlines, although
they are disconnected. \lisa exploits this proximity by connecting these
subarrays' bitlines using a set of isolation transistors.

With the large-bandwidth datapath between subarrays in the same bank, we can
transmit data from one row buffer to the neighbor row buffer through the
connected bitlines \emph{without} going to the memory channel. This is achieved by
exploiting the enabled row buffer (activated with a row of data) to drive the
data. When the destination row buffer is disabled with their bitlines in the
initialization (i.e., precharged) state, the source row buffer is strong enough to
drive the initialized bitlines. Therefore, the destination row buffer can sense
the changes on the bitlines due to the source row buffer and also help drive the
bitlines with the source row buffer's values, essentially latching in the source
data.

Our \lisa substrate cuts inter-subarray transfer latency significantly by
transferring a row of data without using the memory channel. We observe that
\lisa exposes several new opportunities to exploit in-DRAM data transfers
between subarrays within the same bank. In all, we describe five architectural
optimizations that \lisa enables. A brief description of each optimization is
listed in \tabref{intro_opt_wide}. We qualitatively describe all of these
optimizations in this work and quantitatively evaluate the benefits of the
first three optimizations.

In this paper, we make the following main contributions:
\begin{itemize}[leftmargin=0.75cm]

  %\item We provide a detailed description of the open bitline DRAM architecture.
  %  and show that it presents an opportunity to create a high-bandwidth path
  %  between subarrays (Section~\ref{sec:background}).

  \item We propose a new DRAM substrate, \fullname (\lisa), that provides
    high-bandwidth connections between subarrays within the same bank
    at low cost and latency (Section~\ref{sec:lisa}).

  \item We show that \lisa enables efficient implementations of several
    architectural and system optimizations using the same substrate
    (Section~\ref{sec:opt}).

  \item We comprehensively evaluate the performance and energy benefits of the
    three optimizations \lisa enables. \tabref{intro_opt_wide} shows the key
    benefits of these optimizations. Because they are complementary to each
    other, our results show that combining them significantly
    improves system performance by 2.61x and DRAM energy efficiency by
    79.1\% on a 4-core system (Section~\ref{sec:eval}).

  %\item We comprehensively evaluate the performance and energy benefits of
  %  \lisa for three optimizations. First, using \lisa to copy data between
  %  subarrays improves performance by 77.4\% and reduces DRAM energy by 73.4\% on
  %  average over the best prior work across a list of copy-intensive
  %  applications (Section~\ref{sec:eval}).

  %\item Second, using \lisa to perform precharge operations with
  %  two precharge units improves performance by 14.7\% on average for a
  %  variety of 4-core workloads (Section~\ref{sec:eval}).

  %\item Third, \lisavilla enables in-DRAM caching
  %  to improve performance by 3.2\% on average and up to 7.9\% for a 4-core
  %  system. Our results show that these three optimizations are
  %  complementary to each other and combining them provides a significant
  %  improvement in system performance by 2.61x and DRAM energy efficiency by
  %  79.1\% (Section~\ref{sec:eval}).

\end{itemize}


==> sec/lisa/lisa.tex <==
% !TEX root = ../paper.tex

\section{Low-Cost Inter-Linked Subarrays (LISA)} \label{sec:lisa}

We propose a new DRAM substrate, \lisa, which enables fast and energy-efficient
data movement across subarrays within a DRAM chip. First, we discuss the
low-cost design changes to DRAM to enable high-bandwidth connectivity across
neighboring subarrays (Section~\ref{sec:lisa:design}).  We then introduce a new
DRAM command that uses this new connectivity to perform bulk data movement
(Section~\ref{sec:bulk_lisa_transfer}).  Finally, we conduct circuit-level
studies to determine the latency of this command (Sections~\ref{sec:trans_lat}
and~\ref{sec:lisa:variation}).

\subsection{\lisa Design}
\label{sec:lisa:design}

\lisa is built upon two key characteristics of DRAM. First, large data bandwidth
\emph{within} a subarray is already available in today's DRAM chips. A row activation
transfers an entire DRAM row (e.g., 8KB across all chips in a rank) into the row buffer via the bitlines of
the subarray. These bitlines essentially serve as a wide bus that transfers an entire
row of data in parallel to the respective subarray's row buffer. Second, every subarray
has its own set of bitlines, and subarrays within the same bank are placed in
close proximity to each other. Therefore, a subarray's bitlines are very close
to its neighboring subarrays' bitlines, although these bitlines are \emph{not} directly
connected together.\footnote{Note that matching the bitline pitch across
    subarrays is important for a high-yield DRAM
process~\cite{lim-isscc2012,takahashi-jsscc2001}.}

By leveraging these two characteristics, we propose to \emph{build a wide
connection path between subarrays} within the same bank at low cost, to
overcome the problem of a narrow connection path between subarrays in commodity
DRAM chips (i.e., the internal data bus \circled{3} in
\figref{background_bank_sa_detail}). \figref{lisa_links_hpca} shows the
subarray structures in \lisa. To form a new, low-cost inter-subarray datapath
with the same wide bandwidth that already exists inside a subarray, we join
neighboring subarrays' bitlines together using \emph{isolation transistors}. We
call each of these isolation transistors a \emph{\iso}. A link connects the
bitlines for the same column of two adjacent subarrays.

\figputHS{lisa_links_hpca}{1.0}{Inter-linked subarrays in \lisa.}

When the isolation transistor is turned on (i.e., the link is enabled), the
bitlines of two adjacent subarrays are connected. Thus, the sense amplifier of a
subarray that has already driven its bitlines (due to an \act) can also drive
its neighboring subarray's precharged bitlines through the enabled link. This
causes the neighboring sense amplifiers to sense the charge difference, and
simultaneously help drive both sets of bitlines.
When the isolation transistor is turned off (i.e., the link is disabled),
the neighboring subarrays are disconnected from each other and thus operate as
in conventional DRAM.


\ignore{
As a result, an enabled sense amplifier that has already fully driven its bitlines
(to $V_{DD}$ or 0V) can also drive its neighbor subarray's precharged bitline
through an enabled \iso. This causes the neighbor sense amplifiers to sense the
voltage difference, and simultaneously help drive the bitlines.
}
%\figputHW{lisa_design}{Inter-linked subarrays.}
%\figputHS{lisa_design}{0.9}{Inter-linked subarrays.}
%\figputHS{lisa_links_src}{0.9}{Inter-linked subarrays.}
%\figputHW{lisa_links_hpca}{Inter-linked subarrays.}

\subsection{Row Buffer Movement (\xfernorm) Through \lisa}
\label{sec:bulk_lisa_transfer}

Now that we have inserted physical \isos to provide high-bandwidth connections
across subarrays, we must provide a way for the memory controller to make use of
these new connections. Therefore, we introduce a new DRAM command, \xfer, which
triggers an operation to move data from one row buffer (half a row of data) to
another row buffer within the same bank through these \isos. This operation serves
as the building block for our architectural optimizations.

To help explain the \xfer process between two row buffers, we assume that the
\emph{top row buffer} and the \emph{bottom row buffer} in
\figref{lisa_links_hpca} are the source (\src) and destination (\dst) of an
example \xfer operation, respectively, and that \src is activated with the
content of a row from Subarray~0. To perform this \xfer, the memory controller
enables the \isos (\circled{A} and \circled{B}) between \src and \dst, thereby
connecting the two row buffers' bitlines together ($bitline$ of \src to
$bitline$ of \dst, and $\overline{bitline}$ of \src to $\overline{bitline}$ of
\dst).

\figref{lisa_transfer_states_longer_filled} illustrates how \xfer drives the
data from \src to \dst. For clarity, we show only one column from each row
buffer. State \circled{1} shows the initial values of the bitlines (\bl and
\blbar) attached to the row buffers --- \src is activated and has fully driven
its bitlines (indicated by thick bitlines), and \dst is in the precharged state
(thin bitlines indicating a voltage state of \vddhalf). In state \circled{2},
the links between \src and \dst are turned \emph{on}. The charge of the \src
bitline (\bl) flows to the connected bitline (\bl) of \dst, raising the voltage
level of \dst's \bl to \vdddelta. The other bitlines (\blbar) have the opposite
charge flow direction, where the charge flows from the \blbar of \dst to the
\blbar of \src. This phase of charge flowing between the bitlines is known as
\emph{charge sharing}. It triggers \dst's row buffer to sense the increase of
differential voltage between \bl and \blbar, and amplify the voltage difference
further. As a result, \emph{both} \src and \dst start driving the bitlines with
the same values. This \emph{double sense amplification} process pushes both
sets of bitlines to reach the final \emph{fully sensed} state (\circled{3}),
thus completing the \xfer from \src to \dst.

%\figputHW{lisa_transfer_states_longer_filled}{Row buffer movement process using \lisa.}
\figputHS{lisa_transfer_states_longer_filled}{0.85}{Row buffer movement process using \lisa.}

Extending this process, \xfer can move data between two row buffers that are
\emph{not} adjacent to each other as well.  For example, \xfer can move data
from the \src row buffer (in \figref{lisa_links_hpca}) to a row buffer,
\dsttwo, that is \emph{two} subarrays away (i.e., the bottom row buffer of
Subarray~2, not shown in \figref{lisa_links_hpca}). This operation is similar
to the movement shown in \figref{lisa_transfer_states_longer_filled}, except
that the \xfer command turns on \emph{two extra links} ($\L$ \circled{2} in
\figref{lisa_transfer_states_longer_filled}), which connect the bitlines of
\dst to the bitlines of \dsttwo, in state \circled{2}. By enabling \xfer to
perform row buffer movement across non-adjacent subarrays via a single command,
instead of requiring multiple commands, the movement latency and command
bandwidth are reduced.

%\figputHW{lisa_transfer_states_triple}{Row buffer movement process across two
%subarrays using \lisa.}

\subsection{Row Buffer Movement (\xfernorm) Latency}
\label{sec:trans_lat}

To validate the \xfer process over \lisa links and evaluate its latency, we
build a model of \lisa using the Spectre Circuit Simulator~\cite{spectre}, with
the NCSU FreePDK 45nm library~\cite{ncsu-freepdk45}. We configure the DRAM
using the JEDEC DDR3-1600 timings~\cite{jedec-ddr3}, and attach each bitline to
512 DRAM cells~\cite{lee-hpca2013,son-isca2013}. We conservatively perform our
evaluations using \emph{worst-case cells}, with the resistance and capacitance
parameters specified in the ITRS
reports~\cite{itrs-fep-2013,itrs-interconnect-2013} for the metal lanes.
Furthermore, we conservatively model the worst RC drop (and hence latency) by
evaluating cells located at the edges of subarrays.

\newcommand{\samp}[1]{\texttt{SAmp#1}\xspace}

%\figputTS{lisa_clone_spice}{0.85}{SPICE simulation on transferring data across two sense amplifiers with \lisa.}
%\figputT{lisa_clone_spice}{SPICE simulation on transferring data across two sense amplifiers with \lisa.}

We now analyze the process of using one \xfer operation to move data between
\emph{two non-adjacent row buffers} that are two subarrays apart. To help the
explanation, we use an example that performs \xfer from \rb{0} to \rb{2}, as
shown on the left side of \figref{lisa_clone_spice_hpca}. The right side of the
figure shows the voltage of a single bitline $BL$ from each subarray during the
\xfer process over time. The voltage of the $\overline{BL}$ bitlines show the
same behavior, but have inverted values. We now explain this \xfer process step
by step.

\figputHS{lisa_clone_spice_hpca}{0.85}{SPICE simulation results for transferring
data across two subarrays with \lisa.}

First, before the \xfer command is issued, an \act command is sent to \rb{0} at
time~0. After roughly 21ns (\circled{1}), the bitline reaches $V_{DD}$, which
indicates the cells have been fully restored (\tras). Note that, in our
simulation, restoration happens more quickly than the standard-specified \tras
value of 35ns, as the standard includes a guardband on top of the typical cell
restoration time to account for process and temperature
variation~\cite{chandrasekar-date2014, lee-hpca2015}. This amount of margin is
on par with values experimentally observed in commodity DRAMs at
55{\textdegree}C~\cite{lee-hpca2015}.

Second, at 35ns (\circled{2}), the memory controller sends the \xfer command to
move data from \rb{0} to \rb{2}. \xfer simultaneously turns on the \emph{four}
links (circled on the left in \figref{lisa_clone_spice_hpca}) that connect the
subarrays' bitlines.

Third, after a small amount of time (\circled{3}), the voltage of \rb{0}'s
bitline drops to about 0.9V, as the fully-driven bitlines of \rb{0} are now
charge sharing with the precharged bitlines attached to \rb{1} and \rb{2}. This
causes both \rb{1} and \rb{2} to sense the charge difference and start
amplifying the bitline values. Finally, after amplifying the bitlines for a few
nanoseconds (\circled{4} at 40ns), all three bitlines become fully driven with
the value that is originally stored in \rb{0}.

We thus demonstrate that \xfer moves data from one row buffer to a row buffer
two subarrays away at very low latency. Our SPICE simulation shows that the
\xfer latency across two \lisa links is approximately 5ns (\circled{2}
$\rightarrow$ \circled{4}). To be conservative, we do \emph{not} allow data
movement across more than two subarrays with a single \xfer command.\footnote{In
    other words, \xfer has two variants, one that moves data between
    immediately adjacent subarrays
    (\figref{lisa_transfer_states_longer_filled}) and one that moves data
between subarrays that are one subarray apart from each other
(\figref{lisa_clone_spice_hpca}).}

%\figputHS{lisa_clone_spice}{0.85}{SPICE simulation on transferring data across two sense amplifiers with \lisa.}

%However, we only evaluate up to transferring data across two subarrays
%simultaneously in this work. Therefore, the transfer range of each \xfer is at
%most two subarrays.

\subsection{Handling Process and Temperature Variation}
\label{sec:lisa:variation}

On top of using worst-case cells in our SPICE model, we add in a latency
guardband to the \xfer latency to account for process and temperature variation,
as DRAM manufacturers commonly do~\cite{chandrasekar-date2014, lee-hpca2015}.
For instance, the \act timing (\trcd) has been observed to have margins of
13.3\%~\cite{chandrasekar-date2014} and 17.3\%~\cite{lee-hpca2015} for different
types of commodity DRAMs. To conservatively account for process and temperature
variation in \lisa, we add a large timing margin, of \emph{60\%}, to the \xfer
    latency. Even then, \xfer latency is 8ns and \xfer provides a 500~GB/s data
    transfer bandwidth across two subarrays that are one subarray apart from
    each other, which is 26x the bandwidth of a DDR4-2400 DRAM
    channel (19.2~GB/s)~\cite{jedec-ddr4}.


==> sec/lisa/macros.tex <==
\usepackage{ifthen}
\usepackage{calc}
\usepackage{pifont}
\usepackage{color}
\usepackage{fancyhdr}
\usepackage{tikz}
%\usepackage{gnuplot-lua-tikz}
%\usepackage[font={small,bf}]{caption}
%\usepackage{subcaption}
\usepackage{anyfontsize}

\newcounter{hours}
\newcounter{minutes}
\newcommand{\printtime}{%
  \setcounter{hours}{\time/60}%
  \setcounter{minutes}{\time-\value{hours}*60}%
  \thehours:\theminutes}

%\DeclareMathSizes{5}{9}{5}{5}
\newcommand{\bl}[0]{{\small{$BL$}}\xspace}
\newcommand{\blbar}[0]{{\small{$\overline{BL}$}}\xspace}
\newcommand{\vdddelta}[0]{{\small{$V_{DD}/2+\Delta$}}\xspace}
\newcommand{\vddhalf}[0]{{\small{$V_{DD}/2$}}\xspace}


%%%%%%%%%%
% Alias
%%%%%%%%%%
% Set timeofmake to 'true' to print the time the file was compiled
\newboolean{timeofmake}
\setboolean{timeofmake}{false}

\newcommand{\ignore}[1]{}
\newcommand{\unread}[1]{{\color{red}UnreadableComment: \textbf{#1}}\xspace}
\newcommand{\todo}[1]{{\color{red}TODO: \textbf{#1}}\xspace}
\newcommand{\dhl}[1]{{\color{blue} \textbf{Donghyuk: #1}}\xspace}
\newcommand{\kevin}[1]{{\color{brown} \textbf{Kevin: #1}}\xspace}
\newcommand{\sg}[1]{{\color{orange} \textbf{Saugata: #1}}\xspace}
\newcommand{\changes}[1]{\xspace{\color{blue}#1}\xspace}

\newcommand{\refsec}[1]{\S\ref{sec:#1}}

\newcommand{\villa}[0]{{VILLA-DRAM}\xspace}
\newcommand{\villafull}[0]{{variable latency DRAM}\xspace}
\newcommand{\villafullcap}[0]{{VarIabLe LAtency DRAM}\xspace}

\newcommand{\acro}[0]{{LISA}\xspace}
\newcommand{\lisa}[0]{{LISA}\xspace}
\newcommand{\lisarc}[0]{{LISA-RISC}\xspace}
\newcommand{\lisarcnol}[0]{{RISC}\xspace}
\newcommand{\lisarcfull}[0]{{(Rapid Inter-Subarray Copy)}\xspace}
\newcommand{\lisapre}[0]{{LISA-LIP}\xspace}
\newcommand{\lisaprenol}[0]{{LIP}\xspace}
\newcommand{\lisavilla}[0]{{LISA-VILLA}\xspace}
\newcommand{\lisavillanol}[0]{{VILLA}\xspace}
\newcommand{\lisarcvilla}[0]{{LISA-(RISC+VILLA)}\xspace}
\newcommand{\baseline}[0]{\texttt{memcpy}\xspace}
\newcommand{\baselinenorm}[0]{memcpy\xspace}
\newcommand{\xferfull}[0]{{row buffer movement}\xspace}
\newcommand{\xfernorm}[0]{{{RBM}}\xspace}
\newcommand{\xfer}[0]{{RBM}\xspace}
\newcommand{\xfers}[0]{{RBMs}\xspace}
\newcommand{\rb}[1]{\texttt{RB#1}\xspace}

\newcommand{\rc}[0]{{RowClone}\xspace}
\newcommand{\iso}[0]{{link}\xspace}
\newcommand{\isos}[0]{{links}\xspace}
\newcommand{\capfullname}[0]{{Low-Cost Inter-Linked Subarrays}\xspace}
\newcommand{\fullname}[0]{{low-cost inter-linked subarrays}\xspace}
\newcommand{\acrofullname}[0]{{Low-cost Inter-linked SubArrays}\xspace}
\newcommand{\lisafullname}[0]{{\underline{L}ow-cost \underline{I}nter-linked
\underline{S}ub\underline{A}rrays}\xspace}

%\newcommand{\refab}[0]{{\small\emph{$REF_{ab}$}}\xspace}
%\newcommand{\refpb}[0]{{\small\emph{$REF_{pb}$}}\xspace}
%\newcommand{\trefi}[0]{{\small\emph{$tREFI_{ab}$}}\xspace}
%\newcommand{\trefipb}[0]{{\small\emph{$tREFI_{pb}$}}\xspace}
%\newcommand{\trfc}[0]{{\small\emph{$tRFC_{ab}$}}\xspace}
%\newcommand{\trfcpb}[0]{{\small\emph{$tRFC_{pb}$}}\xspace}
%\newcommand{\trc}[0]{{\small\emph{tRC}}\xspace}
%\newcommand{\tras}[0]{{\small\emph{tRAS}}\xspace}
%\newcommand{\trp}[0]{{\small\emph{tRP}}\xspace}
%\newcommand{\trrd}[0]{{\small\emph{tRRD}}\xspace}
%\newcommand{\tfaw}[0]{{\small\emph{tFAW}}\xspace}
%\newcommand{\fgr}[0]{{\small\emph{FGR}}\xspace}
%\newcommand{\trcd}[0]{{\small\emph{tRCD}}\xspace}
%\newcommand{\tcl}[0]{{\small\emph{tCL}}\xspace}
%\newcommand{\tcwl}[0]{{\small\emph{tCWL}}\xspace}
\newcommand{\refab}[0]{{\small{$REF_{ab}$}}\xspace}
\newcommand{\refpb}[0]{{\small{$REF_{pb}$}}\xspace}
\newcommand{\trefi}[0]{{\small{$tREFI_{ab}$}}\xspace}
\newcommand{\trefipb}[0]{{\small{$tREFI_{pb}$}}\xspace}
\newcommand{\trfc}[0]{{\small{$tRFC_{ab}$}}\xspace}
\newcommand{\trfcpb}[0]{{\small{$tRFC_{pb}$}}\xspace}
\newcommand{\trc}[0]{{\small{tRC}}\xspace}
\newcommand{\tras}[0]{{\small{tRAS}}\xspace}
\newcommand{\trp}[0]{{\small{tRP}}\xspace}
\newcommand{\trrd}[0]{{\small{tRRD}}\xspace}
\newcommand{\tfaw}[0]{{\small{tFAW}}\xspace}
\newcommand{\fgr}[0]{{\small{FGR}}\xspace}
\newcommand{\trcd}[0]{{\small{tRCD}}\xspace}
\newcommand{\tcl}[0]{{\small{tCL}}\xspace}
\newcommand{\tcwl}[0]{{\small{tCWL}}\xspace}
\newcommand{\tccd}[0]{{\small{tCCD}}\xspace}
\newcommand{\trtw}[0]{{\small{tRTW}}\xspace}
\newcommand{\twr}[0]{{\small{tWR}}\xspace}
\newcommand{\tbl}[0]{{\small{tBL}}\xspace}

\newcommand{\src}[0]{\texttt{\small{src}}\xspace}
\newcommand{\dst}[0]{\texttt{\small{dst}}\xspace}
\newcommand{\dsttwo}[0]{\texttt{\small{dst2}}\xspace}
\newcommand{\act}[0]{\texttt{\small{ACTIVATE}}\xspace}
\newcommand{\acts}[0]{\texttt{\small{ACTIVATEs}}\xspace}
\newcommand{\crd}[0]{\texttt{\small{READ}}\xspace}
\newcommand{\cwr}[0]{\texttt{\small{WRITE}}\xspace}
\newcommand{\cpre}[0]{\texttt{\small{PRECHARGE}}\xspace}

\newcommand{\putsec}[2]{\vspace{-0.05in}\section{#2}\label{sec:#1}\vspace{-0.075in}}
\newcommand{\putssec}[2]{\vspace{-0.05in}\subsection{#2}\label{ssec:#1}\vspace{-0.075in}}
\newcommand{\putsssec}[2]{\vspace{0.05in}\subsubsection{#2}\label{sssec:#1}\vspace{0.075in}}
\newcommand{\putsssecX}[1]{\vspace{0.0in}\subsubsection*{#1}\vspace{0.0in}}

% RC
\newcommand{\rciasa}[0]{{RC-IntraSA}\xspace}
\newcommand{\rcirsa}[0]{{RC-InterSA}\xspace}
\newcommand{\rcirba}[0]{{RC-InterBA}\xspace}

% Black-background circled text
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.8pt,fill=white,text=black] (char) {#1};}}

\newcommand{\figput}[4][1.0\linewidth]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#3, clip, width=#1]{plots/#2}
\end{center}
\caption{#4 \label{fig:#2}}
\end{minipage}
\end{figure}
}

\newcommand{\figputW}[2]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[clip,width=\linewidth]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputWS}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputH}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth, height=#2]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHW}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHWHeight}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth, height=#3in]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}


\newcommand{\figputGHWHeight}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth,height=#3in]{plots/gnuplots/#1}%
\end{center}
\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGHW}[2]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGTW}[2]{
\begin{figure}[!t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/gnuplots/#1}
\end{center}
\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}


\newcommand{\figputHS}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGHS}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}
\newcommand{\figputGTS}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGTWS}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputTS}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputT}[2]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[clip, width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputTT}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#2, clip, width=1.0\linewidth]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputPlaceHolder}[2]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=0.8, width=1.0\linewidth]{plots/PlaceHolder}
\end{center}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

%\renewcommand{\figurename}{\renewcommand{\baselinestretch}{1.0}\vspace{-0.0in}\footnotesize\sf\bfseries Figure}
%\renewcommand{\tablename}{\renewcommand{\baselinestretch}{1.0}\vspace{-0.0in}\footnotesize\sf\bfseries Table}

\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\eq}[1]{Table~\ref{tab:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\ssecref}[1]{Section~\ref{ssec:#1}}
\newcommand{\sssecref}[1]{Section~\ref{sssec:#1}}



==> sec/lisa/methodology.tex <==
% !TEX root = ../paper.tex

\section{Methodology} \label{sec:meth}

We evaluate our system using a variant of Ramulator~\cite{kim-cal2015},
an open-source cycle-accurate DRAM simulator, driven by traces generated from
Pin~\cite{luk-pldi2005}. We will make our simulator publicly
available~\cite{safari-github}. We use a row buffer policy that closes a row
only when there are no more outstanding requests in the memory controller to
the same row~\cite{rixner-isca2000}. Unless stated otherwise, our simulator
uses the parameters listed in \tabref{sys-config}.

\input{sec/tables/sys_config_table.tex}

\noindent\textbf{Benchmarks and Workloads.} We primarily use benchmarks from
TPC(-C/-H)~\cite{tpc}, DynoGraph (BFS, Page\-Rank)~\cite{dynograph}, SPEC
CPU2006~\cite{spec2006}, and STREAM~\cite{stream}, along with a random-access
microbenchmark similar to HPCC RandomAccess~\cite{randombench}. Because these
benchmarks predominantly stress the CPU and memory while rarely invoking
\baseline, we use the following benchmarks to evaluate different copy
mechanisms: (1)~\texttt{bootup}, (2)~\texttt{forkbench}, and
(3)~\texttt{Unix}~\texttt{shell}. These were shared by the authors of
RowClone~\cite{seshadri-micro2013}. The \texttt{bootup} benchmark consists of a
trace collected while a Debian operating system was booting up. The
\texttt{forkbench} kernel forks a child process that copies 1K pages from the
parent process by randomly accessing them from a 64MB array. The \texttt{Unix}
\texttt{shell} is a script that runs \texttt{find} in a directory along with
\texttt{ls} on each subdirectory. More information on these is in
\cite{seshadri-micro2013}.
%We refer the readers to \cite{seshadri-micro2013} for further details on these
%benchmarks.

To evaluate the benefits of different data copy mechanisms in isolation, we use
a copy-aware page mapping policy that allocates destination pages to certain
DRAM structures (i.e., subarrays, banks) such that only the specified copy
mechanism is used for copy operations. For example, when evaluating
\mbox{\rciasa}, the page mapper allocates the destination page only within the
same subarray as the source page~\cite{seshadri-micro2013}.

To construct multi-core workloads for evaluating the benefits of data copy
mechanisms, we randomly assemble 50 workloads, each comprising 50\%
copy-intensive benchmarks and 50\% non-copy-intensive benchmarks. To evaluate
the benefits of in-DRAM caching and reduced precharge time, we restrict our
workloads to randomly-selected memory-intensive ($\ge$ 5 misses per thousand
instructions) non-copy-intensive benchmarks. Due to the large number of
workloads, we present detailed results for only five workload mixes
(\tabref{wkld-mixes}), along with the average results across all 50 workloads.

\input{sec/tables/wkld_mixes.tex}

\noindent\textbf{Performance Metrics.} We measure single-core and
\mbox{multi-core}
performance using IPC and Weighted Speedup (WS)~\cite{snavely-asplos2000},
respectively. Prior work showed that WS is a measure of system
throughput~\cite{eyerman-ieeemicro2008}. To report DRAM energy consumption, we
use the Micron power calculator~\cite{micron-tr}. We run all workloads for 100
million instructions, as done in many recent
works~\cite{kim-micro2010,kim-isca2012,lee-hpca2013,lee-taco2016,mutlu-micro2007}.

\vspace{3pt} \noindent\textbf{\villa Configuration.} For our simulated \villa,
each fast subarray consists of 32 rows to achieve low latency on sensing,
precharge, and restoration (a typical subarray has 512 rows). Our SPICE
simulation reports the following new timing parameters for a 32-row subarray:
{\small{tRCD}}=7.5ns, {\small{tRP}}=8.5ns, and {\small{tRAS}}=13ns, which are
reduced from the original timings by respectively, 45.5\%, 38.2\%, and 62.9\%.
For each bank, we allocate 4 fast subarrays in addition to the 16 512-row
subarrays, incurring a 1.6\% area overhead. We set the epoch length for our
caching policy to 10,000~cycles.


==> sec/lisa/opt_clone.tex <==
% !TEX root = ../paper.tex

\section{Application 1: Rapid Inter-Subarray Bulk Data Copying (\lisarc)}
\label{sec:lisaclone}

Due to the narrow memory channel width, bulk copy operations used by
applications and operating systems are performance limiters in today's
systems~\cite{jiang-pact2009, kanev-isca2015,
seshadri-micro2013,zhao-iccd2005}. These operations are commonly performed due
to the \texttt{memcpy} and \texttt{memmov}. Recent work reported
that these two operations consume 4-5\% of \emph{all of} Google's datacenter
cycles, making them an important target for lightweight hardware
acceleration~\cite{kanev-isca2015}. As we show in
Section~\ref{sec:lisaclone:shortcomings}, the \mbox{state-of-the-art} solution,
RowClone~\cite{seshadri-micro2013}, has poor performance for such operations
when they are performed \emph{across} subarrays in the same bank.

Our goal is to provide an architectural mechanism to accelerate these
inter-subarray copy operations in DRAM. We propose \lisarc, which uses the
\xfer operation in \lisa to perform rapid data copying.  We describe
the high-level operation of \lisarc (Section~\ref{sec:lisaclone:overview}), and
then provide a detailed look at the memory controller command sequence required
to implement \lisarc (Section~\ref{sec:lisaclone:commands}).

\subsection{Shortcomings of the State-of-the-Art}
\label{sec:lisaclone:shortcomings}


%% Extended RowClone explanation in the previous version %%
\ignore{
To understand this, \figref{intro_rc} shows the organization of a modern DRAM
chip. The chip is divided into a hierarchy of banks, which are further split
into subarrays. Each subarray contains a subset of rows of DRAM cells. The rows
\emph{within} a subarray are interconnected by \emph{bitlines}, which allow the
contents of an \emph{entire row} to be moved between the DRAM cells and the
\emph{row buffer}. Outside of a subarray, DRAM rows are only interconnected
through a narrow 64-bit internal bus.

\figputHW{intro_rc}{Internal DRAM chip organization, also showing the three movement modes of \rc~\cite{seshadri-micro2013}.}

\figref{intro_rc} shows the three cases for data movement within DRAM: (1)
within a subarray, (2) across different banks, and (3) across subarrays within
the same bank. For the first case within a subarray, \rc exploits the bitlines
to transfer the whole row simultaneously, thus outperforming the baseline in
today's system. In the second case across banks, \rc performs slightly better
than the baseline by avoiding data transfer through the channel, even though it
transfers data through the narrow internal 64-bit bus. However, for the third case across
subarrays in a bank, \rc can perform \emph{worse} than today's baseline because
it ties up the internal DRAM bus for a excessive duration (twice the amount
of inter-bank). This blocks critical read or write commands \emph{to other
banks} from executing. As a result, a baseline that moves data through memory
channels, as shown in \figref{intro_baseline}, is still the best performing
mechanism for inter-subarray movement, even though it incurs long latency.
}

Previously, we have described the state-of-the-art work,
\rc~\cite{seshadri-micro2013}, which addresses the problem of costly data
movement over memory channels by coping data completely in DRAM.
However, \rc does \emph{not} provide fast data copy between subarrays.
The main latency benefit of RowClone comes from intra-subarray copy
(\emph{\rciasa} for short) as it copies data at the row granularity. In
contrast, inter-subarray RowClone (\emph{\rcirsa}) requires transferring data at
the cache line granularity (64B) through the internal data bus in DRAM.
Consequently, \rcirsa incurs \emph{16x longer latency} than \rciasa.
Furthermore, \rcirsa is a long \emph{blocking operation} that prevents
reading from or writing to the other banks in the same rank, reducing
bank-level parallelism~\cite{lee-micro2009,mutlu-isca2008}.

%%%% HACK: in order to place this figure in the bottom %%%%
%\begin{figure*}[!hb]
%\stepcounter{figure} % Tweak the figure number
%\begin{minipage}{\linewidth}
%\vspace{6pt}
%\begin{center}
%\includegraphics[scale=0.83]{plots/lisa_timelines_irsa}
%\end{center}
%\vspace{-0.1in}
%\caption{Command service timelines of a row copy for \lisarc and \rcirsa
%(command latencies not drawn to scale). \label{fig:lisa_timelines_irsa}}
%\end{minipage}
%\end{figure*}
%%%%

To demonstrate the ineffectiveness of \rcirsa, we compare it to today's
currently-used copy mechanism, \baseline, which moves data via the memory
channel. In contrast to \mbox{\rcirsa}, which copies data in DRAM, \baseline
copies data by sequentially reading out source data from the memory and then
writing it to the destination data in the on-chip caches. \figref{rc_vs_base}
compares the average system performance and queuing latency of \rcirsa and
\baseline, on a quad-core system across 50 workloads that contain bulk (8KB)
data copies (see Section~\ref{sec:meth} for our methodology). \rcirsa actually
\emph{degrades} system performance by 24\% relative to \baseline, mainly
because \rcirsa increases the overall memory queuing latency by 2.88x, as it
blocks other memory requests from being serviced by the memory controller
performing the \rcirsa copy. In contrast, \baseline is \emph{not} a long or
blocking DRAM command, but rather a long sequence of memory requests that can
be interrupted by other critical memory requests, as the memory scheduler can
issue memory requests out of order~\cite{kim-hpca2010,
kim-micro2010,mutlu-micro2007, mutlu-isca2008, rixner-isca2000,
subramanian-iccd2014, usui-taco2016, zuravleff-patent}.

%%
%\begin{figure}[t] \addtocounter{figure}{-2} % Tweak the figure number
%\includegraphics[width=1.0\linewidth]{plots/gnuplots/rc_vs_base}
%\caption{Comparison of \rc to \baselinenorm over the memory channel, on
%    workloads that perform bulk data copy across subarrays on a 4-core system.
%\label{fig:rc_vs_base}} \addtocounter{figure}{1} % Reset back the figure number
%\end{figure}
%%


%%%% This figure placement cannot place one figure in the top and the other in the bottom
%\ignore{
\figputGHW{rc_vs_base}{Comparison of \rc to \baselinenorm over the memory
    channel, on workloads that perform bulk data copy across subarrays on a
    4-core system.}

\begin{figure*}[!hb]
\begin{minipage}{\linewidth}
\vspace{6pt}
\begin{center}
\includegraphics[scale=0.83]{plots/lisa_timelines_irsa}
\end{center}
\vspace{-0.1in}
\caption{Command service timelines of a row copy for \lisarc and \rcirsa
(command latencies not drawn to scale). \label{fig:lisa_timelines_irsa}}
\end{minipage}
\end{figure*}
%}
%%%%


On the other hand, \rcirsa offers energy savings of 5.1\% on average over
\baseline by \emph{not} transferring the data over the memory channel. Overall,
these results show that neither of the existing mechanisms (\baseline or \rc)
offers \emph{fast and energy-efficient} bulk data copy across subarrays.

\ignore{ Second, the fixed row-size copy granularity of \rciasa can also become
a disadvantage as it cannot control how much data to copy between two rows. The
typical page size in modern operating systems is 4KB, but commodity DDR3/4
memory technology only support 8KB row size~\cite{jedec-ddr3,jedec-ddr4},
creating a mismatch between the copy granularity of \rciasa and page-size data
copies. This can result in potential data loss as \rciasa copies an extra OS
page into another physical page that may be currently used by the operating
system. \todo{? Therefore, the RowClone work assumes a row size of 4KB} Third,
while \rcirsa is copying data, it prevents other banks from reading or writing
data as it uses the internal data bus shared across all banks to transfer data.
\todo{Add this? Fourth, \rciasa restricts its copy range to a smaller physical
address space, that is within a subarray.} }


\subsection{In-DRAM Rapid Inter-Subarray Copy (RISC)}
\label{sec:lisaclone:overview}

Our goal is to design a new mechanism that enables
\emph{low-latency} and \emph{energy-efficient} memory copy between rows \emph{in
different subarrays} within the same bank. To this end, we propose a new in-DRAM
copy mechanism that uses \lisa to exploit the high-bandwidth links between
subarrays. The key idea, step by step, is to: (1)~activate a source row in a
subarray; (2)~rapidly transfer the data in the activated source row buffers to
the destination subarray's row buffers, through LISA's wide inter-subarray
links, without using the narrow internal data bus; and (3)~activate
the destination row, which enables the contents of the destination row buffers
to be latched into the destination row. We call this inter-subarray row-to-row
copy mechanism \emph{\lisa-\underline{R}apid
\underline{I}nter-\underline{S}ubarray \underline{C}opy} (\lisarc).

As \lisarc uses the full row bandwidth provided by \lisa, it reduces the copy
latency by 9.2x compared to \rcirsa (see Section~\ref{sec:comp-copy}). An
additional benefit of using \lisarc is that its inter-subarray copy operations
are performed \emph{completely inside a bank}. As the internal DRAM data bus is
untouched, \emph{other} banks can concurrently serve memory requests,
exploiting bank-level parallelism. This new mechanism is complementary to \rc,
which performs fast \emph{intra-subarray} copies.  Together, our mechanism and
\rc can enable a complete set of fast in-DRAM copy techniques in future
systems. We now explain the step-by-step operation of how \lisarc copies data
across subarrays.

%
\ignore{Our goal is to design a new in-DRAM cloning mechanism that addresses some of the
downsides of \rc with the characteristics of low copy latency and flexible copy
granularity across subarrays within individual banks. This new mechanism will
also be complementary to \rc so that together our mechanism and \rc can enable
a more complete set of in-DRAM copy techniques to accelerate copying or moving a
large amount of data in future systems.

\lisarc offers several benefits over \rc. First, \lisarc enables fast data
transfer within the entire bank, as each transfer between two subarrays utilizes
the full row bandwidth. The copy latency only increases by a small amount (8ns,
Section~\ref{sec:trans_lat}) with every additional two subarrays between the
source and destination subarray. Second, we can enable a finer granularity
data copy between two rows, by providing independent
enable signals for each of the \isos in the same row (e.g., enabling the \isos
for only half of a row buffer).
Third, all inter-subarray copy operations for \lisarc are fully performed
inside the bank, allowing other banks to concurrently serve memory
requests. In addition, \lisarc can also be applied to intra-subarray copying by
simply writing the row buffer content first to the neighbor row buffer, and
then writing it back to its subarray. \lisarc still provides some benefit in
this case, offering finer-grained control over the amount of data being copied.
}
%

\subsection{Detailed Operation of \lisarc}
\label{sec:lisaclone:commands}

\newcommand{\sa}[1]{\texttt{SA#1}\xspace}
\newcommand{\tr}[2]{\texttt{RBM\textsubscript{#1$\rightarrow$#2}}\xspace}
\newcommand{\actcopy}[1]{\texttt{ACT\textsubscript{SA#1}}\xspace}

\figref{lisa_timelines_irsa} shows the command service timelines for both
\lisarc and \rcirsa, for copying a single row of data across two subarrays, as
we show on the left.  Data is copied from subarray \texttt{SA0} to \texttt{SA2}.
We illustrate four row buffers (\texttt{RB0}--\rb{3}): recall from
Section~\ref{sec:background:dram} that in order to activate one row, a subarray
must use \emph{two} row buffers (at the top and bottom), as each row buffer
contains only half a row of data.  As a result, \lisarc must copy half a row at
a time, first moving the contents of \texttt{RB1} into \texttt{RB3}, and then
the contents of \texttt{RB0} into \texttt{RB2}, using two \xfer commands.

% compares the service timelines of different
% inter-subarray copy mechanisms. On the left side of the figure, we show an
% example bank organization with three subarrays
% (\mbox{\texttt{SA0$\leftrightarrow$2}}), along with their row buffers
% (\mbox{\texttt{RB0}$\leftrightarrow$\rb{3}}). A \lisarc operation consists of
% multiple existing DRAM and \xfer commands. We will illustrate how \lisarc
% operates using an example that copies an arbitrary row from \sa{0} to \sa{2}, in
% \figref{lisa_timelines_irsa}. Because a row activation latches a row into two
% row buffers, \lisarc has to copy half a row at a time. We will first describe
% copying the first half of the row.

First, the \lisarc memory controller activates the source row (\actcopy{0}) to
latch its data into two row buffers (\rb{0} and \rb{1}). Second, \lisarc
invokes the first \xfer operation (\tr{1}{3}) to move data from the bottom
source row buffer (\rb{1}) to the respective destination row buffer (\rb{3}),
thereby linking \rb{1} to both \rb{2} and \rb{3}, which activates both \rb{2}
and \rb{3}. After this step, \lisarc \emph{cannot} immediately invoke another
\xfer to transfer the remaining half of the source row in \rb{0} into \rb{2},
as a row buffer (\rb{2}) needs to be in the \emph{precharged state} in order to
receive data from an activated row buffer (\rb{0}). Therefore, \lisarc
completes copying the first half of the source data into the destination row
before invoking the second \xfer, by writing the row buffer (\rb{3}) into the
cells through an activation (\actcopy{2}). This activation enables the contents
of the sense amplifiers (\rb{3}) to be driven into the destination row. To
address the issue that modern DRAM chips do not allow a second \act to an
already-activated bank, we use the \emph{back-to-back} \act command that is
used to support \rc~\cite{seshadri-micro2013}.

%Similar to \rciasa, \lisarc requires a back-to-back \act.

%For example, to copy data
%from \sa{0} to \sa{1}, \lisarc transfers data from \rb{1} to \rb{2} first
%(\tr{1}{2}) followed by an \act on \sa{1} to write the data into \sa{1}. Similar
%to FPM, \lisarc would also require back-to-back \act to the same bank.

Third, to move data from \rb{0} to \rb{2} to complete the copy transaction, we
need to precharge both \rb{1} and \rb{2}. The challenge here is to precharge
all row buffers \emph{except} \rb{0}. This cannot be accomplished in today's
DRAM because a precharge is applied at the bank level to \emph{all} row
buffers. Therefore, we propose to add a new \emph{precharge-exception} command,
which prevents a row buffer from being precharged and keeps it activated. This
bank-wide exception signal is supplied to all row buffers, and when raised for
a particular row buffer, the selected row buffer retains its state while the
other row buffers are precharged. After the precharge-exception
(\texttt{PRE\textsubscript{E}}) is complete, we then invoke the second \xfer
(\tr{0}{2}) to copy \rb{0} to \rb{2}, which is followed by an activation
(\texttt{ACT\textsubscript{SA2}{\small\textprime}}) to write \rb{2} into
\sa{2}. Finally, \lisarc finishes the copy by issuing a \cpre command
(\texttt{PRE} in \figref{lisa_timelines_irsa}) to the bank.

In comparison, the command service timeline of \rcirsa is much longer, as \rc
can copy only \emph{one cache line} of data at a time (as opposed to half a row
buffer).  This requires 128 \emph{serial cache line transfers} to read the data
from \texttt{RB0} and \texttt{RB1} into a temporary row in another bank,
followed by another 128 serial cache line transfers to write the data into
\texttt{RB2} and \texttt{RB3}.  \lisarc, by moving half a row using a single
\xfer command, achieves 9.2x lower latency than \rcirsa.

% Compared to the service timeline of \rcirsa that
% transfers cache line serially through the narrow global data lines, \lisarc
% reduces the latency significantly by 9.2x using the \lisa substrate.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{ Third, after the leading row buffer completes writing. We need to
precharge all the row buffers in the path from the trailing row buffer to the
destination. The challenge here is to precharge everything except for the
trailing row buffer, which cannot be accomplished in today's DRAM because a
precharge is applied at the bank level to all row buffers. Therefore, to support
copying of the trailing row buffer, we propose to add a new
\emph{precharge-exception} signal that prevents a row buffer from being
precharged while keeping the row buffer activated. This exception signal is
supplied to every row buffer, and when it raises for a particular row buffer,
the selected row buffer retains its state while the other row buffers are
precharging. After the exception precharge is complete, we the process from step
two again with a different source row buffer to transfer.

Therefore, it copies the data from one row buffer first before it finishes off
the copy transaction with the second row buffer. For example, to copy data from
\sa{0} to \sa{1}, \lisarc transfers data from \rb{1} to \rb{2} first
(\tr{1}{2}) followed by an \act on \sa{1} to write the data into \sa{1}. Then
it re-initializes the bitlines through a precharge in order to transfer the
second half of the row (\tr{0}{1}). For each additional two hops over two
subarrays, the total latency increases by one transfer (8ns).
\figref{lisa_timelines_irsa} also illustrates a small increase in terms of
transfer latency when comparing a two-hop transfer to a one-hop transfer.
However, for our final evaluations, we simply assume that a one-hop transfer
incurs the same latency as a two-hop transfer. Equation \eqref{eq:1} defines
the total latency of \lisarc, and the transfer latency grows linearly with the
hop count. Lastly, the figure also shows the service timeline of PSM
(inter-subarray) that copies one cache line serially, which incurs longer
latency than using \lisa to perform copies. }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Data Coherence}
\label{sec:copy:coherence}

When a copy is performed in DRAM, one potential disadvantage is that the data
stored in the DRAM may not be the most recent version, as the processor may
have dirty cache lines that belong to the section of memory being copied. Prior
works on in-DRAM migration have proposed techniques to accommodate data
coherence~\cite{seshadri-cal2015,seshadri-micro2013}. Alternatively, we can
accelerate coherence operations by using structures like the \mbox{Dirty-Block}
Index~\cite{seshadri-isca2014}.

\ignore{, which we can also use for \lisarc.  When the memory controller
initiates a copy in DRAM, it also performs an \emph{in-cache} copy of the dirty
lines belonging to the section of memory being copied.  These in-cache copies
are marked as dirty.  This approach avoids forcing the in-DRAM copy
operation to wait for dirty data to be flushed back to memory,
because the cache has the most up-to-date copy for dirty lines that xx cache
before the copy operation has initiated
%as the cache
%copies can occur in parallel, and the newly-copied section in DRAM will be
%automatically updated when these cache copies are written back to DRAM.
}

\subsection{Comparison of Copy Techniques}
\label{sec:comp-copy}

\figref{copy_latency_energy} shows the DRAM latency and DRAM energy consumption
of different \emph{copy commands} for copying a row of data (8KB). The exact
latency and energy numbers are listed in \tabref{copy_latency}.\footnote{Our
    reported numbers differ from prior work~\cite{seshadri-micro2013} because:
(1) we use faster DRAM timing parameters (1600-11-11-11 vs 1066-8-8-8), and (2)
we use the 8KB row size of most commercial DRAM instead of
4KB~\cite{seshadri-micro2013}.} We derive the copy latency of each command
sequence using equations based on the DDR3-1600 timings~\cite{jedec-ddr3}
(available in our technical report~\cite{chang-tr2016}), and the DRAM
energy using the Micron power calculator~\cite{micron-tr}. For \lisarc, we
define a \emph{hop} as the number of subarrays that \lisarc needs to copy data
\emph{across} to move the data from the source subarray to the destination
subarray. For example, if the source and destination subarrays are adjacent to
each other, the number of hops is 1. The DRAM chips that we evaluate have 16
subarrays per bank, so the maximum number of hops is 15.

\figputGTW{copy_latency_energy}{Latency and DRAM energy of 8KB copy.}

% Table on copy latency and energy
\input{sec/tables/copy_latency}

We make two observations from these numbers. First, although \rcirsa incurs
similar latencies as \baseline, it consumes 29.6\% less energy, as it does
\emph{not} transfer data over the channel and DRAM I/O for each copy operation.
However, as we showed in \secref{lisaclone:shortcomings}, \rcirsa incurs a higher system performance
penalty because it is a long-latency \emph{blocking} memory command. Second,
copying between subarrays using \lisa achieves significantly lower
latency and energy compared to \rc, even though the total latency of
\lisarc grows linearly with the hop count.%(i.e., the number of subarrays data must go across).

By exploiting the \lisa substrate, we thus provide a more complete set of
in-DRAM copy mechanisms. Our workload evaluation results show that \lisarc
outperforms \rcirsa and \baseline: its average performance improvement and energy
reduction over the best performing inter-subarray copy mechanism (i.e.,
\baseline) are 66.2\% and 55.4\%, respectively, on a quad-core system, across 50
workloads that perform bulk copies (see Section~\ref{sec:eval_lisaclone}).

%\todo{get rid of copy granularity?}
%
%\input{sec/tables/copy_tradeoff}


==> sec/lisa/opt_clone_hpca_v1.tex <==
\section{Optimization 1: Rapid Inter-Subarray Bulk Data Copying (\lisarc)}
%\subsection{Rapid In-DRAM Data Copying (\lisarc)}
\label{sec:lisaclone}

%\subsection{Motivation for Fast Data Copying or Movement}

Due to the narrow memory channel width, bulk copy or movement operations used by
applications and operating systems are performance limiters in today's
system~\cite{jiang-pact2009, kanev-isca2015, seshadri-micro2013,zhao-iccd2005}.
These operations are commonly performed due to the \texttt{memcpy} and
\texttt{memmov} library calls. Recent work~\cite{kanev-isca2015} has reported
that these two operations consume 4-5\% out of \emph{all of} Google datecenter
cycles, which make them an important target for lightweight hardware
acceleration. In the rest of the section, we first discuss the inefficiency
problem in existing solution and prior work. Then we will propose a mechanism
that leverages the \lisa substrate to overcome the problem, and its detailed
step-by-step command sequence to achieve bulk data copy at low latency.

%\subsection{State-of-the-art In-DRAM Copying Mechanism}
\subsection{Shortcomings of Inter-Subarray Bulk Copying in State-of-the-art Techniques}
%\todo{Title? Shortcomings of State-of-the-art In-DRAM Copying Mechanism}
\label{sec:lisaclone:shortcomings}

Amongst the prior work studying bulk copying, the most recent work by Seshadri
et al.~\cite{seshadri-micro2013} proposes \rc, an in-DRAM copying technique, to
avoid unnecessary data movement over memory channels during memory copy
operations.

\todo{Remove and tighten the rest if we are keeping the intro. \rc consists of
two key mechanisms for copying. The first mechanism, called Fast Parallel Mode
(FPM) or \emph{intra-subarray} cloning, leverages the large subarray-internal
bandwidth to copy data with low latency among rows within the \emph{same
subarray}. The second mechanism, Pipelined Serial Mode (PSM), copies data across
different subarrays in the same bank (inter-subarray) or in different banks
(inter-bank), utilizing the internal data bus within DRAM to transfer \emph{one
cache line} at a time.}

%The serial data movement incurs
%similar copy latency to \\baseline, as it also copies cache lines serially
%over the narrow global data lines and the internal data bus.

\noindent\textbf{Problem.} Unfortunately, \rc has a few shortcomings that limit its
applicability. First, the main latency benefit of RowClone only comes from
intra-subarray RowClone (\rciasa for short) as the data can be copied at the
DRAM row granularity (8KB) within a subarray. In contrast, inter-subarray
RowClone (\rcirsa) requires transferring data at the cache line granularity
(64B) through the global data lines. Consequently, \rcirsa incurs \emph{16x
longer latency} than \rciasa (the detailed operations of these two copy methods
are discussed later in the section).

%We illustrate this slow copy process of
%\rcirsa in \figref{rcirsa_problem}, which shows that copying a source row (src)
%to a destination row (dst) uses the \emph{64-byte} global data lines and the
%internal bus shared across all banks.
%\figputHS{rcirsa_problem}{1}{Slow data copying through \rcirsa.}

Second, \rcirsa is also a \emph{blocking
operation} that prevents other banks within the same rank from reading or
writing data while \rcirsa is copying data because it copies data over the
shared internal bus. Third, the copy range of the fast \rciasa is limited to
only a single subarray. Although the \rcirsa allows a wider copy range than
\rciasa (typically 16 to 32x), it suffers from performance penalty with long
latency.

%In contrast, the much more flexible
%inter-subarray RowClone (\rcirsa) that allows a wider copy range than \rciasa
%(typically 16 to 32x), requires transferring data at the cache line granularity
%(64B) through the global data lines. Consequently, \rcirsa incurs \emph{16x
%longer latency} than \rciasa (the detailed operations of these two copy methods
%are discussed later in the section). We illustrate this slow copy process of
%\rcirsa in \figref{rcirsa_problem}, which shows that copying a source row (src)
%to a destination row (dst) uses the \emph{64-byte} global data lines and the
%internal bus shared across all banks. Due to transferring data over the shared
%internal bus, \rcirsa is also a \emph{blocking operation} that prevents other
%banks within the same rank from reading or writing data.
%
%However, inter-subarray RowClone (\rcirsa), allowing a much
%wider copy range than \rciasa (typically 16 to 32x), requires using the narrow
%64-byte \emph{global data lines} to serially transfer data, thus incurring high
%latency (i.e., 16x higher than \rciasa) as illustrated in
%\figref{rcirsa_problem}.
%
%Furthermore, \rcirsa is a \emph{blocking operation}
%that prevents other banks within the same rank from reading or writing data as
%it uses the internal data bus \emph{shared across all banks} to transfer
%data~\cite{seshadri-micro2013}.


\figref{rc_vs_base} shows the system performance and queueing latency of using
\rcirsa and today's copy mechanism (\baseline) on a quad-core system averaged
across 50 workloads.\footnote{The detailed methodology is discussed in
Section~\ref{sec:meth}.} To perform a bulk \baseline, the cache lines from the
source page are serially read out from the memory and written into the
destination cache lines in the on-chip caches. In contrast to \rcirsa, copying a
large amount of data is not a blocking call in \baseline, but rather a long
sequence of memory requests that can be interrupted over by other demand
requests due to the memory scheduler. Furthermore, it reaps the benefit of using
on-chip caches to serve lines from the source or destination pages at low
latency.

\figputGHW{rc_vs_base}{Comparisons of \rc to \baseline when copying data
across subarrays on a 4-core system.}
%%
\figputWS{lisa_timelines_irsa}{0.83}{Command service timelines of \lisarc
compared to \rc. The commands are not drawn to scale with their latency.}
%%

As shown in \figref{rc_vs_base}, \rcirsa actually \emph{degrades} the average
performance by 24.0\% relative to \baseline due to 2.88x longer memory queueing
latency despite avoiding the round trip to the CPU. However, \rcirsa offers
energy savings of 5.1\% on average over \baseline by not transferring the data
over the memory channel. Overall, these results indicate that neither of the
mechanisms offers \emph{fast and energy-efficient} bulk copy operations across
subarrays.

\ignore{ Second, the fixed row-size copy granularity of \rciasa can also become
a disadvantage as it cannot control how much data to copy between two rows. The
typical page size in modern operating systems is 4KB, but commodity DDR3/4
memory technology only support 8KB row size~\cite{jedec-ddr3,jedec-ddr4},
creating a mismatch between the copy granularity of \rciasa and page-size data
copies. This can result in potential data loss as \rciasa copies an extra OS
page into another physical page that may be currently used by the operating
system. \todo{? Therefore, the RowClone work assumes a row size of 4KB} Third,
while \rcirsa is copying data, it prevents other banks from reading or writing
data as it uses the internal data bus shared across all banks to transfer data.
\todo{Add this? Fourth, \rciasa restricts its copy range to a smaller physical
address space, that is within a subarray.} }

%(e.g., 8MB), due to its applicability only within a subarray.

\subsection{In-DRAM Rapid Inter-Subarray Copy (RISC)}

Our goal is to design a new in-DRAM copy mechanism that enables
\emph{low-latency} and \emph{energy-efficient} memory copies across subarrays
within the same bank. To this end, we propose a new in-DRAM copy mechanism with
\lisa to exploit the high-bandwidth links connected between subarrays. The key
idea is to activate a source row in a subarray, and rapidly transfer the data in
the source row buffers to the destination subarray's row buffers through \lisa
without the need to use the global data lines. By activating the destination row
with its connected row buffers containing the source row data, we can
effectively write the row buffers' content back into the destination row. We
call this copy mechanism \emph{\lisa-\underline{R}apid
\underline{I}nter-\underline{S}ubarray \underline{C}opy (\emph{\lisarc})}.

As a result of using the \lisa substrate's full row bandwidth, \lisarc reduces
the copy latency by by 88.9\% compared to \rcirsa, which we will elaborate in
Section~\ref{sec:comp-copy}. The additional benefit of using \lisarc is that its
inter-subarray copy operations are fully performed \emph{inside} the bank. This
allows other banks to concurrently serve memory requests, exploiting
memory-level parallelism. This new mechanism is complementary to \rc; together
our mechanism and \rc can enable a more complete set of in-DRAM copy techniques
to accelerate copying or moving a large amount of data in future systems. We
will now explain the detailed step-by-step operations on how on \lisarc copies
data across subarrays.

%
\ignore{Our goal is to design a new in-DRAM cloning mechanism that addresses some of the
downsides of \rc with the characteristics of low copy latency and flexible copy
granularity across subarrays within individual banks. This new mechanism will
also be complementary to \rc so that together our mechanism and \rc can enable
a more complete set of in-DRAM copy techniques to accelerate copying or moving a
large amount of data in future systems.

\lisarc offers several benefits over \rc. First, \lisarc enables fast data
transfer within the entire bank, as each transfer between two subarrays utilizes
the full row bandwidth. The copy latency only increases by a small amount (8ns,
Section~\ref{sec:trans_lat}) with every additional two subarrays between the
source and destination subarray. Second, we can enable a finer granularity
data copy between two rows, by providing independent
enable signals for each of the \isos in the same row (e.g., enabling the \isos
for only half of a row buffer).
Third, all inter-subarray copy operations for \lisarc are fully performed
inside the bank, allowing other banks to concurrently serve memory
requests. In addition, \lisarc can also be applied to intra-subarray copying by
simply writing the row buffer content first to the neighbor row buffer, and
then writing it back to its subarray. \lisarc still provides some benefit in
this case, offering finer-grained control over the amount of data being copied.
}
%

\subsection{DRAM Command Sequence of \lisarc}

\newcommand{\sa}[1]{\texttt{SA#1}\xspace}
\newcommand{\rb}[1]{\texttt{RB#1}\xspace}
\newcommand{\tr}[2]{\texttt{RBM\textsubscript{#1$\rightarrow$#2}}\xspace}
\newcommand{\actcopy}[1]{\texttt{ACT\textsubscript{SA#1}}\xspace}

\figref{lisa_timelines_irsa} compares the service timelines of different
inter-subarray copy mechanisms. On the left side of the figure, we show an
example bank organization with three subarrays
(\mbox{\texttt{SA0$\leftrightarrow$2}}), along with their row buffers
(\mbox{\texttt{RB0}$\leftrightarrow$\rb{3}}). A \lisarc operation consists of
multiple existing DRAM and \xfer commands. We will illustrate how \lisarc
operates using an example that copies an arbitrary row from \sa{0} to \sa{2}, in
\figref{lisa_timelines_irsa}. Because a row activation latches a row into two
row buffers, \lisarc has to copy half a row at a time. We will first describe
copying the first half of the row.

First, \lisarc activates the source row (\actcopy{0}) to latch its data into two
buffers (\rb{0} and \rb{1}). Second, \lisarc invokes the first \xfer operation
(\tr{1}{3}) to move data from the bottom source row buffer (\rb{1}) to the
respective destination row buffer (\rb{3}). After this step, \lisarc cannot
immediately invoke another \xfer to transfer the trailing source \rb{0}. The
reason is that row buffers need to be in the \emph{precharge state} in order to
receive data from their neighbor row buffers. But \tr{1}{3} overwrites all the
intermediate row buffers in the chain (both \rb{1} and \rb{2}), which prevents
the source \rb{0} from transferring. Therefore, \lisarc completes copying the
first half of data into the destination row before invoking the second \xfer. It
does so by writing the row buffer (\rb{3}) into the cells through an activation
(\actcopy{2}), which uses the sense amplifiers to restore the latched value back
into the connected cells. To address the issue that modern DRAM chips do not
allow a second \act to an already activated bank, we use the \emph{back-to-back}
\act command that is used to support \rc~\cite{seshadri-micro2013}.

%Similar to \rciasa, \lisarc requires a back-to-back \act.

%For example, to copy data
%from \sa{0} to \sa{1}, \lisarc transfers data from \rb{1} to \rb{2} first
%(\tr{1}{2}) followed by an \act on \sa{1} to write the data into \sa{1}. Similar
%to FPM, \lisarc would also require back-to-back \act to the same bank.

Third, to move data from the trailing row buffer (\rb{0}) to complete the copy
transaction, we need to precharge \rb{1} and \rb{2}. The challenge here is to
precharge everything except for (\rb{0}), which cannot be accomplished in
today's DRAM because a precharge is applied at the bank level to all row
buffers. Therefore, we propose to add a new \emph{precharge-exception} signal,
which prevents a row buffer from being precharged and keeps it activated. This
bank-wide exception signal is supplied to all row buffers, and when raised for a
particular row buffer, the selected row buffer retains its state while the other
row buffers precharge. After the exception precharge
(\texttt{PRE\textsubscript{E}}) is complete, we then invoke the second \xfer and
write the data into cells. Compared to the service timeline of \rcirsa that
transfers cache line serially through the narrow global data lines, \lisarc
reduces the latency significantly by 9.03x using the \lisa substrate.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{ Third, after the leading row buffer completes writing. We need to
precharge all the row buffers in the path from the trailing row buffer to the
destination. The challenge here is to precharge everything except for the
trailing row buffer, which cannot be accomplished in today's DRAM because a
precharge is applied at the bank level to all row buffers. Therefore, to support
copying of the trailing row buffer, we propose to add a new
\emph{precharge-exception} signal that prevents a row buffer from being
precharged while keeping the row buffer activated. This exception signal is
supplied to every row buffer, and when it raises for a particular row buffer,
the selected row buffer retains its state while the other row buffers are
precharging. After the exception precharge is complete, we the process from step
two again with a different source row buffer to transfer.

Therefore, it copies the data from one row buffer first before it finishes off
the copy transaction with the second row buffer. For example, to copy data from
\sa{0} to \sa{1}, \lisarc transfers data from \rb{1} to \rb{2} first (\tr{1}{2})
followed by an \act on \sa{1} to write the data into \sa{1}. Then it re-initializes the
bitlines through a precharge in order to transfer the second half of the row (\tr{0}{1}). For each
additional two hops over two subarrays, the total latency increases by one
transfer (8ns). \figref{lisa_timelines_irsa} also illustrates a small increase in
terms of transfer latency when comparing a two-hop transfer to a one-hop
transfer. However, for our final evaluations, we simply assume that a one-hop transfer
incurs the same latency as a two-hop transfer. Equation \eqref{eq:1} defines the
total latency of \lisarc, and the transfer latency grows linearly with the hop
count. Lastly, the figure also shows the service timeline of PSM (inter-subarray)
that copies one cache line serially, which incurs longer latency than using \lisa
to perform copies.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Comparisons of Copy Techniques}
\label{sec:comp-copy}

\figref{copy_latency_energy} shows the copy latency and energy consumption of
different \emph{copy commands} copying a row of data. We derive the copy latency
using the equations listed in Appendix~\ref{sec:appendix}, which are based on
the DRAM command sequence for each mechanism. The specific latency and energy
numbers are also provided in Appendix~\ref{sec:appendix}.\footnote{Our reported
    numbers differ from prior work~\cite{seshadri-micro2013} because: (1) we use
    faster DRAM timing parameters (1600-11-11-11 vs 1066-8-8-8), and (2) we use
the typical row size of 8KB instead of 4KB~\cite{seshadri-micro2013}.}

\figputGHW{copy_latency_energy}{Copy latency and energy of different copy commands.}

We make several observations from these numbers. First, although \rcirsa incurs
similar latencies as \baseline, it consumes 29.6\% less energy from not
transferring data over the channel and I/O for each copy operation. However, as
discussed previously, \rcirsa incurs higher system performance penalty because
it's a long blocking operation. Second, by transferring data on \lisa, copying
between subarrays can achieve significantly lower latency and energy compared to
\rc despite the total latency of \lisarc grows linearly with the hop count
(i.e., the number of subarrays data is going across).

By exploiting the \lisa substrate, we form a more complete set of in-DRAM copy
mechanisms. Our evaluation results show that \lisarc operations outperforms
\rcirsa and \baseline in today's system. As we shall see in
Section~\ref{sec:eval_lisaclone}, the average performance gains and energy
reduction over the best performing inter-subarray copy mechanism (i.e.,
\baseline) are 59.6\% and 53.6\%, respectively, on a quad-core system running 50
workloads.

%\todo{get rid of copy granularity?}
%
%\input{sec/tables/copy_tradeoff}


==> sec/lisa/opt_pre.tex <==
% !TEX root = ../paper.tex

\section{Application 3: Fast Precharge Using Linked Precharge Units
(\lisapre)}
\label{sec:lisapre}

Our third application aims to accelerate the process of precharge. The
precharge time for a subarray is determined by the drive strength of the
precharge unit. We observe that in modern DRAM, while a subarray is being
precharged, the precharge units (PUs) of \emph{other} subarrays remain idle.

We propose to exploit these idle PUs to accelerate a precharge operation by
connecting them to the subarray that is being precharged. Our mechanism,
\emph{\lisa-\underline{LI}nked \underline{P}recharge} (\lisapre), precharges a
subarray using \emph{two} sets of PUs: one from the row buffer that is being
precharged, and a second set from a neighboring subarray's row buffer (which is
already in the precharged state), by enabling the links between the two
subarrays.

%\lisa can enable this by connecting the fully-driven
%bitlines of the subarray to be precharged with a neighbor subarray's bitlines,
%which are already precharged.

\figref{lisa_pre_states_longer_filled} shows the process of \emph{linked
precharging} using \lisa. Initially, only one subarray (top) is fully activated
(state \circled{1}) while the neighboring (bottom) subarray is in the precharged
state. The neighboring subarray is in the precharged state, as only one subarray
in a bank can be activated at a time, while the other subarrays remain
precharged.
% Also, in today's system, at most only one subarray can be activated while the
% rest has to remain in precharge state.
In state \circled{2}, we begin the precharge operation by disabling the sense
amplifier in the top row buffer and enabling its PU. After we enable the links
between the top and bottom subarrays, the bitlines start sharing charge with
each other, and both PUs \emph{simultaneously} reinitialize the bitlines,
eventually fully pulling the bitlines to $V_{DD}/2$ (state \circled{3}).
Note that we are using \emph{two} PUs to pull down \emph{only one} set of
activated bitlines, which is why the precharge process is shorter.

%\figputHW{lisa_pre_states_longer_filled}{Linked precharging through \lisa.}
\figputHS{lisa_pre_states_longer_filled}{0.9}{Linked precharging through \lisa.}

To evaluate the accelerated precharge process, we use the same methodology
described in Section~\ref{sec:trans_lat} and simulate the linked precharge
operation in SPICE. \figref{lisa_pre_spice_hpca} shows the resulting timing
diagram. During the first 2ns, the wordline is lowered to disconnect the cells
from the bitlines \circled{1}. Then, we enable the \isos to begin precharging
the bitlines \circled{2}. The result shows that the precharge latency reduces
significantly due to having two PUs to perform the precharge. \lisa enables a
shorter precharge latency of approximately 3.5ns \circled{3} versus the
baseline precharge latency of 13.1ns \circled{4}.

\ignore{ This is due not only to having two PUs to perform the precharge, but
also because of charge sharing between the connected bitlines. As we recall from
\figref{lisa_clone_spice_hpca} (\refsec{trans_lat}), when the activated bitline
connects with the precharged bitlines (state \circled{2}), the charge starts to
flow from the activated bitline to the other bitlines, thus helping to bring the
voltage closer to $V_{DD}/2$. Problem: I need to show the other BL's voltage to
prove this, which I do not have. }

\figputHS{lisa_pre_spice_hpca}{0.8}{SPICE simulation of precharge operation.}

To account for \textbf{process and temperature variation}, we add a guardband to
the SPICE-reported latency, increasing it to 5ns (i.e., by \emph{42.9\%}), which
    still achieves 2.6x lower precharge latency than the baseline. Our
    evaluation shows that \mbox{\lisapre} improves performance by 10.3\% on average,
    across 50 \mbox{four-core} workloads (see Section~\ref{sec:eval_lisapre}).


==> sec/lisa/opt_villa.tex <==
% !TEX root = ../paper.tex

\section{Application 2: In-DRAM Caching Using \mbox{Heterogeneous Subarrays
(\lisavilla)}}
\label{sec:villa}

Our second application aims to reduce the DRAM access latency for
frequently-accessed (hot) data. Prior work introduces heterogeneity into DRAM,
where one region has a fast access latency but small capacity (fewer DRAM rows),
while the other has a slow access latency but high capacity (many more
rows)~\cite{lee-hpca2013, son-isca2013}. To yield the highest performance
benefits, the fast region is used as a dynamic cache that stores the hot rows.
There are two design constraints that must be considered: (1)~\emph{ease of
implementation}, as the fast caching structure needs to be low-cost and
non-intrusive; and (2)~\emph{data movement cost}, as the caching mechanism
should adapt to dynamic program phase changes, which can lead to changes in the
set of hot DRAM rows.  As we show in Section~\ref{sec:villa:shortcomings}, prior
work has not balanced the trade-off between these two constraints.

% The fast region is used as a cache for
% the hot data to reduce its access latency. Prior works have looked at similar
% designs and there are two main design parameters that are related to
% heterogeneous designs. First, \emph{ease of design}, the fast caching structure
% needs to be low-cost and non-intrusive to existing DRAM. Second, \emph{migration
% cost}, to adapt to dynamic phase changes in programs, the hot data needs to
% constantly be migrated from the slow region to the fast region. Therefore, the
% efficacy of a heterogeneous design depends on the migration cost of hot data. In
% this work,

Our goal is to design a heterogeneous DRAM that offers fast data movement with
a low-cost and easy-to-implement design. To this end, we propose
\emph{\lisavilla (\underline{V}ar\underline{I}ab\underline{L}e
\underline{LA}tency)}, a mechanism that uses \lisa to provide fast row movement
into the cache when the set of hot DRAM rows changes. \mbox{\lisavilla} is also
easy to implement, as discussed in Section~\ref{sec:villa:dram}. We describe
our hot row caching policy in Section~\ref{sec:villa:caching}.

\subsection{Shortcomings of the State-of-the-Art}
\label{sec:villa:shortcomings}

We observe that two state-of-the-art techniques for heterogeneity
within a DRAM chip are not effective at providing \emph{both}
ease of implementation and low movement cost.

CHARM~\cite{son-isca2013} introduces heterogeneity \emph{within a rank} by
designing a few fast banks with (1)~shorter bitlines for faster data sensing,
and (2)~closer placement to the chip I/O for faster data transfers. To exploit
these low-latency banks, CHARM uses an OS-managed mechanism to statically
allocate hot data to them based on program profile information. Unfortunately,
this approach cannot adapt to program phase changes, limiting its performance
gains. If it were to adopt dynamic hot data management, CHARM would incur high
movement cost over the narrow 64-bit internal data bus in DRAM, as illustrated
in \figref{charm}, since it does not provide high-bandwidth connectivity
between banks.

\input{plots/villa_compare}

TL-DRAM~\cite{lee-hpca2013} provides heterogeneity \emph{within a subarray} by
dividing it into fast (near) and slow (far) segments that have short and long
bitlines, respectively, using isolation transistors. To manage the fast segment
as an OS-transparent hardware cache, TL-DRAM proposes a \emph{fast
intra-subarray movement} scheme similar to RowClone~\cite{seshadri-micro2013}.
The main disadvantage is that TL-DRAM needs to cache each hot row in \emph{two
near segments}, as shown in \figref{tldram}, as each subarray uses two row
buffers on \emph{opposite ends} to sense data in the open-bitline architecture.
This prevents TL-DRAM from using the \emph{full} near segment capacity.
TL-DRAM's area overhead is also sizable (3.15\%) in an open-bitline
architecture. As we can see, neither CHARM nor TL-DRAM strike a good trade-off
between the two design constraints.


\subsection{Variable Latency (VILLA) DRAM}
\label{sec:villa:dram}

We propose to introduce heterogeneity \emph{within a bank} by designing
\emph{heterogeneous-latency subarrays}. We call this heterogeneous DRAM design
\emph{\underline{V}ar\underline{I}ab\underline{L}e \underline{LA}tency DRAM}
(\villa). To design a low-cost fast subarray, we take an approach similar to
prior work, attaching fewer cells to each bitline to reduce the parasitic
capacitance and resistance. This reduces the sensing (\trcd), restoration
(\tras), and precharge (\trp) time of the fast subarrays~\cite{lee-hpca2013,
    micron-rldram3, son-isca2013}. In this work, we focus on managing the fast
    subarrays in hardware, as it offers better adaptivity to dynamic changes in
    the hot data set.

In order to take advantage of \villa, we rely on \lisarc to rapidly copy rows
across subarrays, which significantly reduces the caching latency. We call this
synergistic design, which builds \villa using the \lisa substrate,
\emph{\lisavilla}. Nonetheless, the cost of transferring data to a fast
subarray is still non-negligible, especially if the fast subarray is far from
the subarray where the data to be cached resides. Therefore, an intelligent
cost-aware mechanism is required to make astute decisions on which data to
cache and when.

\subsection{Caching Policy for \lisavilla}
\label{sec:villa:caching}

We design a simple epoch-based caching policy to evaluate the benefits of
caching a row in \lisavilla. Every epoch, we track the number of accesses to
rows by using a set of 1024 saturating counters for each bank.\footnote{The
    hardware cost of these counters is low, requiring only 6KB of storage in
the memory controller (see \secref{hwarea}).} The counter values are halved
every epoch to prevent staleness. At the end of an epoch, we mark the 16 most
frequently-accessed rows as \emph{hot}, and cache them when they are accessed
the next time. For our cache replacement policy, we use the \emph{benefit-based
caching} policy proposed by Lee et al.~\cite{lee-hpca2013}. Specifically, it
uses a benefit counter for each row cached in the fast subarray: whenever a
cached row is accessed, its counter is incremented. The row with the least
benefit is replaced when a new row needs to be inserted. Note that a large body
of work proposed various caching policies (e.g., \cite{hart-compcon1994,
hidaka-ieeemicro90,hsu-isca1993,jiang-hpca2010,kedem-1997,meza-cal2012,qureshi-isca2007,
seshadri-pact2012, yoon-iccd2012}), each of which can potentially be used with
\lisavilla.

Our evaluation shows that \lisavilla improves system performance by 5.1\% on
average, and up to 16.1\%, for a range of 4-core workloads
(see Section~\ref{sec:eval_lisavilla}).


==> sec/lisa/opt_villa_hpca_v1.tex <==
\section{Optimization 2: In-DRAM Caching via Heterogeneous Subarrays (\lisavilla)}
\label{sec:villa}

%\todo{New names? HALS (Hetero Access Lat Subarray). HEAL (HEt A L subarray), HALE
%(H A LatEncy) }

Our second optimization aims to reduce the DRAM access latency for frequently
accessed (hot) data by providing non-uniform access latency to DRAM. To this
end, we leverage the idea of introducing heterogeneity inside \emph{DRAM banks},
with fast subarrays that can cache the hot data. The design of fast subarrays
can be achieved by attaching fewer cells to each bitline to reduce the parasitic
capacitance and resistance, thereby accelerating the sensing (\trcd),
restoration (\tras), and precharge (\trp) time of the fast
subarrays~\cite{micron-rldram3, lee-hpca2013, son-isca2013}. As a result, we can
exploit these fast subarrays to store the hot data to reduce their access
latency. We call this heterogeneous DRAM design,
\emph{\underline{V}ar\underline{I}ab\underline{L}e \underline{LA}tency DRAM} or
\villa.

There are two potential ways to leverage the fast subarray. The first way is to
use it as a \emph{hardware-managed cache} for the regular subarrays, which is
transparent to the operating system (OS). The second way is to expose it as part
of memory to the OS, requiring the programmers or compilers to allocate hot data
in it. Compared to the OS-managed approach, using fast subarrays as
hardware-managed cache simplifies the hardware and software design without
costly usage-monitoring techniques. Therefore, in this work, we focus on the
hardware cache design.

The major \textbf{design challenge} with using \villa lies in enabling \emph{fast
data transfers} between the slow and fast subarrays within the same bank.
%This problem is essentially the same as what we described in the previous
%section on designing an efficient inter-subarray bulk-data copying mechanism.
With the conventional mechanism, transferring a row of data from the DRAM to the
memory controller, then writing the row back to the fast subarray, is too costly
-- high latency and energy consumption. Similarly, using \rcirsa incurs too much
overhead, outweighing the benefits of caching hot data in the fast subarray
(shown in Section~\ref{sec:eval_lisavilla}).

In order to enable \villa, we rely on \lisarc to rapidly copy rows across
subarrays, thus significantly reducing the caching latency. We call this
synergistic design of building \villa on \lisa, \emph{\lisavilla}. Nonetheless,
the cost of transferring data to the fast subarray is still non-negligible.
Therefore, an intelligent cost-aware caching mechanism is required to make
astute decisions on when and which data to cache.

\subsection{Caching Policy for \lisavilla}

In this work, we design a simple epoch-based caching policy to evaluate the
benefit of \lisavilla. Every epoch, we track the number of accesses of rows by
using a set of 1024 saturating counters for each bank. The counter values are
halved every interval to prevent stale values. At the end of an epoch, we mark
the top 16 most frequently accessed rows as hot, and cache them when they are
accessed. For the cache replacement policy, we use the \emph{benefit-based
caching} policy proposed by Lee et al.~\cite{lee-hpca2013}. Specifically, it
uses a benefit counter for each row cached in the fast subarray. When a cached
row is accessed, its counter is incremented. The row with the least benefit is
replaced when a new row needs to be inserted. Note that a large body of work has
proposed various caching policies in memory (e.g., \cite{hart-compcon1994,
kedem-1997,hidaka-ieeemicro90,hsu-isca1993,jiang-hpca2010, yoon-iccd2012}), each
of which can potentially be used on \lisavilla.

The key results show that \lisavilla improves system performance by 5.1\% on
average and up to 16.1\% for a list of 4-core workloads
(Section~\ref{sec:eval_lisavilla}).

\subsection{Qualitative Comparisons to Related Works}

Providing non-uniform DRAM access latency has been studied by multiple prior
works that introduce heterogeneity at different DRAM hierarchy. We will describe
two state-of-the-art works that provide heterogeneity within a DRAM chip. The
first work, TL-DRAM~\cite{lee-hpca2013}, divides each subarray into fast and
slow segments that have short and long bitlines, respectively, using isolation
transistors. The fast segment can be managed by either the hardware as a cache
or the software as part-of-memory, but it shows that hardware caching provides
more benefits than the software approach. Therefore, it proposes a fast
intra-subarray migration scheme similar to RowClone~\cite{seshadri-micro2013} to
support the hardware caching scheme.

The main disadvantage of TL-DRAM is that it needs to cache each hot row in
\emph{two near segments} because each subarray uses two row buffers on two
opposite ends to sense the data in the open-bitline DRAM. Therefore, in each
near segment, only half a row can benefit from low latency whereas the other
half of the row is actually considered in the far segment as it uses the other
row buffer on the far opposite end. By double caching each row, TL-DRAM requires
twice the area overhead compared to \villa for the same amount of caching
capacity. In addition, it may require more \act and \cpre commands to switch
between the two near segments to access the hot rows, incurring extra latency.

The second work, CHARM~\cite{lee-hpca2013}, achieves heterogeneity at the bank
level by designing a few fast banks with (1) shorter bitlines for faster data
sensing and (2) shorter data lines to the I/O for faster data transfers. CHARM
uses an OS-managed mechanism to statically map hot data to the low-latency banks,
based on profiled information from the compiler or programmers. However, relying
on static profiles has the downside of not being able to adapt to dynamic phase
changes in applications, lowering its potential performance gains. Even though CHARM can
adopt a dynamic mechanism to perform page migrations, it will suffer from the
costly inter-bank migration overhead as we have discussed extensively.

Compared to TL-DRAM and CHARM, \villa achieves the best of both worlds by
having: (1) adaptability to dynamic phase changes in applications with a
hardware-managed caching mechanism that benefits from fast data migrations and
(2) simple caching areas that do not require double migrations to cache each hot
row or wasted caching space. In the next section, we will introduce the third
\lisa optimization that is orthogonal to these works.

\ignore{Although the \lisavilla design may provide similar caching benefits as TL-DRAM
and CHARM, our \lisa substrate is more versatile, as it provides other
additional types of performance optimizations that cannot be achieved by either
of these works. Note that the focus of our work is not on designing a new
caching mechanism through asymmetric DRAM access latency, but on designing a new
substrate that enables a wide range of optimizations, including an efficient
mechanism to enable such caching. In the next section, we will introduce the
third \lisa optimization that is orthogonal to these works.}

%%% Notes %%%
%Unfortunately, TL-DRAM integrates
%isolation transistors directly into density-optimized cell arrays whereas \lisa
%places the isolation transistors outside the arrays with the peripherals.
%%% Notes %%%
%fetch granularity of DRAM = a cache line
%so if we want to design a cache, ideally we want it wider like the row buffer
%for spatial locality b/c a cache line is already stored in the cache hierarchy
%so it will have high reuse

%This design decision is to address some potential shortcomings associated with TL-DRAM and CHARM.
%1) TL-DRAM two short segments in open bitline.
%2) migration problem?


==> sec/lisa/other_apps.tex <==
% !TEX root = ../paper.tex

\section{Other Applications Enabled by \lisa}
\label{sec:other_apps}

We describe two additional applications that can potentially benefit from
\lisa. We describe them at a high level, and defer evaluations to future work.

\vspace{3pt} \noindent\textbf{Reducing Subarray Conflicts via Remapping.} When
two memory requests access two different rows in the same bank, they have to be
served serially, even if they are to different subarrays. To mitigate such
\emph{bank conflicts}, Kim et al.~\cite{kim-isca2012} propose
\emph{subarray-level parallelism (SALP)}, which enables multiple subarrays to
remain activated at the same time. However, if two accesses are to the same
subarray, they still have to be served serially. This problem is exacerbated
when \mbox{frequently-accessed} rows reside in the same subarray. To help
alleviate such \emph{subarray conflicts}, \lisa can enable a simple mechanism
that efficiently remaps or moves the conflicting rows to different subarrays by
exploiting fast \xfer operations.

\vspace{3pt} \noindent\textbf{Extending the Range of In-DRAM Bulk Operations.}
To accelerate bitwise operations, Seshadri et al.~\cite{seshadri-cal2015}
propose a new mechanism that performs bulk bitwise AND and OR operations in
DRAM. Their mechanism is restricted to applying bitwise operations
only on rows within the \emph{same subarray} as it requires the copying of
source rows before performing the bitwise operation. The high cost of
\emph{inter-subarray} copies makes the benefit of this mechanism inapplicable to
data residing in rows in different subarrays. LISA can enable efficient
inter-subarray bitwise operations by using \lisarc to copy rows to the same
subarray at low latency and low energy.


%When the mechanism detects frequent occurrence of subarray conflicts, it then
%remaps those conflict-induced rows to different subarrays to ensure better
%access distribution across the bank. We leave exploring the efficacy of this
%subarray-conflict-avoiding mapping policy as part of the future work.
%To demonstrate the effect of subarray conflicts, we employ SALP and allocate X
%more numbers of row buffers for each subarray. Figure X shows that as the
%number of row buffer increases for each subarray, perform increases, up to Z%.

%\subsection{Micro-Pages}
%\label{sec:micro_pages}
\ignore{
\noindent\textbf{Micro-Pages.} To mitigate bank conflicts, Sudan et
al.~\cite{sudan-asplos2010} observe that only a small portion of each OS page is
accessed in a time period. Therefore, they propose to co-locate these small
chunks (micro-pages) from each page into a DRAM row to increase row buffer hit
rate. This technique requires them to reduce the OS page size to 1KB to co-locate
different pages. In addition, it requires a heavy page movement scheme.

\lisa can efficiently implement their proposal. Instead of shrinking the page
size, which is intrusive to the operating system, we can use \lisavilla to cache
the frequently-accessed chunks from every rows inside a bank and modify the
transfer granularity of \lisa to the chunk size (i.e., 1KB, which is a quarter
of each row buffer). This would result in a less heavy-overhead implementation
for micro-pages.
}


==> sec/lisa/related.tex <==
% !TEX root = ../paper.tex

\section{Related Work}
\label{sec:related}

To our knowledge, this is the first work to propose a DRAM substrate that
supports fast data movement between subarrays in the same bank, which enables a
wide variety of applications for DRAM systems. We already provided extensive
comparisons to RowClone~\cite{seshadri-micro2013}, CHARM~\cite{son-isca2013},
and TL-DRAM~\cite{lee-hpca2013}. We now discuss prior works that focus on each
of the optimizations that \lisa enables.

\vspace{3pt}
\noindent\textbf{Bulk Data Transfer Mechanisms.} Prior
works~\cite{gschwind-cf2006, gummaraju-pact2007, kahle-ibmjrd2005} have added
scratchpad memories to reduce CPU pressure during bulk data transfers, which
can also enable sophisticated data movement (e.g., scatter-gather), but they
still require data to first be moved on-chip.
% The PCI-DMA engine only allows bulk data to
% be copied between the CPU and memory~\cite{linux-dma}.
A patent proposes a DRAM that can copy a page across memory
blocks~\cite{seo-patent}, but lacks concrete analysis and evaluation of the
underlying copy operations. Intel I/O Acceleration Technology~\cite{intelioat}
allows for memory-to-memory DMA transfers \emph{across a network}, but cannot
transfer data within main memory.

Zhao et al.~\cite{zhao-iccd2005} propose to add a bulk data movement engine inside the memory
controller to speed up bulk-copy operations. Jiang et
al.~\cite{jiang-pact2009} design a different copy engine, placed within the
cache controller, to alleviate pipeline and cache stalls that occur when these
transfers take place. However, these works do not directly address the problem
of data movement across the narrow memory channel.

A concurrent work by Lu et al.~\cite{lu-micro2015} proposes a heterogeneous
DRAM design similar to \villa, called \mbox{DAS-DRAM}, but with a very
different data movement mechanism from LISA. It introduces a row of
\emph{migration cells} into each subarray to move rows across subarrays.
Unfortunately, the latency of DAS-DRAM is not scalable with movement distance,
because it requires writing the migrating row into each intermediate subarray's
migration cells before the row reaches its destination, which prolongs data
transfer latency. In contrast, LISA provides a \emph{direct path} to transfer
data \emph{between row buffers} without requiring intermediate data writes into
the subarray.

%thus also requiring higher caching area overhead for its DRAM design.
%In contrast, \lisarc quickly transfers the moved data through the links and
%sense amplifiers without writing any data in the intermediate subarray.

\ignore{
DMA engines are currently used to facilitate large-scale data transfers within
processors, but are limited in the types of workloads that they can impact.
PCI-DMA, for example, only allows bulk data to be copied between the CPU and
memory~\cite{linux-dma}.  Scratchpad memories have been used in conjunction
with streaming processors to reduce CPU pressure during these transfers, and
can even be used to enable sophisticated data movement such as scatter-gather,
but still require the data to come on-chip~\cite{gummaraju-pact2007,
gschwind-cf2006, kahle-ibmjrd2005}.  Intel I/O Acceleration Technology allows
for memory-to-memory DMA transfers across a network, but does not enable
transfers within main memory~\cite{intelioat}.  DMA mechanisms typically
require the processor to write to memory-mapped I/O locations, and notify the
processor of completion by raising an interrupt, both of which can be costly
operations.}

%A number of prior works have studied how to reduce the impact of the von
%Neumann bottleneck due to data transfers.  Zhao et al.\ studied the use of a
%bulk data movement engine for servers~\cite{zhao-iccd2005}.
%They speed up these operations by embedding the copy engine
%inside the memory controller.  The copy engine is treated as a coprocessor,
%where the CPU uses a register-based interface to inform the engine of the
%region to copy.  This avoids the long-latency memory operations and interrupts
%required to invoke a DMA transfer.  While the copy engine was a viable solution
%for its time, it took advantage of the fact that the memory controller was
%off-chip and close to DRAM, thereby reducing movement across the memory channel.
%However, the vast majority of today's processors contain integrated memory
%controllers.  The copy engine cannot be moved into DRAM directly, as it can
%only issue load and store requests, thus forcing it to once again use the
%constricted channel.
%
%FastBCI designs a different copy engine, placed within
%the cache controller, in order to alleviate pipeline and cache stalls that
%occur when these transfers take place~\cite{jiang-pact2009}.  FastBCI
%introduces scalar operations that perform copies at large granularities, thus
%avoiding the need for a load-store loop.  These operations can
%non-speculatively retire early, with hardware that tracks instruction
%dependencies on the in-progress copy, thus allowing independent instructions
%to continue execution and retirement.  While FastBCI allows for greater CPU
%throughput, masking some of the performance delays associated with bulk data
%transfer, it does not directly address the unnecessary movement of this data
%between DRAM and the processor chip.
%
%Since \lisa offers a substrate that can
%perform in-DRAM movement without utilizing the memory channel, both of these
%copy engines can be used on top of \lisa to restore and improve their expected
%gains.
%
%RowClone~\cite{seshadri-micro2013} provides an in-DRAM solution for bulk
%data transfer, but can only do so at limited scope and granularity, as we have
%discussed earlier.  We quantitatively show that \lisa not only exploits greater
%opportunities for bulk copy over RowClone, but that it can be used to improve
%other operations as well.

\vspace{3pt}
\noindent\textbf{Caching.} Several prior works (e.g., \cite{hart-compcon1994,
hidaka-ieeemicro90, hsu-isca1993, kedem-1997}) have proposed to add a small
SRAM cache to DRAM chips, which obtains lower access latency at the cost of
high area overhead. Many other works (e.g., \cite{collins-micro1999,
jaleel-pact2008, jaleel-isca2010,piquet-acsac2007, qureshi-isca2006,
qureshi-micro2006, qureshi-isca2007, seshadri-pact2012}) have proposed various
cache management policies. Such caching policies can potentially be integrated
with \lisavilla to achieve a better hit rate in the fast subarrays.


\vspace{3pt}
\noindent\textbf{Reducing DRAM Latency.} Several types of DRAM provide low
latency, such as Micron's RLDRAM~\cite{micron-rldram3} or Fujitsu's
FCDRAM~\cite{sato-vlsic1998}. These have fewer cells connected to each bitline,
which comes with a large overhead~\cite{kim-isca2012, lee-hpca2013}.

%\ignore{Fast Cycle RAM uses a subarray structure to in essence pipeline
%DRAM~\cite{sato-vlsic1998}.  This is achieved by partitioning the array
%vertically, resulting in fewer columns in each subarray. RLDRAM exploits
%subarrays to create a cache-like structure that can be addressed similar to
%SRAM~\cite{micron-rldram3}.  However, both of these approaches require a high
%area overhead to achieve lower access time latencies.}

O et al.~\cite{o-isca2014} propose to add isolation transistors that separate
bitlines from their sense amplifiers so that the bitlines can be precharged
without deactivating the row buffer. This helps to hide the latency impact of
precharge.  These isolation transistors are orthogonal to isolation transistors
in \lisa, which interconnect bitlines of \emph{neighboring subarrays}, and \lisa
can be combined with~\cite{o-isca2014} to further improve performance. LISA can
also be combined with many other proposals that reduce DRAM latency
(e.g.,~\cite{chang-hpca2014,chargecache,kim-isca2012,lee-tech2010,lee-hpca2015,lee-hpca2013}).

%Tiered-latency DRAM rearchitects DRAM subarrays by splitting them into two
%tiers with non-uniform access latencies~\cite{lee-hpca2013}.  Through the use
%of an isolation transistor, a subset of rows can be accessed quickly by
%reducing the effective length of the bitline.  CHARM exploits non-uniformity
%on a bank level in order to balance performance improvements with area
%overhead~\cite{son-isca2013}.  Select banks have their aspect ratio increased
%by reducing the number of wordlines per mat, therefore increasing the number
%of mats.  These mats are then grouped close to I/O, and are used to store
%performance-critical pages as identified by the OS.

%Subarray level parallelism (SALP) takes advantage of the existing subarray
%architecture to overlap multiple memory requests going to the same
%bank~\cite{kim-isca2012}.  As subarrays contain local row buffers, they can
%be activated concurrently with minimal additional hardware, allowing
%overlapping activation and precharge to independent subarrays as well as row
%buffer caching for inactive subarrays.  Row buffer decoupling splits the
%precharging operation into two parts~\cite{o-isca2014}.  Through the use of
%an isolation transistor separating the bitline from the sense amplifier, the
%bitlines can be precharged immediately after row activation.  The sense
%amplifiers are precharged when a row needs to be closed, but since they
%precharge much faster than the bitlines, the effective precharge time observed
%by the memory controller decreases significantly.



==> sec/lisa/tables/4c_copy_norm_ws.tex <==
\begin{table}[h]
\small
\centering
    \setlength{\tabcolsep}{.33em}
    \begin{tabular}{lcc}
      \toprule
      %\textbf{Copy Methods} & Baseline & RC Inter-SA & RC Inter-Bank & RC Intra-SA & LISA-Clone-15\\
      %\midrule
      %\textbf{Weighted Speedup (WS)} & 1.0 & 0.99 & 0.98 & 0.95 \\
      %\textbf{WS Improvement (\%)} & 1.0 & 0.99 & 0.98 & 0.95 \\

      \textbf{Copy Methods} & \textbf{WS} & \textbf{Normalized WS} \\
      \midrule
      Baseline & 1.96 & 1.00\\
      RC Inter-SA & 1.96 & 1.00\\
      RC Inter-Bank & 2.66 & 1.36 \\
      RC Intra-SA & 4.42 & 2.26 \\
      LISA-Clone-15 & 4.17 & 2.13 \\
      LISA-Clone-1 & 4.50 & 2.19 \\
      Ideal & 4.51 & 2.50 \\
      \bottomrule
    \end{tabular}
\caption{Performance comparisons on a 4-core system.}
\label{tab:4c_copy_norm_ws}
\end{table}


==> sec/lisa/tables/copy_tradeoff.tex <==
\begin{table}[h]
\begin{footnotesize}
  \centering
    \begin{tabular}{llll}
        \toprule
        \textbf{Methods} & \textbf{Latency} & \textbf{Copy Range} & \textbf{Copy
    Granularity} \\
        \cmidrule(rl){1-4}

        Baseline & High & All channels & Cache line (64B) \\

        \rcirsa & Medium $\leftrightarrow$ High & All banks & Cache line \\

        \textbf{\lisarc} & Low $\leftrightarrow$ Medium & One bank & Cache line $\leftrightarrow$  Row \\

        \rciasa & Low & One subarray & Row (8KB) \\

        \bottomrule
    \end{tabular}
    %\begin{tabular}{lllll}
    %    \toprule
    %    Methods & Latency & Copy Range & Copy Granularity & Energy\\
    %    \cmidrule(rl){1-5}

    %    Baseline & High & All channels & Cacheline (64B)  & High \\
    %    FPM & Low & One subarray & Row (8KB) & Low\\
    %    PSM & Med. $\leftrightarrow$ High & All banks & Cacheline (64B) &
    %    Med.\\
    %    \lisarc & Low $\leftrightarrow$ Med. & One bank & Cacheline
    %    $\leftrightarrow$  Row & Low\\

    %    \bottomrule
    %\end{tabular}
    \caption{Comparison of copy mechanism properties.}
  \label{tab:copy_tradeoff}%
\end{footnotesize}
\end{table}


==> sec/lisa/tables/dram_cmds.tex <==
\begin{table}[h]
\begin{footnotesize}
  \centering
    %\setlength{\tabcolsep}{.55em}
    \begin{tabular}{llr}
        \toprule
        Commands & Timing Parameters & Time (ns) \\
        \cmidrule(rl){1-3}
        \act $\rightarrow$ \crd/\cwr & \trcd & 13.75ns \\
        \crd $\rightarrow$ Data & \tcl & 13.75ns \\
        \cwr $\rightarrow$ Data & \tcwl & 10ns \\
        \act $\rightarrow$ \cpre & \tras & 35ns \\
        \cpre $\rightarrow$ \act & \trp & 13.75ns \\
        \bottomrule
    \end{tabular}
    \caption{Timing parameters for DRAM commands in DDR3-1600~\cite{jedec-ddr3}.}
  \label{tab:timing_parameters}%
\end{footnotesize}
\end{table}


==> sec/lisa/tables/intro_opt.tex <==
\begin{table}[h]
\begin{small}
  \centering
    \setlength{\tabcolsep}{.50em}
    \begin{tabular}{ll}
        \toprule
        %Index & Description\\
        %\cmidrule(rl){1-4}
        1. & A new bulk-data copy mechanism that uses \lisa to transfer data. \\
        \cmidrule(rl){1-2}

        2. & Precharge subarrays with two precharge units. \\
        \cmidrule(rl){1-2}

        \multirow{2}{*}{3.} & Use \lisa to perform fast in-DRAM caching in \\
                            & a heterogeneous DRAM with fast and slow subarrays. \\
        \cmidrule(rl){1-2}

        \multirow{2}{*}{4.} & Reduce subarray conflicts among frequently \\
                            & accessed rows when subarray-level parallelism is employed. \\

        \cmidrule(rl){1-2}

        \multirow{2}{*}{4.} & Enable fast collocation of frequently accessed \\
                            & sub-pages into a small number of row. \\
        \bottomrule
    \end{tabular}
    \caption{A list of optimizations enabled by \lisa.}
  \label{tab:intro_opt}
\end{small}
\end{table}


==> sec/lisa/tables/intro_opt_wide.tex <==
\begin{table*}[b]
    \begin{small}
        \centering
        %\setlength{\tabcolsep}{.40em}
        \begin{tabular}{p{1.5in}p{3.50in}p{1.78in}}
            \toprule
            \textbf{Problem} & \textbf{Mechanism LISA Enables}  & \textbf{Key
        System Benefits} \\
            \cmidrule(rl){1-3}
            \multirow{3}{*}{\minipage{1.5in}Slow inter-subarray data copying (1363.75ns for
            8KB). \refsec{lisaclone}\endminipage}&
                \underline{\lisarc}$\dagger$: Use \lisa to
            copy data between subarrays in the same bank with short latency --
            151ns, 88.9\% latency and 97.9\% DRAM energy
            reduction over prior work~\cite{seshadri-micro2013}.
            & 59.6\% system performance gain and 53.6\% DRAM energy reduction on
            a 4-core system.\\

            \cmidrule(rl){1-3}
            %High migration cost between heterogeneous subarrays. \refsec{villa}
            High memory access latency. \refsec{villa}
            & \underline{\lisavilla}$\dagger$: We add fast subarrays for caching
            in every bank and use \lisa to migrate/cache data.
            & Up to 16.1\% performance improvement and 5.1\% on average.\\

            \cmidrule(rl){1-3}
            \multirow{3}{*}{\minipage{1.5in}Slow precharge time (13.75ns).
            \refsec{lisapre}\endminipage} &
            \underline{\lisapre}$\dagger$: Use an extra
            precharge unit from the neighbor's subarray through \lisa to accelerate
            the precharge process (5ns -- 63.6\% latency reduction). &
            Up to 13.2\% performance improvement and 8.1\% on average.\\
            %8.1\% system performance gain and X\% DRAM energy reduction on
            %a 4-core system.\\

            %in a heterogeneous DRAM that adds fast subarrays for caching in every
            %bank. & 3.2\% average and 7.9\% maximum performance improvement.\\
            %Slow data transfers inhibit a DRAM design that adds
            %small, fast subarrays as caches. \refsec{villa}
            %& \underline{\lisavilla}$\dagger$: Use \lisa to transfer/cache data in a
            %heterogeneous DRAM that adds fast subarrays for caching in every
            %bank. & 3.2\% average and 7.9\% maximum performance improvement.\\

            \cmidrule(rl){1-3}
            \multirow{2}{*}{Subarray conflicts. \refsec{sa_remap}} & Remaps conflict-inflicting
            rows to different subarrays through \lisa when subarray-level
            parallelism~\cite{kim-isca2012} is employed. & Latency reduction due
            to fewer subarray conflicts. \\

            \cmidrule(rl){1-3} High-cost implementation of
            micro-pages~\cite{sudan-asplos2010}. \refsec{micro_pages} & \lisa enables an efficient
            implementation of prior work that collocates frequently accessed
            sub-pages into a small number of rows. & Performance improvement of
            micro-pages at low cost.\\

            \bottomrule
            \multicolumn{3}{r}{$\dagger$: We quantitatively evaluate the first three optimizations
            in this work.}
        \end{tabular}
        \caption{A list of optimizations \lisa enables.}
        \label{tab:intro_opt_wide}
    \end{small}
\end{table*}

%Slow data transfer latency from slow subarrays to fast subarrays for caching


==> sec/lisa/tables/migration_opt.tex <==
\begin{table*}[b]
    \begin{small}
        \centering
        %\setlength{\tabcolsep}{.40em}
        \begin{tabular}{p{1.45in}p{2.96in}p{2.1in}}

            \toprule
            \textbf{Problem} & \textbf{Mechanism LISA Enables}  & \textbf{Key
        System Benefits} \\
            \cmidrule(rl){1-3}
            \multirow{2}{*}{\minipage{1.5in}Slow inter-subarray data copying
            (\refsec{lisaclone})\endminipage} &
                \underline{\lisarcnol}$\dagger$:
                Bulk data copying between
                subarrays by exploiting LISA's \xfer operation.
                & Reduces (1) latency by 9.03x, (2)
                DRAM energy by 48.1x, over \rc~\cite{seshadri-micro2013}. \\
            %    --
            %151ns, 88.9\% latency reduction over prior work~\cite{seshadri-micro2013}.
            %& 59.6\% system performance gain and 53.6\% DRAM energy reduction.\\

            \cmidrule(rl){1-3}
            %High migration cost between heterogeneous subarrays. \refsec{villa}
            %Imbalanced heterogeneous DRAM designs~\cite{lee-hpca2013,son-isca2013}.

            High memory access latency (\refsec{villa}) &
            \underline{\lisavillanol}$\dagger$:
            Caches hot data via fast inter-subarray movement between
            heterogeneous subarrays within a bank.
            %Uses fast inter-subarray movement
            %to enable heterogeneous subarrays within a bank for caching.
            & Up to 16.1\% performance improvement (5.1\% on average) across 50 workloads.\\

            \cmidrule(rl){1-3}
            \multirow{2}{*}{\minipage{1.5in}Slow precharge time
            (\refsec{lisapre})\endminipage} &
            \underline{\lisaprenol}$\dagger$: Use extra
            precharge units from a neighboring subarray to accelerate the precharge
            process. & Up to 13.2\% performance improvement (8.1\% on average)
            across 50 workloads.\\

            \cmidrule(rl){1-3}
            \multirow{2}{*}{Subarray access conflicts} & Remaps conflicting rows in the
            same subarray to different subarrays when subarray-level
            parallelism~\cite{kim-isca2012} is employed. & Memory latency reduction due
            to fewer subarray conflicts. \\


            \cmidrule(rl){1-3} Costly row movement for \mbox{in-DRAM} Boolean
            logic~\cite{seshadri-cal2015} & Enables fast bulk bitwise AND and OR
            operations on two rows from \emph{different} subarrays. &
            Performance improvement from the extended range of bulk operations.
            \\

            %\cmidrule(rl){1-3} High-cost implementation of
            %micro-pages~\cite{sudan-asplos2010}. & Enable an efficient
            %implementation to quickly colocate frequently accessed
            %sub-pages into a small number of rows. & Performance improvement of
            %micro-pages at low cost.\\

            \bottomrule
            \multicolumn{3}{r}{$\dagger$: We quantitatively evaluate these optimizations in this work.}
        \end{tabular}
        \caption{A list of optimizations that benefit from \lisa's fast inter-subarray
        data movement.}
        \label{tab:migration_opt}
    \end{small}
\end{table*}

%Slow data transfer latency from slow subarrays to fast subarrays for caching


==> sec/lisa/tables/migration_opt_short.tex <==
\begin{table*}[b]
    \begin{small}
        \centering
        %\setlength{\tabcolsep}{.40em}
        \renewcommand{\arraystretch}{0.8}
        \begin{tabular}{p{1.45in}p{2.96in}p{2.1in}}

            \toprule
            \textbf{Problem} & \textbf{Mechanism LISA Enables}  & \textbf{Key
        System Benefits} \\

            \cmidrule(rl){1-3}
            \multirow{2}{*}{Subarray access conflicts} & Remaps conflicting rows in the
            same subarray to different subarrays when subarray-level
            parallelism~\cite{kim-isca2012} is employed. & Memory latency reduction due
            to fewer subarray conflicts. \\


            \cmidrule(rl){1-3} Costly row movement for \mbox{in-DRAM} Boolean
            logic~\cite{seshadri-cal2015} & Enables fast bulk bitwise AND and OR
            operations on two rows from \emph{different} subarrays. &
            Performance improvement from the extended range of bulk logic operations.
            \\

            %\cmidrule(rl){1-3} High-cost implementation of
            %micro-pages~\cite{sudan-asplos2010}. & Enable an efficient
            %implementation to quickly colocate frequently accessed
            %sub-pages into a small number of rows. & Performance improvement of
            %micro-pages at low cost.\\

            \bottomrule
        \end{tabular}
        \caption{Some additional applications that benefit from \lisa's fast inter-subarray
        data movement.}
        \label{tab:migration_opt_short}
    \end{small}
\end{table*}

%Slow data transfer latency from slow subarrays to fast subarrays for caching


==> sec/lisa/thesis_background.tex <==
% !TEX root = ../../paper.tex

\section{DRAM Subarrays}
\label{sec:background:dram}
\label{sec:background}

In this chapter, we focus on operations across subarrays within the \emph{same}
bank, which require us to delve deeper into the physical organization of a bank.
Typically, a bank is subdivided into multiple
\emph{subarrays}~\cite{chang-hpca2014, kim-isca2012, seshadri-micro2013,
  vogelsang-micro2010}, as shown in \figref{background_bank_sa_detail}.
%\footnote{Note that we are illustrating a logical view of the bank.  Throughout
%this section, we abstract away the multiple chips that physically exist within
%a rank for the sake of clarity.} Note that we are illustrating the bank
%structure at a logical level that covers all eight chips in a \texttt{x8} rank
%to abstract away the physical-level detail for clarity.}
Each subarray consists of a 2D-array of DRAM cells that are connected to sense
amplifiers through \emph{bitlines}. Because the size of a sense amplifier is
more than 100x the size of a cell~\cite{lee-hpca2013}, modern DRAM designs fit
in only enough sense amplifiers in a row to sense \emph{half a row of cells}. To
sense the \emph{entire} row of cells, each subarray has bitlines that connect to
\emph{two rows} of sense amplifiers --- one above and one below the cell array
(\circled{1} and \circled{2} in \figref{background_bank_sa_detail}, for Subarray
1). This DRAM design is known as the \emph{open bitline architecture}, and is
commonly used to achieve high-density DRAM~\cite{lim-isscc2012,
  takahashi-jsscc2001}. A single row of
sense amplifiers, which holds the data from \emph{half} a row of activated
cells, is also referred as a \emph{row buffer}.

\figputHS{background_bank_sa_detail}{1.1}{Bank and subarray organization in a
DRAM chip.}

\subsection{DRAM Subarray Operation}
\label{sec:background:access}

Accessing data in a subarray requires two steps. The DRAM row (typically 8KB
across a rank of eight x8 chips) must first be \emph{activated}. Only
after activation completes, a column command (i.e., a \crd/\cwr)
can operate on a piece of data (typically 64B across a rank; the
size of a single cache line) from that row.

When an \act command with a row address is issued, the data stored within a row
in a subarray is read by \emph{two} row buffers (i.e., the row buffer at the
top of the subarray \circled{1} and the one at the bottom \circled{2}). First,
a wordline corresponding to the row address is selected by the subarray's row
decoder. Then, the top row buffer and the bottom row buffer
each sense the charge stored in half of the row's cells through the bitlines,
and amplify the charge to full digital logic values (0 or 1) to latch in the
cells' data.

After an \act finishes latching a row of cells into the row buffers, a
\crd or a \cwr can be issued. Because a typical read/write memory request is
made at the granularity of a single cache line, only a subset of bits are
selected from a subarray's row buffer by the column decoder.
%, typically 64B out of 8KB.
On a \crd, the selected column bits are sent to the global sense
amplifiers through the \emph{internal data bus} (also known as the global data
lines) \circled{3}, which has a narrow width of 64B across a rank of eight
chips. The global sense amplifiers \circled{4} then drive the data to the bank
I/O logic \circled{5}, which sends the data out of the DRAM chip to the memory
controller.

While the row is activated, a consecutive column command to the same row can
access the data from the row buffer without performing an additional \act. This
is called a \emph{row buffer hit}. In order to access a different row, a \cpre
command is required to reinitialize the bitlines' values for another \act. This
re-initialization process is completed by a set of \emph{precharge units}
\circled{6} in the row buffer. For more detail on DRAM commands and internal
DRAM operation, we refer the reader to prior works~\cite{kim-isca2012,
lee-hpca2015, lee-hpca2013, liu-isca2012, seshadri-micro2013, son-isca2013}.


==> sec/parref/0-abstract.tex <==

%%% ONUR: What you have below is way too detailed and not crips. Need
%%% to be more crisp. No need to reintroduce the well-known concept of
%%% banks... See how I rephrased it to be more crisp. There is still
%%% room for improvement.
%%%

%%% ONUR: Second, the downside of per-bank refresh was not organized
%%% well. Instead of saying ``However, ... Furthermore, ...'', it is
%%% much better to say ``There are two key issues. First, ... Second,
%%% ...'' This leads to a much better organization. Having
%%% ``furthermore'' makes it sound like the second problem is less
%%% important.

%%% ONUR: Can you fix these issues in other parts of the paper as
%%% well? The above are fundamental principles in writing a strong
%%% paper. (Let me go through the intro first while you are fixing
%%% these elsewhere)

Modern DRAM cells are periodically refreshed to prevent data loss due
to leakage. Commodity DDR (double data rate) DRAM refreshes cells at
the rank level. This degrades performance significantly because it
prevents an entire DRAM rank from serving memory requests while being
refreshed. DRAM designed for mobile platforms, LPDDR (low power DDR)
DRAM, supports an enhanced mode, called per-bank refresh, that
refreshes cells at the bank level. This enables a bank to be accessed
while another in the same rank is being refreshed, alleviating part of
the negative performance impact of refreshes. Unfortunately, there are
two shortcomings of per-bank refresh employed in today's systems.
First, we observe that the per-bank refresh scheduling scheme does not
exploit the full potential of overlapping refreshes with accesses
across banks because it restricts the banks to be refreshed in a
sequential round-robin order. Second, accesses to a bank that is being
refreshed have to wait.

%%% ONUR: see my more crisp rewrite of the last sentence above.

%memory accesses are forced to
%stall when they collide with refreshes within the same bank.

%To
%alleviate the negative impact of refreshes, DRAM designed for mobile platforms,
%LPDDR (low power double data rate) DRAM, supports a refresh mode that allows
%memory accesses to certain parts of a rank during refresh. Because a rank
%consists of multiple indepedent accessible banks, LPDDR DRAM enables accesses to
%a refreshing rank by refreshing at the bank level. This refresh mode in LPDDR
%DRAM is also called per-bank refresh.


%%% ONUR: The below also needed to be more crisp. I went over it, but
%%% it can benefit from more.
%%% It would be better to organize the \ib mechanism as ``First,
%%% ... Second, ...''as I mentioned above.

To mitigate the negative performance impact of DRAM refresh, we
propose two complementary mechanisms, \ib (\darplong) and \is
(\intersub). The goal is to address the drawbacks of per-bank refresh
by building more efficient techniques to parallelize refreshes and
accesses within DRAM. First, instead of issuing per-bank refreshes in a
round-robin order, as it is done today, \ib issues per-bank refreshes
to idle banks in an out-of-order manner. Furthermore, \ib proactively
schedules refreshes during intervals when a batch of writes are
draining to DRAM. Second, \is exploits the existence of mostly-independent
{\em subarrays} within a bank. With minor modifications to DRAM
organization, it allows a bank to serve memory accesses to an idle
subarray while another subarray is being refreshed. Extensive
evaluations on a wide variety of workloads and systems show that our
mechanisms improve system performance (and energy efficiency) compared
to three \mbox{state-of-the-art} refresh policies and the performance
benefit increases as DRAM density increases.

% 0106
%Modern DRAM cells are periodically refreshed to prevent data loss from leakage.
%These refresh operations degrade system performance because they prevent an
%entire DRAM rank from serving memory requests. To alleviate the negative impact
%of refreshes, DRAM designed for mobile platforms, LPDDR, supports refreshing
%each bank separately in a sequential round-robin order to allow simultaneous
%memory accesses to non-refreshing banks. However, we observe that this per-bank
%refresh mode does not always improve performance and can even degrade
%performance.

% 0107
%Modern DRAM cells are periodically refreshed to prevent data loss from leakage.
%These refresh operations degrade system performance because they prevent an
%entire DRAM rank from serving memory requests. To alleviate the negative impact
%of refreshes, DRAM designed for mobile platforms, LPDDR, supports refreshing
%each bank separately in a sequential round-robin order to allow simultaneous
%memory accesses to non-refreshing banks. However, we observe that this strict
%in-order scheduling prevents it from exploiting the full benefit of overlapping
%refreshes with accesses across banks. Furthermore, memory accesses are forced
%to stall when they collide with refreshes within the same bank.
%
%To mitigate the negative performance impact of DRAM refreshes, we propose two
%complementary mechanisms, \ib (\darplong) and \is (\intersub). The goal is to
%hide refresh latency by serving refreshes to banks or subarrays in parallel
%with memory accesses. Instead of issuing per-bank refreshes in a round-robin
%order, as it is done today, \ib issues per-bank refreshes to idle banks in an
%out-of-order manner. Furthermore, \ib proactively schedules refreshes during
%intervals when a batch of writes are draining to DRAM. \is enables a bank to
%serve memory accesses from an idle subarray while another subarray is being
%refreshed. Extensive evaluations on a wide variety of workloads show that our
%mechanisms improve multi-core system performance compared to three
%\mbox{state-of-the-art} refresh policies and the performance benefit increases
%as DRAM density increases.


==> sec/parref/1-intro.tex <==
\section{Introduction} \label{sec:intro}

Modern main memory is predominantly built using \emph{dynamic random
  access memory} (DRAM) cells. A DRAM cell consists of a capacitor to
store one bit of data as electrical charge. The capacitor leaks charge
over time, causing stored data to change. As a result, DRAM requires
an operation called \emph{refresh} that periodically restores
electrical charge in DRAM cells to maintain data integrity.

%% ONUR: THe new organization is better but the writing is really not
%% crisp. See below for things to fix.

%% Refresh as a problem

%%% ONUR: The paragreph below. Fine in terms of content. However,
%%% there are grammar issues and unexplained numbers. For example,
%%% where does the 12.4% number come from?
%%% ``Dram is under refresh operations'' is very awkward.

%%% ``Because DRAM is required to refresh more cells within the same
%%% refresh interval, the refresh overhead will increase.''
%%% --> ONUR: The explanation above was very awkward as well. You will
%%% --> need to make your writing crisp and the flow much better.

%%% ONUR: I made the performance point a footnote, as it was breaking
%%% the flow. Please be very conscious of the flow. I removed it after
%%% further consideration as it is better to merge it with the 29% number.

%%% ONUR: What is the refresh mechanism used to obatin the 12.4% and
%%% 29% numbers?
% Kevin: All-bank refresh.
%%% ONUR2: OK, please double check all numbers in he paper. All
%%% numbers in the paper and explanations in text should be
%%% consistent.

%\footnote{This causes 12.4\% performance degradation on an
%  8-core system using 8Gb DDR3 DRAM as we show in
%  Section~\ref{XXX}}.

Each DRAM cell must be refreshed periodically every {\em refresh interval} as
specified by the DRAM standards~\cite{jedec-ddr3,jedec-lpddr3}. The exact
refresh interval time depends on the DRAM type (e.g., DDR or LPDDR) and the
operating temperature.  While DRAM is being refreshed, it becomes unavailable to
serve memory requests. As a result, refresh latency significantly degrades
system performance~\cite{liu-isca2012, mukundan-isca2013,
nair-hpca2013,stuecheli-micro2010} by delaying in-flight memory requests. This
problem will become more prevalent as DRAM density increases, leading to more
DRAM rows to be refreshed within the same refresh interval.  DRAM chip density
is expected to increase from 8Gb to 32Gb by 2020 as it doubles every two to
three years~\cite{itrs-dram}. Our evaluations show that DRAM refresh, as it is
performed today, causes an average performance degradation of 8.2\% and 19.9\%
for 8Gb and 32Gb DRAM chips, respectively, on a variety of memory-intensive
workloads running on an 8-core system. Hence, it is important to develop
practical mechanisms to mitigate the performance penalty of DRAM refresh.

%%% ONUR: The below is not organized well. Please rewrite. The
%%% organization of the abstract is much better. Do not start with the
%%% sentence ``We now provide a quick summary ...'' Not good. It is
%%% better to integrate this summary into the explanation.

%%% ONUR: Here is a much better way to start: There are two major ways
%%% refresh operations are performed in modern DRAM systems: {\em
%%% all-bank refresh} and {\em per-bank refresh}.

%%% ONUR: See what I have done below. The flow is much better but the
%%% specific sentences can still be made better.

There are two major ways refresh operations are performed in modern DRAM
systems: {\em all-bank refresh (or, rank-level refresh)} and {\em per-bank
refresh}. These methods differ in what levels of the DRAM hierarchy refresh
operations tie up to. A modern DRAM system is organized as a hierarchy of ranks and
banks. Each rank is composed of multiple banks. Different ranks and banks can be
accessed independently. Each bank contains a number of rows (e.g., 16-32K in
modern chips). Because successively refreshing {\em all} rows in a DRAM chip
%,of which there are tens of thousands in,
would cause very high delay by tying up
the entire DRAM device, modern memory controllers issue a number of refresh
commands that are evenly distributed throughout the refresh
interval~\cite{jedec-ddr3,jedec-lpddr3,liu-isca2013,liu-isca2012,nair-hpca2013}.
Each refresh command refreshes a small number of rows.\footnote{The time between
two refresh commands is fixed to an amount that is dependent on the DRAM type
and temperature.} The two common refresh methods of today differ in where in
the DRAM hierarchy the rows refreshed by a refresh command reside.

In {\em all-bank refresh}, employed by both commodity DDR and LPDDR
DRAM chips, a refresh command operates at the rank level: it refreshes
a number of rows in {\em all} banks of a rank concurrently. This
causes every bank within a rank to be unavailable to serve memory
requests until the refresh command is complete.  Therefore, it
degrades performance significantly, as we demonstrate in
Section~\ref{sec:motivation} and as others have
demonstrated~\cite{liu-isca2012, mukundan-isca2013,
  nair-hpca2013,stuecheli-micro2010}. In {\em per-bank refresh},
employed by LPDDR DRAM~\cite{jedec-lpddr3, micronLPDDR2_2Gb} as an
alternative refresh mode, a refresh command operates at the bank
level: it refreshes a number of rows in only a single bank of a rank
at a time.\footnote{One can think of per-bank refresh as splitting up
  a single large all-bank refresh operation performed on an entire
  rank into smaller groups of refresh operations performed on each
  bank.} This enables a bank to be accessed while another in the same
rank is being refreshed, alleviating part of the negative performance
impact of refreshes (as we show in
Section~\ref{sec:motivation}). Unfortunately, per-bank refresh suffers
from two shortcomings that limit the ability of DRAM to serve requests
while refresh operations are being performed. First, we observe that
the per-bank refresh scheduling scheme does not exploit the full
potential of overlapping refreshes with accesses across banks because
it restricts the banks to be refreshed in a strict sequential {\em
  round-robin order}~\cite{jedec-lpddr3}. Second, accesses to a bank
that is being refreshed still have to wait as there is no way today to
perform a refresh and an access to the same bank concurrently. We find
that, due to these shortcomings, a significant performance degradation
still exists with per-bank refresh (Section~\ref{sec:motivation}).

%% DRAM/Refresh background
\ignore{

%%% ONUR: OLD COMMENT: this really needs to be either better integrated or needs to go into background...
%%% ONUR: NEW COMMENT: See my rewrite above. The below is not flowing well and is not organized crisply.

We now provide a quick summary on how refresh works in today's commodity DDR
DRAM. Modern DRAM is organized as a hierarchy of ranks, banks, and subarrays.
Each rank is composed of multiple banks and each bank contains subarrays. A subarray
consists of a 2-D arrays of cells organized in rows and columns. Because modern
DRAM devices contain thousands of rows, refreshing all of them in succession
incurs high latency. Instead, memory controllers send a number of refresh
commands that are evenly distributed throughout the refresh
interval~\cite{jedec-ddr3,jedec-lpddr3,nair-hpca2013}. The time between two
refresh commands is fixed to an amount that is dependent
on the DRAM type and temperature. As a result, each
refresh command refreshes some numbers of rows in DRAM. When commodity DDR DRAM
receives a refresh command, it starts to perform refresh operations at the rank
level, refreshing multiple rows across banks. Therefore, this refresh scheme is
also called \emph{all-bank refresh}, causing every bank within a rank to become
unavailable to serve requests during refresh.

%% Per-bank refresh
To help alleviate refresh latency, LPDDR DRAM~\cite{jedec-lpddr3,
micronLPDDR2_2Gb} supports a refresh mode that splits up an all-bank refresh
operation into multiple smaller groups of refreshes. Each of these refreshes is
called a \emph{per-bank refresh} and it is issued periodically to only one bank
at a time in a strict \emph{round-robin order} as opposed to the entire rank of DRAM.
In contrast to using all-bank refresh that locks up DRAM by refreshing every
bank, using per-bank refresh allows partial access to DRAM, specifically the
non-refreshing banks, while a single bank is under refresh. Our evaluations show
that per-bank refresh improves system performance by 4.0\% over the conventional
all-bank refresh on an 8-core system.
But, we find that per-bank refresh has two main issues. First, it does
not maximize the potential benefit from overlapping refreshes with accesses
across banks due to its restrictive in-order scheduling policy. Second, it stalls
accesses to a bank that is being refreshed.
}

%%% ONUR: The below paragraph is good.
Our goal is to alleviate the shortcomings of per-bank refresh by enabling more
efficient parallelization of refreshes and accesses within DRAM. The major ideas
are to (1) provide a more flexible scheduling policy for traditional per-bank
refresh and (2) exploit the internal {\em subarray} structure of a bank to
enable parallelization of refreshes and accesses within a bank. To this end, we
propose two complementary techniques.

%%% ONUR: The below is well organized. References needed; see
%%% below. Better to add back the turnaround time explanation.

%%% ONUR2: Round robin reference should come earlier so I moved it up.
The first technique, \emph{\darplong (\darp)}, is a new refresh
scheduling policy based on two key ideas: \emph{\ooolong} and
\emph{\warplong}. The first idea enables the memory controller to
specify an idle bank to be refreshed as opposed to the
state-of-the-art per-bank refresh policy that refreshes banks in a
strict round-robin order. By monitoring the bank request queues'
occupancies, \darp avoids refreshing a bank that has pending memory
requests and instead refreshes an idle bank to maximize
parallelization of refreshes and accesses. The second idea hides
refresh latency with write accesses by proactively scheduling per-bank
refreshes during the time period when banks are serving write
requests. There are two reasons why we attempt to parallelize refresh
operations with write accesses. First, modern systems typically buffer
write requests in memory controllers and drain them to DRAM in a batch
to mitigate the \mbox{\emph{bus turnaround}}
penalty~\cite{chatterjee-hpca2012,lee-tech2010,stuecheli-isca2010}.
Write batching allows our mechanism to proactively schedule a per-bank
refresh to a bank while other banks are serving the accumulated write
requests, thus enabling more parallelization of refreshes and writes
to hide refresh latency.  Second, although \ib can potentially delay
write requests to some of the banks, this does not significantly
affect system performance. The reason is that DRAM writes (which are
writebacks from the last-level
cache~\cite{lee-tech2010,stuecheli-isca2010}) are not latency-critical
as processors do not stall to wait for them to finish.
%%% ONUR2: ``does not affect performance'' was too strong. Better to qualify it with ``significantly''

%Therefore, a write request can be delayed for some period of time without
%affecting performance. Taking advantage of this observation, \ib selects a bank
%with a few writes to perform per-bank refresh.

%%% ONUR: The above paragraph ends a bit abruptly

%%% ONUR: See my changes below. The problem was ``the technique'' was
%%% kind of introduced twice... Better to say its full name right away
%%% in the first sentence to preserve ``English sentence-level
%%% parallelism'' with the first technique's description in the above
%%% paragraph.

%%% ONUR: Please add the citations below. Please also fix the
%%% formatting.

%%% ONUR2: ``K. Itoh, VLSI Memory Chip Design. Springer, 2001.''
%%% Reference has extra spaces? Please check...

The second technique, \emph{\intersub (\is)}, takes advantage of the
fact that a DRAM bank is composed of multiple \emph{subarrays} and
each subarray has its own local \emph{sense
  amplifiers}~\cite{itoh-vlsi, kim-isca2012, lee-hpca2013,
  moon-isscc2009,vogelsangmoon-micro2010}. We observe that only a few
subarrays are refreshed within a bank when the other subarrays and the
DRAM I/O bus remain completely idle. Based on this observation,
\emph{\is} enables a bank to be accessible while being refreshed: it
can serve read or write requests to idle subarrays while other
subarrays in the bank are being refreshed. Therefore, \is reduces the
interference of refreshes on demand requests at the cost of very
modest modifications to DRAM devices.
%%% ONUR2: Second to last sentence above was not good. Fixed now.

We make the following major \textbf{contributions}:

\begin{itemize}

\item We propose a new per-bank refresh scheduling policy, \darp
  (\darplong), to proactively schedule refreshes to banks that are
  idle or that are draining writes.

\item We propose a new DRAM refresh mechanism, \is (\intersub), to
  enable a bank to serve memory requests in idle subarrays while other
  subarrays are being refreshed.

%\item We perform extensive evaluations and analysis of \emph{per-bank} refresh
%mode. We show that it improves performance when there are sufficient memory
%request streams provided in a multi-core system to exploit its benefit of
%\mbox{bank-level} parallelism, but degrades performance in a single-core system
%with limited amount of outstanding memory requests.

%\item Combining the two complementary mechanisms improves system performance of an 8-core
%system by 3.3\%/7.2\%/15.2\% on average across 100 workloads and up to
%7.1\%/14.5\%/27.0\% over per-bank refresh for 8/16/32Gb DRAM devices. Compared
%to previously proposed elastic refresh~\cite{stuecheli-micro2010}, our mechanisms improve system
%performance significantly (Section~\ref{sec:multi-core-results}).

%%% ONUR: You cannot simply introduce DSARP without explaining
%%% it. This last contribution needs a rewrite. You evaluate the
%%% benefits of all proposals. However, you choose to report the
%%% combination in the below contribution description. Please rewrite.
%%% Also, the evaluation contribution is not powerful. You evaluate
%%% other core counts and configurations as well. You may not report
%%% them here, but the reader needs to understand the context and
%%% extent of evaluation here. See my rewrite now.

\item We comprehensively evaluate the performance and energy benefits
  of \ib and \is, and their combination, \emph{\combo}, compared to
  three state-of-the-art refresh policies across a wide variety of
  workloads and system configurations.  One particular evaluation
  shows that \combo improves system performance by 3.3\%/7.2\%/15.2\%
  on average (and up to 7.1\%/14.5\%/27.0\%) across 100 workloads over
  the best previous mechanism (per-bank refresh) for 8/16/32Gb DRAM
  devices. \combo's performance gain increases as workload memory
  intensity and core count increase.

%%% ONUR2: Last sentence was bad. It had DARP. That should be DSARP,
%%% right? No need to say ``other evaluations'' (this weakens the
%%% sentence; it is obvious that these results are obtained via
%%% evaluation as the first sentence in the contribution states).

%%% ONUR2: Please proofread the entire paper carefully.

\end{itemize}



==> sec/parref/2-background-camera.tex <==
\section{Background}
\label{sec:background}

\subsection{DRAM System Organization}
\label{sec:dram-org}
At a high level, a DRAM system is
organized as a hierarchy of ranks and banks as shown in
\figref{dram-organization-v2}. Each rank consists of multiple banks that share
an internal bus for reading/writing data.\footnote{A typical DRAM system has 2
ranks connected to each channel and 8 banks per rank.} Because each bank acts as
an independent entity, banks can serve multiple memory requests in parallel,
offering \emph{bank-level
parallelism}~\cite{kim-micro2010,lee-micro2009,mutlu-isca2008}.

%%% ONUR: Show at least one more rank in this figure. You can do this
%%% by having the top rank cover most of the bottom one.
\figputHS{dram-organization-v2}{1.0}{DRAM system organization.}

%%% ONUR: Please fix the grammar everywhere. I fix some but may miss
%%% some also. Common issues include 1) plural/singular mismatch for
%%% subject and verb, 2) lack of sentence-level parallelism in
%%% parallel language constructs, 3) inconsistent capitalization of
%%% words in captions.
A DRAM bank is further sub-divided into multiple
\emph{subarrays}~\cite{kim-isca2012, seshadri-micro2013, vogelsangmoon-micro2010} as shown in
\figref{bank-organization}.
%Subarrays are fundamental structures with which all DRAMs that we know of are
%using to allow wires to remain short, fast, and low power~\cite{itoh-vlsi}.
A subarray consists of a 2-D array of cells organized in rows and
columns.\footnote{Physically, DRAM has 32 to 64 subarrays, which
  varies depending on the number of rows (typically 16-32K) within a
  bank. We divide them into 8 subarray groups and refer to a subarray
  group as a subarray~\cite{kim-isca2012}.} Each DRAM cell has two
components: 1) a \emph{capacitor} that stores one bit of data as
electrical charge and 2) an \emph{access transistor} that connects the
capacitor to a wire called \emph{bitline} that is shared by a column
of cells. The access transistor is controlled by a wire called
\emph{wordline} that is shared by a row of cells.  When a wordline is
raised to $V_{DD}$, a row of cells becomes connected to the bitlines,
allowing reading or writing data to the connected row of cells. The
component that reads or writes a bit of data on a bitline is called a
\emph{sense amplifier}, shared by an entire column of cells. A row of
sense amplifiers is also called a \emph{row buffer}. All subarrays'
row buffers are connected to an I/O buffer~\cite{khoetal-isscc2009,
  moon-isscc2009} that reads and writes data from/to the bank's I/O
bus.

%%% ONUR2: Minor nit: The capitalization of first letters of words of
%%% different references is inconsistent. The PARBS reference has all
%%% important words' first letters capitalized, whereas the Mukundan
%%% reference does not. It would be good to fix this, but this is a
%%% nit.

%%% ONUR: Give a good idea of how many rows in a subarray, how many
%%% subarrays in a bank, how many banks in a rank, how many ranks in a
%%% module... Provide typical numbers. This can be done with a footnote.

%%% ONUR: Show the ``row'' within the subarray in this figure.
\figputHS{bank-organization}{0.8}{DRAM bank and subarray organization.}


%%% ONUR: ``Because there are thousands of rows in DRAM,''
%%% --> in a DRAM chip?
%%% --> ``tens of thousands'' is much better.

\subsection{DRAM Refresh} %\textbf{All-Bank Refresh (\refab)}.
\subsubsection{All-Bank Refresh (\refab)} The minimum time interval during which
any cell can retain its electrical charge without being refreshed is called the
\emph{minimum retention time}, which depends on the operating temperature and
DRAM type. Because there are tens of thousands of rows in DRAM, refreshing all
of them in bulk incurs high latency. Instead, memory controllers send a number
of refresh commands that are evenly distributed throughout the retention time to
trigger refresh operations, as shown in \figref{ab_timeline}. Because a typical
refresh command in a commodity DDR DRAM chip operates at an entire rank level,
it is also called an \emph{all-bank refresh} or \emph{\refab} for
short~\cite{jedec-ddr3,jedec-lpddr3,micronLPDDR2_2Gb}. The timeline shows that the time
between two \refab commands is specified by \trefi (e.g., 7.8$\mu$s for 64ms
retention time). Therefore, refreshing a rank requires $\sfrac{64ms}{7.8\mu
s}\approx8192$ refreshes and each operation refreshes exactly $\sfrac{1}{8192}$
of the rank's rows.

%\footnote{The equality is inexact because the standard allows eight refresh
%commands to be issued early or late.}

When a rank receives a refresh command, it sends the command to a DRAM-internal
refresh unit that selects which specific rows or banks to refresh. A \refab
command triggers the refresh unit to refresh a number of rows in every bank for
a period of time called \trfc (\figref{ab_timeline}). During \trfc, banks are
not refreshed simultaneously. Instead, refresh operations are staggered
(pipelined) across banks~\cite{mukundan-isca2013}. The main reason is that
refreshing every bank simultaneously would draw more current than what the power
delivery network can sustain, leading to potentially incorrect DRAM
operation~\cite{mukundan-isca2013, shevgoor-micro2013}. Because a \refab command
triggers refreshes on all the banks within a rank, the rank cannot process any
memory requests during \trfc, The length of \trfc is a function of the number of
rows to be refreshed.

%%% ONUR2: The above has grammar issues and was not crisp. I fixed it.
%%% Example: potential incorrect --> potentially incorrect

%%% ONUR: Unclear what ``temporal coverage'' means in these figures. ``Timeline''
%%% ONUR: Also, the distance between the two refresh commands separated with ... is too small for both fig a and b.
%%% ONUR: Can you try to fix this?
%%% ONUR: Also, comparing (a) and (b), is it your intent to show that
%%% it takes *longer* to complete all 8 REFpb's than it takes to
%%% complete a REFab.
\input{plots/refresh_background}

\subsubsection{Per-Bank Refresh (\refpb)}
%Because an all-bank refresh occupies every bank in a rank, it prevents the rank
%from serving any requests during refresh.
To allow partial access to DRAM during refresh, LPDDR DRAM (which is
designed for mobile platforms), supports an additional
finer-granularity refresh scheme, called \emph{per-bank refresh}
(\refpb for short)~\cite{jedec-lpddr3,micronLPDDR2_2Gb}. It splits up
a \refab operation into eight separate operations scattered across
eight banks (\figref{pb_timeline}).  Therefore, a \refpb command is
issued eight times more frequently than a \refab command (i.e.,
\trefipb = \trefi / 8).

Similar to issuing a \refab, a controller simply sends a \refpb
command to DRAM every \trefipb without specifying which particular
bank to refresh. Instead, when a rank's internal refresh unit receives
a \refpb command, it refreshes only one bank for each command
following a \emph{sequential round-robin order} as shown in
\figref{pb_timeline}. The refresh unit uses an internal counter to
keep track of which bank to refresh next.

By scattering refresh operations from \refab into multiple and
non-overlapping per-bank refresh operations, the refresh latency of
\refpb (\trfcpb) becomes shorter than \trfc. Disallowing \refpb
operations from overlapping with each other is a design decision made
by the LPDDR DRAM standard committee~\cite{jedec-lpddr3}. The reason
is simplicity: to avoid the need to introduce new timing constraints,
such as the timing between two overlapped refresh
operations.\footnote{At slightly increased complexity, one can
  potentially propose a modified standard that allows overlapped
  refresh of a subset of banks within a rank.}
%one may potentially draw up a new specification
%that enables DRAM to refresh any arbitrary number of banks in parallel
%through a single command.
%%% ONUR2: Last sentence above did not convey what you are trying to
%%% say. Please rephrase. I do not understand what you are trying to
%%% say because it is not clear.

%Note that \trfcpb (refresh
%latency of \refpb) is shorter than \trfc because banks are not
%refreshed simultaneously during all-bank refresh. Instead, refresh
%operations are staggered (pipelined) across banks. The main reason is
%that refreshing every bank simultaneously would draw more current than
%what the power delivery network can sustain, leading to potential
%incorrect DRAM operations~\cite{mukundan-isca2013,
%  shevgoor-micro2013}.  \refpb operations are also disallowed to
%overlap with each other across different banks based on the current
%standard~\cite{jedec-lpddr3}.

%%% ONUR: This sentence comes abruptly and is not well explained. It
%%% contradicts the picture in 8a, which shows that *all* banks are
%%% refreshed simultaneously in all-bank refresh. You need to think
%%% about the organization of this discussion. It is probably better
%%% to make it a separate paragraph. Please rethink to be very clear...
%%% ``Note that \trfcpb (refresh latency of \refpb) is shorter than
%%% \trfc because banks are not refreshed simultaneously during
%%% all-bank refresh. Instead, refresh operations are staggered
%%% (pipelined) across banks. The main reason is ...''

%%% ONUR: Also, see my comments on the figure. Basically, think
%%% exactly what you are going to tell the reader in the first two
%%% paragraphs of the ``per-bank refresh'' section and in what order
%%% you will tell these. Then, rephrase and reorder. What you have is
%%% a good start but there is an organization/ordering/what-to-tell
%%% issue.

%%% ONUR: You say: ``\refpb operations are also disallowed to overlap
%%% with each other across different banks based on the current
%%% standard~\cite{jedec-lpddr3}.'' Why is this the case? Anything
%%% fundamental?


%%% ONUR: Below. Please provide a conclusion saying service time is
%%% saved. Also, please rewrite the first sentence to be more clear.

With the support of \refpb, LPDDR DRAM can serve memory requests to
non-refreshing banks in parallel with a refresh operation in a single
bank.  \figref{per-bank-refresh-timeline} shows pictorially how \refpb
provides performance benefits over \refab from parallelization of
refreshes and reads.  \refpb reduces refresh interference on reads by
issuing a refresh to Bank 0 while Bank 1 is serving
reads. Subsequently, it refreshes Bank 1 to allow Bank 0 to serve a
read. As a result, \refpb alleviates part of the performance loss due
to refreshes by enabling parallelization of refreshes and accesses
across banks.
%%% ONUR: It is important to have a conclusion here.


%With the support for \refpb, LPDDR DRAM can serve memory requests in
%other non-refreshing banks and send data back to the processor while a
%bank is under refresh.
%\figref{per-bank-refresh-timeline} shows
%pictorially how \refpb provides performance benefits over \refab from
%parallelization of refreshes and reads. \refpb reduces refresh
%interference on reads by issuing a refresh to Bank 0 while Bank 1 is
%serving reads. Subsequently, it refreshes Bank 1 to allow Bank 0 to
%serve a read.
%%%% ONUR: It is important to have a conclusion here.

%%% ONUR2: Saved Cycles in REFpb --> Saved Cycles w/ REFpb

\input{plots/per-bank-refresh-timeline}


==> sec/parref/3-motivation-camera.tex <==
\section{Motivation}
\label{sec:motivation}

%%% ONUR: Need to be more crisp and better organized here. Overall
%%% organization is fine, but individual sentences and arguments need
%%% more clarity. I took my pass now, but there is still room for
%%% improvement.

In this section, we first describe the scaling trend of commonly used
all-bank refresh in both LPDDR and DDR DRAM as chip density increases
in the future. We then provide a quantitative analysis of all-bank
refresh to show its performance impact on multi-core systems followed
by performance comparisons to per-bank refresh that is only supported
in LPDDR.


\subsection{Increasing Performance Impact of Refresh}
\label{sec:refresh-challenge}

%%% ONUR: ``Performance bottleneck of refresh'' was awkward.
%%%  ``Refresh as a performance bottleneck'' is better but see what I
%%%  have above.

During the \trfc time period, the entire memory rank is locked up, preventing
the memory controller from sending any memory request. As a result, refresh
operations degrade system performance by increasing the latency of memory
accesses. The negative impact on system performance is expected to be
exacerbated as \trfc increases with higher DRAM density. The value of \trfc is
currently 350ns for an 8Gb memory device~\cite{jedec-ddr3}. \figref{rfc_trend}
shows our estimated trend of \trfc for future DRAM generations using linear
extrapolation on the currently available and previous DRAM devices. The same
methodology is used in prior works~\cite{liu-isca2012,stuecheli-micro2010}.
\emph{Projection 1} is an extrapolation based on 1, 2, and 4Gb devices;
\emph{Projection 2} is based on 4 and 8Gb devices. We use the more optimistic
\emph{Projection 2} for our evaluations. As it shows, \trfc may reach up to
1.6$\mu$s for future 64Gb DRAM devices. This long period of unavailability to
process memory accesses is detrimental to system performance.

%%% ONUR: Please start x axis from 1. 0 does not make sense.
\figputGHS{rfc_trend}{1.0}{Refresh latency (\captrfc) trend.}

To demonstrate the negative system performance impact of DRAM refresh,
we evaluate 100 randomly mixed workloads categorized to five different
groups based on memory intensity on an 8-core system using various
DRAM densities.\footnote{Detailed methodology is described in
  Section~\ref{methodology}, including workloads, simulation
  methodology, and performance metrics.\label{fnote}} We use up to
32Gb DRAM density that the ITRS predicts to be manufactured by
2020~\cite{itrs-dram}. \figref{perf_loss_mpki} shows the average
performance loss due to all-bank refresh compared to an ideal baseline
without any refreshes for each memory-intensity category. The
performance degradation due to refresh becomes more severe as either
DRAM chip density (i.e., \trfc) or workload memory intensity increases
(both of which are trends in systems), demonstrating that it is
increasingly important to address the problem of DRAM refresh.
%%% ONUR: refresh issues --> This was very vague at the end of last sentence above.

%%% ONUR: caption: ``Memory Intensive'' --> ``Memory-intensive''; In --> in
\figputGHS{perf_loss_mpki}{1.0}{Performance degradation due to refresh.}

%%% ONUR: For the below paragraph:
%%% 1. ``they are'': unclear? who are?

%%% ONUR2: an LPDDR2 (instead of a LPDDR2)
%%% ONUR2: a 2Gb LPDDR2 (instead of an 2Gb LPDDR2)

Even though the current DDR3 standard does not support \refpb, we believe that
it is important to evaluate the performance impact of \refpb on DDR3 DRAM
because DDR3 DRAM chips are widely deployed in desktops and servers.
Furthermore, adding per-bank refresh support to a DDR3 DRAM chip should be
non-intrusive because it does not change the internal bank organization. We
estimate the refresh latency of \refpb in a DDR3 chip based on the values used
in an LPDDR2 chip. In a 2Gb LPDDR2 chip, the per-bank refresh latency (\trfcpb)
is 90ns and the all-bank refresh latency (\trfc) is 210ns, which takes
\emph{2.3x} longer than \trfcpb~\cite{micronLPDDR2_2Gb}.\footnote{LPDDR2 has a
shorter \trfc than DDR3 because LPDDR2 1) has a retention time of 32ms instead
of 64ms in DDR3 under normal operating temperature and 2) each operation
refreshes fewer rows.} We apply this multiplicative factor to \trfc to calculate
\trfcpb.
%As a result, the estimated \trfcpb is 152ns with \trfc of 350ns in an 8Gb DDR3
%device.

Based on the estimated \trfcpb values, we evaluate the performance impact of
\refpb on the same 8-core system and workloads.\textsuperscript{\ref{fnote}}
\figref{perf_loss_all} shows the average performance degradation of \refab and
\refpb compared to an ideal baseline without any refreshes. Even though \refpb
provides performance gains over \refab by allowing DRAM accesses to
non-refreshing banks, its performance degradation becomes exacerbated as \trfcpb
increases with higher DRAM density. With 32Gb DRAM chips using \refpb, the
performance loss due to DRAM refresh is still a significant 16.6\% on average,
which motivates us to address issues related to \refpb.

%%% ONUR: see my rewrite of the above sentence.

\figputGHS{perf_loss_all}{1.0}{Performance loss due to \caprefab and \caprefpb.}

%%% ONUR: I modified the below as well. Still can be better.

\subsection{Our Goal} We identify two main problems that \refpb faces. First,
\refpb commands are scheduled in a very restrictive manner in today's systems.
Memory controllers have to send \refpb commands in a sequential round-robin
order without any flexibility. Therefore, the current implementation does not
exploit the full benefit from overlapping refreshes with accesses across banks.
Second, \refpb cannot serve accesses to a refreshing bank until the refresh of
that bank is complete.  Our goal is to provide practical mechanisms to address
these two problems so that we can minimize the performance overhead of DRAM
refresh. %latency.

%Our goal is to mitigate the negative performance impact due to DRAM
%refresh and to provide performance improvement over existing refresh schemes
%by proposing practical mechanisms to address these two problems.

%%%%%%%%%%%%%%%%%%%%%
% 0106 %
%%%%%%%%%%%%%%%%%%%%%
%\refpb consistently reduces refresh
%penalty on system performance over \refab because \refpb
%allows a multi-core system to utilize the available non-refreshing banks while
%only a single bank is refreshing. However, similar to \refab, the performance
%degradation of \refpb also becomes exacerbated with higher DRAM density due to increased
%\trfcpb. With 32Gb DRAM, there is a large potential performance
%improvement if we eliminate all refreshes.
%%%%%%%%%%%%%%%%%%%%%

%\figputHS{motivation-perf-loss}{0.8}{Performance loss of all-bank and per-bank
%refresh compared to an ideal no-refresh baseline averaged across all 8-core
%workloads.}
%\figputGHS{perf_loss_all}{1.0}{Performance loss due to \refab and \refpb.}

%\subsection{Our Goal}
%
%Although our evaluations show that \refpb provides performance improvement over
%the conventional \refab in a multi-core system, the opportunity to further
%reduce performance loss from \refpb becomes more significant as DRAM density
%increases.
%Our goal is to mitigate the negative performance impact due to DRAM
%refresh and provide performance improvement over existing refresh schemes.


==> sec/parref/4-mech.tex <==
\section{Mechanisms}
\label{sec:mechanism}

\subsection{Overview}

%%% ONUR: I made the beloew more crisp. It can still be made
%%% better. In particular, the two sentences that started with ``The
%%% second component'' were repetitive and not providing the key
%%% insight of hiding refresh latency with write latency. It is
%%% important to provide this.

We propose two mechanisms, \emph{\darplong (\darp)} and
\emph{\intersub (\is)}, that hide refresh latency by parallelizing
refreshes with memory accesses across \emph{banks} and
\emph{subarrays}, respectively. \darp is a new refresh scheduling
policy that consists of two components. The first component is
\emph{\ooolong} that enables the memory controller to specify a
particular (idle) bank to be refreshed as opposed to the standard
per-bank refresh policy that refreshes banks in a strict round-robin
order. With out-of-order refresh scheduling, \darp can avoid
refreshing (non-idle) banks with pending memory requests, thereby
avoiding the refresh latency for those requests. The second component
is \emph{\warplong} that proactively issues per-bank refresh to a bank
while DRAM is draining write batches to other banks, thereby
overlapping refresh latency with write latency. The second mechanism,
\is, allows a bank to serve memory accesses in idle subarrays while
other subarrays within the same bank are being refreshed. \is exploits
the fact that refreshing a row is contained within a subarray, without
affecting the other subarrays' components and the I/O bus used for
transferring data. We now describe each mechanism in detail.

%The first component is \emph{\ooolong} that enables the memory controller to
%specify an idle bank to be refreshed as opposed to state-of-the-art per-bank
%refresh policy that strictly refreshes banks in a round-robin order. Therefore,
%\darp avoids refreshing a bank that has pending memory requests to increase
%parallelization of refreshes and accesses.

%decouples the sequential bank selection logic
%from DRAM and instead enables the memory controller to specify which bank to
%refresh.

%It takes advantage of the fact that a write request is off
%the critical path for processor progress. Therefore, delaying a write request in
%a bank does not directly impact the performance of any processor.

%leverages the observation from prior
%research~\cite{kim-isca2012} that multiple subarrays can be accessed in parallel
%with minor DRAM changes. While the prior work mainly focuses on reducing DRAM
%latency due to bank conflicts, we propose a mechanism to allow a bank to
%parallelize memory accesses in idle subarrays with refreshes in other subarrays.

\subsection{\darplong}

%Section~\ref{sec:refresh-challenge}
%explains an alternate refresh mode called \emph{per-bank refresh}
%(\refpb) that refreshes one bank for each auto refresh command. However, the
%current per-bank refresh mechanisms disallow a memory controller from specifying which bank
%to refresh. Instead, DRAM has an internal logic that strictly refreshes banks
%with a \emph{sequential round-robin order} in a rank.

%\textbf{\ooolongCap}.
\subsubsection{\ooolongCap} The limitation of the current per-bank refresh
mechanism is that it disallows a memory controller from specifying
which bank to refresh. Instead, a DRAM chip has internal logic that
strictly refreshes banks in a \emph{sequential round-robin order}.
Because DRAM lacks visibility into a memory controller's state (e.g.,
request queues' occupancy), simply using an in-order \refpb policy can
unnecessarily refresh a bank that has multiple pending memory requests
to be served when other banks may be free to serve a refresh
command. To address this problem, we propose the first component of
\darp, \emph{\ooolong}. The idea is to remove the bank selection logic
from DRAM and make it the memory controller's responsibility to
determine which bank to refresh. As a result, the memory controller
can refresh an idle bank to enhance parallelization of refreshes and
accesses, avoiding refreshing a bank that has pending memory requests
as much as possible.

Due to \refpb reordering, the memory controller needs to guarantee
that deviating from the original in-order schedule still preserves
data integrity. To achieve this, we take advantage of the fact that
the contemporary DDR JEDEC standard~\cite{jedec-ddr3,jedec-ddr4}
actually provides some refresh scheduling flexibility. The standard
allows up to \emph{eight} all-bank refresh commands to be issued late
(postponed) or early (pulled-in). This implies that each bank can
tolerate up to eight \refpb to be postponed or pulled-in. Therefore,
the memory controller ensures that reordering \refpb preserves data
integrity by limiting the number of postponed or pulled-in commands.
%the memory controller not only provides \refpb reordering, but also ensures
%data integrity by limiting the number of postponed or pulled-in commands.
%complying to the JEDEC standard.

\figref{darp_flow_chart} shows the algorithm of our mechanism. The
\ooolong scheduler makes a refresh decision every DRAM cycle. There
are three key steps.  First, when the memory controller hits a
per-bank refresh schedule time (every \trefipb), it postpones the
scheduled \refpb if the to-be-refreshed bank (\texttt{\emph{R}}) has pending demand
requests (read or write) {\em and} it has postponed fewer refreshes
than the limit of eight (\circled{1}). The hardware counter that is
used to keep track of whether or not a refresh can be postponed for each
bank is called the \emph{refresh credit (ref\_credit)}. The counter
decrements on a postponed refresh and increments on a pulled-in
refresh for each bank. Therefore, a \refpb command can be postponed if
the bank's ref\_credit stays above -8. Otherwise the memory controller
is required to send a \refpb command to comply with the
standard. Second, the memory controller prioritizes issuing commands
for a demand request if a refresh is not sent at any
given time (\circled{2}). Third, if the memory controller cannot issue
any commands for demand requests due to the timing constraints, it
instead randomly selects one bank (\texttt{\emph{B}}) from a list of banks that have no
pending demand requests to refresh. Such a refresh command is either a
previously postponed \refpb or a new pulled-in \refpb (\circled{3}).

%%% ONUR2: In this flowchart, there are two ref_credit's, right? One
%%% is for the selected bank in this cycle, and the other is for the
%%% randomly selected bank. Can you please change the notation to
%%% denote that these are two potentially different credit counters?

%%% ONUR2: You can do this by saying ``Every Cycle, Select a Bank R to
%%% Refresh'' instead of ``Every Cycle'' and call its ref_credit as
%%% ref_creditR (subscript R), and call the ref_credit of B as
%%% ref_creditB (subscript B)

\figputHS{darp_flow_chart}{0.85}{Algorithm of \ooolong.}

%%% ONUR: Above description of the algorithm:
%%% The algorithm is not clear. The reasons for actions 1, 2, 3 are not provided.
%%% ONUR: See below my 4 points...

%%% 1. You say: ``it tries to postpone the scheduled REFpb by checking
%%% if the target bank has exceeded the postpone limit of eight
%%% refreshes''
%%% --> should this not be ``has NOT exceeded''? I am confused
%%% --> what is the reason for doing this? You postpone a refresh
%%%     regardless of whether or not the bank has a pending request?
%%% --> Be clear in your description of why you do what you do in 1.

%%% 2. Is the algorithm per bank? If so, why do you select a random
%%% bank to refresh in Step 3? The explanation is confusing. Please
%%% provide the high-level reasons why you make the design choices you
%%% have done in steps 1,2,3 of Fig 8. Step 2 is the most clear, but
%%% steps 1 and 3 are confusing.

%%% 3. The beginning of the algorithm description is also not
%%% clear. You say: ``when the memory controller hits a per-bank
%%% refresh schedule time''. It was not clear that there was a target
%%% bank. If the algorithm is ``per each bank'' then why is there a
%%% random selection of a bank in step 3? Please rethink the algorithm
%%% explanation.

%%% 4. Is the ``Gone through all banks?'' loop done in a single cycle
%%% in this flowchart?
% Kevin: The main takeaway is that we want to randomly pick one bank that has no
% demand requests to refresh. Although the process is explained as a loop, the
% real implementation does not have to be a loop (perhaps a tree). It's done in
% a single cycle in the simulator, but it may take longer than 1 cycle in real
% implementation.
%%% ONUR2: I got it now. It can be done in a single cycle. Basically
%%% you keep one bank to refresh in a cycle, not more than one,
%%% correct?
% Kevin: That is correct.

%%% ONUR2: The above explanation has become much better now. I have
%%% fixed some things (see above), but it is now much easier to
%%% understand now.

%%%%%%%%%%%%%%%%%%%%%%%
% OLD STUFF
%%%%%%%%%%%%%%%%%%%%%%%
%As shown in Algorithm~\ref{algo:ooo-algo}, the \ooolong scheduler makes refresh
%decisions every 1) \trefi and 2) DRAM cycle. First, the scheduler uses the
%\trefi schedule that tracks the round-robin bank order as a \emph{checkpoint} to
%determine if a bank exceeds eight postponed or pulled-in refreshes, as opposed
%to the baseline where the memory controller issues a refresh command every \trefi.
%During the checkpoint, if the refresh limit is not reached, the scheduler postpones
%refreshing the bank. Otherwise the scheduler is forced to refresh the bank to
%ensure data integrity. The \emph{refresh credit} is the key component used to
%keep track of the refresh progress for each bank. The credit decrements on a
%postponed refresh and increments on a pulled-in refresh. Second, every DRAM
%cycle, if the scheduler cannot issue any command for demand requests, the
%scheduler instead issues the previously postponed or pulled-in refresh command
%to a randomly selected bank that is idle.

%The key component is
%a refresh credit that keeps track of how many refreshes have been postponed or
%pulled-in for each bank so that the memory controller does not exceed the
%defined threshold of eight refresh commands for each bank. The credit is
%initialized to a value of zero, indicating that all refreshes have been issued
%following \trefi. Whenever a refresh command is postponed, the credit decrements
%by one; on the contrary, it increments by one when a refresh is pulled in.
%The
%scheduler proactively postpones a refresh command to a bank if the bank's credit
%is above the threshold (greater than $-8$ given that the credit decrements for
%postponed refreshes). When the memory controller has no demand requests to
%issue, the \refpb refresh scheduler issues a refresh command to a randomly
%selected bank that is idle without any pending memory requests.

% -- OLD ALGO
%\input{sec/algos/ooo-algo}
%%%%%%%%%%%%%%%%%%%%%%%

%\textbf{\warplongCap}.
\subsubsection{\warplongCap} The key idea of the second component of \darp is to
actively avoid refresh interference on read requests and instead enable more
parallelization of refreshes with \emph{write requests}. We make two
observations that lead to our idea. First, {\em write batching} in DRAM creates
an opportunity to overlap a refresh operation with a sequence of writes, without
interfering with reads. A modern memory controller typically buffers DRAM writes
and drains them to DRAM in a batch to amortize the \emph{bus turnaround
latency}, also called \emph{tWTR} or
\emph{tRTW}~\cite{jedec-ddr3,kim-isca2012,lee-tech2010}, which is the additional
latency incurred from switching between serving writes to reads because DRAM I/O
bus is half-duplex. Typical systems start draining writes when the write buffer
occupancy exceeds a certain threshold until the buffer reaches a low watermark.
This draining time period is called the \emph{writeback mode}, during which no
rank within the draining channel can serve read
requests~\cite{chatterjee-hpca2012,lee-tech2010,stuecheli-isca2010}. Second,
DRAM writes are not latency-critical because processors do not stall to wait for
them: DRAM writes are due to dirty cache line evictions from the last-level
cache~\cite{lee-tech2010,stuecheli-isca2010}.

%%% ONUR2: The above was rough at places. I fixed it.

%%%%%%%%%%
%\subsubsection{\warplongCap} The key idea of our second component in \darp is
%to actively avoid issuing refresh commands with read requests and instead
%enable more parallelization of refreshes with \emph{write requests}. We make
%the following observations that lead to our idea. First, write batching creates
%an opportunity for a refresh operation to overlap with a sequence of writes
%without interfering with reads. The reason that writes are issued to DRAMs in a
%batch is to amortize the additional latency incurred in transitioning from
%serving writes to reads (or vice versa). Because a DRAM I/O bus is not
%full-duplex which disallows reading and writing data to the memory
%simultaneously, turning around the bus into a particular direction for either
%reading or writing data (toward the memory or processor) incurs an additional
%latency called \emph{tWTR} (7.5ns for an 8Gb device~\cite{micronDDR3_4Gb}).
%Therefore, to avoid excessive bus turnarounds, writes are accumulated in the
%write buffer and drained in a batch when the buffer occupancy exceeds a certain
%threshold until the buffer reaches a low watermark. This time period of DRAM
%draining write requests is called the \emph{writeback mode}, during which all
%ranks within the draining channel can only serve write requests. Second, writes
%to DRAMs are not on the critical path for processors in most systems. This is
%because they get generated due to dirty cache line evictions from the
%last-level cache. Therefore, writes are much more tolerant to additional memory
%latency caused by DRAM refresh that prevents a bank from serving memory
%accesses.
%%%%%%%%%%

%%% ONUR: The above paragraph needs to be more crisp. Especially the
%%% part about ``writes not being on the critical path is not well
%%% written. Can you please rewrite? The same explanation in the new
%%% introduction was much better.

%%% ONUR: Last sentence above did not fit well when you bring in
%%% refreshes... I rewrote it. (Talking about writes being delayed by
%%% refreshes was premature)



%%% ONUR: The beginning of the below paragraph is very good. It puts
%%% in context the two observations you make above.

Given that writes are not latency-critical and are drained in a batch
for some time interval, we propose the second component of \darp,
\emph{\warplong}, that attempts to maximize parallelization of
refreshes and writes. \Warplong selects the bank with the minimum
number of pending demand requests (both read and write) and preempts
the bank's writes with a per-bank refresh. As a result, the bank's
refresh operation is hidden by the writes in other banks.

%%% ONUR2: ``elongate the writeback mode'', not ``elongate the length
%%% of writeback mode''

The reasons why we select the bank with the lowest number of demand
requests as a refresh candidate during writeback mode are
two-fold. First, the goal of the writeback mode is to drain writes as
fast as possible to reach a low watermark that determines the end of
the writeback
mode~\cite{chatterjee-hpca2012,lee-tech2010,stuecheli-isca2010}. Extra
time delay on writes can potentially elongate the writeback mode by
increasing queueing delay and reducing the number of writes served in
parallel across banks. Refreshing the bank with the lowest write
request count (zero or more) has the smallest impact on the writeback
mode length because other banks can continue serving their writes to
reach to the low watermark. Second, if the refresh scheduled to a bank
during the writeback mode happens to extend beyond writeback mode, it
is likely that the refresh 1) does not delay immediate reads within
the same bank because the selected bank has no reads or 2) delays
reads in a bank that has less contention. Note that we only preempt
one bank for refresh because the JEDEC standard~\cite{jedec-lpddr3}
disallows overlapping per-bank refresh operations across banks within
a rank.

%%% ONUR2: Only one bank. How do you relax this standard when you
%%% parallelize subarray access and refresh? DO you still have one
%%% bank refreshed at a time, i.e., one subarray in the entire rank
%%% refreshed at a time?
% Kevin: Only one bank can be refreshed at once. Using SARP does not break this
% constraint. I think parallelizing "refreshes" across banks is another topic
% itself.

%%% ONUR: The above is not clear to me. ``Preempted refresh''? I
%%% thought you preempted writes? I am very confused with the above
%%% explanation.
%%% Please clarify all the explanations in the above paragraph: Last
%%% sentence before ``Second,'' is unclear. ``Second, ...'' itself is
%%% unclear due to ``preempted refresh''. In the next sentence, you
%%% use ``preempt'' for a bank...

%Even though the extra delay
%on writes in a single bank does not impact the processors'
%performance directly, the delay can potentially elongate the length of writeback
%mode by increasing queueing delay in banks and reducing bank-level parallelism
%that allows parallelization of some operations (e.g., row activation) of writes
%across banks.

%Second, preempting a bank with the lowest write count creates imbalances
%in write queue occupancy as some banks may need to drain more writes than
%before. This allows other banks to be preempted with refreshes in the upcoming
%writeback mode.

\figref{inter-bank-service-timeline} shows the service timeline and
benefits of \warplong. There are \textbf{two scenarios} when the
scheduling policy parallelizes refreshes with writes to increase
DRAM's availability to serve read
requests. \figref{inter-bank-postpone} shows the first scenario when
the scheduler \emph{postpones} issuing a \refpb command to avoid
delaying a read request in Bank 0 and instead serves the refresh in
parallel with writes from Bank 1, effectively hiding the refresh
latency in the writeback mode. Even though the refresh can potentially
delay individual write requests during writeback mode, the delay does
not impact performance as long as the length of writeback mode remains
the same as in the baseline due to longer prioritized write request
streams in other banks. In the second scenario shown in
\figref{inter-bank-pull}, the scheduler proactively \emph{pulls in} a
\refpb command early in Bank 0 to fully hide the refresh latency from
the later read request while Bank 1 is draining writes during the
writeback mode (note that the read request cannot be scheduled during
the writeback mode).

%%% ONUR: Very nice figure. Please emphasize the ``Saved Cycles''...
\input{plots/inter-bank-service-timeline}

The crucial observation is that \warplong improves performance because
it avoids stalling the read requests due to refreshes by postponing or
pulling in refreshes in parallel with writes without extending the
writeback period.

%%% ORIGINAL - too mechanical, no conclusion%%%
\ignore{\figref{inter-bank-service-timeline} shows the service timeline and benefits of
\ib. There are \textbf{two scenarios} when the scheduling policy parallelizes
refresh operations with writes to increase DRAM's availability to serve read
requests. The first scenario is when the scheduler \emph{postpones} issuing a
\refpb to allow a DRAM bank to serve read requests. Then when the DRAM enters
writeback mode issuing write requests to other banks, the scheduler can send
the postponed refresh to the bank. As a result, the refresh operation is
parallelized with writes, effectively hiding the refresh latency in the
writeback mode to reduce the negative impact of refresh on read requests. Even
though refresh can potentially delay individual write requests during
writeback mode, the delay may not impact performance as long as the length
of writeback mode remains approximately the same due to longer prioritized
write request streams in other banks. \figref{inter-bank-postpone} shows the
performance benefit of postponing a refresh and overlapping it with writes.

In the second scenario, the scheduler takes preventive action by issuing a \refpb
command early when there is an opportunity to fully hide the refresh latency
during the writeback mode. As shown in \figref{inter-bank-pull}, the scheduler
speculatively \emph{pulls in} a \refpb command during the writeback mode before
it reaches its refresh schedule in order to free up an upcoming refresh
interval to serve a read request.}
%%% END ORIGINAL - too mechanical, no conclusion%%%

Algorithm~\ref{algo:warp-algo} shows the operation of \warplong. When
the memory controller enters the writeback mode, the scheduler selects
a bank candidate for refresh when there is no pending refresh. A bank
is selected for refresh under the following criteria: 1) the bank has
the lowest number of demand requests among all banks and 2) its
refresh credit has not exceeded the maximum \emph{pulled-in} refresh
threshold. After a bank is selected for refresh, its credit increments
by one to allow an additional refresh postponement.

%%% ONUR: Please make sure the algorithm is correct. I did not check this carefully.
\input{sec/algos/interbank-algo}

%%% ONUR2: You did the right thing in Algo 1 and specified a bank
%%% associated with ref_credit: ref_credit[b], please do this as I
%%% described for the flowchart earlier as well.

%%% ONUR2: Caption of Algo 1: write-refresh parallelization --> Write-refresh parallelization

%\textbf{Refresh scheduling flexibility with per-bank refreshes.}
%JEDEC standard~\cite{jedec-ddr3} provides refresh scheduling
%flexibility by allowing refresh commands to be delayed or pulled-in early (up
%to eight all/per-bank refresh commands). Therefore using this flexibility on
%per-bank refresh introduces additional flexibility for refresh scheduling
%policies and it creates opportunities for a memory controller to overlap refresh
%latency with memory accesses at different points in time.

\subsubsection{Implementation}
\darp incurs a small overhead in the memory controller and DRAM
without affecting the DRAM cell array organization. There are five
main modifications. First, each refresh credit is implemented with a
hardware integer counter that either increments or decrements by up to
eight when a refresh command is pulled-in or postponed,
respectively. Thus, the storage overhead is very modest with 4 bits
per bank (32 bits per rank). Second, \darp requires logic to monitor
the status of various existing queues and schedule refreshes as
described. Despite reordering refresh commands, all DRAM timing
constraints are followed, notably \trrd and \trfcpb that limit when
\refpb can be issued to DRAM.  Third, the DRAM command decoder needs
modification to decode the bank ID that is sent on the address bus
with the \refpb command.  Fourth, the refresh logic that is located
outside of the banks and arrays needs to be modified to take in the
specified bank ID. Fifth, each bank requires a separate row counter to
keep track of which rows to refresh as the number of postponed or
pulled-in refresh commands differs across banks.  Our proposal limits
the modification to the least invasive part of the DRAM without
changing the structure of the dense arrays that consume the majority
of the chip area.

\subsection{\intersub} Even though \darp allows refreshes and accesses to occur
in parallel across different banks, \darp cannot deal with their collision
\emph{within a bank}. To tackle this problem, we propose \emph{\sarp
(\intersub)} that exploits the existence of subarrays within a bank. The key
observation leading to our second mechanism is that refresh occupies only a few
\emph{subarrays} within a bank whereas the other \emph{subarrays} and the
\emph{I/O bus} remain idle during the process of refreshing. The reasons for
this are two-fold.  First, refreshing a row requires only its subarray's sense
amplifiers that restore the charge in the row without transferring any data
through the I/O bus.  Second, each subarray has its own set of \emph{sense
amplifiers} that are not shared with other subarrays.

Based on this observation, SARP's key idea is to allow memory accesses
to an \emph{idle} subarray while another subarray is refreshing.
\figref{subarray-service-timeline} shows the service timeline and the
performance benefit of our mechanism. As shown, \is reduces the read
latency by performing the read operation to Subarray 1 in parallel
with the refresh in Subarray 0. Compared to \ib, \is provides the
following advantages: 1) \is is applicable to both all-bank and
per-bank refresh, 2) \is enables memory accesses to a refreshing bank,
which cannot be achieved with \ib, and 3) \is also utilizes bank-level
parallelism by serving memory requests from multiple banks while the
entire rank is under refresh. \is requires modifications to 1) the
DRAM architecture because two distinct wordlines in different
subarrays need to be raised simultaneously, which cannot be done in
today's DRAM due to the shared peripheral logic among subarrays, 2)
the memory controller such that it can keep track of which subarray is
under refresh in order to send the appropriate memory request to an
idle subarray.

%%% ONUR: I modified the last sentence to be more coherent. There was
%%% no need for ``However,'' there as SARP also requires modifications
%%% to DRAM and the memory controller. The above modifications seem
%%% redundant with what is described in implementation. However, it
%%% may be OK to keep it here as it is now rephrased.

%\input{plots/subarray-service-timeline}
\figputHW{subarray-service-timeline}{Service timeline of a refresh and a read request to two
different subarrays within the same bank.}

%%% ONUR2: The top says ``All-Bank Refresh'' but this should really be
%%% ``All-Bank or Per-Bank Refresh''. Please fix.

%%% ONUR: I changed the heading below because this section talks only
%%% about DRAM bank implementation.
\subsubsection{DRAM Bank Implementation for \is} \label{sec:sarp_implementation}
As opposed to \ib, \is requires modifications to DRAM to support accessing
subarrays individually. While subarrays are equipped with dedicated local
peripheral logic, what prevents the subarrays from being operated independently
is the global peripheral logic that is shared by all subarrays within a bank.

%%% ONUR2: Fig 11: Please fix the subcaptions as:
%%% (a) Existing Organization without SARP
%%% (b) New Organization with SARP

\figref{detail-bank-organization} shows a detailed view of an existing DRAM
bank's organization. There are two major shared peripheral components within a
bank that prevent modern DRAM chips to refresh at subarray level. First, each
bank has a \emph{global row decoder} that decodes the incoming row's addresses.
To read or write a row, memory controllers first issue an \act command with the
row's address.
% in order to latch the row's content into the row buffer.
Upon receiving this command, the bank feeds the row address to the \emph{global
row decoder} that broadcasts the partially decoded address to all subarrays
within the bank. After further decoding, the row's subarray then raises its
wordline to begin transferring the row's cells' content to the row
buffer.\footnote{The detailed step-to-step explanation of the activation process
can be found in prior
works~\cite{kim-isca2012,lee-hpca2013,seshadri-micro2013}.} During the transfer,
the row buffer also restores the charge in the row. Similar to an \act,
refreshing a row requires the refresh unit to \act the row to restore its
electrical charge (only the refresh row counter is shown for clarity in
\figref{detail-bank-organization}).
%is triggered by a command that is similar to \act from the refresh unit.
Because a bank has only one global row decoder and one pair of address wires
(for subarray row address and ID), it cannot simultaneously activate two
different rows (one for a memory access and the other for a refresh).
%support two \act addresses (one from a memory access and one from a refresh) to
%activate two different rows.

Second, when the memory controller sends a read or write command, the required
column from the activated row is routed through the \emph{global bitlines} into
the \emph{global I/O buffer} (both of which are shared across all subarrays' row
buffers) and is transferred to the I/O bus (all shown in
\figref{bank-organization}). This is done by asserting a \emph{column select}
signal that is routed globally to {\em all} subarrays, which enables {\em all}
subarrays' row buffers to be concurrently connected to the global bitlines.
Since this signal connects all subarrays' row buffers to the global bitlines at
the same time, if more than one activated row buffer (i.e., activated subarray)
exists in the bank, an electrical short-circuit occurs, leading to incorrect
operation. As a result, two subarrays cannot be kept activated when one is being
read or written to, which prevents a refresh to one subarray from happening
concurrently with an access in a different subarray in today's DRAM.

%%% ONUR2: The above was still not clear. I fixed it. It is important
%%% to think like a reader who wants things to flow logically and
%%% clearly.

%\figref{detail-bank-organization} shows a detailed view of an existing
%DRAM bank's organization. There are two major shared peripheral
%components within a bank. First, the \emph{global row-decoder}
%specifies a unique row whose address is broadcast to all subarrays
%within the bank. As a result, only one subarray (to which the row
%belongs) can be activated, while all other subarrays are prevented
%from being activated. Second, the global I/O buffer is shared across
%subarrays. When the memory controller attempts to access data from any
%one of the activated subarrays, not just the one, but all activated
%subarrays connect their local row buffers to the global I/O buffer
%through the global bitlines – leading to an electrical short-circuit
%when there is more than one activated subarray. As a result, two
%subarrays cannot be kept activated concurrently when one is being
%read.  The key enabler of \is is to reduce the sharing of the global
%peripheral logic (global row decoders and global bitlines) to allow
%accesses to non-refreshing subarrays while others are refreshing.

%%% ONUR: See what I added above: ``As a result, two subarrays cannot
%%% be kept activated concurrently when one is being read.'' This was
%%% very important.
%%% ONUR: Please make the above much more crisp. It was missing
%%% explanations and had incorrect words, which I fixed. It still
%%% needs a careful look and polishing.

%%% ONUR: Figure 11a:
%%% - The sharing of the global I/O buffer is not coming out from the
%%%   figure. Can you please draw the global bitlines? I really cannot
%%%   see where the column select transistors are controlling access
%%%   to... The readers will be confused. Please fix. This is your
%%%   opportunity to do a good job with a very clear DRAM figure.

%%% - Why is there a single subarray in Fig 11b? You need to maintain
%%%   consistency with Fig 11a so that people can understand the -
%%%   differences well.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% ONUR: The below explanation of Fig 11b is very tough to follow. Please
%%% reorganize and rethink.

%%% ONUR: 0. You start with: ``First, we decouple the refresh row counter
%%% into two separate counters''. You do not say why you do this. What
%%% does this enable? You can say, ``First, to enable ...,''

%%% ONUR: 1. You say: ``Note that there is only one of each counter in a
%%% DRAM chip, as they are shared by every bank.'' I do not understand
%%% this. Why? The readers will have the same problem.

%%% ONUR: 2. You say: ``the subarray counter increments when it wraps around
%%% to zero''. I do not know what this means. Does it not increment
%%% when it does not wrap around? Need to rethink.

%%% ONUR: 3. This sentence is broken: ``The comparator determines if the
%%% subarray matches with the refresh-subarray counter and there is
%%% also a refresh enable signal.'' The refresh enable signal is
%%% introduced in a very awkward way here. Please rethink as you have
%%% an organizational problem here.

%%% ONUR: 4. You say: ``If there is a match, the subarray is selected for
%%% refresh. Then the subarray’s row buffer is disconnected from the
%%% global bitlines to prevent short-circuit''. Not enough. Why is
%%% preventing short circuit a good idea. It is because another
%%% subarray can be accessed through the global bitlines, right? You
%%% realy need to be explicit and clear in writing here.

%%% ONUR: Basically, you really need to rethink the last paragraph of
%%% Section 4.3.1 to be much more clear. Principles:
%%% 1. always give the reason for the modification first
%%% 2. then describe the modification very clearly and crisply
%%% 3. Do not introduce terminology in the middle of describing your modification
%%% 4. Strive for ultimate clarity and good flow (SALP paper has this, so does TL-DRAM, for example)

\input{plots/inter-sub-implementation}

The key idea of \is is to allow the concurrent activation of multiple subarrays,
but to only connect the accessed subarray's row buffer to the global bitlines
while another subarray is refreshing.\footnote{As described in
Section~\ref{sec:dram-org}, we refer to a subarray as a collection of multiple
physical subarrays. A modern refresh operation concurrently refreshes every
physical subarray within a collection.}  \figref{inter-sub-implementation} shows
our proposed changes to the DRAM microarchitecture. There are two major enablers
of \is.

%%% ONUR2: I read until here...

The first enabler of \is allows both refresh and access commands to
simultaneously select their designated rows and subarrays with three
new components. The first component (\circled{1}) provides the subarray and
row addresses for refreshes without relying on the global row
decoder. To achieve this, it decouples the refresh row counter into a
\emph{refresh-subarray} counter and a \emph{local-row} counter that
keep track of the currently refreshing subarray and the row address
within that subarray, respectively. The second component (\circled{2})
allows each subarray to activate a row for either a refresh or an
access through two muxes. One mux is a row-address selector and the
other one is a subarray selector. The third component (\circled{3})
serves as a control unit that chooses a subarray for refresh. The
\texttt{\small{REF?}} block indicates if the bank is currently under
refresh and the \texttt{\small{=ID?}} comparator determines if the
corresponding subarray's ID matches with the refreshing subarray
counter for refresh. These three components form a new address path
for the refresh unit to supply refresh addresses in parallel with
addresses for memory accesses.
%%% ONUR2: A question: Can the REF subarray value be supplied by the
%%% memory controller? Is that what is needed in SARP or DSARP? Or
%%% does the DRAM internally determine which subarray to be refreshed?
%%% Please clrify for me first. Is this clear somewhere in text?
%%% ONUR2: I think what I asked for right above comes in the ``memory
%%% controller'' changes section, right? Please see my changes to that
%%% section.
% Kevin: The DRAM internally selects which subarray to refresh. Your explanation
% in the footnote is correct.

The second enabler of \is allows accesses to one activated subarray while
another subarray is kept activated for refreshes. We add an \emph{AND} gate
(\circled{4}) to each subarray that ensures the refreshing subarray's row buffer
is {\em not} connected to the global bitlines when the {\em column select}
signal is asserted on an access. At any instance, there is at most one activated
subarray among all non-refreshing subarrays because the global row decoder
activates only one subarray at a time. With the two proposed enablers, \is
allows one activated subarray for refreshes in parallel with another activated
subarray that serves data to the global bitlines.
%%% ONUR2: I simplified the explanation above. There is no need to
%%% bring in component 3 again here.

%%% ONUR2: PLease make sure Fig 11 is *absolutely* correct in
%%% connections and routing.

%To enable \is, we propose to make the following changes to the DRAM
%microarchitecture, as shown in
%\figref{inter-sub-implementation}. First, we decouple the refresh row
%counter into two separate counters: \emph{subarray} counter and
%\emph{local-row} counter that keep track of the current refreshed
%subarray and the row address within the subarray, respectively
%(\circled{1} in \figref{inter-sub-implementation}). The local-row
%counter is set based on the number of rows within a subarray and the
%subarray counter increments when it wraps around to zero. As a result,
%we route these counters with global wires across the bank to provide
%refresh selection instead of connecting them to the global row
%decoder. Note that there is only one of each counter in a DRAM chip,
%as they are shared by every bank. Second, to enable raising wordlines
%in a different subarray from the one being refreshed, we add two muxes
%that take inputs from the global row decoder and the refresh counters
%(\circled{2}). As a result, the refreshing subarray's local row
%decoder receives the row address from the refresh row counter while
%another subarray is accessed with the row address specified by the
%memory controller. Third, we add a small amount of logic (one
%\emph{comparator}, one \emph{NAND} gate, and one \emph{AND} gate) to
%supply select signals to the muxes to pick either the row address from
%the refresh counter or the memory controller. The comparator
%determines if the subarray matches with the refresh-subarray counter
%and there is also a refresh enable signal. If there is a match, the
%subarray is selected for refresh. Then the subarray's row buffer is
%disconnected from the global bitlines to prevent short-circuit
%(\circled{3}).
%%% ONUR: The above needs to be rewritten. I did not touch it because
%%% I would like you to take a good, serious cut at it.


%%% ONUR: See my above comments on Fig 11 a and b. The caption is not
%%% good. ``DRAM bank without and with SARP.'' is a better caption.
%\input{plots/inter-sub-implementation}

\subsubsection{Detecting Subarray Conflicts in the Memory Controller} To avoid
accessing a refreshing subarray, which is determined internally by the DRAM chip
in our current mechanism, the memory controller needs to know the current
refreshing subarray and the number of subarrays. We create shadow copies of the
\emph{refresh-subarray} and \emph{local-row} counters in the memory controller
to keep track of the currently-refreshing subarray.
%To detect the number of subarrays within a bank,
We store the number of subarrays in an EEPROM called the \emph{serial presence
detect (SPD)}~\cite{jedec-spd}, which stores various timing and DRAM
organization information in existing DRAM modules. The memory controller reads
this information at system boot time so that it can issue commands
correctly.\footnote{Note that it is possible to extend our mechanisms such that
the memory controller specifies the subarray to be refreshed instead of the DRAM
chip. This requires changes to the DRAM interface.}

%To prevent sending a memory access to a refreshing subarray, the memory
%controller needs to know the number of subarrays and the current refreshing
%subarray. Instead of changing the interface of DRAM to expose this information
%through extra pins, we create shadow copies of the refresh \emph{subarray} and
%\emph{local-row} counters in the memory controller, which increment accordingly
%when a refresh command is issued to a rank. However, we still need to know the
%number of subarrays within a bank to set a maximum bound on the row counter so
%that it wraps around correctly. To do so, we store the number of subarrays in
%an EEPROM called the \emph{serial presence detect (SPD)}~\cite{jedec-spd} that
%stores various timing and DRAM organization information in existing DRAM
%modules. The memory controller reads these information at system boot time so
%that it can issue commands correctly.

%%% ONUR: cite SPD please
%%% ONUR: You can reduce the discussion in 4.3.2, if space is
%%% needed. However, this will need to be done carefully.

%%% ONUR: is it ``four activation window'' or ``four activation windows''?
%%% ONUR: four row activations are allowed to operate --> very very awkward wording.
%%% ONUR: Why not call ``activation'' an activate command? I tried to fix this by calling it row activation.

\subsubsection{Power Integrity} Because an \act draws a lot of current, DRAM
standards define two timing parameters to constrain the activity rate
of DRAM so that \acts do not over-stress the power delivery
network~\cite{jedec-ddr3,shevgoor-micro2013}.  The first parameter is
the \emph{row-to-row activation delay} (\trrd) that specifies the
minimum waiting time between two subsequent \act commands within a
DRAM device. The second is called the \emph{four activate window}
(\tfaw) that defines the length of a rolling window during which a
maximum of four \acts can be in progress. Because a refresh operation
requires activating rows to restore charge in DRAM cells, \is consumes
additional power by allowing accesses during refresh. To limit the
power consumption due to \acts, we further constrain the activity rate
by increasing both \tfaw and \trrd, as shown below. This results in
fewer \act commands issued during refresh.
%To compensate for the power overhead, we increase the \trrd and \tfaw to extend
%time interval between \acts, thus limiting the activity rate during refresh.
%The following equations show the re-adjusted \trrd and \tfaw timing parameters.

%%% ONUR: I do not understand what ``To limit this power overhead
%%% during refresh-access parallelization, we increase both \trrd and
%%% \tfaw to extend the spacing between activations during
%%% refresh. The following equations define the re-adjusted timing''
%%% means. Please be clear.

%%% ONUR2: The above is better now. Can still make it better.

%{
%\small
%\vspace{-0.15in}
%\begin{align}
%\label{eq:1}
% &I_{ACT} = I_{DD0} - \frac{(I_{DD3N} * tRAS + I_{DD2N} * (tRC - tRAS))}{tRC} \\
%\label{eq:2}
% &I_{REF} = I_{DD5B} - I_{DD3N} \\
%\label{eq:3}
% &PowerOverhead_{FAW} = \frac{4*I_{ACT} + I_{REF}}{4*I_{ACT}} \\
%\label{eq:4}
% &t_{FAW\_SARP} = t_{FAW} * PowerOverhead_{FAW} \\
%\label{eq:5}
% &t_{RRD\_SARP} = t_{RRD} * PowerOverhead_{FAW}
%\end{align}
%}

{
\small
%\footnotesize
\vspace{-0.15in}
\begin{align}
\label{eq:1}
 &PowerOverhead_{FAW} = \frac{4*I_{ACT} + I_{REF}}{4*I_{ACT}} \\
\label{eq:2}
 &t_{FAW\_SARP} = t_{FAW} * PowerOverhead_{FAW} \\
\label{eq:3}
 &t_{RRD\_SARP} = t_{RRD} * PowerOverhead_{FAW}
\end{align}
\vspace{-0.2in}
}

%%% ONUR: Micron, not MICRON.

%\eqref{eq:1} and \eqref{eq:2} show the current values of an activation and a
{\small $I_{ACT}$} and {\small $I_{REF}$} represent the current values
of an \act and a refresh, respectively, based on the Micron
Power Calculator~\cite{micron-tr}. We calculate the power overhead of
parallelizing a refresh over a {\em four activate window} using
\eqref{eq:1}. Then we apply this power overhead to both \tfaw
\eqref{eq:2} and \trrd \eqref{eq:3}, which are enforced during refresh
operations. Based on the $IDD$ values in the Micron 8Gb
DRAM~\cite{micronDDR3_8Gb} data sheet, \is increases \tfaw and \trrd
by 2.1x during all-bank refresh operations. Each per-bank refresh consumes 8x
lower current than an all-bank refresh, thus increasing \tfaw and \trrd by only
13.8\%.

%%% ONUR: What is the area overhead of DARP? Why not report that as well?

%\textbf{Die Area Overhead}.
\subsubsection{Die Area Overhead} In our evaluations, we use 8 subarrays per
bank and 8 banks per DRAM chip. Based on this configuration, we calculate the
area overhead of \is using parameters from a Rambus DRAM model at 55$nm$
technology~\cite{rambus_powermodel}, the best publicly available model that we
know of, and find it to be 0.71\% in a 2Gb DDR3 DRAM chip with a die area of
73.5$mm^2$. The power overhead of the additional components is negligible
compared to the entire DRAM chip.
%the overall area overhead of \is is 0.71\% in a 2Gb DDR3 DRAM chip with a die
%area of 73.5$mm^2$ using 55$nm$ technology~\cite{rambus_powermodel}.

%%% ONUR: Summary is OK, but you can get rid of it due to space
%%% constraints. Do not delete it, just \ignore it. It is much more
%%% important to use the space to explain the mechanisms and
%%% implementations more clearly. The biggest benefit of the summary
%%% is the introduction of the term DSARP, which needs to be done
%%% elsewhere when the summary is removed. Do not forget to say
%%% ``called DSARP'' when you introduce the acronym.
\ignore{
\subsection{Summary} We  proposed two mechanisms to hide
refresh latency by parallelizing refresh operations with memory
accesses at different granularities within the DRAM architecture. Our
first mechanism, \darp, exploits the refresh scheduling flexibility in
JEDEC standards to enable the memory controller to make more
intelligent decisions on when and which specific bank to refresh. The
second mechanism, \is, pushes the boundaries of today's DRAMs to
enable a DRAM to serve memory requests in idle subarrays while another
subarray is under refresh. As a result, it requires modifications to
the existing DRAM microarchitecture to achieve refresh-access
parallelization without impacting the array structures.  \is is
complementary to \darp and the combination of both, called \combo,
offers additive performance benefits with the implementation cost
incurred from both mechanisms.}


==> sec/parref/5-meth.tex <==
\section{Methodology}
\label{methodology}

%%% Main scurves results
%\input{plots/main-scurves}
%\figputGTS{scurves}{1.0}{Multi-core system performance improvement over baseline
%all-bank refresh using various DRAM densities.}
\figputGTS{scurves}{1.0}{Multi-core system performance improvement over
\caprefab across 100 workloads.}

To evaluate our mechanisms, we use an in-house cycle-level x86
multi-core simulator with a front end driven by
Pin~\cite{luk-pldi2005} and an in-house cycle-accurate DRAM timing
model validated against DRAMSim2~\cite{rosenfeld-cal2011}. Unless
stated otherwise, our system configuration is as shown in
Table~\ref{table:sys-config}.

%%% ONUR: Why do you evaluate with only 8 MSHRs? This is a really
%%% unnecessary limitation. What is the sensitivity of performance
%%% results to MSHRs? As researchers, it is very important to research
%%% processors that can have high MLP.

% Methodology configuration table
\input{sec/tables/sys_config_table}
%%% ONUR: Fix DRAM to span only two rows and make it look nice by centering the word ``DRAM'' in two rows.

%%% ONUR: Add the refresh related parameters to the table please. You
%%% need tRFC and tREFI (and any other relevant parameter even if the
%%% DDR3 datasheet specifies it. These are such critical parameters
%%% that they should be listed, not the least because you provide the
%%% extrapolated values below.

In addition to 8Gb DRAM, we also evaluate systems using 16Gb and 32Gb
near-future DRAM chips~\cite{itrs-dram}. Because commodity DDR DRAM does not
have support for \refpb, we estimate the \trfcpb values for DDR3 based on the
ratio of \trfc to \trfcpb in LPDDR2~\cite{micronLPDDR2_2Gb} as described in
Section~\ref{sec:refresh-challenge}. We evaluate our systems with 32ms retention
time, which is a typical setting for a server environment and LPDDR DRAM, as
also evaluated in previous work~\cite{nair-hpca2013,stuecheli-micro2010}.
%When the write queue becomes full, the memory controller starts draining writes until
%the queue reaches a low watermark.

We use benchmarks from \emph{SPEC CPU2006~\cite{spec2006}, STREAM~\cite{stream},
TPC~\cite{tpc}}, and a microbenchmark with random-access behavior similar to
HPCC RandomAccess~\cite{randombench}. We classify each benchmark as either
memory intensive (MPKI $\ge$ 10) or memory non-intensive (MPKI $<$ 10). We then
form five intensity categories based on the fraction of memory intensive
benchmarks within a workload: 0\%, 25\%, 50\%, 75\%, and 100\%. Each category
contains 20 randomly mixed workloads, totaling to 100 workloads for our main
evaluations. For sensitivity studies in Sections~\ref{sec:sense_core},
\ref{sec:sense_tfaw}, \ref{sec:sense_sa}, and \ref{sec:sense_ref}, we run 16
randomly selected memory-intensive workloads using 32Gb DRAM to observe the
performance trend.
%Every workload runs 256 million cycles to ensure the same number of refreshes.
%We measure system performance with the commonly-used \emph{weighted
%speedup}~\cite{snavely-asplos2000, eyerman-ieeemicro2008} metric.

We measure system performance with the commonly-used \emph{weighted
  speedup (WS)}~\cite{eyerman-ieeemicro2008,snavely-asplos2000}
metric. To report the DRAM system power, we use the methodology from
the \emph{Micron power calculator}~\cite{micron-tr}. The DRAM device
parameters are obtained from~\cite{micronDDR3_8Gb}. Every workload
runs for 256 million cycles to ensure the same number of refreshes. We
report DRAM system power as \emph{energy per memory access serviced}
to fairly compare across different workloads.


==> sec/parref/6-eval.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we evaluate the performance of the following
mechanisms: 1) the \emph{all-bank} refresh scheme (\refab), 2) the
\emph{per-bank} refresh scheme (\refpb), 3) elastic
refresh~\cite{stuecheli-micro2010}, 4) our first mechanism, \ib, 5)
our second mechanism, \is, that is applied to either \refab (\isab) or
\refpb (\ispb), 6) the combination of \ib and \ispb, called \combo,
and 7) an ideal scheme that eliminates refresh. Elastic
refresh~\cite{stuecheli-micro2010} takes advantage of the refresh
scheduling flexibility in the DDR standard: it postpones a refresh if
the refresh is predicted to interfere with a demand request, based on
a prediction of how long a rank will be idle, i.e., without any demand
request (see Section~\ref{sec:related} for more detail).

%predicts how long a
%rank will be idle (i.e., without any memory requests) and postpones a
%refresh if

%the rank idle time is too short to hide the refresh latency


%it postpones each refresh command by a time delay that varies based on the number
%of postponed refreshes and the estimated average rank idle time (see
%Section~\ref{sec:related} for more detail).

%it attempts to predict how long a memory rank will remain idle (without a demand) when a
%refresh is about to be scheduled and issues the refresh when the
%predicted idle period is long enough to prevent refresh from
%interfering with demand requests (see Section~\ref{sec:related} for
%more detail).
%%% ONUR2: The last sentence was not clear in explaining elastic
%%% refresh well. This prediction of idle period is done when a
%%% refresh is about to be scheduled right? Basically, elastic refresh
%%% delays the refresh if it will interfere with demands. Correct?
%%% Please be clear in the description by rephrasing well if the above
%%% is incorrect.

%%% ONUR: Above: DSARP combines DARP and SARPpb, right? SARPpb should
%%% be specified, no? (I know this is implicit as DARP assumes
%%% per-bank refresh, but it is important to be ultra clear and make
%%% the busy reader not think)

\subsection{Multi-Core Results}
\label{sec:multi-core-results}


%%% ONUR: Why are SARPab results not plotted in Fig 12 and Table 2?
%%% The paper would be more comprehensive with them, even if you do
%%% not discuss these specific results. (Update: I saw SARPab is
%%% included later. It would be more complete to include it here
%%% also. You do not need to change the explanation much. However,
%%% what you have currently is fine, too.)

%%% ONUR: Fig 12. Please try to have the sorted workload number as the
%%% x axis in the Fig 12 graphs. The reader would like to see what
%%% fraction of workloads show what speedup range. Increments of 10 is
%%% a good idea. You can make this a small font.
\figref{scurves} plots the system performance improvement of \refpb, \ib, \ispb,
and \combo over the all-bank refresh baseline (\refab) using various densities
across 100 workloads (sorted based on the performance improvement due to \ib).
The x-axis shows the sorted workload numbers as categorized into five
memory-intensive groups with 0 to 19 starting in the least memory-intensive
group and 80 to 99 in the most memory-intensive one.
Table~\ref{table:scurve_summary} shows the maximum and geometric mean of system
performance improvement due to our mechanisms over \refpb and \refab for
different DRAM densities. We draw five key conclusions from these results.

%%% ONUR2: I had not meant sort workload numbers by intensity... but,
%%% this is interesting still as it gives some indication. Can you
%%% cram more numbers into the x axis by reducing font size just a
%%% bit?

%%% ONUR: Why do you provide ``max'' performance improvements in the
%%% below paragraph? Your AVG results are very good. Can you rephrase
%%% such that you provide average numbers? (Keep the old paragraph in
%%% \ignore just in case)
\ignore{
First, \ib provides system performance gains over both \refpb and
\refab schemes in different DRAM densities with up to 11.0\% and
23.1\% improvement in 16Gb DRAM, respectively. The reason is that \ib
hides refresh latency with writes and issues refresh commands in
out-of-order fashion to reduce refresh interference on reads. Second,
\ispb provides significant system performance improvement over \ib and
refresh baselines for all the evaluated DRAM density as \ispb enables
accesses to idle subarrays in the refreshing banks. \ispb improves
system performance by up to 21.5\% and 28.0\% over \refpb and \refab
in 32Gb DRAM, respectively.  Third, as DRAM density increases, the
performance benefit of \ispb over \ib gets larger. This is because
longer refresh latency becomes more difficult to hide behind writes or
idle banks for \ib. This is also the reason why the performance
improvement due to \ib drops slightly at 32Gb compared to 16Gb.  On
the other hand, \ispb is able to allow a long-refreshing bank to serve
some memory requests in its subarrays.}

First, \ib provides system performance gains over both \refpb and
\refab schemes: 2.8\%/4.9\%/3.8\% and 7.4\%/9.8\%/8.3\% on average in
8/16/32Gb DRAMs, respectively. The reason is that \ib hides refresh
latency with writes and issues refresh commands in out-of-order
fashion to reduce refresh interference on reads. Second, \ispb
provides significant system performance improvement over \ib and
refresh baselines for all the evaluated DRAM densities as \ispb
enables accesses to idle subarrays in the refreshing banks.  \ispb's
average system performance improvement over \refpb and \refab is
3.3\%/6.7\%/13.7\% and 7.9\%/11.7\%/18.6\% in 8/16/32Gb DRAMs,
respectively.  Third, as density increases, the performance
benefit of \ispb over \ib gets larger. This is because the longer
refresh latency becomes more difficult to hide behind writes or idle
banks for \ib. This is also the reason why the performance improvement
due to \ib drops slightly at 32Gb compared to 16Gb.  On the other
hand, \ispb is able to allow a long-refreshing bank to serve some
memory requests in its subarrays.

%%% ONUR2: Is there a need to still bolden some of the rows in Table
%%% 2?

%%% ONUR: ``Third'' explanation above is nice! Keep such crisp
%%% explanations coming.

Fourth, combining both \ispb and \darp (\combo) provides additive system
performance improvement by allowing even more parallelization of
refreshes and memory accesses. As DRAM density (refresh latency)
increases, the benefit becomes more apparent, resulting in improvement
up to 27.0\% and 36.6\% over \refpb and \refab in 32Gb DRAM,
respectively.

Fifth, \refpb performs worse than \refab for some workloads (the
curves of \refpb dropping below one) and the problem is exacerbated
with longer refresh latency. Because \refpb commands cannot overlap
with each other~\cite{jedec-lpddr3}, their latencies are
serialized. In contrast, \refab operates on every bank in parallel, which is
triggered by a single command that partially overlaps refreshes across
different banks~\cite{mukundan-isca2013}. Therefore, in a pathological
case, the \refpb latency for refreshing every bank (eight in most
DRAMs) in a rank is {\small$8 \times \trfcpb = 8 \times
  \frac{\trfc}{2.3} \approx 3.5 \times \trfc$}, whereas all-bank
refresh takes \trfc (see Section~\ref{sec:refresh-challenge}). If a
workload cannot
%lacks bank-level parallelism to
effectively utilize multiple banks during a per-bank refresh operation, \refpb
may potentially degrade system performance compared to \refab.
%%% ONUR: The above explanation is good, but please remind the reader
%%% where the number 2.3 is coming from. See what I did above and fill in.

\input{sec/tables/scurve_summary}

%%% ONUR: the performance --> performance (unles you say the performance of ...)
%%% ONUR: the system performance --> system performance (ditto)
\subsubsection{All Mechanisms' Results}
Figure~\ref{fig:multi-core-perf-density-sweep} shows the average
performance improvement due to all the evaluated refresh mechanisms
over \refab.  The weighted speedup value for \refab is 5.5/5.3/4.8
using 8/16/32Gb DRAM density.  We draw three major conclusions. First,
using \is on all-bank refresh (\isab) also significantly improves
system performance. This is because \is allows a rank to continue
serving memory requests while it is refreshing. Second, elastic
refresh does not substantially improve performance, with an average of
1.8\% over all-bank refresh.  This is because elastic refresh does not
attempt to pull in refresh opportunistically, nor does it try to
overlap refresh latency with other memory accesses. The observation is
consistent with prior work~\cite{nair-hpca2013}. Third, \combo
captures most of the benefit of the ideal baseline ("No REF"),
performing within 0.9\%, 1.2\%, and 3.7\% of the ideal for 8, 16, and
32Gb DRAM, respectively.
%%% ONUR: Why does SARP ab do better than SARPpb with 32Gb? Same
%%% reason as why REFab does better than REFpb as described earlier
%%% for 32Gb?
%%% ONUR: This begs the question even more: Does DSARP employ SARPab or SARPpb?

\figputGHS{multi-core-perf-density-sweep}{1.0}{Average system performance
improvement over \caprefab.}
%over baseline all-bank refresh with various DRAM chip densities.}

%%% ONUR: performance of \darp's two components -->  the performance of \darp's two components
\subsubsection{Performance Breakdown of \ib} To understand the observed
performance gain in more detail, we evaluate the performance of \darp's two
components separately. \emph{\Ooolong} improves performance by 3.2\%/3.9\%/3.0\%
on average and up to 16.8\%/21.3\%/20.2\% compared to \refab in 8/16/32Gb DRAMs.
Adding \emph{\warplong} to \emph{\ooolong} (\ib) provides additional performance
gains of 4.3\%/5.8\%/5.2\% on average by hiding refresh latency with write
accesses.

%The evaluations show that adding \emph{\warplong} to \emph{\ooolong} improves
%performance by 1.6\%/1.4\%/0.3\% on average and up to 6.0\%/3.0\%/1.2\%
%compared to using \ooolong alone on 8/16/32Gb DRAM devices. The results show
%that \warplong attains better performance gains at lower density because the
%refresh latency (\trfc) is shorter than the length of writeback mode at lower
%density, allowing more refreshes to be hidden behind writes. But, as the
%refresh latency elongates, there are fewer opportunities to hide refreshes
%behind writes as the total writeback interval remains roughly constant for the
%same workload.

%%% ONUR: Above: What is the perf improvement of OoO per bank refresh
%%% alone first? (Give this please) Then, give the perf improvement of
%%% wr-refresh parallelization alone. Then give them both
%%% together. This would be the best way of treating this section.

%%% ONUR: Alternatively, please have complete results in a technical
%%% report and cite the technical report for fully detailed results
%%% for all DRAM densities as I described above, This tech report is
%%% needed as you may not be able to fit in all these results in the
%%% current paper.

%%% ONUR: Is it true that the total writeback interval remains
%%% constant with the same workload?

%%% ONUR: The below section is very crisp and clear. Good!
\subsubsection{Energy}

Our techniques reduce energy per memory access compared to existing
policies, as shown in \figref{energy_reduction}. The main reason is
that the performance improvement reduces average static energy for
each memory access. Note that these results conservatively assume the
same power parameters for 8, 16, and 32 Gb chips, so the savings in
energy would likely be more significant if realistic power parameters
are used for the more power-hungry 16 and 32 Gb nodes.

%%% ONUR: Caption is occupying too much space. Try playing with the
%%% format so that valuable white space is not wasted.
\figputGHS{energy_reduction}{1.0}{Energy consumption. Value on top indicates
percentage reduction of \combo compared to
\caprefab.}

\subsubsection{Effect of Memory Intensity}
Figure~\ref{fig:mpki_ws} shows the performance improvement of \combo
compared to \refab and \refpb on workloads categorized by memory
intensity (\% of memory-intensive benchmarks in a workload),
respectively. We observe that \combo outperforms \refab and \refpb
consistently. Although the performance improvement of \combo over
\refab increases with higher memory intensity, the gain over \refpb
begins to plateau when the memory intensity grows beyond 25\%. This is
because \refpb's benefit over \refab also increases with memory
intensity as \refpb enables more accesses to be be parallelized with
refreshes. Nonetheless, our mechanism provides the highest system
performance compared to prior refresh policies.

\figputGHS{mpki_ws}{1.0}{WS improvement of {\small \combo}
over {\small \caprefab} and {\small \caprefpb} as memory intensity and DRAM density vary.}

%%% ONUR: In general, your captions are very long. Try to make them
%%% shorter and definitely change the format of how that looks (lots
%%% of space waste there now) -- the above caption seems fine though
%%% as there is nothing else that explains the figure in the figure.

\subsubsection{Effect of Core Count}
\label{sec:sense_core}

Table~\ref{table:core_sweep} shows the weighted speedup, harmonic speedup,
fairness, and energy-per-access improvement due to \combo compared to \refab for
systems with 2, 4, and 8 cores. For all three systems, \combo consistently
outperforms the baseline without unfairly penalizing any specific application.
We conclude that \combo is an effective mechanism to improve performance,
fairness and energy of multi-core systems employing high-density DRAM.

\input{sec/tables/core_sweep}
%\vspace{-0.1in}
%%% ONUR: How about harmonic speedup improvement? There was a reason
%%% this was nit included?

%%% ONUR: Very good and crisp explanation of tFAW below.
\subsection{Effect of \tfaw}
\label{sec:sense_tfaw}
Table~\ref{table:faw_sweep} shows the performance improvement of \ispb
over \refpb when we vary \tfaw in DRAM cycles (20 cycles for the
baseline as specified by the data sheet) and when \trrd scales
proportionally with \tfaw.\footnote{We evaluate only \ispb because it
  is sensitive to \tfaw and \trrd as it extends these parameters
  during parallelization of refreshes and accesses to compensate for
  the power overhead.} As \tfaw reduces, the performance benefit of
\ispb increases over \refpb. This is because reduced \tfaw enables
more accesses/refreshes to happen in parallel, which our mechanism
takes advantage of.

\input{sec/tables/sarp_faw_sweep}
\vspace{-0.08in}

\subsection{Effect of Subarrays-Per-Bank}
\label{sec:sense_sa}
%With more subarrays with in a bank, the benefit of using \is increases
%because the probability of memory requests to a refreshing subarray
%reduces.
Table~\ref{table:sa_sweep} shows that the average performance
gain of \ispb over \refpb increases as the number of subarrays
increases in 32Gb DRAM. This is because with more subarrays, the
probability of memory requests to a refreshing subarray reduces.

\input{sec/tables/subarray_sweep}
\vspace{-0.08in}

\subsection{Effect of Refresh Interval}
\label{sec:sense_ref}

For our studies so far, we use 32ms retention time (i.e., \trefi =
3.9$\mu$s) that represents a typical setting for a server environment
and LPDDR DRAM~\cite{jedec-lpddr3}. Table~\ref{table:64ms_summary}
shows the performance improvement of \combo over two baseline refresh
schemes using retention time of \emph{64ms} (i.e., \trefipb =
7.8$\mu$s). \combo consistently provides performance gains over both
refresh schemes. The maximum performance improvement over \refpb is
higher than that over \refab at 32Gb because \refpb actually degrades
performance compared to \refab for some workloads, as discussed in the
32ms results (Section~\ref{sec:multi-core-results}).

\input{sec/tables/64ms_summary}

\subsection{DDR4 Fine Granularity Refresh}
\label{sec:ddr4}

DDR4 DRAM supports a new refresh mode called \emph{fine granularity
  refresh (FGR)} in an attempt to mitigate the increasing refresh
latency (\trfc)~\cite{jedec-ddr4}. \fgr trades off shorter \trfc with
faster refresh rate ($\sfrac{1}{\trefi}$) that increases by either 2x
or 4x. \figref{ddr4_ref} shows the effect of \fgr in comparison to
\refab, \emph{adaptive refresh policy (AR)}~\cite{mukundan-isca2013},
and \combo. 2x and 4x \fgr actually reduce average system performance
by 3.9\%/4.0\%/4.3\% and 8.1\%/13.7\%/15.1\% compared to \refab with
8/16/32Gb densities, respectively. As the refresh rate increases by
2x/4x (higher refresh penalty), \trfc does not scale down with the
same constant factors. Instead, \trfc reduces by 1.35x/1.63x with
2x/4x higher rate~\cite{jedec-ddr4}, thus increasing the worst-case
refresh latency by 1.48x/2.45x. This performance degradation due to
\fgr has also been observed in Mukundan et
al.~\cite{mukundan-isca2013}.  AR~\cite{mukundan-isca2013} dynamically
switches between 1x (i.e., \refab) and 4x refresh modes to mitigate
the downsides of \fgr.  AR performs slightly worse than \refab (within
1\%) for all densities. Because using 4x \fgr greatly degrades
performance, AR can only mitigate the large loss from the 4x mode and
cannot improve performance over \refab. On the other hand, \combo is a
more effective mechanism to tolerate the long refresh latency than
both \fgr and AR as it overlaps refresh latency with access latency
without increasing the refresh rate.

%%% ONUR: See what I did above. It was not well organized before, and
%%% the benefits of DSARP over FGR and AR were not coming out. Please
%%% add the reference.

\figputGHS{ddr4_ref}{1.0}{Performance comparisons to FGR and AR~\cite{mukundan-isca2013}.}


==> sec/parref/7-related.tex <==
\section{Related Work}
\label{sec:related}

To our knowledge, this is the first work to comprehensively study the
effect of per-bank refresh and propose 1) a refresh scheduling policy
built on top of per-bank refresh and 2) a mechanism that achieves
parallelization of refresh and memory accesses {\em within} a
refreshing bank. We discuss prior works that mitigate the negative
effects of DRAM refresh and compare them to our mechanisms.
%%% ONUR: Note how I organized the above. It was not well
%%% organized. ``We also ...'' always reduces the strength of the
%%% thing that is said afterwards.

%To our knowledge, this is the first work to comprehensively study the effect
%of per-bank refresh and propose a refresh scheduling policy that is built on
%top of per-bank refresh. In addition, we propose a mechanism that achieves
%parallelization of refresh and memory accesses within a refreshing bank. In
%this section, we discuss prior works that have proposed different mechanisms
%to mitigate the negative effects of DRAM refresh. We refer a refresh as a
%conventional \mbox{all-bank} refresh unless stated otherwise.

%%% ONUR: Note how I rephrased the below. Again, organization and flow
%%% was not as good before. Also, the comparison sentence at the end
%%% was a bit weak.

%\textbf{Refresh Scheduling.} Stuecheli et al.~\cite{stuecheli-micro2010} propose
%elastic refresh that we discussed and evaluated in Section~\ref{sec:evaluation}.
%%Elastic refresh attempts to predict how long a memory rank will remain idle
%%(without a demand) periodically.
%%Then it postpones the refresh by a time delay
%Elastic refresh postpones refreshes by a time delay
%that varies based on the number of postponed refreshes and the predicted rank
%idle time to avoid interfering with demand requests. Elastic refresh has two
%shortcomings. First, it becomes less effective when the average rank idle period
%is shorter than \trfc as the refresh latency cannot be fully hidden in that
%period. This occurs especially with 1) more memory-intensive workloads that
%inherently have less idleness and 2) higher density DRAM chips that have higher
%\trfc. Second, elastic refresh incurs more refresh latency when it {\em
%incorrectly} predicts a time period as idle when it actually has pending
%requests.  In contrast, our mechanisms parallelize refresh operations with
%accesses even if there is no idle period and therefore outperform elastic
%refresh.

\textbf{Refresh Scheduling.} Stuecheli et al.~\cite{stuecheli-micro2010}
propose elastic refresh, which we discussed and evaluated in
Section~\ref{sec:evaluation}. Elastic refresh postpones refreshes by a time
delay that varies based on the number of postponed refreshes and the predicted
rank idle time to avoid interfering with demand requests. Elastic refresh has
two shortcomings. First, it becomes less effective when the average rank idle
period is shorter than \trfc as the refresh latency cannot be fully hidden in
that period. This occurs especially with 1) more memory-intensive workloads
that inherently have less idleness and 2) higher density DRAM chips that have
higher \trfc. Second, elastic refresh incurs more refresh latency when it {\em
incorrectly} predicts a time period as idle when it actually has pending
requests. In contrast, our mechanisms parallelize refresh operations with
accesses even if there is no idle period and therefore outperform elastic
refresh.

%\textbf{Refresh Scheduling.} Stuecheli et al.~\cite{stuecheli-micro2010}
%propose a mechanism, elastic refresh, that we have already explained and
%compared to in Section~\ref{sec:evaluation}. In sum, elastic refresh has three
%shortcomings.  First, it becomes less effective when the average idle period
%is shorter than \trfc as the refresh latency cannot be fully hidden in the
%idle period. Second, it has less opportunity to find long idle periods to
%schedule a refresh operation for more memory-intensive workloads and for
%higher density DRAM that has longer \trfc values. Third, elastic refresh
%incurs more refresh latency when it incorrectly predicts a time period that
%has pending requests as idle. In contrast to our mechanisms, elastic refresh
%does not parallelize refresh operations with accesses and it requires idle
%periods. As a result, our mechanisms are more effective when there is no idle
%period as we parallelize refresh operations with accesses to hide refresh
%latency.

Ishii et al.~\cite{ishii-msc2012} propose a write scheduling policy
that prioritizes write draining over read requests in a rank while
another rank is refreshing (even if the write queue has not reached
the threshold to trigger write mode). This technique is {\em only}
applicable in multi-ranked memory systems.  Our mechanisms are {\em
  also} applicable to single-ranked memory systems by enabling
parallelization of refreshes and accesses at the bank and subarray
levels, and they can be combined with Ishii et
al.~\cite{ishii-msc2012}.

%Because their mechanism is orthogonal to ours, it can be combined with ours
%schemes.
%%% ONUR2: Bad English in the abive commented-out sentence.

%%% ONUR: The above technique is also different, right? It does not
%%% pull-in or postpone refreshes, instead it decides to go into WB
%%% mode when a rank is refreshing, correct? As such, can it not be
%%% combined with your techniques? If so, better to say this, too.
%%% ONUR: Also see how I clarified ``the threshold.''

%Ishii et al.~\cite{ishii-msc2012} propose a write scheduling policy that
%prioritizes write draining over read requests in a rank while another rank is
%performing refresh even if the write queue hasn't reached the threshold.
%However, it is unclear why the proposal prioritizes writes over reads when a
%rank can serve any type of requests independently of another rank. In addition,
%this technique is only applicable in a multi-rank memory subsystem. Our
%mechanisms differ from theirs as we enable parallelization
%of refresh and memory accesses at the bank and subarray level.

Mukundan et al.~\cite{mukundan-isca2013} propose scheduling techniques (in
addition to adaptive refresh discussed in Section~\ref{sec:ddr4}) to address the
problem of {\em command queue seizure}, whereby a command queue gets filled up
with commands to a refreshing rank, blocking commands to {\em another}
non-refreshing rank.  In our work, we use a different memory controller design
that does not have command queues, similarly to prior
work~\cite{herrero-tc2013}. Our controller generates a command for a scheduled
request {\em right before} the request is sent to DRAM instead of pre-generating
the commands and queueing them up. Thus, our baseline design does not suffer
from the problem of command queue seizure.

%In addition to adaptive refresh discussed in Section~\ref{sec:ddr4}, Mukundan et
%al.~\cite{mukundan-isca2013} propose other scheduling techniques to address the
%problem of command queue seizure, whereby a command queue gets filled up with
%commands to a refreshing rank, blocking commands to another non-refreshing rank.
%In our work, we use a different memory controller design that does not have
%command queues. The key distinction is that our controller generates a command
%for a scheduled request right before it is sent to DRAM instead of
%pre-generating the commands and queueing them up. Thus, our design ensures that
%command queue seizure does not happen. A similar design has been used in prior
%work~\cite{herrero-tc2013}.

\textbf{Subarray-Level Parallelism (SALP).} Kim et
al.~\cite{kim-isca2012} propose SALP to reduce bank serialization
latency by enabling {\em multiple accesses} to different subarrays
within a bank to proceed in a pipelined manner. In contrast to SALP,
our mechanism (\is) parallelizes {\em refreshes and accesses} to
different subarrays within the same bank. Therefore, \is exploits the
existence of subarrays for a different purpose and in a different way
from SALP. As Section~\ref{sec:sarp_implementation} describes, we
reduce the sharing of the peripheral circuits for refreshes and
accesses, not for arbitrary accesses. As such, our implementation is
not only different, but also less intrusive than SALP: \is does not
require new DRAM commands and timing constraints.

%Such an implementation regarding refresh is not discussed and
%explored in SALP.

%\textbf{Subarray-Level Parallelism.} Kim et al. propose a technique called
%“subarray-level parallelism” (SALP)~\cite{kim-isca2012} to improve DRAM
%performance. SALP reduces bank serialization latency by enabling multiple
%accesses to different subarrays within a bank to proceed in parallel. The key
%difference between \is (our proposal) and SALP is that unlike \is, SALP cannot
%parallelize a refresh operation in one subarray with an access to another
%subarray in the same bank. In SALP, a single row counter provides the refresh
%row address that passes through the row-address MUX shared with the row address
%provided by the memory controller as shown in \figref{detail-bank-organization}.
%Because a single refresh command initiates a \emph{sequence} of rows to be
%refreshed internally, the memory controller is oblivious to when the refresh
%logic is sending the refresh row address through the bus to the row-address MUX.
%As a result, an externally issued command can collide with a refresh row address
%within a bank, resulting in unknown outcome for the external command from the
%memory controller. To solve this problem, we reduce the sharing of the
%peripheral circuits for the refresh row address and the externally issued row
%address within a bank. Specifically, we separate the row counter into two
%separate counters and route these counters with global wires across the bank to
%provide refresh selection. Such a modification along with the appropriate bank
%control logic enables \is to parallelize refreshes with accesses, which cannot
%be achieved with the current implementation of SALP.

\textbf{Refresh Pausing.} Nair et al.~\cite{nair-hpca2013} propose
pausing a refresh operation to serve pending memory requests. To make
pausing a refresh possible, the authors assume that DRAM refreshes
multiple rows \emph{sequentially}. Thus, there is a short recovery
time, called a "refresh pausing point" (RPP), after refreshing each
row so that the memory controller can signal the DRAM to stop
refreshing subsequent rows. However, DRAM manufacturers currently
design their chips to refresh multiple rows in \emph{parallel} (or, in
a {\em staggered/pipelined} way, as explained
in~\cite{mukundan-isca2013}).
%Therefore, the current implementation of refresh
%pausing requires modification to become effective in modern DRAM due to lack of
%RPPs.
%%% ONUR: Do you really need the sentence that starts with
%%% ``Therefore'' at the very end above? Maybe shorten it while
%%% keeping the strength?

%The authors show that
%the latency to refresh eight rows ($8 \times \trc$) individually by issuing
%explicit activation commands from a memory controller is \emph{less} than the
%refresh latency (\trfc) resulting from a refresh command.
%However, DRAM manufacturers currently design their chips to refresh multiple
%rows in \emph{parallel} (staggered/pipelined as explained in
%~\cite{mukundan-isca2013}). The current 8Gb DDR3 DRAM data
%sheets~\cite{jedec-ddr3,micronDDR3_8Gb} actually show that 8 $\times$ \trc $>$
%\trfc with \trc ranging from 45ns to 52.5ns (as opposed to 39ns used
%in~\cite{nair-hpca2013}) with \trfc remaining at 350ns.
%ddr4: 44.5ns - 50ns
%ddr3-1066: 50.625 for the exact same params as in the micron datasheet

%\textbf{Refresh Pausing.}
%Nair et al.~\cite{nair-hpca2013} propose refresh pausing in attempt to pause a
%refresh to serve memory requests. To make pausing a refresh possible, the
%authors assume that there is a short recovery time, called a "refresh pausing
%point" (RPP), after refreshing each row so that the memory controller can signal
%the DRAM to stop refreshing subsequent rows. The reason RPPs exist is that they
%assume rows are \emph{sequentially} refreshed during refresh and the latency
%to refresh eight rows sequentially ($8 \times \trc$) is \emph{less} than the
%refresh latency (\trfc). However, DRAM manufacturers currently design their
%chips so that multiple rows are refreshed in \emph{parallel}
%(staggered/pipelined as explained in ~\cite{mukundan-isca2013}). Using the same
%8Gb DDR3 DRAM data sheets~\cite{jedec-ddr3,micronDDR3_8Gb} actually shows that
%8 $\times$ \trc $>$ \trfc with \trc ranging from 45ns to 52.5ns (as opposed
%to 39ns used in their paper) with \trfc remaining at 350ns. Therefore, to make
%refresh pausing viable, one would need to justify the existence of Refresh
%Pausing Points.

\textbf{eDRAM Concurrent Refresh.} Kirihata et al.~\cite{kirihata-jssc2005}
propose a mechanism to enable a bank to refresh independently while another bank
is being accessed in embedded DRAM (eDRAM). Our work differs
from~\cite{kirihata-jssc2005} in two major ways. First, unlike
SARP,~\cite{kirihata-jssc2005} parallelizes refreshes only across banks, not
{\em within} each bank.  Second, there are significant differences between DRAM
and eDRAM architectures, which make it non-trivial to
apply~\cite{kirihata-jssc2005}'s mechanism directly to DRAM. In particular,
eDRAMs have no standardized timing/power integrity constraints and access
protocol, making it simpler for each bank to independently manage its refresh
schedule. In contrast, refreshes in DRAM need to be managed by the memory
controller to ensure that parallelizing refreshes with accesses does not violate
other constraints.
%%% ONUR: Good, above. See my slight changes to make it better and put more emphasis.

%\textbf{eDRAM Concurrent Refresh.} Kirihata et al.~\cite{kirihata-jssc2005}
%propose a mechanism to enable a bank to refresh independently while another bank
%is being accessed in embedded DRAM (eDRAM). Our work differs
%from~\cite{kirihata-jssc2005} in two important ways. First, unlike SARP, their
%proposal parallelizes refreshes only across banks and not within banks. In this
%regard, their work shares more similarities with per-bank refresh in LPDDR
%DRAMs. Second, there are significant differences between DRAM and eDRAM
%architectures, which make it non-trivial to apply their technique directly to
%DRAM architectures. In particular, eDRAMs have no standardized timing/power
%integrity constraints and access protocol, making it simpler for each bank to
%independently manage its refresh schedule. In contrast, refreshes in DRAM need
%to be managed by the memory controller to ensure that parallelizing refreshes
%with accesses does not violate other constraints.

\textbf{Retention-Aware Refresh.} Prior works
(e.g.,~\cite{liu-isca2012, venkatesan-hpca2006}) propose mechanisms to
reduce unnecessary refresh operations by taking advantage of the fact
that different DRAM cells have widely different retention
times~\cite{liu-isca2013}. These works assume that the retention time
of DRAM cells can be \emph{accurately} profiled and they depend on
having this accurate profile in order to guarantee data
integrity~\cite{liu-isca2013}. However, as shown
in~\cite{liu-isca2013}, accurately determining the retention time
profile of DRAM is an unsolved research problem due to the Variable
Retention Time and Data Pattern Dependence phenomena, which can cause
the retention time of a cell to fluctuate over time.  As such,
retention-aware refresh techniques need to overcome the profiling
challenges to be viable.

%%% ONUR: See my rephrasing of the above paragraph.

%leak charge at different
%rates due to various factors, such as process variation, leading to


==> sec/parref/7-related_dhl.tex <==
\section{Related Work}
\label{sec:related}

To our knowledge, this is the first work to comprehensively study the effect of
per-bank refresh and propose a refresh scheduling policy built on top of
per-bank refresh. We also propose a mechanism that achieves parallelization of
refresh and memory accesses within a refreshing bank. In this section, we
discuss prior works that mitigate the negative effects of DRAM refresh and
compare them to our mechanisms.

%To our knowledge, this is the first work to comprehensively study the effect
%of per-bank refresh and propose a refresh scheduling policy that is built on
%top of per-bank refresh. In addition, we propose a mechanism that achieves
%parallelization of refresh and memory accesses within a refreshing bank. In
%this section, we discuss prior works that have proposed different mechanisms
%to mitigate the negative effects of DRAM refresh. We refer a refresh as a
%conventional \mbox{all-bank} refresh unless stated otherwise.

\textbf{Refresh Scheduling.} Stuecheli et al.~\cite{stuecheli-micro2010}
propose elastic refresh that is discussed and evaluated in
Section~\ref{sec:evaluation}. In sum, elastic refresh has two shortcomings.
First, it becomes less effective when the average idle period is shorter than
\trfc as the refresh latency cannot be fully
hidden in the idle period. This occurs when
using more memory-intensive workloads with less idleness and
higher density DRAM with longer \trfc.
Second, elastic refresh incurs more refresh latency
when it incorrectly predicts a time period that has pending requests as idle.
In contrast to elastic refresh, our mechanisms parallelize refresh operations
with accesses even if there is no idle period.

%\textbf{Refresh Scheduling.} Stuecheli et al.~\cite{stuecheli-micro2010}
%propose a mechanism, elastic refresh, that we have already explained and
%compared to in Section~\ref{sec:evaluation}. In sum, elastic refresh has three
%shortcomings.  First, it becomes less effective when the average idle period
%is shorter than \trfc as the refresh latency cannot be fully hidden in the
%idle period. Second, it has less opportunity to find long idle periods to
%schedule a refresh operation for more memory-intensive workloads and for
%higher density DRAM that has longer \trfc values. Third, elastic refresh
%incurs more refresh latency when it incorrectly predicts a time period that
%has pending requests as idle. In contrast to our mechanisms, elastic refresh
%does not parallelize refresh operations with accesses and it requires idle
%periods. As a result, our mechanisms are more effective when there is no idle
%period as we parallelize refresh operations with accesses to hide refresh
%latency.

Ishii et al.~\cite{ishii-msc2012} propose a write scheduling policy that
prioritizes write draining over read requests in a rank while another rank is
refreshing even if the write queue hasn't reached the threshold. While
this technique is only applicable in multi-rank memory systems, our
mechanisms are also applicable to single-rank memory systems by enabling
parallelization of refreshes and accesses at the bank and subarray level.

%Ishii et al.~\cite{ishii-msc2012} propose a write scheduling policy that
%prioritizes write draining over read requests in a rank while another rank is
%performing refresh even if the write queue hasn't reached the threshold.
%However, it is unclear why the proposal prioritizes writes over reads when a
%rank can serve any type of requests independently of another rank. In addition,
%this technique is only applicable in a multi-rank memory subsystem. Our
%mechanisms differ from theirs as we enable parallelization
%of refresh and memory accesses at the bank and subarray level.

Mukundan et al.~\cite{mukundan-isca2013} propose scheduling techniques in
addition to adaptive refresh discussed in Section~\ref{sec:ddr4} to address the
problem of command queue seizure, whereby a command queue gets filled up with
commands to a refreshing rank, blocking commands to another non-refreshing rank.
In our work, we use a different memory controller design that does not have
command queues as similar to prior work~\cite{herrero-tc2013}. The key
distinction is that our controller generates a command for a scheduled request
right before it is sent to DRAM instead of pre-generating the commands and
queueing them up. Thus, our design does not suffer from command queue seizure.

%In addition to adaptive refresh discussed in Section~\ref{sec:ddr4}, Mukundan et
%al.~\cite{mukundan-isca2013} propose other scheduling techniques to address the
%problem of command queue seizure, whereby a command queue gets filled up with
%commands to a refreshing rank, blocking commands to another non-refreshing rank.
%In our work, we use a different memory controller design that does not have
%command queues. The key distinction is that our controller generates a command
%for a scheduled request right before it is sent to DRAM instead of
%pre-generating the commands and queueing them up. Thus, our design ensures that
%command queue seizure does not happen. A similar design has been used in prior
%work~\cite{herrero-tc2013}.

\textbf{Subarray-Level Parallelism.} Kim et al. propose a technique called
“subarray-level parallelism” (SALP)~\cite{kim-isca2012} to reduce bank
serialization latency by enabling multiple accesses to different subarrays
within a bank to proceed in parallel. In contrast to SALP, our mechanism (\is)
parallelizes refreshes and accesses to different subarrays within the same bank.
As described in Section~\ref{sec:sarp_implementation}, we reduce the sharing of the
peripheral circuits for refreshes and accesses. Such an implementation regarding
refresh is not discussed and explored in SALP. Therefore, \is enables
independent subarray operations in a different way from SALP.

%\textbf{Subarray-Level Parallelism.} Kim et al. propose a technique called
%“subarray-level parallelism” (SALP)~\cite{kim-isca2012} to improve DRAM
%performance. SALP reduces bank serialization latency by enabling multiple
%accesses to different subarrays within a bank to proceed in parallel. The key
%difference between \is (our proposal) and SALP is that unlike \is, SALP cannot
%parallelize a refresh operation in one subarray with an access to another
%subarray in the same bank. In SALP, a single row counter provides the refresh
%row address that passes through the row-address MUX shared with the row address
%provided by the memory controller as shown in \figref{detail-bank-organization}.
%Because a single refresh command initiates a \emph{sequence} of rows to be
%refreshed internally, the memory controller is oblivious to when the refresh
%logic is sending the refresh row address through the bus to the row-address MUX.
%As a result, an externally issued command can collide with a refresh row address
%within a bank, resulting in unknown outcome for the external command from the
%memory controller. To solve this problem, we reduce the sharing of the
%peripheral circuits for the refresh row address and the externally issued row
%address within a bank. Specifically, we separate the row counter into two
%separate counters and route these counters with global wires across the bank to
%provide refresh selection. Such a modification along with the appropriate bank
%control logic enables \is to parallelize refreshes with accesses, which cannot
%be achieved with the current implementation of SALP.

\textbf{Refresh Pausing.} Nair et al.~\cite{nair-hpca2013} propose refresh
pausing that pauses a refresh to serve memory requests. To make pausing a
refresh possible, the authors assume that DRAM refreshes multiple rows
\emph{sequentially}. Thus, there is a short recovery time, called a "refresh
pausing point" (RPP), after refreshing each row so that the memory controller
can signal the DRAM to stop refreshing subsequent rows. However, DRAM
manufacturers currently design their chips to refresh multiple rows in
\emph{parallel} (staggered/pipelined as explained in ~\cite{mukundan-isca2013}).
Therefore, the current implementation of refresh pausing requires modification
to become effective in modern DRAM due to lack of RPPs.

%The authors show that
%the latency to refresh eight rows ($8 \times \trc$) individually by issuing
%explicit activation commands from a memory controller is \emph{less} than the
%refresh latency (\trfc) resulting from a refresh command.
%However, DRAM manufacturers currently design their chips to refresh multiple
%rows in \emph{parallel} (staggered/pipelined as explained in
%~\cite{mukundan-isca2013}). The current 8Gb DDR3 DRAM data
%sheets~\cite{jedec-ddr3,micronDDR3_8Gb} actually show that 8 $\times$ \trc $>$
%\trfc with \trc ranging from 45ns to 52.5ns (as opposed to 39ns used
%in~\cite{nair-hpca2013}) with \trfc remaining at 350ns.
%ddr4: 44.5ns - 50ns
%ddr3-1066: 50.625 for the exact same params as in the micron datasheet

%\textbf{Refresh Pausing.}
%Nair et al.~\cite{nair-hpca2013} propose refresh pausing in attempt to pause a
%refresh to serve memory requests. To make pausing a refresh possible, the
%authors assume that there is a short recovery time, called a "refresh pausing
%point" (RPP), after refreshing each row so that the memory controller can signal
%the DRAM to stop refreshing subsequent rows. The reason RPPs exist is that they
%assume rows are \emph{sequentially} refreshed during refresh and the latency
%to refresh eight rows sequentially ($8 \times \trc$) is \emph{less} than the
%refresh latency (\trfc). However, DRAM manufacturers currently design their
%chips so that multiple rows are refreshed in \emph{parallel}
%(staggered/pipelined as explained in ~\cite{mukundan-isca2013}). Using the same
%8Gb DDR3 DRAM data sheets~\cite{jedec-ddr3,micronDDR3_8Gb} actually shows that
%8 $\times$ \trc $>$ \trfc with \trc ranging from 45ns to 52.5ns (as opposed
%to 39ns used in their paper) with \trfc remaining at 350ns. Therefore, to make
%refresh pausing viable, one would need to justify the existence of Refresh
%Pausing Points.

\textbf{eDRAM Concurrent Refresh.} Kirihata et al.~\cite{kirihata-jssc2005}
propose a mechanism to enable a bank to refresh independently while another
bank is being accessed in embedded DRAM (eDRAM). Our work differs
from~\cite{kirihata-jssc2005} in two important ways. First, unlike SARP, their
proposal parallelizes refreshes only across banks and not within banks.
Second, there are significant differences between DRAM and eDRAM architectures,
which make it non-trivial to apply their technique directly to DRAM
architectures. In particular, eDRAMs have no standardized timing/power
integrity constraints and access protocol, making it simpler for each bank to
independently manage its refresh schedule. In contrast, refreshes in DRAM need
to be managed by the memory controller to ensure that parallelizing refreshes
with accesses does not violate other constraints.

%\textbf{eDRAM Concurrent Refresh.} Kirihata et al.~\cite{kirihata-jssc2005}
%propose a mechanism to enable a bank to refresh independently while another bank
%is being accessed in embedded DRAM (eDRAM). Our work differs
%from~\cite{kirihata-jssc2005} in two important ways. First, unlike SARP, their
%proposal parallelizes refreshes only across banks and not within banks. In this
%regard, their work shares more similarities with per-bank refresh in LPDDR
%DRAMs. Second, there are significant differences between DRAM and eDRAM
%architectures, which make it non-trivial to apply their technique directly to
%DRAM architectures. In particular, eDRAMs have no standardized timing/power
%integrity constraints and access protocol, making it simpler for each bank to
%independently manage its refresh schedule. In contrast, refreshes in DRAM need
%to be managed by the memory controller to ensure that parallelizing refreshes
%with accesses does not violate other constraints.

\textbf{Retention-Aware Refresh.} Prior works (e.g.,~\cite{liu-isca2012,
venkatesan-hpca2006}) have proposed mechanisms to take advantage of the fact
that DRAM cells leak charge at different rates due to various factors, such as
process variation, leading to different retention time for each cell. However,
these prior works have the same disadvantage of assuming that the retention
time of DRAM cells can be \emph{accurately} profiled and their mechanisms all
depend on having this profile in order to guarantee that DRAM refresh is
handled in a timely manner. Ensuring profile accuracy has the difficulties of
facing physical phenomena of Variable Retention Time (VRT) and Data Pattern
Dependence (DPD)~\cite{liu-isca2013} that can cause the retention time of a
cell to fluctuate over time. Therefore, these mechanisms need to overcome the
profiling challenges to be viable.


==> sec/parref/8-conclusion.tex <==
\section{Conclusion}

We introduced two new complementary techniques, \ib (\darplong) and
\is (\intersub), to mitigate the DRAM refresh penalty by enhancing
\emph{refresh-access parallelization} at the bank and subarray levels,
respectively.  \darp 1) issues per-bank refreshes to idle banks in an
out-of-order manner instead of issuing refreshes in a strict
round-robin order, 2) proactively schedules per-bank refreshes during
intervals when a batch of writes are draining to DRAM.  \is enables a
bank to serve requests from idle subarrays in parallel with other
subarrays that are being refreshed. Our extensive evaluations on a
wide variety of systems and workloads show that these mechanisms
significantly improve system performance and outperform
state-of-the-art refresh policies, approaching the performance of
ideally eliminating all refreshes. We conclude that \ib and \is are
effective in hiding the refresh latency penalty in modern and
near-future DRAM systems, and that their benefits increase as DRAM
density increases.

%%% ONUR: I increased the strength of this. Please see above. This is
%%% much stronger now.


==> sec/parref/algos/interbank-algo.tex.0527 <==
\begin{algorithm}
\caption{\small Parallelizing Refreshes with Write Requests}
\label{algo:interbank-algo}
\footnotesize{
\textbf{\underline{Definition:}}
\begin{algorithmic}
\STATE \begin{itemize}
    \item \textit{N}: number of banks per rank
    \item \textit{write\_queue[N]}: an array of queues storing write requests
    \item \textit{refresh\_queue[N]}: an array of queues storing refresh requests
    \item \textit{ref\_credit[N]}: an array of credits keeping track of the number of
    postponed and pulled-in refreshes
    \item \textit{next\_ref\_bank}: the bank to be refreshed next after \trefi refreshes
    \item \textit{max\_postpone}: maximum number of allowed postponed refreshes
    \item \textit{max\_pull}: maximum number of allowed pulled-in refreshes
    \item \textit{refreshBank(b)}: refresh the specified bank
    \end{itemize}
\end{algorithmic}

\textbf{\underline{Every tREFI:}}
\begin{algorithmic}
\IF{\textit{ref\_credit[\textit{next\_ref\_bank}]} > -\textit{max\_postpone}}
    \STATE \textit{ref\_credit[\textit{next\_ref\_bank}]} -= 1
    \COMMENT {Postpone refresh}
\ELSE
    \STATE \textit{refreshBank(\textit{next\_ref\_bank})}
\ENDIF
\end{algorithmic}

\textbf{\underline{During Writeback Mode:}}
\begin{algorithmic}
\IF {no write request is scheduled}
\FOR{\textbf{each} $b$ in N}
    \IF {$refresh\_queue[b].isEmpty()$ AND $b.isIdle()$ AND $ref\_credit[b] <
    max\_pull$ AND $\frac{\trc \times
    write\_requests\_left} {writeback\_BLP} > tRFC$}
        \STATE \textit{refreshBank($b$)}
        \COMMENT {Issue either a postponed or pulled-in refresh}
        \STATE \textit{ref\_credit[$b$]} += 1
        \STATE break
    \ENDIF
\ENDFOR
\ENDIF
\end{algorithmic}
}
\end{algorithm}


==> sec/parref/algos/ooo-algo.tex <==
\begin{algorithm}
\caption{\small \ooolongCap}
\label{algo:ooo-algo}
\footnotesize{
\textbf{\underline{Definition:}}
\begin{algorithmic}
\STATE \begin{itemize}
    \item \textit{ref\_credit[number of banks]}: an array of credits keeping track of the number of
    postponed and pulled-in refreshes
    \item \textit{max\_postpone}: maximum number of allowed postponed refreshes
    \item \textit{max\_pull}: maximum number of allowed pulled-in refreshes
    \item \textit{refresh\_candidate}: a list of bank IDs with no
    pending read requests
    \item \textit{ref\_bank}: the bank to be refreshed in the sequential
    round-robin order
    \end{itemize}
\end{algorithmic}

\textbf{\underline{Every tREFI:}}
\begin{algorithmic}
\IF{\textit{ref\_credit[\textit{ref\_bank}]} > -\textit{max\_postpone}}
    \STATE \textit{ref\_credit[\textit{ref\_bank}]} -= 1
    \COMMENT {\textbf{Postpone refresh}}
\ELSE
    \STATE \textit{refreshBank(\textit{ref\_bank})}
    \COMMENT {\textbf{A forced refresh}}
\ENDIF
\end{algorithmic}

\textbf{\underline{Every Cycle:}}
\begin{algorithmic}
\IF{no demand request issued}
    \FOR{\textbf{each} \textit{bank} in \textit{refresh\_candidate}}
        \IF{-\textit{max\_postpone} < \textit{ref\_credit[\textit{bank}]} <
        \textit{max\_pull}}
            \STATE \textit{refreshBank(\textit{bank})}
            \COMMENT {\textbf{Either a postponed or pulled-in refresh}}
            \STATE break
        \ENDIF
    \ENDFOR
\ENDIF
\end{algorithmic}
}
\end{algorithm}


==> sec/proposal_related.tex <==
\section{Related Work}

\subsection{Low Latency DRAM Architecture}

Many previous works have proposed various DRAM architectures to provide
low-latency operations. We will describe the relevant works by dividing them into
different categories based on their similarity.

\subsubsection{Commodity Low Latency DIMM}

RLDRAM~\cite{micron-rldram3} and FCRAM~\cite{sato-vlsic1998} enable lower DRAM
timing parameters by reducing the length of bitlines (i.e., with fewer number of
cells attached to each bitline). Because the bitline parasitic capacitance
reduces with its length, shorter bitlines enable faster sensing between the
cells and the sense amplifiers, thus reducing the latency of DRAM operations.
The main drawback of this simple approach is that it leads to lower chip density
from a large amount of area overhead (30-40\% for FCRAM, 40-80\% for RLDRAM) due
to the additional peripheral logic (e.g., row decoders)~\cite{kim-isca2012}.

%because more subarrays are allocated with
%shorter bitlines, thus incurring additional area from the peripheral logics
%(e.g., row decoders and sense amplifiers) in each subarray.

\subsubsection{Cached DRAM}

Several prior works (e.g., \cite{ hart-compcon1994, hidaka-ieeemicro90,
hsu-isca1993,kedem-1997}) have proposed to add a small SRAM cache to DRAM chips
to lower the access latency for hot data. The main disadvantage of these works
is that the SRAM cache incurs a high area overhead and design
complexity~\cite{kim-isca2012}.

\subsubsection{Heterogeneous DRAM}

Prior work introduces heterogeneity into DRAM, where one region has a fast
access latency but fewer DRAM rows, while the other has a slower access latency
but many more rows~\cite{lee-hpca2013, son-isca2013}. The fast region is mainly
utilized as a caching area for the frequently access data. We briefly describe
two state-of-the-art works that offer different heterogeneous DRAM designs.

\ignore{Lee et al.~\cite{lee-hpca2013} proposed TL-DRAM that divides
each subarray into fast and slow segments that have short and long bitlines,
respectively, using isolation transistors. TL-DRAM reduces the memory latency by
caching data from slow segments into fast segments. The main shortcoming of
TL-DRAM is that the isolation transistors are intrusive to the cell array due to
their larger pitch size compared to the pitch between two cells, thus reducing
the array's density.}
%Since the data from the slow
%segment can be transferred to the fast segment at very low latency, TL-DRAM can
%be exploited using an OS-transparent hardware caching scheme.
%. An isolation transistor is typically several times larger than a
%cell. As a result, adding an isolation to each bitline inside an array affects
%the \emph{pitch} between cells, reducing the cell array density.

CHARM~\cite{son-isca2013} introduces heterogeneity \emph{within a rank} by
designing a few fast banks with (1)~shorter bitlines for faster data sensing,
and (2)~closer placement to the chip I/O for faster data transfers. To exploit
these low-latency banks, CHARM uses an OS-managed mechanism to statically map
hot data to these banks, based on profiled information from the compiler or
programmers. Unfortunately, this approach cannot adapt to program phase changes,
limiting its performance gains. If it were to adopt dynamic hot data management,
CHARM would incur high migration costs over the narrow 64-bit bus \figref{background_bank_sa_detail}.

\ignore{Son et al.~\cite{son-isca2013} proposed CHARM by adding heterogeneity at
the bank level. CHARM allocates a few fast banks with (1) shorter bitlines for
faster data sensing and (2) shorter data lines to the I/O for faster data
transfers. Although CHARM prevents the problem of intrusive design to cell
arrays, its design cannot be exploited with a hardware caching scheme. It
requires the OS to map hot data to low-latency banks, based on profiled
information from the compiler or programmers. The reason is that the caching
latency from a slow bank to a fast bank is so high that it overshadows the
benefits from caching in the fast banks.}

TL-DRAM~\cite{lee-hpca2013} provides heterogeneity \emph{within a subarray} by
dividing it into fast (near) and slow (far) segments that have short and long
bitlines, respectively, using isolation transistors. The fast segment is managed
as an OS-transparent hardware cache. The main disadvantage is that it needs to
cache each hot row in \emph{two near segments} as each subarray uses two row
buffers on \emph{opposite ends} to sense data in the open-bitline architecture
(Section~\ref{sec:bank-org}). This prevents TL-DRAM from using the full near
segment capacity. As we can see, neither CHARM nor TL-DRAM strike a good design
balance for their heterogeneous DRAM. In Section~\ref{sec:villa}, we describe a
new heterogeneous DRAM design that fully utilizes the caching area with low
migration cost.

Another work has proposed a different form of heterogeneous DRAM by exploiting
latency variation due to temperature in existing DRAM chips. Modern DRAM is
designed to follow the JEDEC standard that defines a set of timing parameters,
which determine the DRAM access latency. Since DRAM can be employed in systems
under a wide range of environment, the timings are provisioned for the worst
case scenario (e.g., high temperature). Chandrasekar et
al.~\cite{chandrasekar-date2014} and Lee et al.~\cite{lee-hpca2015} evaluated
the potential DRAM timing parameter reduction by exploiting the safety margin
added due to process or temperature variation. They showed that some amount of
reduction on DRAM timing parameters exhibit no DRAM errors because typical
systems do not operate under worst-case environment.

Based on this observation, Lee et al.~\cite{lee-hpca2015} further propose a
mechanism that dynamically optimizes the DRAM timing parameters based on the
operating temperature to reduce access latency. However, such a mechanism
applies uniform timing parameters that guarantee reliability for \emph{every}
DRAM cell. In part of our proposal (Section~\ref{sec:proposal_1}), we describe a
way to further exploit potential timing reduction by employing timing parameters
based on the location of the cells, which express different behavior.

\subsection{Low-Latency Data Migration}
\label{sec:rowclone}

Migrating a large amount of data across memory is a long latency operation that
significantly degrades system performance in today's system. The main reason is
that data has to move over the narrow memory channels multiple times when it's
read from the memory to the processor, then written back to the memory. To avoid
costly transfers over memory channels for bulk data migration, Seshadri et
al.~\cite{seshadri-micro2013} propose, RowClone, to perform migration within
DRAM chips, thus reducing the migration latency.

However, it has two main drawbacks that limit its efficacy. First, RowClone's
main benefits are limited to \emph{within} a subarray, which typically only
consists of 512 rows of DRAM cells, resulting in a very small amount of
migration range. Second, performing data migration across subarrays is much
slower than within a subarray. This is because \rc transfers data over the
narrow DRAM-internal data bus (i.e., 64 bits). In fact, we observe that RowClone
performs worse than today's baseline (by 24\% across 50 workloads in a quad-core
system) when migrating data across subarrays as it ties up the internal DRAM bus
for an excessive duration.

\subsection{DRAM Refresh Latency Mitigation}

%\mbox{}\\ \indent \textbf{Retention-Aware Refresh.}
Prior works (e.g.,~\cite{liu-isca2012,
venkatesan-hpca2006}) have proposed mechanisms to reduce unnecessary refresh
operations by taking advantage of the fact that different DRAM cells have widely
different retention times~\cite{liu-isca2013}. These works assume that the
retention time of DRAM cells can be \emph{accurately} profiled and they depend
on having this accurate profile in order to guarantee data
integrity~\cite{liu-isca2013}. However, as shown in~\cite{liu-isca2013},
accurately determining the retention time profile of DRAM is an unsolved
research problem due to the Variable Retention Time and Data Pattern Dependence
phenomena, which can cause the retention time of a cell to fluctuate over time.
As such, retention-aware refresh techniques need to overcome the profiling
challenges to be viable.

%\textbf{Refresh Pausing.}
Nair et al.~\cite{nair-hpca2013} propose pausing a
refresh operation to serve pending memory requests. To make pausing a refresh
possible, the authors assume that DRAM refreshes multiple rows
\emph{sequentially}. Thus, there is a short recovery time, called a "refresh
pausing point" (RPP), after refreshing each row so that the memory controller
can signal the DRAM to stop refreshing subsequent rows. However, DRAM
manufacturers currently design their chips to refresh multiple rows in
\emph{parallel} (or, in a {\em staggered/pipelined} way, as explained
in~\cite{mukundan-isca2013}).



\ignore{\subsection{Increased DRAM Parallelism}

Kim et al.~\cite{kim-isca2012} proposed Subarray level parallelism (SALP) to
take advantage of the existing subarray architecture to overlap multiple memory
requests going to the same bank. As subarrays contain local row buffers, they
can be activated concurrently with minimal additional hardware, allowing
overlapping activation and precharge to independent subarrays as well as row
buffer caching for inactive subarrays. Row buffer decoupling splits the
precharging operation into two parts~\cite{o-isca2014}. Through the use of an
isolation transistor separating the bitline from the sense amplifier, the
bitlines can be precharged immediately after row activation. The sense
amplifiers are precharged when a row needs to be closed, but since they
precharge much faster than the bitlines, the effective precharge time observed
by the memory controller decreases significantly.}

%\subsection{Reduced DRAM Timing Parameters}
%Another recent approach O et al. [34] propose to add isolation transistors that
%separate bitlines from their sense amplifiers, so the bitlines can be
%precharged without deactivating the row buffer. This helps hide the latency
%impact of precharge.
%Another recent approach is to decouple sense amplifiers from long
%bitlines~\cite{o-isca2014} to accelerate sense amplifiers' sensing time and
%precharge operations, resulting in reduced DRAM access latency.


==> sec/scatchpad <==
========related work========
\ignore{
Techniques like out-of-order
execution~\cite{tomasulo-ibmj67}, non-blocking caches~\cite{kroft-isca81},  and
runahead execution~\cite{mutlu-isca2005, mutlu-hpca2003, mutlu-micro2005}

strive
to overlap the latency of future DRAM accesses with the current stalling DRAM
access so that the future memory-stall time is reduced for the processor.

Prior works~\cite{mutlu-isca2005, mutlu-hpca2003,
  mutlu-micro2005} propose runahead execution that continues to fetch and
execute instructions when the processor stalls on memory. The goal of runahead
is to

The concept of generating and servicing multiple
DRAM accesses in parallel is called Memory Level Parallelism
(MLP)

%As a result, the processor tolerates long
%memory latency by generating prefetch requests through pre-execution of the
%memory-stalled application.

Large instruction windows
Runahead hpca03, micro05, isca05
MLP design
}


==> sec/tables/data_patt_pvalue.tex <==
\begin{table}[h]
  \small
  \centering
    %\setlength{\tabcolsep}{.65em}
    \begin{tabular}{crrr}
        \toprule
        %\multirow{2}{*}{Supply Voltage} & \multicolumn{3}{c}{\bf Vendor} \\
        Supply & \multicolumn{3}{c}{\bf Vendor} \\

         \cmidrule(lr){2-4}
        Voltage & \multicolumn{1}{c}{A} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{C} \\
        \midrule
        1.305  & --- & --- & --- \\
        1.250  & --- & --- & \textbf{0.000000} \\
        1.200   & --- & --- & 0.029947 \\
        1.175 & --- & --- & 0.856793 \\
        1.150  & --- & --- & 0.872205 \\
        1.125 & --- & 0.375906 & 0.897489 \\
        1.100 & \textbf{0.028592} & 0.375906 & \textbf{0.000000} \\
        1.075 & 0.103073 & 0.907960 & $\triangle$ \\
        1.050 & $\triangle$  & 0.651482 & $\triangle$ \\
        1.025 & $\triangle$  & \textbf{0.025167} & $\triangle$ \\
        \bottomrule
    \end{tabular}

  \caption{Calculated p-values from the BERs across three data patterns at each
    supply voltage level. A p-value less \fixIII{than} 0.05 indicates that the BER is
    statistically different across the three data patterns (indicated in bold). \fix{--- indicates
    that the BER is zero. \fixIV{$\triangle$ indicates that we cannot reliably access data from the DIMM}.}\vspace{-15pt}}
  \label{tab:pval}
\end{table}

%  VendorA
%  Voltage level: 1.075  F-value 2.391019 p-val 0.103073
%  Voltage level: 1.100  F-value 3.744221 p-val 0.028592
%  Voltage level: 1.125  F-value      nan p-val      nan
%  Voltage level: 1.150  F-value      nan p-val      nan
%  Voltage level: 1.175  F-value      nan p-val      nan
%  Voltage level: 1.200  F-value      nan p-val      nan
%  Voltage level: 1.250  F-value      nan p-val      nan
%  Voltage level: 1.350  F-value      nan p-val      nan
%  VendorB
%  Voltage level: 1.025  F-value 4.410440 p-val 0.025167
%  Voltage level: 1.050  F-value 0.432612 p-val 0.651482
%  Voltage level: 1.075  F-value 0.096762 p-val 0.907960
%  Voltage level: 1.100  F-value 1.000000 p-val 0.375906
%  Voltage level: 1.125  F-value 1.000000 p-val 0.375906
%  Voltage level: 1.150  F-value      nan p-val      nan
%  Voltage level: 1.175  F-value      nan p-val      nan
%  Voltage level: 1.200  F-value      nan p-val      nan
%  Voltage level: 1.250  F-value      nan p-val      nan
%  Voltage level: 1.350  F-value      nan p-val      nan
%  VendorC
%  Voltage level: 1.100  F-value 9005365.820037 p-val 0.
%  Voltage level: 1.125  F-value 0.108415 p-val 0.897489
%  Voltage level: 1.150  F-value 0.137147 p-val 0.872205
%  Voltage level: 1.175  F-value 0.155090 p-val 0.856793
%  Voltage level: 1.200  F-value 3.796615 p-val 0.029947
%  Voltage level: 1.250  F-value 115.070830 p-val 0.0000
%  Voltage level: 1.350  F-value      nan p-val      nan


==> sec/tables/dimm_table.tex <==
\begin{table}[h]
%\reftiny
  \centering
    \setlength{\tabcolsep}{.35em}
    %\begin{tabular}{ccccc}
    %    \toprule
    %    \multirow{2}{*}{Vendor} & Number & Timing (ns) &
    %    Assembly & \multirow{2}{*}{Capacity} \\
    %    & of Family & (tRCD/tRP/tRAS) & Year & \\
    %    \midrule
    %    A (10 DIMMs}) & 2 & 13.75/13.75/35 & 2015-16 & 2GB\\
    %    B (12 DIMMs) & 1 & 13.75/13.75/35 & 2014-15 & 2GB \\
    %    C (9 DIMMs) & 2 & 13.75/13.75/35 & 2015 & 2GB \\
    %    \bottomrule
    %\end{tabular}
    \begin{tabular}{cccc}
        \toprule
        \multirow{2}{*}{Vendor} & Total Number & Timing (ns) &
        Assembly  \\
        & of Chips & (\trcd/\trp/\tras) & Year  \\
        \midrule
        %A (10 DIMMs) & 2 & 13.75/13.75/35 & 2015-16\\
        %B (12 DIMMs) & 1 & 13.75/13.75/35 & 2014-15 \\
        %C (9 DIMMs) & 2 & 13.75/13.75/35 & 2015 \\
        A (10 DIMMs) & 40 & 13.75/13.75/35 & 2015-16\\
        B (12 DIMMs) & 48 & 13.75/13.75/35 & 2014-15 \\
        C (9 DIMMs) & 36 & 13.75/13.75/35 & 2015 \\
        \bottomrule
    \end{tabular}
  \caption{\fixIII{Main} properties of the tested DIMMs.}
  \label{tab:dimm_list}
\end{table}


==> sec/tables/ecc.tex <==
\begin{table}[h]
%\reftiny
  \centering
    \setlength{\tabcolsep}{.65em}
    \begin{tabular}{ccrrrrr}
        \toprule
        \multirow{2}{3em}{\centering Vendor} & \multirow{2}{5em}{\centering Correctable Timing} & \multicolumn{5}{c}{Voltage}  \\
        \cmidrule(lr){3-7}
        & & 1.05 & 1.075 & 1.1 & 1.125 & 1.15  \\
        \midrule
        \multirow{3}{3em}{\centering A \\ \tiny 10 DIMMs \quad}
         & tRCD & - & - & 1/1 & - & - \\
         & tRP & - & - & - & - & - \\

        \cmidrule(lr){1-7}
        \multirow{3}{3em}{\centering B \\ \tiny 12 DIMMs \quad}
         & tRCD & 2/5 & 3/5 & 1/1 & 0 & 0 \\
         & tRP & 2/5 & 6/7 & 2/5 & 0/1 & - \\

        \cmidrule(lr){1-7}
        \multirow{3}{3em}{\centering C \\ \tiny 9 DIMMs \qquad}
         & tRCD & 0 & 0 & 0 & 3/4 & 3/3 \\
         & tRP & - & - & 0/1 & 0/5 & 0/5 \\
        \bottomrule
    \end{tabular}

  \caption{Performance results of memory non-intensive workloads with different
  \varr values.}
  \label{tab:non_mem_intensive_results}
\end{table}


==> sec/tables/module_legend.tex <==
\begin{tabular}{l}
\small
{$\,$} \\

{$\ast$ The manufacturing date in the format of year-week
(yy-ww). For example, 15-01 indicates that the DIMM was manufactured during}\\
{the first week of 2015.} \\

{$\,$} \vspace{-7pt}\\

$\dagger$ The timing factors associated with each DIMM:\\
\hspace{0.1in}$Freq$: the channel frequency\\
\hspace{0.1in}$tRCD$: the minimum required latency for an \act to complete \\
\hspace{0.1in}$tRP$: the minimum required latency for a \pre to complete \\
\hspace{0.1in}$tRAS$: the minimum required latency for to restore the charge in an activated row of cells \\

{$\,$} \vspace{-7pt}\\

{$\ddagger$ The maximum DRAM module size supported by our testing platform is 2GB.} \\

{$\,$} \vspace{-7pt}\\

{$\star$ The number of DRAM chips mounted on each DRAM module. }\\

{$\,$} \vspace{-7pt}\\

{$\S$ The DRAM die versions that are marked on the chip package. } \\

{$\,$} \vspace{-7pt}\\

${\circ}$ The \emph{minimum voltage level} that allows error-free \changes{operation}, as
described in \ssecref{volt_sensitivity}.

{$\,$} \\

\end{tabular}


==> sec/tables/modules.tex <==
\definecolor{lightgray}{gray}{0.95}

\begin{table}[h]

\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{1pt}
\centering
\scriptsize
%\footnotesize

\begin{tabular}{ccccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \scriptsize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \scriptsize \centering Module} &
                     {\em \scriptsize \centering Date$^{\ast}$} &
\multicolumn{4}{c}{\em \scriptsize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \scriptsize \centering Organization} &
\multicolumn{4}{c}{\em \scriptsize \centering Chip}
%& \multicolumn{2}{c}{\em \scriptsize \centering Timing}
\\

\cmidrule(lr){3-3} \cmidrule(lr){4-7} \cmidrule(lr){8-9} \cmidrule(lr){10-13}

 &
 & {\em \scriptsize (yy-ww)}
 & {\em \scriptsize Freq~(MT/s)}
 & {\em \scriptsize tRCD (ns)}
 & {\em \scriptsize tRP (ns)}
 & {\em \scriptsize tRAS (ns)}
 & {\em \scriptsize Size (GB)$^{\ddagger}$}
 & {\em \scriptsize Chips$^{\star}$}
 & {\em \scriptsize Size (Gb)}
 & {\em \scriptsize Pins}
 & {\em \scriptsize Die Version$^{\S}$}
 & {\em \scriptsize \fix{V\textsubscript{min}} (V)$^{\circ}$}
 \\

\midrule

%['crucialb41', 'crucialb42''micronb48',
%'micronb49', 'micronb50', 'micronb51', 'micronb52', 'micronb55', 'micronb56',
%'micronb57'
%'samsungo8', 'samsungo9', 'samsungo10', 'samsungo11', 'samsungo12', 'samsungo13',
%'samsungo14', 'samsungo15', 'samsungo16', 'samsungo17', 'samsungo18', 'samsungo19', ]
%, 'hynixp64', 'hynixp65', 'hynixp66', 'hynixp67', 'hynixp69', 'hynixp71', 'hynixp73', 'hynixp74', 'hynixp75',


 & \module{A}{ 1}{} & 15-46 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{B}$ & 1.100 \\
 & \module{A}{ 2}{} & 15-47 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{B}$ & 1.125 \\
 & \module{A}{ 3}{} & 15-44 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{F}$ & 1.125 \\
 & \module{A}{ 4}{} & 16-01 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{F}$ & 1.125 \\
 & \module{A}{ 5}{} & 16-01 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{F}$ & 1.125 \\
 & \module{A}{ 6}{} & 16-10 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{F}$ & 1.125 \\
 & \module{A}{ 7}{} & 16-12 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{F}$ & 1.125 \\
 & \module{A}{ 8}{} & 16-09 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{F}$ & 1.125 \\
 & \module{A}{ 9}{} & 16-11 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{F}$ & 1.100 \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering
  Total of \\ \centering 10 DIMMs}
 & \module{A}{10}{} & 16-10 & 1600 & 13.75 & 13.75 & 35 & 2
& 4 & 4 & $\times$16  & $\mathcal{F}$ & 1.125 \\

\midrule

 & \module{B}{ 1}{} & 14-34 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.100 \\
 & \module{B}{ 2}{} & 14-34 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.150 \\
 & \module{B}{ 3}{} & 14-26 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.100 \\
 & \module{B}{ 4}{} & 14-30 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.100 \\
 & \module{B}{ 5}{} & 14-34 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.125 \\
 & \module{B}{ 6}{} & 14-32 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.125 \\
 & \module{B}{ 7}{} & 14-34 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.100 \\
 & \module{B}{ 8}{} & 14-30 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.125 \\
 & \module{B}{ 9}{} & 14-23 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.125 \\
 & \module{B}{10}{} & 14-21 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.125 \\
 & \module{B}{11}{} & 14-31 & 1600 & 13.75 & 13.75 & 35 & 2 &
4 & 4 & $\times$16  & $\mathcal{Q}$ & 1.100 \\
\multirow{-12}{5em}{\centering {\large\em B} \\ {\tiny \quad \\} \centering
  Total of \\ \centering 12 DIMMs}
 & \module{B}{12}{} & 15-08 & 1600 & 13.75 & 13.75 & 35  & 2 & 4 & 4 &
$\times$16  & $\mathcal{Q}$ & 1.100 \\

\midrule

 & \module{C}{ 1}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2 & 4 & 4 & $\times$16
& $\mathcal{A}$ & 1.300 \\
 & \module{C}{ 2}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2
& 4 & 4 & $\times$16 & $\mathcal{A}$ & 1.250 \\
 & \module{C}{ 3}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2
& 4 & 4 & $\times$16  & $\mathcal{A}$ & 1.150 \\
 & \module{C}{ 4}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2
& 4 & 4 & $\times$16  & $\mathcal{A}$ & 1.150 \\
 & \module{C}{ 5}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2
& 4 & 4 & $\times$16  & $\mathcal{C}$ & 1.300 \\
 & \module{C}{ 6}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2
& 4 & 4 & $\times$16  & $\mathcal{C}$ & 1.300 \\
 & \module{C}{ 7}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2
& 4 & 4 & $\times$16  & $\mathcal{C}$ & 1.300 \\
 & \module{C}{ 8}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2
& 4 & 4 & $\times$16  & $\mathcal{C}$ & 1.250 \\
\multirow{-9}{5em}{\centering {\large\em C} \\ {\tiny \quad \\} \centering
  Total of \\ \centering 9 DIMMs}
 & \module{C}{9}{} & 15-33 & 1600 & 13.75 & 13.75 & 35  & 2
& 4 & 4 & $\times$16  & $\mathcal{C}$ & 1.300 \\

\bottomrule
\end{tabular}

\input{sec/voltron_final/tables/module_legend}

%\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em A} (sorted by manufacturing date)}
\caption{Characteristics of the evaluated DDR3L DIMMs.}
\vspace{-35pt}
\label{tab:modules}
\end{table}


==> sec/tables/motivation_freq_scaling.tex <==
\begin{table}[h]
%\reftiny
  \centering
    \setlength{\tabcolsep}{.35em}
    \begin{tabular}{ccccc}
        \toprule
        Workload & Speedup & Bandwidth & DRAM Energy & System Energy \\
        \midrule
        \emph{mcf} & \textbf{-19\%} & -20\% & -11\% & -2\% \\
        \emph{perl} & -2\% & -2\% & \textbf{-30\%} & -2\% \\
        \bottomrule
    \end{tabular}
  \caption{Workload behavior when the channel frequency reduces by half from
    1600 MT/s to 800 MT/s.}
  \label{tab:motivation}
\end{table}


==> sec/tables/mwork.tex <==
\definecolor{lightgray}{gray}{0.95}

\begin{table*}[h]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing}
\\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\bottomrule
\end{tabular}
%\input{tbl/module_legend}
%\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em A} (sorted by manufacturing date)}
%\label{tbl:vendor1}
\end{table*}

\ignore{
\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering \mycolorii{Vulnerability Ratio}$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule

%% MICRON
\cellcolor{white} & \module{B}{ 1}{} & 10-09 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 2}{} & 10-22 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 3}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 4}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 5}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 6}{} & 11-26 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 7}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.1  & --   \\
\cellcolor{white} & \module{B}{ 8}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 479  & --   \\
\cellcolor{white} & \module{B}{ 9}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 1.9  & --   \\
\cellcolor{white} & \module{B}{10}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 4.3  & --   \\
\cellcolor{white} & \module{B}{11}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 161  & --   \\
\cellcolor{white} & \module{B}{12}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.3  & --   \\
\cellcolor{white} & \module{B}{13}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 16.0 & --   \\
\cellcolor{white} & \module{B}{14}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 8.6  & --   \\
\cellcolor{white} & \module{B}{15}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{B}{16}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{B}{17}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{18}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{19}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{20}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{21}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 4.3  & 11.4 \\
\cellcolor{white} & \module{B}{22}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 472  & --   \\
\cellcolor{white} & \module{B}{23}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 279  & --   \\
\cellcolor{white} & \module{B}{24}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 3276 & --   \\
\cellcolor{white} & \module{B}{25}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{B}{26}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{B}{27}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{28}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 78.3 & 8.2  \\
\cellcolor{white} & \module{B}{29}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 23.4 & 5.8  \\
\multirow{-32}{5em}{\centering {\large\em B} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{B}{30}{} & 14-09 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\bottomrule
\end{tabular}

\input{tbl/module_legend}

\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em B} (sorted by manufacturing date)}
\label{tbl:vendor2}
\end{table*}


\newpage

\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering \mycolor{Vulnerability Ratio}$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule


%% SAMSUNG
\cellcolor{white} & \module{C}{ 1}{} & 08-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 2}{} & 09-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{E}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 3}{} & 10-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 4}{} & 11-16 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 5}{} & 11-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 6}{} & 11-25 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 7}{} & 11-37 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 2.6  \\
\cellcolor{white} & \module{C}{ 8}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 32.9 \\
\cellcolor{white} & \module{C}{ 9}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 42.3 \\
\cellcolor{white} & \module{C}{10}{} & 11-49 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{11}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 104  \\
\cellcolor{white} & \module{C}{12}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 117  \\
\cellcolor{white} & \module{C}{13}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 291  \\
\cellcolor{white} & \module{C}{14}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{15}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 97.0 \\
\cellcolor{white} & \module{C}{16}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 493  \\
\cellcolor{white} & \module{C}{17}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 61.8 \\
\cellcolor{white} & \module{C}{18}{} & 12-25 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.2  & 3.3  \\
\cellcolor{white} & \module{C}{19}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 473  & 3.1  \\
\cellcolor{white} & \module{C}{20}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 5.4  & 2.7  \\
\cellcolor{white} & \module{C}{21}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 3.5  & 3.0  \\
\cellcolor{white} & \module{C}{22}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 545  & 3.0  \\
\cellcolor{white} & \module{C}{23}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.7  & 3.0  \\
\cellcolor{white} & \module{C}{24}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 27.2 & 2.9  \\
\cellcolor{white} & \module{C}{25}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.3  \\
\cellcolor{white} & \module{C}{26}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 54.2 & 19.1 \\
\cellcolor{white} & \module{C}{27}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.1  \\
\cellcolor{white} & \module{C}{28}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 29.0 & 5.4  \\
\cellcolor{white} & \module{C}{29}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 120  & 6.7  \\
\cellcolor{white} & \module{C}{30}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 196  & 3.2  \\
\cellcolor{white} & \module{C}{31}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 599  & 8.5  \\
\cellcolor{white} & \module{C}{32}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 51.6 & --   \\
\cellcolor{white} & \module{C}{33}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.5  \\
\cellcolor{white} & \module{C}{34}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.6  \\
\cellcolor{white} & \module{C}{35}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.6  \\
\multirow{-38}{5em}{\centering {\large\em C} \\ {\tiny \quad \\} \centering Total of \\ \centering 36 DIMMs}
\cellcolor{white} & \module{C}{36}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.9  \\
\bottomrule
\end{tabular}

\input{tbl/module_legend}

\caption{Sample Population of 36 DDR3 DIMMs from Vendor {\em C} (sorted by manufacturing date)}
\label{tbl:vendor3}

\end{table*}
}


==> sec/tables/non_mem_intensive.tex <==
\begin{table}[h]
%\scriptsize
%\reftiny
  \centering
    \setlength{\tabcolsep}{.45em}
    \begin{tabular}{crrrrr}
        \toprule
        \textbf{\varr} & 1.3V & 1.2V & 1.1V & 1.0V & 0.9V  \\
        \midrule
        %System Performance Loss (\%) & 0.6 & 2 & 4 & 8 & 17 \\
        %DRAM Energy Savings (\%) & 3 & 8 & 12 & 15 & 14 \\
        %System Energy Savings (\%) & 1 & 3 & 4 & 5 & 3\\

        \textbf{System Performance Loss} (\%) & 0.5 & 1.4 & 3.5 & 7.1 & 14.2 \\
        \textbf{DRAM Power Savings} (\%) & 3.4 & 10.4 & 16.5 & 22.7 & 29.0 \\
        %\textbf{DRAM Energy Savings} (\%) & 2.8 & 8.7 & 12.9 & 16.0 & 16.3 \\
        % V 0.90  val 29.04 |  V 1.00  val 22.65 |  V 1.10  val 16.50 |  V 1.20
        % val 10.36 |  V 1.30  val  3.36
        \textbf{System Energy Savings} (\%) & 0.8 & 2.5 & 3.5 & 4.0 & 2.9 \\

        \bottomrule
    \end{tabular}

  \caption{System performance loss and energy savings due to array voltage
    scaling for \fix{non-memory-intensive} workloads.}
  \label{tab:non_mem_intensive_results}
\end{table}


==> sec/tables/sys_config_table.tex <==
\begin{table}[h]
  \renewcommand{\arraystretch}{0.9}
  %\scriptsize
  %\small
  %\reftiny
  \centering
    \setlength{\tabcolsep}{.6em}
    \begin{tabular}{ll}
        \toprule
        \multirow{2}{*}{Processor} & 4 ARM Cortex-A9 cores~\cite{arma9}, 2GHz, \\
        & 192-entry instruction window \\
        \midrule
        Cache & L1: 64KB/core, L2: 512KB/core, L3: 2MB shared \\
        \midrule
        Memory & \multirow{2}{*}{64/64-entry read/write request queue,
            FR-FCFS~\cite{rixner-isca2000,zuravleff-patent}} \\
        Controller & \\
        \midrule
        \multirow{2}{*}{DRAM} & DDR3L-1600~\cite{jedec-ddr3l}\\
        & 2 channels (1 rank and 8 banks per channel) \\
        \bottomrule
    \end{tabular}
  \caption{Evaluated system configuration.}
  \label{tab:sys-config}
\end{table}


==> sec/tables/test.tex <==
%\reftiny


==> sec/tables/varr_latency.tex <==
\begin{table}[h]
  %\renewcommand{\arraystretch}{0.8}
  %\small
  %\reftiny
  \centering
    \setlength{\tabcolsep}{.5em}
    \begin{tabular}{ll|ll}
        \toprule
        \varr & tRCD - tRP - tRAS (ns) & \varr & tRCD - tRP - tRAS (ns) \\
        \midrule
        %\cmidrule(lr){1-2}
        %\cmidrule(lr){3-4}

        1.35 & 13.75 - 13.75 - 36.25 &  1.10 & 15.00 - 16.25 - 40.00 \\
        1.30 & 13.75 - 13.75 - 36.25 &  1.05 & 16.25 - 17.50 - 41.25 \\
        1.25 & 13.75 - 15.00 - 36.25 &  1.00 & 17.50 - 18.75 - 45.00 \\
        1.20 & 13.75 - 15.00 - 37.50 &  0.95 & 18.75 - 21.25 - 48.75 \\
        1.15 & 15.00 - 15.00 - 37.50 &  0.90 & 21.25 - 26.25 - 52.50 \\
        \bottomrule
    \end{tabular}
  \caption{DRAM latency \fixIV{required for correct operation} for each evaluated \varr.}
  \label{tab:varr_latency}
\end{table}


==> sec/tables/workload_list.tex <==
\begin{table}[h]
  \renewcommand{\arraystretch}{0.92}
  \centering
    \setlength{\tabcolsep}{.3em}
    %\begin{tabular}{clclcl}
    %    \toprule
    %    Number & Name & Number & Name & Number & Name\\
    %    \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}
    %    0 & YCSB-a & 9 & calculix & 18 & milc \\
    %    1 & YCSB-b & 10 & gamess & 19 & namd \\
    %    2 & YCSB-c & 11 & gcc & 20 & omnetpp \\
    %    3 & YCSB-d & 12 & GemsFDTD & 21 & perlbench \\
    %    4 & YCSB-e & 13 & gobmk & 22 & povray \\
    %    5 & astar & 14 & h264ref & 23 & sjeng \\
    %    6 & bwaves & 15 & hmmer & 24 & soplex \\
    %    7 & bzip2 & 16 & libquantum & 25 & sphinx3 \\
    %    8 & cactusADM & 17 & mcf & 26 & zeusmp \\
    %    \bottomrule
    %\end{tabular}
    \footnotesize
    \begin{tabular}{clrc|clrc|clr}
        \toprule
        Number & Name & \fixV{L3} MPKI & & Number & Name & L3 MPKI & & Number & Name & L3 MPKI\\
        %\cmidrule(lr){1-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9}
        %\cmidrule(lr){1-3} \cmidrule(lr){5-7} \cmidrule(lr){9-11}
        \midrule
        0 & YCSB-a    & 6.66 & & 9  & calculix    & 0.01  & & 18 & milc     & 27.91 \\
        1 & YCSB-b    & 5.95 & & 10 & gamess      & 0.01  & & 19 & namd     & 2.76 \\
        2 & YCSB-c    & 5.74 & & 11 & gcc         & 3.20  & & 20 & omnetpp  & 27.87\\
        3 & YCSB-d    & 5.30 & & 12 & GemsFDTD    & 39.17 & & 21 & perlbench& 0.95 \\
        4 & YCSB-e    & 6.07 & & 13 & gobmk       & 3.94  & & 22 & povray   & 0.01 \\
        5 & astar     & 3.43 & & 14 & h264ref     & 2.14  & & 23 & sjeng    & 0.73 \\
        6 & bwaves    & 19.97& & 15 & hmmer       & 6.33  & & 24 & soplex   & 64.98\\
        7 & bzip2     & 8.23 & & 16 & libquantum  & 37.95 & & 25 & sphinx3  & 13.59\\
        8 & cactusADM & 6.79 & & 17 & mcf         & 123.65& & 26 & zeusmp   & 4.88 \\
        \bottomrule
    \end{tabular}

  \caption{Evaluated benchmarks with their \fixIII{respective} L3 MPKI values.}
  \label{tab:workload_list}
\end{table}


==> sec/voltron_final/abstract.tex <==
% !TEX root=../paper.tex

The energy consumption of DRAM is a critical concern in modern computing
systems. Improvements in manufacturing process technology have allowed DRAM
vendors to lower the DRAM supply voltage conservatively, which reduces some of
the DRAM energy consumption. We would like to reduce the DRAM supply voltage
more aggressively, to further reduce energy. Aggressive supply
voltage reduction requires a thorough understanding of the effect voltage
scaling has on DRAM access latency and DRAM reliability.

In this paper, we take a comprehensive approach to understanding and exploiting
the latency and reliability characteristics of modern DRAM when the supply
voltage is lowered below the \fixII{nominal voltage level} specified by
\fixIV{DRAM standards}. Using an FPGA-based testing platform, we perform an
experimental study of 124 real DDR3L (low-voltage) DRAM chips manufactured
recently by three major DRAM vendors. We find that reducing the supply voltage
below a certain point introduces bit errors in the data, and we comprehensively
characterize the behavior of these errors. We discover that these errors can be
avoided by increasing the latency of three major DRAM operations (activation,
restoration, and precharge). \fixII{We perform} detailed DRAM circuit
simulations to validate and explain our experimental findings. We also
characterize the various relationships between reduced supply voltage and error
locations, stored data patterns, DRAM temperature, and data retention.

Based on our observations, we propose a new DRAM energy reduction mechanism,
called \emph{Voltron}. The key idea of Voltron is to use a performance model to
determine \fix{by} how much we can reduce the supply voltage without introducing errors
and without exceeding a user-specified threshold for performance loss. Our
evaluations show that Voltron reduces the average DRAM and system energy
consumption by 10.5\% and 7.3\%, respectively, while limiting the average system
performance loss to only 1.8\%, for a variety of \fix{memory-intensive} quad-core
workloads. We also show that Voltron significantly outperforms prior dynamic
voltage and frequency scaling mechanisms for DRAM.


==> sec/voltron_final/background_motivation.tex <==
% !TEX root=../paper.tex

\section{Background and Motivation}
\label{sec:background}

In this section, we first provide necessary DRAM background and terminology. We then
discuss related work on reducing the voltage and/or frequency of DRAM, to motivate
the need for our study.

\subsection{DRAM Organization}
\label{ssec:dram_org}

\figref{dram-organization} shows a high-level overview of \fixII{a modern}
memory system organization. A processor (CPU) is connected to a DRAM module via
a \emph{memory channel}, which is a bus used to transfer data and commands
between the processor and DRAM. A DRAM module is also called a \emph{dual
  in-line memory module} (\fixII{DIMM}) and it consists of multiple \emph{DRAM
  chips}, which are controlled together\fixIV{.\footnote{\fixIV{In this paper, we
study DIMMs that contain a single \emph{rank} (i.e., a group of chips in a
single DIMM that operate in lockstep).}}} \changes{Within each DRAM chip,
  illustrated in \figref{chip-organization}, we categorize the internal
  components into two broad categories: \myitem{i} the \emph{DRAM array}, which
  consists of multiple banks of DRAM cells organized into rows and columns, and
  \myitem{ii} \emph{peripheral circuitry}, which consists of the circuits that
  sit outside of the DRAM array. For a more detailed view of the components in a
  DRAM chip, we refer the reader to prior
  work\fixII{s}\fixIV{~\cite{vogelsang-micro2010, kim-isca2012, lee-hpca2013,
      liu-isca2012, lee-hpca2015, hassan-hpca2016, chang2016low,
      chang-thesis2017, lee-thesis2016, kim-thesis2015, lee-sigmetrics2017,
      chang-sigmetrics2016,lee-pact2015,seshadri-micro2013,seshadri-arxiv2016,lee-arxiv2016,chang-hpca2014,seshadri-thesis2016,seshadri-micro2015}}.}

%\figputHS{DRAM}{1.0}{DRAM system and chip organization.}
%\vspace{-0.1in}
\input{sections/subplots/background}
%\vspace{-0.05in}

\ignore{\fixIV{The DRAM array in each DRAM chip} is divided into multiple banks
  (typically eight \fixIV{in DDR3 DRAM~\cite{jedec-ddr3l, jedec-ddr3}}).
  \fixIV{Because the chips are controlled together, the arrays from each
    chip behave as if they are a single larger array.  Thus, each bank spans across
    all of the chips in the module. }
}

A DRAM array is divided into multiple banks (typically eight \fixIV{in DDR3
DRAM~\cite{jedec-ddr3l, jedec-ddr3}}) that can process DRAM commands
independently from each other to increase parallelism. A bank \fixIV{contains} a
2-dimensional array of DRAM cells. Each cell uses a capacitor to store \fixIV{a
  single bit} of data. Each array of cells is connected to a row of sense
amplifiers via vertical wires, called \emph{bitlines}. \fixII{This} row of sense
amplifiers \fixII{is called the} \emph{row buffer}. The row buffer senses the
data stored in one row of DRAM cells and serves as a temporary buffer for the
data. A typical row \fixIV{in a DRAM module (i.e., across all of the DRAM chips
  in the module)} is 8KB wide, comprising 128 \fixIV{64-byte} cache lines.

%A modern DRAM chip consists of a large number of cell arrays (e.g., 1K for
%a 4Gb chip), as the number of arrays grows with higher DRAM chip capacity. Each DRAM
%cell uses a capacitor to store 1~bit of data. Each array is attached to a \emph{row
%buffer} that consists of sense amplifiers. The row buffer senses the data
%stored in one row of DRAM cells from the cell array, and serves as a temporary buffer
%for the data.  A typical row is 8KB wide, comprising 128~cache lines.

The peripheral circuitry has three major components. First, the I/O component is
used to receive commands or transfer data between the DRAM \fixIV{chip} and the
processor via the memory channel. Second, a typical DRAM chip uses a delay-lock
loop (DLL) to synchronize its data signal with the external clock to coordinate
data transfers on the memory channel.
%since a DRAM chip's clock is supplied from an external system clock, Note that
%certain DRAM architectures (e.g., LPDDR) do not integrate the DLL within the
%chip~\cite{malladi-isca2012, yoon-isca2012}.
Third, the control logic decodes DRAM commands sent across the memory channel
and selects the row \fixIV{and column} of cells to read data from or write data into.

\subsection{Accessing Data in DRAM}
\label{ssec:access_data}

To access data stored in DRAM, \fixII{the} \emph{memory controller} (shown in
\figref{dram-organization}) issues DRAM commands across the memory channel
to the DRAM chips. Reading a cache line from DRAM requires three essential
commands, as shown in \figref{background_timeline}: \act, \crd, and \pre.
Each command requires some time to complete, and the DRAM
\fixII{standard}~\cite{jedec-ddr3l} define\fixII{s} the latency of the commands
\fixII{with} a set of \emph{timing parameters}. The memory controller can be
programmed to obey different sets of timing parameters through the
BIOS~\cite{intel-xmp, lee-hpca2015, amd-bkdg, amd-opteron}.

\figputHS{background_timeline}{0.9}{DRAM commands and timing parameters
when reading one cache line of data.}

\paratitle{Activate Command} To open the target row of data in the bank
that contains the desired cache line, the memory controller first
\fixII{issues} an \act command \fixII{to the target DRAM bank}. During
activation, the electrical charge stored in the target row starts to
propagate to the row buffer. The charge propagation triggers the row buffer
to latch the data stored in the row after some amount of time. The latency
of an \act command, or the \fixII{\emph{activation latency}}, is defined as
the minimum amount of time \fixII{that is required to pass} from the issue
time of an \act until the issue time of a column command (i.e., \crd or
\cwr). The timing parameter for the activation latency is called \trcd, as
shown in \figref{background_timeline}, and is typically set to 13ns in
DDR3L~\cite{micronDDR3L_2Gb}.

Since an activation drains charge from the target row's cells to latch
\fixII{the cells'} data into the row buffer, the \fixII{cells'} charge needs to
be restored to prevent data loss. The row buffer performs \emph{charge
restoration} simultaneously with activation. Once the cells' charge is
fully restored, the row can be closed \fixII{(and thus the DRAM array be
prepared for the next access)} by \fixII{issuing} a \pre command \fixII{to the
DRAM bank}. The DRAM standard specifies the restoration latency as the
minimum amount of time the controller must wait after \act before issuing
\pre. The timing parameter for restoration is called \tras, as shown in
\figref{background_timeline}, and is typically set to 35ns in
DDR3L~\cite{micronDDR3L_2Gb}.

\paratitle{Read Command} Once the row data is latched in the row buffer after
the \act command, the memory controller \fixII{issues} a \crd command. The row
buffer contains multiple cache lines of data (8KB), and the \crd command enables
\fixIV{all $n$ DRAM chips in the} DRAM module to select the desired cache line
(64B) from the row buffer. \fixIV{Each DRAM chip on the module then drives
  \fixV{($\sfrac{1}{n}$)\textsuperscript{th}} of the cache line from the row buffer to
  the I/O component within the peripheral circuitry.}
%The entire module then drives \fixII{a portion of the cache line} from the row
%buffer to the I/O component within the peripheral circuitry \fixII{of every
%DRAM chip in the module}.
The peripheral circuitry \fixII{of each chip} then sends \fixIV{its
  \fixV{($\sfrac{1}{n}$)\textsuperscript{th}} of the cache line} across the memory
channel to the memory controller. \response{Note that the column access time to
  read and write the cache line is defined by the timing parameters \tcl and
  \tcwl, respectively, \fixII{as shown in \figref{background_timeline}}. Unlike
  the activation latency (\trcd),  \tcl and \tcwl are
  \fixIV{\emph{DRAM-internal}} timings that are determined by a clock inside
  DRAM~\cite{micronDDR3L_2Gb}. Therefore, our \fix{FPGA-based} experimental
  \fixIII{infrastructure} (described in \secref{fpga}) \emph{cannot} evaluate
  the effect of changing \tcl and \tcwl.}

\paratitle{Precharge Command} After reading the data from the row buffer,
the memory controller may contain a request that needs to access data from
a \emph{different} row within the same bank.  To prepare \fixII{the bank to service
this request}, the memory controller \fixII{issues} a \pre command \fixII{to
the bank}, which closes the currently-activated row and resets the bank
\fixII{in preparation} for the next \act command. Because closing the
activated row and resetting the bank takes some time, the standard
specifies the precharge latency as the minimum amount of time the
controller must wait \fixII{for} after \fixII{issuing} \pre before \fixII{it
issues an} \act. The timing parameter for precharge is called \trp, as
shown in \figref{background_timeline}, and is typically set to 13ns in
DDR3L~\cite{micronDDR3L_2Gb}.

% Another important aspect of the timing parameters (latencies) is that they are
% determined by the elapsed time from issuing one DRAM command until the
% subsequent command. Since the memory controller is responsible for scheduling
% and issuing DRAM commands, memory controller has the flexibility to adjust the
% DRAM access latency of activation, restoration, and precharge in any number of
% DRAM cycles even if the resulting latency can cause incorrect operations in
% DRAM.\footnote{Many today's processors allow the users to adjust the timing
%   parameters through BIOS albeit the adjustable values are bounded within
%   certain range.} In today's systems, a controller maintains a set of timing
% parameters specified by the DRAM vendors and they take a fixed amount of time
% for every DRAM cell.

\changes{
    \subsection{Effect of DRAM Voltage and Frequency on Power
    \fixII{Consumption}}
\label{sec:dram_power}

DRAM power \fixII{is divided} into dynamic and static power. \fixII{Dynamic}
power \fixII{is} the power consumed by executing the access commands: \act,
\pre, and \crd/\cwr. \fixIV{Each} \act and \pre consumes \fixIV{power in the
  DRAM array and the peripheral circuitry due to the activity in the DRAM
  array and control logic.} \fixII{Each} \crd/\cwr consumes power in the DRAM
array by accessing data in the row buffer, and in the peripheral circuitry by
driving data on the channel. On the other hand, static power \fixII{is} the
power that is consumed \emph{regardless} of the DRAM accesses, and it is mainly
due to transistor leakage. DRAM power is governed by both the supply voltage and
\fixII{operating clock} frequency: $Power \propto Voltage^2 \times
Frequency$~\cite{david-icac2011}. As shown in \fixIV{this} equation, power consumption
scales quadratically with supply voltage, and linearly with frequency.

DRAM supply voltage is distributed to both the DRAM array and the
peripheral circuitry through \fixII{respective} power pins on the
%($V_{DD}$ and $V_{DDQ}$, respectively)
DRAM chip, \fixII{dedicated separately to the DRAM array and the peripheral
circuitry}. We call the voltage supplied to the DRAM array, \varr, and the
voltage supplied to the peripheral circuitry, \vperi. Each DRAM standard
requires a specific nominal supply voltage value, which depends on many
factors, such as the architectural design and process technology. In this
work, we focus on the widely used DDR3L DRAM design that requires a nominal
supply voltage of 1.35V~\cite{jedec-ddr3l}. To remain operational when the
\fixII{supply} voltage is unstable, DRAM can tolerate a small amount of
\fixIV{deviation from the nominal supply}
voltage. In particular, DDR3L DRAM \fixII{is specified to} operate
with a supply voltage ranging from 1.283V to 1.45V~\cite{micronDDR3L_2Gb}.

%Modern DDR DRAM chips are \emph{synchronous} state machines, driven by an
%external clock signal from the memory controller. This allows the memory
%controller to have timing control on when to send commands to or receive data
%from DRAM.
The DRAM \fixII{channel} frequency value of a DDR DRAM chip is typically
specified \fixIV{using the} \emph{channel data rate}, measured in mega-transfers per second
(MT/s). The size of each data transfer is dependent on the width of the data
bus, which ranges from 4 to 16~bits for a DDR3L chip~\cite{micronDDR3L_2Gb}.
Since a modern DDR channel transfers data on both the positive and \fixII{the}
negative clock edge\fixII{s (hence the term \emph{double data rate}, or DDR)},
the channel frequency \fixII{is} \emph{half of the data rate}. For example, a
DDR data rate of 1600 MT/s means that the frequency \fixII{is} 800 MHz. To run
the channel at a specified data rate, the peripheral circuitry requires a
certain minimum voltage (\vperi) for stable operation. As a result, the supply
voltage scales directly \fixIV{(i.e., linearly)} with DRAM frequency, and it
determines the maximum operating
frequency~\cite{deng-asplos2011,david-icac2011}.

\ignore{
  % Detailed on frequency
Modern DDR DRAM chips are \emph{synchronous} state machines, driven by an
external clock signal from the memory controller. This allows the memory
controller to have timing control on when to send commands to or receive data
from DRAM. The DRAM frequency value of a DDR DRAM chip is typically specified in
channel data rate, measured in mega-transfers per second (MT/s). The size of
each data transfer is dependent on the width of the data bus, which ranges from
4 to 16 bits for a DDR3L chip~\cite{micronDDR3L_2Gb}. Since a modern DDR channel
transfers data on both the positive and negative clock edge, the channel
frequency operates at half of the data rate. For example, a DDR data rate of
1600 MT/s means that the channel operates at 800 MHz.\footnote{\reftiny Note that
  several prior works (imprecisely) use MT/s and MHz interchangeably to discuss
  channel frequency.} A DRAM chip typically supports several frequency values
(e.g., 1066, 1333, 1600 MT/s) that can be chosen by the processor only during the
system boot time. The DRAM frequency not only affects the data throughput, but
also the DRAM power. Except for the dynamic power of \act and \pre, which are
\emph{asynchronous operations}, the remaining DRAM power scales \emph{linearly} with
frequency: $Power \propto Frequency$.
}
}

\subsection{Memory Voltage and Frequency Scaling}
\label{ssec:dvfs}

\ignore{The memory system has become a major energy consumer in modern computing
systems, consuming 40\% of the total system energy in
servers~\cite{hoelzle-book2009,ibmpower7-hpca}, and 40\% of the total system
power in GPUs~\cite{paul-isca2015}).}

One \fixII{proposed} approach to reducing memory energy consumption is to scale
the voltage and/or the frequency of DRAM based on the \fixIV{observed memory
  channel} utilization. We briefly describe two different ways of scaling
frequency and/or voltage below.

%This approach is motivated by voltage and frequency scaling within CPUs, which
%is widely used by today's systems to reduce CPU energy consumption at the cost
%of a modest performance loss~\cite{intel-speedstep, amd-powernow,
%ibmpower7-hpca}.

%One approach to reduce memory energy consumption is to scale the voltage and/or
%frequency of DRAM. This approach is motivated by voltage and frequency scaling
%within CPUs, which is widely used by today's systems to reduce CPU energy
%consumption at the cost of a moderate performance loss~\cite{intel-speedstep,
%amd-powernow, ibm-power7}. The effectiveness of voltage and/or frequency
%scaling is governed by the dynamic power consumption (P): $P \propto Voltage^2
%\times Frequency$. Thus, power scales quadratically with supply voltage, and
%linearly with frequency.


\paratitle{Frequency Scaling} To \fix{enable the power reduction} \fixII{that
comes with reduced} \fixIV{DRAM} frequency, prior works propose to apply
\emph{dynamic frequency scaling} (DFS) by adjusting the DRAM \fixIV{channel}
frequency based on \fixIV{the} memory bandwidth demand \fixIV{from the DRAM
  channel}~\cite{deng-asplos2011,deng-islped2012,deng-micro2012, paul-isca2015,
  begum-iiswc2015,sundriyal2016}. A major \fixIV{consequence of} lowering the
frequency is the \fixII{likely} performance loss that occurs, as it takes a
longer time to transfer data across the DRAM channel \fixIV{while operating at a
  lower frequency}. The clocking logic within the peripheral circuitry requires
a \emph{fixed number of DRAM cycles} to transfer the data, \fixII{since} DRAM
sends data on each edge of the clock cycle. For a 64-bit memory channel with a
64B~cache line size, the transfer typically takes four DRAM
cycles~\cite{jedec-ddr3}. Since \fixII{lowering} the frequency increases the
time required for each cycle, the total amount of time spent on data transfer,
in nanoseconds, increases accordingly. As a result, \fix{not only does memory
  latency increase, but} \fixIII{also} memory \fix{data} throughput decreases,
\fixII{making} DFS \fixII{undesirable to use} when the running workload's memory
bandwidth \fixII{demand} \fixIV{or memory latency sensitivity} is high. The
extra transfer \fix{latency from DRAM} can also cause longer queuing times for
requests waiting at the memory controller\fixIII{~\cite{lee-tech2010,
    ipek-isca08,
    kim-rtas2014,subramanian-iccd2014,subramanian-tpds2016,kim-rts2016}},
further exacerbating the performance loss \fixII{and potentially delaying
  latency-critical applications}~\cite{deng-asplos2011,david-icac2011}.

% Note that decreasing the channel frequency reduces the dynamic power of DRAM
% periphery and background (static) power, but not the dynamic power of arrays
% because array operations (e.g., \act) are not dependent on channel
% frequency~\cite{micron-tr}. Therefore, in contrast to the fixed cycle time for
% data transfers, changing the frequency does not affect the \emph{wall-clock time
%   (ns) of timing parameters}, since their clock cycles actually decrease with
% slower frequency. For example, halving a DDR3L DIMM's channel frequency from
% 2133 MT/s to 1066 MT/s also halves the \act latency from 14 cycles to 7 cycles,
% but the wall-clock time of an \act remains the same at
% 13ns~\cite{micronDDR3L_2Gb}.

\paratitle{Voltage and Frequency Scaling} While decreasing the channel
frequency \fixII{reduces} the peripheral circuitry power and static power, it
does \fix{\emph{not}} affect the dynamic power consumed by the operations performed on
the DRAM array (i.e., activation, restoration, precharge). This is because
\fixII{DRAM array operations} are asynchronous\fix{, i.e., independent of}
the channel frequency~\cite{micron-tr}. As a result, these operations
require a fixed \fixIII{time (in nanoseconds)} to complete.  For example, the
activation latency in a DDR3L DRAM module \fixII{is} 13ns, regardless of the DRAM
frequency~\cite{micronDDR3L_2Gb}.  If the channel frequency is \fixII{doubled
from 1066~MT/s to 2133~MT/s}, the memory controller \fixII{doubles} the
number of cycles for the \act timing parameter (i.e., \trcd) (from 7~cycles
to 14~cycles), to maintain the 13ns latency.

%While decreasing the channel frequency reduces the peripheral circuitry and
%background power, it does not affect the dynamic power consumed by the cell
%arrays. This is because the operations performed on the cell array (i.e.,
%activation, restoration, precharge) behave according to RC circuit behavior, and
%are not dependent on the channel frequency~\cite{micron-tr}.  As a result, these
%operations require a fixed number of nanoseconds to complete.  For example, the
%activation latency in a DDR3L module takes 13ns, regardless of the channel
%frequency~\cite{micronDDR3L_2Gb}.  If the channel frequency is halved from
%2133~MT/s to 1066~MT/s, the memory controller cuts the number of cycles for the
%\act timing parameter (i.e., \trcd) in half (from 14~cycles to 7~cycles), to
%maintain the 13ns latency.

\changes{ In order to reduce the dynamic power consumption of the DRAM
array as well, prior work \fixII{proposes} \emph{dynamic voltage and
frequency scaling} (DVFS) for DRAM, which reduces the supply voltage along
with the \fixII{channel} frequency~\cite{david-icac2011}. This mechanism
selects a DRAM frequency based on the current memory bandwidth utilization
and finds the \emph{minimum operating voltage} (\vmin) for that frequency.
\vmin is defined to be the lowest voltage that still provides ``stable
operation'' for DRAM (i.e., no errors occur within the data). There are two
significant limitations for this proposed DRAM DVFS mechanism. The first
limitation is due to a lack of understanding of how voltage scaling affects
the DRAM behavior. No prior work \fixIV{provides} experimental characterization
or analysis of \fixII{the effect of} reducing \fixIV{the DRAM supply} voltage \fixII{on latency,
reliability, and data retention} in real DRAM chips. As the DRAM behavior \fix{under reduced-voltage operation}
is unknown \fixII{to \fix{satisfactorily} maintain the latency and reliability of DRAM}, the
\fixII{proposed DVFS} mechanism~\cite{david-icac2011} can reduce \fixII{supply}
voltage only \emph{very conservatively}. The second limitation is that this
prior work
\fixII{reduces the
supply} voltage only when it \fixII{reduces the channel frequency, since
a lower channel frequency requires a lower supply voltage for stable operation.}
%requires \fixII{reducing the channel} frequency to \fixII{reduce
%supply} voltage since a given channel frequency
%lower  minimum operating voltage redues
As a result, \fixII{DRAM} DVFS results in the same
performance issues experienced by \fixII{the DRAM} DFS mechanisms. In
\ssecref{pavc_eval}, we evaluate \fixII{the main} prior
work~\cite{david-icac2011} on memory DVFS to quantitatively demonstrate its
\fixII{benefits and limitations}.}

% To further reduce DRAM power consumption, one prior work
% shows that DRAM's voltage can be reduced along with lower
% frequency~\cite{david-icac2011}. It finds a minimum voltage for ``stable
% operations'' at a fixed frequency and it does not change the timing parameters.
% Unfortunately, there is a lack of information on how voltage scaling affects the
% DRAM characteristics and what constitutes a ``stable operation'' under a voltage
% level.

\changes{ \subsection{Our Goal} The goal of this work is to \myitem{i}
\fixII{experimentally} characterize and analyze \emph{real modern DRAM chips} operating at different
supply voltage levels, \fixII{in order to develop a solid and thorough
understanding of how \fix{reduced-voltage} operation affects latency,
reliability, and data retention in DRAM;} and \myitem{ii} develop a mechanism that can reduce DRAM
energy consumption \fix{by reducing DRAM voltage,} without having to sacrifice
memory \fixII{data} throughput,
\fixII{based on the insights obtained from \fixIV{comprehensive} experimental}
characterization. Understanding how DRAM characteristics change at different
voltage levels is imperative not only for enabling memory DVFS in real systems,
but also for developing other low-power \fixII{and low-energy} DRAM designs that can effectively reduce
the DRAM voltage. We \fixII{experimentally analyze} the \fixII{effect} of
reducing \fixII{supply} voltage \fixII{of modern} DRAM chips
in \secref{dram_exp}, and \fixII{introduce} our \fixII{proposed new} mechanism \fixII{for
reducing DRAM energy} in \secref{varray}. }


==> sec/voltron_final/cell_ops <==
\section{DRAM Cell Operation}
\label{dram_cell_op}

In this section, we explain the how the DRAM cell and its state change during
the three fundamental operations: activation, restoration, and precharge
(see \ssecref{access_data}).
\figref{dram_curve} shows the bitline voltage level during these operations with
\vdd set to 1.35V. An \act command and a \pre command are issued at 0ns and 50ns,
respectively. To further help understand the operations, we use
\figref{dram_state} to describe the state of the cell, bitline, and sense
amplifier during the same time frame as \figref{dram_curve}. A bitline is used
to connect a cell with its sense amplifier (in the row buffer) for data
accesses. Accessing data in a DRAM cell consists of four major steps:

\begin{figure}[!h]
    \centering
   \subcaptionbox{DRAM bitline voltage.\label{fig:dram_curve}}
    {
        \includegraphics[scale=0.8]{plots/dram_curve}
    }
    %
    \subcaptionbox{DRAM state.\label{fig:dram_state}}
    {
        \includegraphics[scale=0.8]{plots/dram_state}
    }
    \caption{DRAM phases during a DRAM access.}
\end{figure}

\paratitle{Precharge} Initially, each cell in the DRAM is in a charged
state (for data value 1) or a discharged state (for data value 0) at 0ns ($T0$). The
amount of filled gray color represents the amount of charge in the cell. In our
shown example, we assume the cell is fully charged, storing a data value of 1.
The bitline voltage is maintained at a voltage of $\frac{1}{2}$\vdd.

\paratitle{Charge Sharing} An \act command connects a row of cells to their
bitlines. This triggers the charge stored in the cells to start flowing to the
bitlines (or the other way around, depending on the initial charge level in the
cell) via a process called \emph{charge sharing} (at time $T1$). In our example,
the cell is initially charged. Hence, it perturbs the bitline's voltage from
$\frac{1}{2}$\vdd to $\frac{1}{2}$\vdd$+\delta$ by a small amount of charge
($\delta$).

\paratitle{Sensing and Amplification} After the charge sharing phase, the
sense amplifier senses the voltage perturbation on the bitline towards either
\vdd or 0. Following the same direction, it starts to amplify the bitline
voltage by injecting more charge into the bitline and the cell. When
the bitline voltage surpasses 75\% of \vdd (at time $T2$), the binary data becomes latched in
the sense amplifier, thus ensuring that the correct data can be read by a \crd
command. These two phases are also known as the activation phase. The activation
latency is the time elapsed from $T0$ to $T2$, which is defined as \trcd.

\paratitle{Restoration} After the row is activated and each sense
amplifier latches in the binary data of its cell, the DRAM starts to restore the
connected cell's charge back to its original fully-charged state (at time $T3$).
This phase is known as restoration, and its latency (from $T0$ to $T3$) is
defined as \tras.

To activate a different row of cells within the same array of the activated row,
the memory controller sends a \pre command to disconnect the cells from the
bitline. Then, the sense amplifier brings the bitline back to $\frac{1}{2}$\vdd
(at time $T4$). The precharge latency is defined at \trp, from the issue time of
\pre (50ns) to $T4$.




==> sec/voltron_final/conclusion.tex <==
% !TEX root=../paper.tex

%\vspace{-0.1in}
\section{Conclusion}

\changes{ This paper provides the first experimental study that comprehensively
characterizes and analyzes the behavior of DRAM chips when the supply voltage is
reduced below its nominal value. We demonstrate, \fixIV{using 124 DDR3L DRAM
  chips}, that the \fix{DRAM} supply voltage can be reliably reduced to a
certain level, beyond which errors arise within the data. We then experimentally
demonstrate the relationship between the supply voltage and the latency of the
fundamental DRAM operations (activation, restoration, and precharge). \fixIV{We
  show that bit errors caused by reduced-voltage operation can be eliminated by
  increasing the latency of the three fundamental DRAM operations.} By
\fix{changing} the memory controller configuration to allow for the longer
latency of these operations, we can thus \emph{further} lower the supply voltage
without inducing errors in the data. We also \fixIV{experimentally} characterize
the relationship between reduced supply voltage and error locations, stored data
patterns, temperature, and data retention.

%In addition, we investigate the spatial distribution of bit errors when the
%supply voltage is lowered, and study the impact of a reduced supply voltage on
%retention time.

Based on these observations, we propose and evaluate \voltron, a low-cost energy
reduction mechanism that reduces DRAM energy \emph{without} \fix{affecting}
memory data throughput. \voltron reduces the supply voltage for \emph{only} the
DRAM array, while maintaining the nominal voltage for the peripheral circuitry
to continue operating the memory channel at a high frequency. \voltron uses a
new piecewise linear performance model to find the array supply voltage that
maximizes the system energy reduction within a given performance loss target.
\fix{Our experimental evaluations across a wide variety of workloads}
demonstrate that \voltron significantly reduces system energy \fix{consumption}
with only \fix{very} modest performance loss.

We conclude that it is very promising to understand and exploit reduced-voltage
operation in modern DRAM chips. We hope that the experimental characterization,
analysis, and optimization techniques presented in this paper will enable the
development of other new mechanisms that can effectively \fixIII{exploit the
trade-offs between voltage, reliability, and latency in DRAM to improve system
performance, efficiency, and/or reliability.}}


==> sec/voltron_final/experimental_methodology.tex <==
% !TEX root=../paper.tex

\section{Experimental Methodology}
\label{sec:fpga}

To study the behavior of real DRAM chips under \fixII{reduced} voltage, we build
an FPGA-based infrastructure based on SoftMC~\cite{hassan-hpca2017}, which
allows us to have precise control over the DRAM modules. This method was used in
many previous works\fixIII{~\cite{jung-memsys2016, jung-patmos2016,
    kim-isca2014, chang-sigmetrics2016, khan-sigmetrics2014,
    khan-dsn2016,hassan-hpca2017,lee-sigmetrics2017,mathew-rapido2017,
    lee-hpca2015, qureshi-dsn2015, khan2016case, lee-thesis2016,
    chang-thesis2017, kim-thesis2015, liu-isca2013}} as an effective way to
explore different DRAM characteristics (e.g., latency, reliability, \fixVI{and}
\fixIV{data retention time}) that have not been known or exposed to the public
by DRAM manufacturers. Our testing platform consists of a Xilinx ML605 FPGA
board and a host PC that communicates with the FPGA via a PCIe bus
(\figref{fpga}). We adjust the supply voltage to the DRAM by using a USB
interface adapter~\cite{ti-usb} that enables us to tune the power rail connected
to the DRAM module directly. The power rail is connected to all the power pins
of every chip on the module (as shown in Appendix~\ref{sec:pin_layout}).

\figputHS{fpga}{0.5}{FPGA-based DRAM testing platform.}

\paratitle{Characterized DRAM Modules} In total, we tested 31 DRAM DIMMs,
comprising \fix{of} 124 DDR3L (low-voltage) chips, from the three \fixII{major}
DRAM chip vendors that hold more than 90\% of the DRAM market
share~\cite{bauer-mckinsey2016}.  Each chip has a 4Gb density. Thus,
\fixII{each} of our DIMMs \fixII{has} a 2GB capacity. The DIMMs support up to a
1600 MT/s channel frequency. Due to \fixII{our} FPGA's maximum operating
frequency limitations, all of our tests are conducted at 800 MT/s.  Note that
the experiments we perform \fixII{do \emph{not} require us to adjust} the
channel frequency. \tabref{dimm_list} describes the relevant information about
\fixIV{the} tested DIMMs. \fixIV{Appendix~\ref{sec:dimm_info} provides
  detailed information on each DIMM}. Unless otherwise specified, we test our
DIMMs at an ambient temperature of 20$\pm$1\celsius. We examine the effects of
high \fixIV{ambient} temperature \fixIV{(i.e., 70$\pm1\celsius$)} in
Section~\ref{ssec:temperature}.

%For vendor A
%and C, we tested DIMMs with two distinct models. A DIMM model contains certain
%information on the process technology and array design used in the chips.

% \vspace{-0.05in}
\input{sections/tables/dimm_table}
% \vspace{-0.1in}

\paratitle{DRAM Tests} \label{ssec:dramtest} At a high level, we develop a test
(Test~\ref{test}) that writes/reads data to\fixII{/from} \emph{every} row in the
\emph{entire} DIMM, \fixIV{for a given supply voltage}. The test takes in
several different input parameters: activation latency (\trcd), precharge
latency (\trp), and data pattern. The goal of the test is to examine if any
errors occur under \fixIV{the given supply voltage with} the different input
parameters.
%Test~\ref{test} shows the test pseudocode.

%\vspace{-0.05in}
\input{sections/algos/test}
%\vspace{-0.05in}

In the test, we iteratively test two consecutive rows at a time. The two rows
hold data that are the inverse of each other (i.e., $\mathit{data}$ and
$\overline{\mathit{data}}$). Reducing \trp lowers the amount of time the
precharge unit has to reset the bitline voltage from either \vddbl (bit value 1)
or \vddzero (bit value 0) to \vddblhalf. If \trp were reduced too much, the
bitlines would float at some other intermediate voltage value between \vddblhalf
and \emph{full/zero voltage}. As a result, the next activation can potentially
start before the bitlines are fully precharged. If we were to use the same data
pattern in both rows, the sense amplifier would require \emph{less} time to
sense the value during the next activation, as the bitline is already
\emph{biased} \fixII{toward} those values. By using the \emph{inverse} of
\fixII{the data pattern in} the row \fixII{that is} precharged for the next row
\fixII{that is} activated, we ensure that the partially-precharged state of the
bitlines does \emph{not} unfairly favor the \fix{access to the} next
row~\cite{chang-sigmetrics2016}.
% This ensures that when we reduce \trp, the partially-precharged state from one
% row will not favor the data pattern in the next row to be
% activated~\cite{chang-sigmetrics2016}.
In total, we use three different groups of data patterns for our test: (0x00,
0xff), (0xaa, 0x33), and (0xcc, 0x55). Each specifies the $\mathit{data}$ and
$\overline{\mathit{data}}$, placed in consecutive rows in the same bank.

\ignore{
\noindent\textbf{Voltage and Latency Adjustments.} Since our hypothesis is that
latency needs to increase as supply voltage reduces to prevent errors in the
data. We start by testing our DIMMs under the nominal voltage of 1.35V and
decrement the voltage by a step of 0.05V (50mV). We keep decrementing the
voltage until we can no longer find any latency values that can access data
without any errors. The DIMM at that voltage cannot be reliably accessed likely
due to I/O signaling issues, rather than the internal array.

Under each voltage step, we first run the VoltageTest (Test~\ref{test} shown
above) using the nominal latency values. If we can correctly access all data
without any errors (line 8 in Test~\ref{test}), we repeat the same test with a
\emph{decremented tRCD} value. If no errors are shown, we run the test with a
\emph{decremented tRP} value. We repeat this process until we hit a latency
value pairs that result in errors. If the nominal latency result with errors to
begin with, we reverse the process by \emph{incrementing} the latencies until we
find the latencies that do not exhibit any errors. Due to the clock frequency
limitation of our FPGA board, we can only adjust the latency at a granularity of
2.5ns. Although this granularity covers an 18\% latency range of the nominal
latency, it is able to help us to find a potential range of where the latency
lies at voltage reduces, as we will show in the later section. To fill in the
2.5ns gap, we will show how we approximate the latency values at a continuous
range of voltage by developing a DRAM SPICE model based on the experimental
results (\ssecref{spice}).

In summary, we run at least 30 rounds of our test under each latency pair and
voltage level for each DIMM, summing up to more than 64800 rounds of tests
across all 31 DIMMs. To facilitate future research we will release our
infrastructure source code and experimental data for all tested DRAM chips.
}


==> sec/voltron_final/experimental_results.tex <==
% !TEX root=../paper.tex

\section{Characterization of DRAM Under Reduced Voltage}
\label{sec:dram_exp}

In this section, we present our major observations from our detailed
experimental characterization of 31 commodity DIMMs \changes{(124 chips)} from
three vendors, when \changes{the DIMMs} operate under \fix{reduced} supply
voltage (i.e., below the nominal voltage level specified by \fixIV{the DRAM
  standard}).
First, we analyze the reliability of DRAM chips as we reduce the \changes{supply}
voltage without changing the DRAM access latency (\ssecref{volt_sensitivity}).
Our experiments \changes{are designed} to identify if lowering \changes{the
  supply} voltage induces bit errors (i.e., \emph{bit flips}) in data.
\fix{Second}, we present our findings on the effect of increasing the activation
and precharge latencies for DRAM operating under \fixIV{reduced} supply voltage
(\ssecref{low_volt_latency}). The purpose of this experiment is to understand
the trade-off between access latencies (which \fix{impact} performance) and the
supply voltage of DRAM \fixIII{(which impacts energy consumption)}. We use detailed circuit-level DRAM simulations to
validate \changes{and explain} our observations on the relationship between
access latency and supply voltage. \fix{Third}, we examine the spatial locality
of errors \changes{induced due to reduced-voltage operation} (\ssecref{spatial})
and the distribution of errors in the data sent across the memory channel
(\ssecref{ecc}).  \fix{Fourth}, we study the effect of temperature on
\changes{reduced}-voltage operation (\ssecref{temperature}). \fix{Fifth}, we
study \fix{the effect of reduced voltage on the} data retention times within
DRAM (\ssecref{refresh}). We present a summary of our findings in
\ssecref{char_summary}.

\subsection{DRAM Reliability as Supply Voltage Decreases}
\label{ssec:volt_sensitivity}

We first study the reliability of DRAM chips under low voltage, which was not
studied by prior works on DRAM voltage scaling
\fix{(e.g.,~\cite{david-icac2011}).} For these experiments, we use the minimum
activation and precharge latencies that we experimentally determine to be
reliable (i.e., they do not induce any errors) under the nominal voltage of
1.35V \changes{at 20$\pm$1$\celsius$ temperature}. As shown in \fix{prior
  works~\cite{chang-sigmetrics2016, lee-hpca2015, chandrasekar-date2014,
    lee-sigmetrics2017, hassan-hpca2017, chang-thesis2017, lee-thesis2016,
liu-isca2012, agrawal-hpca2014, qureshi-dsn2015,
venkatesan-hpca2006,bhati-isca2015,lin-iccd2012,ohsawa-islped1998,
patel-isca2017, khan-sigmetrics2014, khan-dsn2016, khan2016case}},
\changes{DRAM} manufacturers adopt a pessimistic standard latency that
\fix{incorporates} a large margin as a \fix{safeguard to ensure that each chip
  \fixIII{deployed in the field} operates correctly under a wide range of
  conditions.  Examples of these conditions include process variation, which
  causes some chips or some cells within a chip to be slower than others, or
  high operating temperatures, which can affect the time required to perform
  various operations within DRAM.}
% provision against worst-case scenarios, such as process variation that causes
% some production chips or \fix{some cells to be slower than others and}
% \fix{worst-case operations conditions (e.g., highest allowed temperature by
% the standard).}
Since our goal is to understand how the inherent DRAM latencies vary with
voltage, we \fixIII{conduct} our experiments \emph{without} such an excessive
margin. We identify that the reliable \trcd and \trp latencies are
\changes{both} 10ns (instead of \fix{the 13.75ns latency} specified by the
\fix{DRAM} standard) at \fix{20$\celsius$}, which agree with the values reported
by prior work on DRAM latency characterization\fix{~\cite{chang-sigmetrics2016,
    lee-hpca2015, chang-thesis2017, lee-thesis2016}}.

Using the \fix{\emph{reliable minimum latency values} (i.e., 10ns for all of the
DIMMs),} we run Test~\ref{test}, which accesses every bit within a DIMM at the
granularity of a 64B cache line. In total, there are 32~million cache lines in a \fix{2GB}
DIMM. We vary the supply voltage from the nominal voltage of 1.35V down to
1.20V, using a step size of 0.05V (50mV). Then, we change to a smaller step \fix{size} of
0.025V (25mV), until we reach the lowest voltage \fix{at which} the DIMM can
\fix{operate reliably (i.e., without any errors) while employing the reliable minimum latency values.}
%tolerate \fix{by eliminating all the errors with high latency values.} without
%generating at least a single bit error even under
\fix{(We examine methods to further reduce the \fixIII{supply} voltage in
  \ssecref{low_volt_latency}.)} For each voltage step, we run 30~rounds of
Test~\ref{test} for each DIMM.  \figref{dimm_errors_all} shows the fraction of
cache lines that \changes{experience} at least 1~bit of error (i.e., 1~bit flip)
in each DIMM \changes{(represented by each curve)}, \fixIV{categorized based
  on vendor.}

%\figputHW{dimm_errors_all}{Fraction of erroneous cache lines in each DIMM as
\figputHS{dimm_errors_all}{0.8}{The fraction of erroneous cache lines in each DIMM as
we reduce the supply voltage, with a fixed access latency.}

We make three observations. First, when each DIMM runs below a certain voltage
level, errors start occurring. We refer to the \emph{minimum voltage level} of
each DIMM that allows error-free \changes{operation} as \vmin. For example, most
DIMMs from Vendor~C have $V_{min}=1.30V$.
%
\changes{Below \vmin, we observe errors because the fundamental DRAM array
operations (i.e., activation, restoration, precharge) \emph{cannot} fully
complete within the time interval specified by the latency parameters (e.g.,
\trcd, \tras) at low voltage.}
%We explain below \changes{(in \emph{Source of Errors} subtopic)} why errors
%occur when we reduce the voltage beyond \vmin.
%
Second, not all cache lines exhibit errors for all supply voltage values below
\vmin. Instead, the number of erroneous cache lines \changes{for each DIMM}
increases as we reduce the voltage further below \vmin. Specifically, Vendor A's
DIMMs \fix{experience a} near-exponential increase \fix{in} errors as \fix{the} supply voltage reduces
below \vmin. This is mainly due to the \emph{manufacturing process and
  architectural variation}, which introduces strength and size variation across
the different DRAM cells within a chip\fixIII{~\cite{kim-edl2009, li11,
    chang-sigmetrics2016, lee-sigmetrics2017, lee-hpca2015,
    chandrasekar-date2014, lee-thesis2016, kim-thesis2015, chang-thesis2017}}. \changes{Third, variation in \vmin exists not only
  across DIMMs from different vendors, but also across DIMMs from the same
  vendor.} However, the variation across DIMMs \fix{from} the same vendor is
much smaller compared to cross-vendor variation, since the fabrication process
and circuit designs can differ drastically across vendors. These results
demonstrate that reducing voltage beyond \vmin, without altering the access
latency, has a negative impact on \fix{DRAM} reliability.

% by causing more erroneous cache lines with lower voltage.

We also conduct an analysis of \fixIII{storing different \emph{data patterns}} on the error rate
\fixIII{during reduced-voltage operation} (see Appendix~\ref{sec:datapatt}).  In summary, our results show that the data
pattern does \emph{not} \changes{have a} consistent effect on the rate of errors
induced by reduced-voltage operation. For most supply voltage values, the data
pattern does \emph{not} have a statistically significant effect on the error
rate.

\paratitle{Source of Errors} To understand why errors occur in data as the
supply voltage \fixIV{reduces} below \vmin, we \changes{perform} circuit-level SPICE
simulations~\cite{nagel-spice,massobrio1993semiconductor}, which reveal more
detail on how the cell arrays operate. \fix{We develop a} SPICE model of the DRAM array \fix{that} uses a
sense amplifier design from prior work~\cite{baker-dram} with the \SI{45}{\nano\meter}
transistor model from the Predictive Technology Model (PTM)~\cite{ptm,
  zhao-isqed2006}. \fix{Appendix~\ref{spice_model} provides a detailed description of our SPICE
simulation model, which we have open-sourced~\cite{volt-github}.}

We vary the supply voltage of the DRAM array (\vdd) \fix{in our SPICE simulations} from
1.35V to 0.90V.
\figref{spice_act+pre_v3} shows the bitline voltage during activation and
precharge for different \vdd values. Times 0ns and 50ns correspond to when the
DRAM receives the \act and the \pre commands, respectively. An \act causes the
bitline voltage to increase from \vddhalf to \vdd in order to sense the stored
data value of ``1''. A \pre resets the bitline voltage back to \vddhalf in order
\fix{to enable the issuing of a later}
\act to another row within the same bank. In the figure, we mark the
points where the bitline reaches \fix{the} \circled{1} \emph{ready-to-access} voltage,
which we assume to be 75\% of \vdd; \circled{2} \emph{ready-to-precharge}
voltage, which we assume to be 98\% of \vdd; and \circled{3}
\emph{ready-to-activate} voltage, which we assume to be within 2\% of \vddhalf.
These points \fix{represent the minimum \trcd, \tras, and \trp values, respectively,}
required for reliable DRAM operation.
%For readers who wish to understand more detail on how bitline voltage
%\changes{changes under different} DRAM operations, we refer them to
%Appendix~\ref{dram_cell_op}, where we \changes{explain how the bitline voltage
%changes during the three DRAM operations}.
For readers who wish to understand \fix{the bitline voltage behavior in more detail,}
%  on how bitline voltage \changes{changes under different} DRAM operations,
\fix{we refer them to recent
works~\cite{lee-hpca2015,lee-hpca2013,hassan-hpca2016, lee-sigmetrics2017, lee-thesis2016} that provide
extensive background on how the bitline voltage changes during the three DRAM
operations.}

% To understand why errors occur in data as voltage reduces, we turn to DRAM
% circuit-level SPICE simulations, which reveal more details on how internal DRAM
% arrays operate. Our SPICE model uses a sense amplifier design from prior
% work~\cite{baker-dram} and we use the 45nm transistor model from Predictive
% Technology Model (PTM)~\cite{ptm, zhao-isqed2006}. \figref{spice_act+pre_v2}
% shows the bitline voltage during the activation and precharge phase from 1.35V
% to 0.9V. Times 0ns and 50ns correspond to when the DRAM receives the \act and
% the \pre command, respectively. We mark the activation latency (\trcd),
% restoration latency (\tras), and precharge latency (\trp) for each voltage
% value. For readers who wish to understand more details on how bitline voltage
% behaves during DRAM operations, we refer them to Appendix~\ref{dram_cell_op},
% where we provide further explanation.

%\figputHW{dram_error_spice}{Effect of reduced-voltage on DRAM activation,
%restoration, and precharge.} The major observation is that the bitline voltage
%increases at different rate depending on the voltage, thus affecting the
%latency of DRAM operations. When the nominal voltage (1.35V) is used, the time
%(\trcd) it takes for the sense amplifier to drive the bitline to the
%ready-to-access voltage (75\% of voltage) is shorter compared to 1.0V. With
%lower \vdd, the sense amplifier requires more time to reach the 75\% threshold,
%increasing activation latency. Similarly, the time (\tras) that is needed to
%restore the cell (to 98\% \varr) and the time (\trp) for the bitline to reset
%back to \varrhalf increase with lower \vdd at 1.0V.

\figputHS{spice_act+pre_v3}{1}{Effect of reduced array supply
voltage on activation, restoration, and precharge, from SPICE simulations.}

We make two observations from our SPICE simulations. First, we observe that the
bitline voltage during activation increases at a different rate depending on the
\changes{supply} voltage \fix{of} the DRAM array (\vdd). \changes{Thus},
\fix{the} \changes{supply voltage affects} the latency of the three DRAM
operations (activation, restoration, and precharge). When the nominal voltage
level (1.35V) is used \fix{for \vdd}, the time (\trcd) it takes for the sense
amplifier to drive the bitline to the \emph{ready-to-access voltage
  \changes{level}} (75\% of \vdd) is much shorter than the time \fix{to do so at
  a} lower \vdd. As \vdd decreases, the sense amplifier needs more time to latch
in the data, increasing the activation latency. \ignore{Similarly, the
  \changes{restoration latency} (\tras)\changes{, i.e., the} time needed to
  restore the cell to 98\% \changes{of} \vdd and the \changes{precharge latency}
  (\trp), \changes{i.e, the time} for the bitline to reset back to \vddhalf
  increase as \vdd decreases.} Similarly, the \changes{restoration latency}
(\tras) and the \changes{precharge latency} (\trp) increase as \vdd decreases.

Second, the latencies of the three fundamental DRAM array operations (i.e.,
activation, restoration, precharge) \changes{do} \emph{not} correlate with the
channel (or clock) frequency \fixIV{(not shown in \figref{spice_act+pre_v3})}. This is
because these operations are clock-independent \changes{asynchronous} operations
that are a function of the cell capacitance, bitline capacitance, and
\vdd~\cite{keeth-dram-tutorial}.\fix{\footnote{\fix{In
      Appendix~\ref{spice_model}, we show a detailed circuit schematic of a DRAM
      array that operates asynchronously\fixIII{, which forms the basis of our
        SPICE circuit simulation model~\cite{volt-github}}.}}} As a result, the
channel frequency is \emph{independent} of the three fundamental \changes{DRAM}
operations.

Therefore, we hypothesize that DRAM errors occur at lower supply voltages
because the \fix{three} DRAM \fix{array} operations have insufficient latency to
fully complete \fix{at lower voltage levels}. In the next section, we
\changes{experimentally} investigate the effect of increasing latency values as
we vary the supply voltage \changes{on real DRAM chips}.

\subsection{Longer Access Latency Mitigates Voltage-Induced Errors}
\label{ssec:low_volt_latency}

% separate subsections
%To confirm our hypothesis from \ssecref{volt_sensitivity} that a lower
%supply voltage requires a longer access latency \changes{for reliable DRAM
%operation, we first perform experiments on real DIMMs. Next, based on the
%results of our experiments, we build a DRAM SPICE circuit to simulate the
%DRAM reliability for DRAM timing parameters and supply voltages at finer
%granularity than our experimental platform provides. We generalize our SPICE
%simulation results by deriving a mathematical expression to model the
%latency required to reliably access DRAM under different supply voltages.}
%
%\subsubsection{Experimental Evaluation of the DRAM Reliability at Low Voltage}
%\label{sssec:exp_eval}

To confirm our hypothesis from \ssecref{volt_sensitivity} that a lower supply
voltage requires a longer access latency, we test our DIMMs at supply voltages
below the nominal voltage (1.35V) while incrementally increasing the activation
and precharge latencies \changes{to be} as high as 20ns (2x higher than the
tested latency in \ssecref{volt_sensitivity}). At each supply voltage value, we
call the minimum required activation and precharge latencies that do \emph{not}
exhibit any errors \trcdmin and \trpmin, respectively.

\figref{fpga_latency_range} shows the distribution of \trcdmin (top row) and
\trpmin (bottom row) measured for all DIMMs across three vendors as we vary the
supply voltage. Each circle represents a \trcdmin or \trpmin value. A circle's
size indicates the DIMM population size, with bigger circles representing more
DIMMs. The number above each circle indicates the fraction of DIMMs that work
reliably at the specified voltage and latency. Also, we
% plot a boundary using dashed lines with semi-transparent color filled between
% them. The boundary represents
shade the range of potential \trcdmin and \trpmin values. Since our
infrastructure can adjust the latencies at a granularity of
2.5ns, a \trcdmin or \trpmin value of 10ns is only an approximation of the
minimum value, as the precise \trcdmin or \trpmin falls between 7.5ns and 10ns.
We make three major observations.

\input{sections/subplots/min_latency}

% Old
% \figref{fpga_latency_range} shows the distribution of \trcdmin (top row) and
% \trpmin (bottom row) for all DIMMs across three vendors as voltage varies. Each
% circle represents the measured \trcdmin or \trpmin. A circle's size indicates
% the population size, with bigger circle representing more DIMMs. In addition, we
% also plot a boundary using dashed lines with semi-transparent color filled
% between them. The boundary represents the range of potential \trcdmin and
% \trpmin values because our infrastructure can only adjust the latency at a
% granularity of 2.5ns. Therefore, a measured \trcdmin at 10ns is only an
% approximation since the precise \trcdmin can likely fall in between 7.5ns and
% 10ns. Our major observations are as follows.

First, when the supply voltage falls below \vmin\footnote{\fix{In
    \ssecref{volt_sensitivity}, we define \vmin as the minimum voltage level of
    each DIMM that allows error-free operation. \tabref{modules} in Appendix~\ref{sec:dimm_info}
shows the \vmin value we found for each DIMM.}},
% DIMMs from Vendors A, B, and C have \vmin
%     values of 1.125V, 1.15V, and 1.3V, respectively.}
the tested DIMMs show
that an increase of at least 2.5ns is needed for \trcdmin and \trpmin to read
data without errors. For example, some DIMMs require at least a 2.5ns increase
\fix{of} \trcdmin or \trpmin to read data without errors at 1.100V, 1.125V, and 1.25V
from \fix{Vendors}~A, B, and C, respectively. Since our testing platform can only
identify the minimum latency at a granularity of 2.5ns\fixIII{~\cite{hassan-hpca2017}}, we use circuit-level
simulations \fix{to obtain} a more precise latency measurement of \trcdmin and \trpmin
(\fix{which we describe} in the latter part of this section).

Second, DIMMs from different vendors \changes{exhibit} very different behavior
on how much \trcdmin and \trpmin need to increase for reliable operation as
supply voltage falls below \vmin. Compared to other vendors, many more of
Vendor~C's DIMMs require higher \trcdmin and \trpmin to operate at a lower \vdd.
This is particularly the case for the precharge latency, \fixIV{\trpmin}. For
instance, 60\% of Vendor~C's DIMMs require a \trpmin of 12.5ns to read data
without errors at 1.25V, whereas this increase is not necessary at all for
\fix{DIMMs from Vendor~A, which \emph{all} operate reliably at \fixIII{1.15V}.}
This reveals that different vendors may have different circuit architectures or
manufacturing process technologies, \fixIII{which lead to variations in} the
\fix{additional} latency required to compensate for a reduced \vdd in DIMMs.

% Old
%
% Second, DIMMs from different vendors shows very different behavior on the
% required increase of \trcdmin and \trpmin. Vendor C's DIMMs require a 2.5ns
% increase on \trcdmin and \trpmin at a voltage level higher than others. This is
% especially apparent for the precharge latency (\trpmin). More than half of the
% DIMMs require us to set the \trpmin to 12.5ns at 1.25V to prevent errors,
% whereas this increase is not required at all for Vendor A. This result suggests
% that different vendors have different circuit architectures or process
% technologies, causing the latency to vary between them.

Third, \changes{at very low supply voltages}, not all of the DIMMs have valid
\trcdmin and \trpmin values less than or equal to 20ns that \changes{enable
  error-free operation of the DIMM}. We see that the circle size gets smaller as
the \fixIV{supply} voltage reduces, indicating that the number of DIMMs
\fix{that can operate reliably (even at higher latency) reduces.} For example,
Vendor~A's DIMMs can no longer operate \changes{reliably (\fix{i.e.,}
  error-free)} when the voltage is below 1.1V.
% We determine that a DIMM does not have valid \trcdmin and \trpmin when using a
% value of 20ns still observes errors.
We tested a small subset of DIMMs with latencies of more than 50ns and found
that these very high latencies still do \emph{not} prevent errors from
occurring. We hypothesize that this is because of signal integrity issues on the
channel, causing bits to flip during data transfer at very low supply voltages.

\fix{We correlate our characterization results with} our SPICE simulation results
from \ssecref{volt_sensitivity}, demonstrating that there is a direct
relationship between supply voltage and access latency. This \fix{new
  observation on the trade-off between supply voltage and access latency} is not
discussed or \fix{demonstrated} in prior work \changes{on DRAM voltage
  scaling}~\cite{david-icac2011}, where the access latency (in nanoseconds)
remains \emph{fixed} when performing memory DVFS. \changes{In conclusion, we
  demonstrate both experimentally and in circuit simulations that increasing the
  access latency (i.e., \trcd and \trp) allows us to lower the supply voltage
  while still reliably accessing data without errors.}

% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! %
% SPICE model
\input{sections/spice}
% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! %

\subsection{Spatial Locality of Errors}
\label{ssec:spatial}

While reducing the supply voltage induces errors when the DRAM latency is not
long enough, we also show that not all DRAM locations experience errors at all
supply voltage levels. To understand the locality of the errors induced by a low
supply voltage, we show the probability of each DRAM row in a DIMM
\fix{experiencing} at least one bit of error across all experiments.
\response{We present results for two \fixIV{representative} DIMMs from two
  different vendors\fix{, as} the observations from these two DIMMs are similar
  to those we make \fixIV{for} the other tested DIMMs. Our results collected
  from \fix{each of the 31} DIMMs are publicly available~\cite{volt-github}.}

\figref{locality_C} shows the probability of each row \fix{experiencing} at
least a one-bit error due to reduced voltage in the two representative DIMMs.
For each DIMM, we choose the supply voltage when errors start appearing (i.e.,
the voltage \fix{level} one step below \vmin), and we do \emph{not} increase the
DRAM access latency \fixIV{(i.e., 10ns for both \trcd and \trp)}. The x-axis
and y-axis indicate the bank number and row number (in thousands), respectively.
Our tested DIMMs are divided into eight banks, and each bank consists of
32K~rows of cells.\footnote{Additional results showing the error locations at
  different voltage \fix{levels} are in Appendix~\ref{spatial}.}

\input{sections/subplots/loc}
%\vspace{-0.1in}

Our main observation is that errors tend to cluster at certain locations. For
our representative DIMMs, we see that errors tend to cluster at certain rows
across multiple banks for Vendor~B. On the contrary, Vendor~C's DIMMs exhibit
errors in certain banks but not in other banks. We hypothesize that the error
concentration can be a result of \myitem{i} manufacturing process variation,
resulting in less robust components at certain locations, as observed in
Vendor~B\fix{'s DIMMs}; or \myitem{ii} architectural design variations in the power delivery
network. However, it is hard to verify our hypotheses without knowing the
specifics of the DRAM circuit design, which is proprietary information that
varies across different DRAM models within and across vendors.

Another implication of the spatial concentration of errors under low voltage is
that \emph{only those regions with errors require a higher access latency to
  read or write data correctly}, whereas error-free regions can be accessed
reliably with the standard latency. \fix{In \ssecref{eval_el}, \fixIII{we
    discuss} and evaluate a technique that exploits this \fixIV{spatial}
  locality \fixV{of errors} to improve system performance.}

% === section ECC ===
\input{sections/ecc}

\subsection{Effect of Temperature}
\label{ssec:temperature}

Temperature is an important external factor that can affect the behavior of
DRAM\fixIII{~\cite{schroeder-sigmetrics2009,el-sayed-sigmetrics2012,
    liu-isca2013, khan-sigmetrics2014, lee-hpca2015, liu-isca2012, kim-isca2014,
    lee-thesis2016}}. Prior works have studied the impact of temperature on
reliability\fixIII{~\cite{schroeder-sigmetrics2009, el-sayed-sigmetrics2012,
    kim-isca2014,kim-thesis2015}},
latency\fixIII{~\cite{lee-hpca2015,chang-sigmetrics2016, chang-thesis2017,
    lee-thesis2016}}, and retention
time~\cite{khan-sigmetrics2014,liu-isca2013,liu-isca2012,qureshi-dsn2015} at the
nominal supply voltage. However, no prior work has studied \dhlfix{the effect of
  temperature on the latency \fix{at which DRAM operates reliably},} as the
supply voltage changes.

To reduce the test time, we test 13~representative DIMMs under a high ambient
temperature of 70$\celsius$ using a closed-loop temperature
controller~\cite{hassan-hpca2017}. \figref{temperature} shows \fix{the} \trcdmin
and \trpmin values of tested DIMMs, categorized by \fix{vendor, at} 20$\celsius$
and 70$\celsius$. \fix{The error bars indicate the minimum and maximum latency
  values across all \fixIII{DIMMs we} tested that are from the same vendor. We
  increase the horizontal spacing between the low and high temperature data
  points at each voltage level to improve readability.}

%\figputHW{temperature}{Effect of high temperature (70$\celsius$) on latency.}
\figputHS{temperature}{0.8}{Effect of high \fix{ambient} temperature (70$\celsius$) on minimum
  reliable operation latency at reduced voltage.}

We make two observations. First, temperature impacts vendors differently. On
Vendor~A's DIMMs, temperature does not have an observable impact on the
\dhlfix{reliable operation} latencies. \fix{Since our platform can test
  latencies with  a step size of only 2.5ns, it is possible that the effect of high
  temperature on the reliable minimum operating latency for Vendor~A's DIMMs
  may be within 2.5ns.}
%However, we cannot conclude that Vendor~A's DIMMs do not require a higher
%latency for reliability at a higher temperature, as our platform . Thus, it is
%likely that the high temperature's effect on latency is within 2.5ns.
On the other hand, the temperature effect on latency is measurable on DIMMs from
Vendors~B and C. DIMMs from Vendor~B are not strongly affected by temperature
when the supply voltage is above 1.15V. \fix{The precharge latency for
Vendor~C's DIMMs is affected by high temperature} at supply voltages of 1.35V and
1.30V, \fix{leading to an increase in the minimum} latency from 10ns to 12.5ns.
When the voltage is below 1.25V, the impact \fix{of high temperature on
precharge latency is} not observable, as the precharge
latency already needs to be raised by 2.5ns, to 12.5ns, at 20$\celsius$. Second,
the precharge latency is more sensitive to temperature than the activation
latency. Across all of our tested DIMMs, \trp increases \fix{with high
  temperature} under a greater number of supply voltage \fix{levels}, whereas
\trcd is less likely to be perturbed by temperature.

Since temperature can affect latency behavior under different voltage levels,
techniques that compensate for temperature changes can be used to dynamically
adjust the activation and precharge latencies, as proposed by prior
work~\cite{lee-hpca2015, lee-thesis2016}.

% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! %
\input{sections/refresh}
% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! %

\subsection{Summary}
\label{ssec:char_summary}

\changes{We have presented extensive characterization results and analyses on
DRAM chip \fix{latency, reliability, and data retention time} behavior under
various supply voltage levels. We summarize our findings in six key points.
First, DRAM reliability worsens \fixIV{(i.e., more errors start appearing)} as
we reduce the supply voltage below \vmin. Second, we discover that
voltage-induced errors occur mainly because, at low supply voltages, the DRAM
access latency is no longer sufficient to allow the fundamental DRAM operations
to complete. Third, via both experiments on real DRAM chips and SPICE
simulations, we show that increasing the latency of activation, restoration, and
precharge \fix{operations in DRAM} can mitigate errors under low supply voltage
levels until a certain voltage level. Fourth, we show that voltage-induced
errors \fixIV{exhibit} strong spatial locality \fixIV{in a DRAM chip},
clustering at certain locations \fixIV{(i.e., \fixV{certain} banks and rows)}. Fifth,
temperature affects the reliable access latency at low supply voltage levels
\fix{and the effect is very vendor-dependent}. Sixth, we find that reducing the
supply voltage does \emph{not} require increasing the standard DRAM refresh
\fix{rate} for reliable \fixIII{operation below 70$\celsius$}.}


==> sec/voltron_final/extended_voltron_eval.tex <==
% !TEX root=../paper.tex

% == Extension results ==
\ignore{
\subsection{Comparison to Memory DVFS}

In this section, we quantitatively compare Voltron against \textit{\memdvfs}, a
dynamic DRAM frequency and voltage scaling mechanism proposed by a prior
work~\cite{david-icac2011}, which we already described in \ssecref{dvfs}.
Similar to the configuration used in the prior work, we enable \memdvfs to
dynamically switch between three frequency steps: 1600, 1333, and 1066 MT/s,
which employ 1.35V, 1.3V, and 1.25V, respectively.

\figref{memdvfs} shows the system performance loss and system energy savings due
to \memdvfs and \voltron. Each metric (y-axis) is shown in a single plot that
uses boxplots to show the distribution among multiple workloads, which are
categorized into high and low memory intensity (x-axis). Each box demonstrates
the quartiles of the population and the whiskers indicate the minimum and
maximum value. The red dot on each box indicates the mean. We make several major
observations.

\input{sections/subplots/voltron_memdvfs}

First, for the \fix{memory-intensive} workloads, \memdvfs has almost zero effect on
system energy and performance. The reason is that \memdvfs avoids scaling DRAM
frequency when an application's memory bandwidth is above a fixed threshold
since reducing the frequency can result in a large performance loss due to lower
data throughput. As \fix{memory-intensive} applications have high memory bandwidth
consumption that is easily above the threshold, \memdvfs cannot perform
frequency and voltage scaling during most of the applications' runtime. These
results are consistent with that of reported in \memdvfs\cite{david-icac2011}. In
contrast, \voltron reduces system energy by 7.0\% on average for the \fix{memory-intensive}
workloads at the cost of 2.9\% system performance loss, which meets the
specified target of 5\%.

Second, both \memdvfs and \voltron reduce system energy consumption for low
memory-intensity workloads. By reducing the DRAM array voltage to a lower value
than \memdvfs, \voltron is able to provide slightly higher reduction. Third,
although \voltron reduces the system energy at a small performance loss, the
system energy efficiency, in terms of \emph{performance per watt}, still
improves by 7.4\% and 3.3\% for \fix{memory-intensive and non-memory-intensive} workloads,
respectively, on average over the baseline. We demonstrate that \voltron is a new
optimization technique that enables energy efficiency improvement not only on
non-memory-intensive applications, but also on memory-intensive workloads that
prior work cannot achieve.
}
%memdvfs: namd 64 in lowest setting 25 in normal

\response{
\subsection{Effect of Exploiting \fixIV{Spatial} Locality \fixV{of Errors}}
\label{ssec:eval_el}
In \ssecref{spatial}, our experimental results show that errors due to reduced
voltage concentrate in certain regions, specifically in select DRAM banks for some
vendors' DIMMs. This implies that when we lower the voltage, only the banks with errors require a higher
access latency to read or write data correctly, whereas error-free banks can
be accessed reliably with the standard latency. Therefore, in this section, we
enhance our \voltron mechanism by exploiting the spatial locality of
\fixIV{errors caused by reduced-voltage operations}. The key idea is to dynamically change the access latency \fixIII{on a
  per-bank basis (i.e., based on the
DRAM banks being accessed)} to account for the reliability of each bank.
% as certain banks do not require increased latency to
%access data reliably.
\fixIII{In other words, we would like to increase the latency only for banks
that would otherwise experience \emph{errors}, and do so just enough such that these banks operate
reliably.}

\fix{For our evaluation, we model the behavior based on a subset
  \fixIII{(three)} of Vendor C's DIMMs, which show that the number of banks with
  errors increases as we reduce the \fixIV{supply} voltage
  \fixIII{(\ssecref{spatial})}. We observe that these DIMMs start experiencing
  errors at 1.1V using the standard latency values. However, only one bank
  observes errors when we reduce the voltage level from 1.15V to 1.1V
  \fixIII{(i.e., 50mV reduction)}. We evaluate a \fixIV{conservative} model that
  increases the number of banks that need higher latency by one for every 50mV
  reduction from the nominal voltage of 1.35V. Note that this model is
  conservative, because we start increasing the latency when the voltage is
  reduced to 1.3V, which is much higher than the lowest voltage level (1.15V)
  for which we observe that DIMMs operate reliably without \fixIV{requiring} a
  latency increase. Based on this conservative model, we choose the banks
  \fixIV{whose latencies should} increase \emph{sequentially} starting from the
  first bank, while the remaining banks operate at the standard latency. For
  example, at 1.25V (100mV lower than the nominal voltage of 1.35V), \voltron
  needs to increase the latency for the first two out of the eight banks to
  ensure reliable \fixIII{operation}. }

%the number of banks that experiences errors decreases by one when the voltage
%drops by 50mV from 1.15V to 1.1V. Every 50mV reduction from the nominal voltage
%of 1.35V increases the number of banks that need higher latency by one. For
%example, at 1.3V and 1.2V, \voltron needs to increase the latency for one and
%three out of the eight banks, respectively.

\fix{\figref{voltron_bankloc} compares the system performance and energy
efficiency of our bank-error locality aware version of \voltron (denoted as
\emph{Voltron+BL}) to the previously-evaluated \voltron mechanism, which is not
aware of such locality.} \fix{By increasing the memory latency for only} a
subset of banks at each voltage step, Voltron+BL reduces the average performance
loss from 2.9\% to 1.8\% and \fix{increases} the average system energy savings
from 7.0\% to 7.3\% for \fix{memory-intensive} workloads, with similar
improvements for \fix{non-memory-intensive} workloads. We show that enhancing
\voltron by adding awareness of the spatial locality of errors can further
mitigate the latency penalty due to reduced voltage, \fixIV{even with \fixV{the}
  conservative bank error locality model we assume and evaluate in this
  example.} \fix{We believe that a mechanism that exploits \fixIV{spatial} error
  locality at a finer granularity could lead to even higher performance and
  energy savings, but we leave \fixIV{such an evaluation} to future work.}

\input{sections/subplots/voltron_bank_loc}

%\begin{figure}[h]
%\begin{minipage}{\linewidth}
%\begin{center}
%\includegraphics[scale=1.1]{sim_results/paper_plots/voltron_bankloc/voltron_paper_intensive_bankloc}
%\end{center}
%\vspace{-0.1in}
%\caption{Benefit of exploiting bank locality in \voltron (denoted as Voltron+BL). \label{fig:voltron_bankloc}}
%\end{minipage}
%\end{figure}


\subsection{Effect on Heterogeneous Workloads}
\label{ssec:eval_hetero}

So far, we have evaluated \voltron on \fixIII{\emph{homogeneous} multi-core} workloads, where
each workload consists of the same benchmark running on all cores. In this
section, we evaluate the effect of \voltron on \textit{heterogeneous} workloads,
where each workload consists of \emph{different} benchmarks running on each
core. We categorize the workloads based on the fraction of memory-intensive
benchmarks in the workload (0\%, 25\%, 50\%, 75\%, and 100\%). Each category
consists of 10~workloads, resulting in a total of 50~workloads across all
categories.

%\figref{voltron_hetero} compares the performance and energy efficiency of
%\voltron (with a target performance loss of 5\%) to \memdvfs for
%heterogeneous workloads.
%The system energy savings provided by \voltron grow as

\fix{\figref{voltron_hetero} shows the system performance loss and energy
efficiency improvement (in terms of performance per watt) with \voltron and with
\memdvfs for heterogeneous workloads. The error bars indicate the 95\%
confidence interval \fixIII{across all workloads in the category}. We make two
observations from the figure.}
%compares the energy efficiency \fix{improvement} (in terms of performance per
%watt) due to \voltron (with a target performance loss of 5\%) and \memdvfs for
%heterogeneous workloads.
\fix{First, for each category of the heterogeneous workloads, \voltron is able
  to meet the 5\% performance loss target on average.
%  \voltron inurs less than 5\%
%average system performance loss for each category of the heterogeneous
%workloads.
However, since \voltron is not designed to provide a \emph{hard} performance
guarantee for every single workload, \voltron exceeds the performance loss
target for 10 out of the 50~workloads, though it exceeds the target by only
0.76\% on average. Second,} the energy efficiency improvement due to
\voltron\fixIII{\ becomes larger} as the memory intensity of the workload
increases. This is because the fraction of system energy coming from memory
grows with higher memory intensity, \fixIII{due to the higher amount of} memory
traffic. Therefore, the memory energy reduction from \voltron has \fix{a
  greater} impact at the system level with more \fix{memory-intensive}
workloads. On the other hand, \memdvfs becomes \emph{less} effective with higher
memory intensity, as the memory bandwidth \fixIV{utilization more frequently}
exceeds the fixed threshold \fixIII{employed by \memdvfs}. Thus, \memdvfs has
\fix{a} smaller opportunity to scale the frequency and voltage. \fix{We conclude
  that \voltron is an effective mechanism that can adapt to different
  applications' characteristics to improve system energy efficiency.}

% Multiple metric plot
\input{sections/subplots/voltron_hetero}

%\figputHSL{sim_results/paper_plots/hetero_wklds/voltron_hetero_cat_wklds_perfwattgains}{1.1}{voltron_hetero}{Performance
%  and energy efficiency of Voltron across different heterogeneous workload
%  mixes.}

\subsection{Effect of Varying the Performance Target}
\label{ssec:vary_perf_target}

\figref{voltron_sweep} shows the performance loss and energy efficiency
\fixV{improvement due to} \voltron as we vary the system performance loss target for
\fixIV{both homogeneous and} heterogeneous workloads. For each target, we use a
boxplot to show the distribution across all workloads. In total, we evaluate
\voltron on 1001 combinations of workloads and performance targets: \fixIV{27
  homogeneous workloads $\times$ 13 targets + 50 heterogeneous workloads
  $\times$ 13 targets}. The first major observation is that \voltron's
performance-aware voltage control mechanism adapts to different performance
targets by dynamically selecting different voltage values at runtime. Across all
1001~runs, \voltron\fixIII{\ keeps performance within the performance loss}
target for 84.5\% of them. Even though \voltron cannot enforce a
\fixIII{\emph{hard}} performance guarantee for all workloads, \fixIII{it}
exceeds the target by only 0.68\% on average for those workloads \fixIII{where
  it does} not strictly meet the target.

\input{sections/subplots/target_sweep}

Second, system energy efficiency increases with higher performance loss targets,
but the gains plateau at around a target of 10\%. Beyond the 10\% target,
\voltron starts selecting smaller \varr values (e.g., 0.9V) that result in much
higher memory latency, which in turn increases both the CPU runtime and system
energy. \fix{In \ssecref{scaling_eval}, we observed that employing a \varr value
  less than 1.0V can result in smaller system energy savings than using
  \varr=1.0V.}

\fixIV{We conclude that,}
compared to prior work on memory DVFS, \voltron is a more
flexible mechanism, as it allows the \fixIV{users or system} designers to select
a performance and energy trade-off that best suits their target system or
applications.

\subsection{Sensitivity to the Profile Interval Length}
\label{ssec:interval}

\figref{interval} shows the average \fixV{system} energy efficiency improvement
due to \voltron with different profile interval lengths \fixIV{measured across
  27 homogeneous workloads}. As the \fixIV{profile} interval length increases
beyond two million cycles, we observe that the energy efficiency \fixIII{benefit
  of \voltron} \fixV{starts reducing}. This is because longer intervals prevent
\voltron from making \fixV{faster \varr} adjustments based on the
\fixV{collected new profile} information. Nonetheless, \voltron consistently
improves system energy efficiency \fixIV{for all evaluated profile interval
  lengths}.

\begin{figure}[h]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[scale=1.1]{sim_results/paper_plots/voltron_homo_intervals/voltron_intervals_more_perfwattgains}
\end{center}
\vspace{-0.1in}
\caption{Sensitivity of Voltron's \fixIV{system energy efficiency improvement} to profile interval length.\label{fig:interval}}
\end{minipage}
\end{figure}

} % end response


==> sec/voltron_final/intro.tex <==
% !TEX root=../paper.tex

\section{Introduction}

In a wide range of modern computing systems, spanning from warehouse-scale data
centers to mobile platforms, energy consumption is a first-order
concern~\cite{hoelzle-book2009,ibm-power7,deng-asplos2011,
  david-icac2011,malladi-isca2012,yoon-isca2012,choi-memcon2013,superfri,mutlu-imw2013}.
In these systems, the energy consumed by the DRAM-based main memory system
constitutes a significant fraction of the total energy.  For example,
\fix{experimental} studies of production systems have shown that DRAM consumes
40\% of the total energy in servers~\cite{hoelzle-book2009,ibmpower7-hpca}
\fixII{and 40\%} of the total power in graphics cards~\cite{paul-isca2015}.

The energy consumed by DRAM is correlated with the \emph{supply voltage} used
within the DRAM chips. The supply voltage is distributed to the two major
components within DRAM: the \emph{DRAM array} and the \emph{peripheral
  circuitry}~\cite{vogelsang-micro2010,lee-thesis2016}. The DRAM array consists
of thousands of capacitor-based DRAM cells, which store data as charge within
the capacitor. \changes{Accessing data stored in the \emph{DRAM array} requires
  a DRAM chip to perform a series of fundamental \fix{operations:} activation,
  restoration, and precharge.\footnote{We explain the detail of each of these
    operations in \secref{background}.} A memory controller \fix{orchestrates}
  each of the DRAM operations \fixII{while obeying the DRAM} timing parameters.
  On the other hand, the \emph{peripheral circuitry} consists of control logic
  and I/O drivers that connect the DRAM array to the memory channel, which is
  responsible for transferring commands and data between the memory controller
  and the DRAM chip. Since the DRAM supply voltage is distributed to both the
  DRAM array and the peripheral circuitry, \fixII{changing} the supply voltage
  would affect the energy consumption of both components in the entire DRAM
  chip.}

%The energy consumed by DRAM is correlated with the \emph{supply voltage} used
%within the DRAM chips.  The supply voltage is distributed to the two major
%components within DRAM: the \emph{DRAM array} and the \emph{peripheral
%circuitry}~\cite{vogelsang-micro2010}. The DRAM array consists of thousands of
%capacitor-based DRAM cells, which store data as charge within the capacitor.
%Due to the underlying capacitor used in each cell, accessing data stored within
%the cells requires a DRAM chip to perform a series of fundamental operations
%that are \emph{independent} of clock frequency. At the CPU, a memory controller
%sequences each of the DRAM operations based on a series of timing parameters.
%On the other hand, the peripheral circuitry consists of control logic and I/O
%drivers that connect the DRAM array to the memory channel. To transfer data
%between DRAM and the CPU at a high throughput, the peripheral circuitry needs
%to be clocked at a high frequency, \todo{which requires a certain minimum
%voltage for stable operations. Therefore, the supply voltage determines the
%maximum memory data throughput.}

To reduce the energy consumed by DRAM, vendors have developed low-voltage
variants of DDR (Double Data Rate) memory, such as LPDDR4 (Low-Power
DDR4)~\cite{jedec-lpddr4} and DDR3L (DDR3 Low-voltage)~\cite{jedec-ddr3l}. For
example, in DDR3L, the internal architecture remains the same as DDR3 DRAM, but
vendors lower the nominal supply voltage to both the DRAM array and the
peripheral circuitry \fix{via} improvements in manufacturing process technology.
In this work, we would like to reduce DRAM energy by \emph{further reducing DRAM
  supply voltage}. Vendors choose a conservatively high supply voltage, to
provide a \emph{guardband} that allows DRAM chips with worst-case process
variation to operate without errors \fixIV{under the worst-case operating
  conditions}~\cite{david-icac2011}.
% Although modern DRAM chips employ additional guardband on the nominal voltage
% for the worst-case scenarios (e.g., process variation)~\cite{david-icac2011},
The exact amount of supply voltage guardband varies across chips, and lowering
the voltage below the guardband can result in erroneous or even undefined
behavior. Therefore, we need to understand how DRAM chips behave during
reduced-voltage operation. To our knowledge, no previously published work
examines the effect of using a wide range of different supply voltage values on
the reliability, latency, and retention characteristics of DRAM chips.

% Prior works
%\ignore{
%Other work~\cite{david-icac2011}
%takes inspiration from \emph{dynamic voltage and
%frequency scaling} (DVFS) techniques that are widely used in commercial CPUs
%to reduce power dissipation~\cite{intel-speedstep, amd-powernow, ibm-power7}.
%DVFS for DRAM is designed to scale the supply voltage below the nominal voltage value
%at runtime, by reducing
%both the voltage and frequency of the DRAM~\cite{david-icac2011}.  One drawback
%of DVFS for DRAM is that in order to significantly reduce the supply voltage,
%the DVFS mechanism \emph{must} reduce the frequency of the peripheral
%circuitry, as the maximum operating frequency is a function of the voltage.
%This reduces the rate at which the peripheral circuitry can send data across
%the memory channel, which thus reduces the throughput of the DRAM.
%In order to minimize the performance impact of the reduced throughput,
%DVFS for DRAM performs voltage and frequency scaling only when DRAM bandwidth
%utilization is low.
%}

% Many state-of-the-art works have proposed different DRAM power optimizations,
% such as modifying DRAM chip architecture to reduce access
% power~\cite{udipi-isca2010,zhang-isca2014,cooper-balis-ieeemicro2010},
% increasing idleness for more DRAM low-power modes~\cite{lebeck-asplos2000,
%   fan-islped2001,aggarwal-hpca2008, bi-hpca2010}, or adjusting DRAM frequency
% or/and voltage dynamically~\cite{deng-asplos2011,david-icac2011,
%   paul-isca2015,begum-iiswc2015}. In particular, \emph{dynamic voltage and
%   frequency scaling (DVFS)} is an effective optimization used in commercial CPUs
% to reduce power and (likely) energy consumption~\cite{intel-speedstep,
%   amd-powernow, ibm-power7}. As a result, these recent works focus on applying this
% conventional DVFS technique to DRAM based on memory bandwidth utilization.

%\ignore{ We aim to develop a mechanism where the DRAM supply voltage (and
%therefore DRAM energy consumption) can be reduced without sacrificing
%throughput.  As the throughput is a function of the peripheral circuitry voltage
%and frequency, we can preserve throughput by reducing the supply voltage to
%\emph{only} the DRAM cell array. However, we cannot blindly reduce the cell
%array voltage, as the voltage reduction may affect reliability. As the cell
%array exhibits RC circuit behavior, we need to carefully understand the effect
%that voltage reduction has on the cell array.  Our goal in this work is to
%characterize the relationship between supply voltage reductions and the behavior
%of the DRAM cell array, and to use the insight from this characterization to
%drive our mechanism design. }

% DRAM voltage required for correct data retrieval is known to be correlated with
% the frequency at which DRAM is clocked, i.e., voltage can be reduced if
% frequency is reduced. Nonetheless, to our knowledge, no work has published
% information about the influence of using a wide range of different voltage
% values on various other DRAM characteristics, e.g., reliability and DRAM
% latency. Current literature primarily focuses on designing new control policies
% on when to adjust frequency and voltage of memory to reduce DRAM power without
% demonstrating the effect on DRAM when performing voltage scaling
% ~\cite{david-icac2011}. Furthermore, given a fixed frequency, prior works simply
% select a voltage that is empirically determined to read the correct data without
% knowing how DRAM behaves with lower supply voltage. In this work, our major goal
% is to characterize and analyze \emph{real modern DRAM chips} operating under
% different supply voltage levels. Understanding DRAM characteristics due to
% different voltage levels is imperative not only for enabling memory DVFS in real
% systems, but also for developing other low-power DRAM designs that use low
% voltage.
%
% %Unlike CPU, DRAM-based memory consists DRAM cells that each stores data as
% %charge on a capacitor. Since the amount of charge stored in each cell is
% %directly correlated with the DRAM voltage, scaling voltage introduces
% %additional implications on DRAM operations which are responsible to sense and
% %supply the charge in the cells.

\changes{\textbf{Our goal} in this work is to \myitem{i}~characterize and
understand the relationship between supply voltage reduction and various
characteristics of DRAM, including DRAM reliability, latency, and data
retention; and \myitem{ii}~use the insights derived from this characterization
and understanding to design a new mechanism that can aggressively lower the
supply voltage to reduce DRAM energy consumption while keeping performance loss
under a bound.} To this end, we build an FPGA-based testing platform that allows
us to tune the DRAM supply voltage~\cite{hassan-hpca2017}. Using this testing
platform, we perform experiments on 124~real DDR3L DRAM chips~\cite{jedec-ddr3l}
\fixII{from \fix{three} major vendors}, contained within 31~dual in-line memory
modules (DIMMs). Our comprehensive experimental characterization provides four
major observations on how DRAM \fixII{latency, reliability, and data retention
  time are} affected by reduced supply voltage.

First, we observe that we can reliably access data when DRAM supply voltage is
lowered below the nominal voltage, {\em until a certain voltage value}, \vmin,
which is the minimum voltage level at which no bit errors occur. Furthermore, we
find that we can reduce the voltage below \vmin to attain further energy
savings, but that errors start occurring in some of the data read from memory.
As we drop the voltage further below \vmin, the number of erroneous bits of data
increases exponentially \fixII{with the voltage drop}.

Second, we observe that while reducing the voltage below \vmin introduces bit
errors in the data, we can prevent these errors if we \emph{increase} the latency of
the three fundamental DRAM operations (activation, restoration, and precharge).
When the supply voltage is reduced, the capacitor charge takes a longer time to
change, thereby causing these DRAM operations to become slower to complete.
Errors are introduced into the data when the memory controller does \emph{not}
account for this slowdown in the DRAM operations.  We find that if the memory
controller allocates extra time for these operations to finish when the supply
voltage is below \vmin, errors no longer occur. We validate, analyze, and
explain this behavior using \fixII{detailed} circuit-level simulations.

Third, we observe that when only a small number of errors occur due to reduced
supply voltage, these errors tend to \emph{cluster} physically in certain
\emph{regions} of a DRAM chip, as opposed to being randomly distributed
throughout the chip.  This observation implies that when we reduce the supply
voltage to the DRAM array, we need to increase the fundamental operation
latencies for \emph{only} the regions where errors can occur.

% AFTER SUBMISSION
%Thus, we can
%exploit low-cost mechanisms to track these regions, and can avoid increasing the
%latencies (and thus avoid reducing the performance) for the rest of the cell
%array when we reduce the array voltage.

% Third, we find that when a small number of errors start occurring due to reduced
% voltage, they cluster in certain \emph{regions} of a DRAM chip instead of being
% distributed randomly. This observation implies that only certain regions require
% higher access latency to operate DRAM without errors when scaling voltage. This
% allows us exploit low-cost mechanisms to mitigate performance loss under low
% voltage by using higher latency in only those error-inflicting regions.

Fourth, we observe that reducing the supply voltage does \emph{not} impact the
data retention guarantees of DRAM.  Commodity DRAM chips guarantee that all
cells can safely retain data for 64ms, after which the cells are
\emph{refreshed} to replenish charge that leaks out of the capacitors. Even when
we reduce the supply voltage, the rate at which charge leaks from the capacitors
is so slow that no data is lost during the 64ms \fixIV{refresh interval} at
20$\celsius$ and 70$\celsius$ \fix{ambient temperature}.

% Fourth, we study the effect of voltage on DRAM retention time -- the amount of
% time that a DRAM cell can safely retain data without being refreshed. Our
% results show that the impact of reduced voltage can only be observed at a
% retention time (512ms) that is much higher than the standard refresh frequency
% (64ms), showing on average less than one cell out of billions of cells observes
% a bit flip. However, by refreshing cells every 64ms, we observe no bit flips
% with all the reduced voltage value that we tested.

% Our experimental observations lead us to propose a new power optimization that
% addresses a major limitation of memory DVFS proposed by prior
% works~\cite{deng-micro2012, david-icac2011}. Frequency scaling in DRAM refers to
% changing DRAM \emph{channel (bus)} frequency, affecting available memory
% bandwidth. Frequency control algorithm proposed by these works lowers the
% channel frequency only when an application has small memory bandwidth demand to
% avoid large performance loss. As a result, DRAM DVFS has little opportunity when
% an application's performance is sensitive to memory bandwidth as reducing the
% channel frequency can severely degrade system performance.

% Our power optimization goal is to enable DRAM power reduction while retaining
% the same high memory bus frequency. We propose to reduce the supply voltage to
% only cell arrays without tuning the voltage to the periphery circuits in DRAM. A
% DRAM chip can be divided into two major components: DRAM cell arrays and
% peripheral circuitry~\cite{vogelsang-micro2010}. The periphery circuitry refers
% to the structure outside of the arrays, mainly consisting of control logic and
% I/O that drives/received data through the memory channel. The cell array
% operations (e.g., activate and precharege) are not dependent on the channel
% frequency and our experiments show that these operations' latency scale
% accordingly with voltage. Hence, reducing voltage to cell arrays increases the
% latency, but it does not affect the bandwidth of DRAM channels.

%Introduce: array voltage reduction.
%two ways:
%1. Talk about it right away saying that we already know latency goes up with
%lower voltage. But then how about frequency? it turns out DRAM splits into
%arrays and peri. And array ops are completely independent of frequency, so this
%enables us to do a limited version of voltage scaling without touching
%frequency. Why do this? B/c high bw case.
%
%2. Talk about frequency scaling and its limitation. Mainly hw bw case. It turns
%out freq and volt are split. And based on our observation, latency is
%independent of frequency, so we can introduce array volt scaling.

Based on our experimental observations, we propose a new low-cost DRAM energy
\fix{reduction} mechanism called \emph{Voltron}. \changes{The key idea of
  Voltron is to use a performance model to determine \fixIV{by} how much we can
  reduce the DRAM array voltage at runtime without introducing errors and
  without exceeding a user-specified threshold for \fixII{acceptable}
  performance loss.} Voltron consists of two components: \fix{\emph{array
    voltage scaling} and \emph{performance-aware voltage control}}.

\emph{Array voltage scaling}
leverages minimal hardware modifications within DRAM to reduce the
voltage of \emph{only} the DRAM array, without affecting the voltage
of the peripheral circuitry. \changes{If Voltron were to reduce the voltage of the
peripheral circuitry, we would have to reduce the operating frequency of DRAM.
This is because the \emph{maximum} operating frequency of DRAM is a
function of the peripheral circuitry voltage~\cite{david-icac2011}.
A reduction in the operating frequency reduces the memory data throughput, which
can significantly harm the performance of applications that require high memory
\fix{bandwidth}, \fixIV{as we demonstrate in this paper.}}
%  (as we demonstrate quantitatively in \ssecref{avs})
% \changes{One limitation of
%   reducing the supply voltage (to both the peripheral circuitry and DRAM array)
%   is that it requires the peripheral circuitry to operate at lower frequency, as
%   the maximum operating frequency is a function of the
%   voltage~\cite{david-icac2011}. This reduces the rate at which DRAM can send
%   data across the memory channel, which thus reduces the memory throughput. In
%   order to reduce DRAM energy without sacrificing memory bandwidth, }

\emph{Performance-aware voltage control} uses \fixII{performance counters}
within the processor to build a piecewise linear model of how the performance of
an application decreases as the DRAM array supply voltage is lowered (due to
longer operation latency to prevent errors), and uses the model to select a
supply voltage that \fixII{keeps performance above} a
\fixIV{user/system-specified} performance target.

%Unlike prior works~\cite{deng-asplos2011,
%  david-icac2011, paul-isca2015, begum-iiswc2015}, Voltron does not reduce
%memory throughput, and can reduce the supply voltage even during periods of high
%memory utilization.

Our evaluations of Voltron show that it \fix{significantly reduces} both DRAM and system energy
consumption, at the expense of very modest performance degradation. For example,
at \fixII{an average} performance loss of only 1.8\% over seven \fix{memory-intensive}
quad-core workloads from SPEC2006, Voltron reduces DRAM energy consumption by an
average of 10.5\%, which translates to an overall system energy consumption of
7.3\%. We also show that \voltron effectively saves DRAM and system energy on
even \fix{non-memory-intensive} applications, with very little performance impact.

% Evaluations of our proposed technique on reducing cell array voltage shows both
% lower DRAM and system energy consumption at the cost of very modest performance
% degradation. In addition, we propose a new management policy, called
% \emph{Voltron}, that selects an array voltage based on users' requirement on
% performance loss. The key idea of Voltron is to predict the potential
% performance loss under a range of different voltage inputs based on a piecewise
% linear model. The model incorporates inputs from a few of an application's
% hardware footprints -- memory intensity and stall time. Through this model,
% Voltron provides DRAM and system energy savings by 11\% and 7\%, respectively,
% at the cost of 3\% performance loss for a list of memory intensive workloads.

This work makes the following major contributions:
\squishlist
%\item We perform the first detailed experimental characterization of the effects
%of reduced-voltage operation on DRAM latency, reliability and data retention, by
%comprehensively testing and analyzing 124 real DRAM chips from three major DRAM
%vendors.

\item We perform the first detailed experimental characterization \fix{of how
the reliability and latency of \fixIII{modern DRAM chips are} affected when the
supply voltage is lowered below the nominal voltage level.  We comprehensively
test and analyze} 124 real DRAM chips from three major DRAM vendors. \fixII{Our
characterization reveals four new major observations, which can be useful for
developing new mechanisms \fixIV{that improve or better trade off between}
DRAM energy/power, latency, and/or reliability.}

% \item We experimentally characterize real DRAM chips using a wide range of
%   reduced voltage values below nominal supply voltage. Lowering voltage induces
%   errors in data read from DRAM when the voltage is below a certain point.

\item We experimentally demonstrate that reducing the supply voltage below a
  certain point introduces bit errors in the data read from DRAM. We show that we
  can avoid these bit errors by increasing the DRAM access latency when the
  supply voltage is reduced.

  % The access latency
  % determines the amount of time allotted for the three fundamental
  % DRAM operations (activation, restoration, and precharge).

% \item We demonstrate that \emph{only certain regions} within a DRAM
%   chip require a longer access latency when DRAM supply voltage is reduced.
%   We demonstrate that supply voltage reductions do not impact the data
%   retention guarantees of modern DRAM chips.

\item We propose Voltron, a mechanism that \fixII{\myitem{i}~reduces the supply
voltage to only the DRAM array without affecting the peripheral circuitry, and
\myitem{ii}~uses a performance model to select a voltage that does not degrade
performance beyond a chosen threshold.  We show that Voltron is effective at
improving system energy consumption, with only a small impact on performance.}

\item \fix{We open-source our FPGA-based experimental characterization \fixIII{infrastructure} and
DRAM circuit simulation infrastructure, \fixIV{used in this paper}, for \fixIII{evaluating} reduced-voltage operation~\cite{volt-github}.}

\ignore{reduces DRAM and system energy consumption
without introducing errors and without incurring significant application performance
loss. Voltron \fixII{\myitem{i}} reduces the supply voltage to only the DRAM array without
affecting the peripheral circuitry, to avoid hurting memory data throughput, and
\fixII{\myitem{ii}} uses a performance model to select a voltage that does not degrade performance
by more than a threshold.}

\ignore{Onur says: "We show that Voltron is effective at improving system energy
consumption, with only a small impact on performance." This is a bit redundant
with the previous sentence.}

  \ignore{ Voltron reduces DRAM and system energy consumption by an average of
  10.8\% and 7.4\%, respectively, with only a 3.5\% reduction in system
  performance over seven \fix{memory-intensive} quad-core workloads.}

% \item We propose a new low-power mechanism that scales voltage to DRAM
%   arrays without affecting other peripheral circuitry in order to clock DRAM at
%   high frequency. We propose a management policy called \voltron to
%   automatically select an array voltage that saves energy consumption while
%   bounding performance loss. We find that \voltron reduces DRAM and system
%   energy by 11\% and 7\%, respectively, with 3\% system performance loss on
%   average in a 4-core system.

\squishend


==> sec/voltron_final/related.tex <==
% !TEX root=../paper.tex

\section{Related Work}

\response{To our knowledge, this is the \fixIII{first work}} to \myitem{i}
experimentally \changes{characterize the reliability and performance of modern
  low-power DRAM chips under different supply voltages}, and \myitem{ii}
\fixIV{introduce} a new mechanism that reduces DRAM energy while retaining high
memory \fixIV{data} throughput by \fixIV{adjusting} the DRAM array voltage. We
briefly discuss other prior work in DRAM energy reduction.

\ignore{\paratitle{DRAM Frequency and Voltage Scaling} Many prior works have proposed to
reduce DRAM energy by adjusting the memory channel frequency and/or the DRAM
supply voltage dynamically. Deng et al.~\cite{deng-asplos2011} propose MemScale,
which scales the frequency of DRAM at runtime based on a performance predictor
of an in-order processor. Other work focuses on developing management policies
to improve system energy efficiency by coordinating DRAM \emph{DFS} with DVFS on
the CPU~\cite{deng-micro2012, deng-islped2012, begum-iiswc2015} or
GPU~\cite{paul-isca2015}. In addition to frequency scaling, David et
al.~\cite{david-icac2011} propose to scale the DRAM supply voltage along with
the memory channel frequency, based on the memory bandwidth utilization of
applications.}

\paratitle{DRAM Frequency and Voltage Scaling} \changes{We have already
discussed the most relevant works on DRAM frequency and voltage scaling, and
provided qualitative comparisons in \ssecref{dvfs}.} \changes{ None of these
works provide a comprehensive experimental analysis \fixIII{of} the impact of
using a wide range of supply voltages on DRAM reliability, latency, and refresh.
In contrast to all these works, our work focuses on a detailed experimental
characterization of real DRAM chips as the supply voltage varies. Our study
provides fundamental observations for potential mechanisms that can mitigate
DRAM and system energy consumption. Furthermore, frequency scaling hurts memory
throughput, and thus significantly degrades \fixIV{the} system performance of
\fixIV{especially} memory-intensive workloads (see \ssecref{avs} for our
quantitative comparison). We demonstrate the importance \fix{and benefits} of
\fix{exploiting} our \fix{experimental} observations by proposing \voltron, one
\fixIV{new example} mechanism that uses our observations to reduce DRAM and system
energy without sacrificing memory throughput. }

%and thus provides meager energy savings for memory-intensive applications.
%We demonstrate the importance of these observations by proposing \voltron, one
%potential mechanism that uses our observations to reduce DRAM and system energy
%without sacrificing memory throughput.

%\todo{Expand here}
%a couple of sentences on throughput and tie it back array voltage selection
%these dont decouple array from the lvoltage

% Our
% study provides foundation for techniques that aim to utilize memory voltage
% scaling as part of the power management policy. For example, we propose and
% evaluate a new power optimization technique that reduces the system energy
% consumption for bandwidth-sensitive workloads based on our experimental study.

\ignore{vs. our work. They focus on benchmarks that don't utilize BW. There are
BW sensitive apps, such as GPU, but is good at hiding latency. We focus on mem
intensive workloads. In addition, we conduct experimental study on the DRAM
behavior which prior work does not have. Our approach can be combine with these
works to enable a comprehensive technique to improve energy efficiency for a
wide range of workloads. Contradicting comments...bc we show that freq scale
doesn't quite work for compute-intensive workloads. Unclear what the breakdown
between CPU and DRAM in these prior works. }

\paratitle{Low-Power Modes for DRAM} Modern DRAM chips support various low-power
standby modes. \fix{Entering and exiting these modes incurs some amount of
  latency, which delays memory requests that must be serviced.}
%that can be utilized at the cost of increased latency to exit these modes when
%a memory request must be serviced.
To increase the opportunities to exploit these low-power modes, several prior
works propose mechanisms that increase periods of memory idleness through data
placement (e.g.,~\cite{lebeck-asplos2000, fan-islped2001}) and memory traffic
reshaping (e.g.,~\cite{aggarwal-hpca2008, bi-hpca2010, amin-islped2010,
  lyuh-dac2004, diniz-isca2007}). Exploiting low-power modes is orthogonal to
our work on studying the impact of \fixIV{reduced-voltage operation in DRAM}.
Furthermore, low-power modes have a smaller effect on memory-intensive
workloads, which exhibit little idleness in memory accesses, \fixIV{whereas, as
  we showed in \ssecref{pavc_eval}, our mechanism is especially effective on
  memory-intensive workloads.}

\paratitle{Low-Power DDR DRAM Chips} Low-power DDR (LPDDR)~\cite{jedec-lpddr3,
jedec-lpddr4} is a specific type of DRAM that is optimized for low-power systems
like mobile devices. To reduce power consumption, LPDDRx (currently in its 4th
generation) employs a few major design changes that differ from conventional
DDRx chips. First, LPDDRx uses a low-voltage swing I/O interface that consumes
40\% less I/O power than DDR4 DRAM~\cite{choi-memcon2013}. Second, it supports
additional low-power modes with a lower supply voltage. Since the LPDDRx array
design remains the same as DDRx, our observations on the correlation between
access latency and array voltage are applicable to LPDDRx DRAM \fixIV{as well}.
Our proposed \voltron approach can provide significant benefits in LPDDRx,
\fixIII{since array} energy consumption is significantly \emph{higher} than the
energy consumption of \fixIII{peripheral circuitry in LPDDRx
  chips}~\cite{choi-memcon2013}. \changes{We leave the detailed evaluation of
  LPDDRx chips for future work since our current experimental platform is not
  capable of evaluating them.}

\paratitle{Low-Power DRAM Architectures} \fixIV{Prior} works
(e.g.,~\cite{udipi-isca2010, zhang-isca2014, cooper-balis-ieeemicro2010,
  chatterjee-hpca2017}) propose to modify the DRAM chip architecture to reduce
the \act power by activating only a fraction of a row instead of the entire row.
Another common technique, called sub-ranking, reduces dynamic DRAM power by
accessing data from a subset of chips from a DRAM module~\cite{zheng-micro2008,
  yoon-isca2011, ware-iccd2006}. \fix{A couple of} prior
works~\cite{malladi-isca2012, yoon-isca2012} propose DRAM module architectures
that integrate many low-frequency LPDDR chips to enable DRAM power reduction.
These proposed changes to DRAM chips or DIMMs are orthogonal to our work.

\fix{ \paratitle{Reducing Refresh Power} In modern DRAM chips, although
different DRAM cells have widely different retention times~\cite{liu-isca2013,
  kim-edl2009}, memory controllers conservatively refresh \emph{all} of the
cells based on the retention time of a small fraction of weak cells, which have
the longest retention time out of all of the cells. To reduce DRAM refresh
power, many prior works (e.g., \fixV{\cite{liu-isca2012, agrawal-hpca2014,
    qureshi-dsn2015, liu-isca2013,
    venkatesan-hpca2006,bhati-isca2015,lin-iccd2012,ohsawa-islped1998,
    patel-isca2017, khan-sigmetrics2014, khan-dsn2016, khan2016case}}) propose
mechanisms to reduce unnecessary refresh operations, and, thus, refresh power,
by characterizing the retention time profile (i.e., the \fixIV{data} retention
behavior of each cell) within the DRAM chips. However, these techniques do not
reduce the power of \emph{other} DRAM operations, and these prior works do
\emph{not} provide an experimental characterization of the effect of reduced
voltage level\fixIV{s} on \fixIV{data} retention time.
%, such as the \act power

% only on refresh power, which is only a small power component in today's DRAM
%we show it's quite small in today's DRAM. It's also not big to future dram as
%scaling to 64gb may be unlikely due to the difficulty of build trench capacitor.

\paratitle{Improving DRAM Energy Efficiency by Reducing Latency or
Improving Parallelism} \fixIV{Various} prior works
(e.g.,\fixIV{~\cite{hassan-hpca2016, lee-hpca2015, chang-hpca2014,
lee-thesis2016, lee-hpca2013,
lee-sigmetrics2017,lee-arxiv2016,kim-isca2012, lee-thesis2016,
lee-taco2016, seshadri-micro2013, chang2016low, lee-pact2015}}) improve
DRAM energy efficiency by reducing the execution time through techniques
that reduce the DRAM access latency or improve parallelism between memory
requests.  These mechanisms are orthogonal to ours, because they do
\fixIV{not reduce} the voltage level of DRAM. }

\fixIII{\paratitle{Experimental Studies of DRAM Chips} Recent works
\fixIV{experimentally investigate various} reliability, \fixIV{data} retention,
and latency characteristics of modern DRAM chips~\cite{liu-isca2012,
  liu-isca2013, kim-isca2014, chang-sigmetrics2016, lee-hpca2015,
  lee-sigmetrics2017, chandrasekar-date2014, khan-sigmetrics2014,
  jung-memsys2016, jung-patmos2016,
  hassan-hpca2017,khan-dsn2016,patel-isca2017,lee-arxiv2016,lee-thesis2016,kim-thesis2015,
  meza2015revisiting, schroeder-sigmetrics2009, sridharan-asplos2015,
  sridharan2012study}. None of these works study these characteristics under
reduced-voltage operation, which we do in this paper.}

% Paul et al.~\cite{paul-isca2015} propose a power management scheme that
% coordinates DVFS of GPU and DRAM.

\fixIII{\paratitle{Reduced-Voltage Operation in SRAM Caches} Prior works propose
different techniques to enable SRAM caches to operate under reduced voltage
levels
(e.g.,~\cite{alameldeen-isca2011,alameldeen-tc2011,wilkerson-ieeemicro2009,chishti-micro2009,roberts-dsd2007,wilkerson-isca2008}).
These works are orthogonal to our experimental study because we focus on
\fixIV{understanding and enabling reduced-voltage operation in} DRAM, which is a
\fixIV{significantly} different memory technology than SRAM.}


==> sec/voltron_final/spice_exp.tex <==
To further understand the relationship between access latency and voltage,
we express the access latency as a mathematical function. Since the SPICE
simulation employs a series of circuit
models~\cite{nagel-spice,massobrio1993semiconductor}, we can simplify the
latency growth function with only the \vdd parameter given \emph{our}
specific transistor, resistance, and capacitance parameters. \sg{this is
unclear still - what is the latency growth function?}

We represent the latency as an exponential function of \varr
%(abbreviated as $V$)
in Equation~\ref{exp_decay}. $\lambda$ is the decay rate of the latency,  and
$y_{0}$ represents the initial latency value when \varr is 0, with an offset of
$\epsilon$. In this work, we bound the value of \varr from 0.9V to 1.35V for our
SPICE simulations.

\vspace{-0.15in}
\begin{align}
    y(V_{array})=y_{0} \cdot e^{-\lambda V_{array}} + \epsilon
    \label{exp_decay}
\end{align}
\vspace{-0.15in}

\tabref{exp_func_params} shows the coefficients of the exponential function
after fitting the function to our SPICE simulation results. We calculate the
coefficients using the SciPy~\cite{scipy} non-linear regression, which minimizes
least squares. To measure how well the regression function fits to the SPICE
results, we report $R^2$, which ranges from 0\% (i.e., does not fit at all) to
100\% (i.e., a perfect fit). Our exponential function matches very closely with
our SPICE simulation results, with a 99.91\% and 99.85\% $R^2$ for the activation
and precharge latencies, respectively.

\begin{table}[h]
    \renewcommand{\arraystretch}{0.9}
    \small
    \centering
    \setlength{\tabcolsep}{.7em}
    \begin{tabular}{crrrc}
        \toprule
        \textbf{Latency} & \multicolumn{1}{c}{$y_{0}$} & \multicolumn{1}{c}{$\lambda$} & \multicolumn{1}{c}{$\epsilon$} & \multicolumn{1}{c}{$R^{2}$ (\%)}\\
        \midrule
        Activation & 9471.58 & 7.15 & 6.72 & \textbf{99.91} \\
        Precharge & 26299.34 & 8.33 & 7.71 & \textbf{99.85} \\
        \bottomrule
    \end{tabular}
    \caption{Coefficients and goodness of fit of Equation~\ref{exp_decay}.}
    \label{tab:exp_func_params}
\end{table}

Our SPICE simulations not only
validate that a lower supply voltage requires longer access latency, but also provide
us with a model that generates much more precise latency values given a certain
supply voltage.

%%%%% END SPICE MODEL %%%%%


==> sec/voltron_final/subplots/loc_samsung.tex <==
\begin{figure}[!h]
    \centering
    \subcaptionbox{1.05V}[\linewidth]
    {
        \includegraphics{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.050000_fix_row}.pdf}
    }

    \subcaptionbox{1.025V}[\linewidth]
    {
        \includegraphics{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.025000_fix_row}.pdf}
    }
    \caption{Spatial distribution of errors in a Vendor B's DIMM.}
    \label{fig:locality_B}
\end{figure}


==> sec/voltron_final/subplots/motivation.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    {
        \includegraphics[width=\linewidth]{plots/powerbreakdown/power_breakdown_Freq_power_isca}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/powerbreakdown/power_breakdown_Freq_energy_isca}
        \vspace{-0.1in}
    }

    \caption{Power and energy consumption due to different DRAM frequency.}
    \label{fig:voltron}
\end{figure}


==> sec/voltron_final/subplots/voltron.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    %\subcaptionbox{1}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_perfloss}
        %\includegraphics[scale=1.0]{plots/voltron_perfloss}
        \vspace{-0.1in}
    }

    %\subcaptionbox{2}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_dramenergysavings}
        %\includegraphics[scale=1.0]{plots/voltron_dramenergysavings}
        \vspace{-0.1in}
    }

    %\subcaptionbox{3}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_sysenergysavings}
        %\includegraphics[scale=1.0]{plots/voltron_sysenergysavings}
        %\vspace{-0.1in}
    }
    \vspace{-0.1in}
    \caption{Comparison between \voltron and an oracle with a system performance
      loss bound of 5\%.}
    \label{fig:voltron}
\end{figure}


==> sec/voltron_final/subplots/voltron_interval.tex <==
\begin{figure}[!h]
    \centering
    %\captionsetup[subfigure]{justification=left}
    %\subcaptionbox{1}[\linewidth]

    \subcaptionbox*{}[0.49\linewidth][l]
    {
      \includegraphics[scale=1]{sim_results/paper_plots/voltron_homo_intervals/voltron_intervals_drampowersavings}
    }
    \subcaptionbox*{}[0.49\linewidth][r]
    {
      \includegraphics[scale=1]{sim_results/paper_plots/voltron_homo_intervals/voltron_intervals_perfwattgains}
    }
    \vspace{-0.25in}

    \caption{\response{Performance sensitivity of \voltron to profile intervals.}}}
    \label{fig:interval}
\end{figure}


==> sec/voltron_final/subplots/vsweep.tex <==
% plots/vsweep_norm_dram_energy.pdf  plots/vsweep_norm_ipc.pdf
% plots/vsweep_norm_system_energy.pdf  plots/vsweep_norm_ws.pdf
\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{justification=centering}
    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_ipc}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_dram_energy}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_system_energy}
        \vspace{-0.1in}
    }
    \caption{Impact of adjusting DRAM array voltage on system performance and energy
    savings.}
    \label{fig:vsweep}
\end{figure*}


==> sec/voltron_final/system_evaluation.tex <==
% !TEX root=../paper.tex

\section{System Evaluation}
\label{sec:eval}

In this section, we evaluate the system-level \fixIV{performance and energy}
impact of \voltron.  We present our evaluation methodology in \ssecref{meth}.
Next, we study the energy savings and performance loss when we use array voltage
scaling without any control (\ssecref{scaling_eval}).  We study how
performance-aware voltage control delivers overall system energy reduction with
only a modest \fix{amount of} performance loss
(\fixIII{Sections~\ref{ssec:pavc_eval} and \ref{ssec:energy_breakdown}}). We
then evaluate \fix{an enhanced version of} \voltron\fix{, which exploits}
spatial error locality (\ssecref{eval_el}). Finally,
Sections~\ref{ssec:eval_hetero} to \ref{ssec:interval} present sensitivity
studies of \voltron\fix{\ to various system and algorithm parameters}.

\subsection{Methodology}
%\section{Evaluation Methodology}
\label{ssec:meth}

We evaluate \voltron using Ramulator~\cite{kim-cal2015}, a detailed and
\fixV{and cycle-accurate}
  \fix{open-source DRAM simulator~\cite{ram-github}}, integrated with a
  multi-core performance simulator. We model a low-power mobile system that
  consists of 4 ARM cores and DDR3L DRAM. \tabref{sys-config} shows our system
  parameters. Such a system resembles existing commodity devices, such as the
  Google Chromebook~\cite{chromebook} \fix{or the NVIDIA} SHIELD
  tablet~\cite{shield}. To model power and energy consumption, we use
  McPAT~\cite{mcpat:micro} for the processor and DRAMPower~\cite{drampower} for
  the DRAM-based memory system. \fix{We open-source the code of Voltron
    \cite{volt-github}.}

%\vspace{-0.05in}
\input{sections/tables/sys_config_table}
%\vspace{-0.05in}

\tabref{varr_latency} lists the latency values we evaluate for each DRAM array
voltage (\varr). The latency values are obtained from our SPICE model using data
from real devices (\ssecref{low_volt_latency}), \fix{which is available
  online~\cite{volt-github}}.\footnote{\fixIV{In this work, we do not have
  experimental data on the restoration latency (\tras) under reduced-voltage
  operation. This is because our reduced-voltage tests access cache lines
  sequentially from each DRAM row, and \tras overlaps with the latency of
  reading all of the cache lines from the row.  Instead of designing a separate
  test to measure \tras, we use our circuit simulation model
  (\ssecref{low_volt_latency}) to derive \tras values for reliable operation
  under different voltage levels. We leave the thorough experimental evaluation
  of \tras under reduced-voltage operation to future work.}} To account for
  manufacturing process variation,
we conservatively add in the same latency guardband (i.e., 38\%) used by
manufacturers at the nominal voltage level of 1.35V to each of our \fix{latency
  values}. We then round up each latency \fix{value} to the nearest clock cycle
time (i.e., 1.25ns).

%\vspace{-0.05in}
\input{sections/tables/varr_latency}
%\vspace{-0.05in}

\paratitle{Workloads} We evaluate 27~benchmarks from SPEC
CPU2006~\cite{spec2006} and YCSB~\cite{cooper-socc2010}, as shown in
\tabref{workload_list} \fix{along with each benchmark's \fixIII{L3 cache} MPKI,
  i.e., memory intensity}. \fix{We use the 27~benchmarks to form
  \emph{homogeneous} and \emph{heterogeneous} \fixIV{multiprogrammed}
  workloads.} \fix{For each \emph{homogeneous workload}, we replicate one of our
  benchmarks} by running one copy on each core to form a four-core
\fixIV{multiprogrammed} workload, as done in many past works \fixIII{that
  evaluate multi-core system performance}~\cite{lee-hpca2015,
  chang-sigmetrics2016, lee-hpca2013, nair-isca2013, nair-micro2014,
  shafiee-hpca2014, shevgoor-micro2013, chatterjee-micro2012}. \fixIV{Evaluating
  homogeneous workloads enables easier analysis and understanding of the
  system.} \fix{For each \emph{heterogeneous workload}, we combine four
  \emph{different} benchmarks \fix{to create a four-core workload}. We
  categorize the heterogeneous workloads by varying the fraction of
  \fix{memory-intensive} benchmarks in each workload (0\%, 25\%, 50\%, 75\%, and
  100\%). Each category consists of 10~workloads, resulting in a total of
  50~workloads across all categories.} Our simulation executes at least
500~million instructions on each core. \fix{We calculate system energy as} the
product of the average dissipated power (from both CPU and DRAM) and the
workload runtime. We measure system performance with the commonly-used
\emph{weighted speedup} (WS) metric~\cite{snavely-asplos2000}, which is a
measure of job throughput on a multi-core system~\cite{eyerman-ieeemicro2008}.

%Specifically,
%$WS = \sum_{i=1}^N{\frac{IPC_{i}^{shared}}{IPC_{i}^{alone}}}$. $N$ is the number
%of cores in the system. ${IPC_{i}^{shared}}$ is the IPC of an application that
%runs on $core_i$ while other applications are running on the other cores.
%${IPC_{i}^{alone}}$ is the IPC of an application when it runs alone in the
%system without any other applications. Essentially, WS is the sum of every
%application's slowdown compared to when it runs alone on the same system.

\input{sections/tables/workload_list}

%\todo{GPGPU with HBM, similar to a mobile system. For hiding latency
%purpose. It doesn't have to be BW intensive.}
%\highlight{* Ideal: Pure Vdd without any changes to the latency and BW}
%\highlight{* Vdd = Vcore + Vperi. Vperi tuning -> slower bus}
%\highlight{* Vcore tuning -> core latency}
%\highlight{* Vdd -> Tunes both bus freq and core latency}

%\kevin{more details on the DRAM power and energy calculation}. Talk about how we
%calculate the energy from the array. 1) the dynamic component scales with v2 and
%2) the area of array vs periphery and scale that fraction with v2.

%\vspace{-0.1in}

%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\subsection{Dynamic DRAM Energy Results}

Since higher DRAM access latency can potentially increase the energy
consumption, we perform a first order study to evaluate the \emph{dynamic}
energy consumption of the three fundamental access operations that we
demonstrate to be affected by \varr: \myitem{i} activation, \myitem{ii}
precharge, and \myitem{iii} restoration.

\figref{spice_energy_savings} shows the normalized dynamic energy consumption of
the three operations as voltage varies. As \varr lowers, the power consumption
of these operations reduces with high latency. We calculate their energy by
multiplying their power consumption with its latency at each \varr point. The
results show that even though latency increases, the power reduction still saves
\emph{dynamic} energy per operation. However, the dynamic energy savings have
diminished returns when \varr reduces below 1.1V since the latency is increasing
at an exponential rate (shown previously in Eq.~\ref{exp_decay},
\ssecref{spice}). For precharge, the dynamic energy of precharge starts to give
negative returns on energy savings. These results show that decreasing \varr
directly reduces the energy consumption of DRAM operations, but lower \varr does
not necessarily provide more energy savings. Now, we evaluate the system
performance and energy savings by taking into account other dynamic and static
energy consumption in both the DRAM and CPU.

\input{sections/subplots/spice_power_energy}
}
%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Impact of Array Voltage Scaling}
\label{ssec:scaling_eval}

In this section, we evaluate how array voltage scaling (\ssecref{avs}) affects
the system energy consumption and application performance \fix{of our homogeneous workloads} at different \varr
values. We split our discussion into two parts: the results for \fix{memory-intensive}
workloads (i.e., applications where MPKI \fix{$\geq$} 15 for each core), and the results
for \fix{non-memory-intensive} workloads.

%\paratitle{Memory-Intensive Workloads} \figref{vsweep_high_mpki} shows the
%system performance (WS) loss, DRAM energy reduction, and system energy reduction,
%compared to a baseline DRAM with 1.35V, when we vary \varr from 1.30V to 0.90V.
%We make three observations from these results.

\paratitle{Memory-Intensive Workloads} \figref{vsweep_high_mpki} shows the
system performance (WS) loss, DRAM power reduction, and system energy reduction,
compared to a baseline DRAM with 1.35V, when we vary \varr from 1.30V to 0.90V.
We make three observations from these results.

\input{sections/subplots/vsweep_high_mpki}

%%%%%%%% All benchmarks results %%%%%%%%%%%%%
%%%%%%\input{sections/subplots/vsweep}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First, system performance loss \fixIII{increases} as we lower \varr, due to the increased
DRAM access latency. However, different workloads \fix{experience} a different
rate of performance loss, as they tolerate memory latency differently. Among the
\fix{memory-intensive} workloads, \emph{mcf} exhibits the lowest performance
degradation since it has the highest memory intensity and \fix{high memory-level
  parallelism}, leading to high queuing delays in the memory controller. The
queuing delays \fix{and memory-level parallelism} hide the longer DRAM access
latency \fix{more than in other workloads}. Other workloads lose more
performance because they are \fixIII{less able to tolerate/hide the} increased latency. Therefore,
workloads with very high memory intensity \fix{and memory-level parallelism can
  be less sensitive} to the increased memory latency.

%more sensitive to memory bandwidth than to latency~\cite{kim-micro2010}.

Second, DRAM power savings increase with lower \varr since reducing the DRAM
array voltage decreases \emph{both} the dynamic and static power components of
DRAM. \fix{However, \emph{system} energy savings does \fixIII{\emph{not}}
  monotonically increase with lower \varr.} We find that using $V_{array}$=0.9V
\fix{provides} lower system energy savings than \fixIV{using} $V_{array}$=1.0V,
as the processor takes \emph{much longer} to run the applications \fixIV{at
  $V_{array}$=0.9V}. In this case, the increase in static DRAM and CPU energy
\fix{outweighs} the dynamic DRAM energy savings.

%Second, DRAM energy savings increase as we lower \varr until 1.0V for most
%workloads, since reducing the DRAM array voltage lowers \emph{both} the dynamic
%and static energy components of DRAM.
%%While the DRAM power continues to reduce the energy does not
%We find that using $V_{array}$=0.9V \fix{provides} lower energy savings than
%$V_{array}$=1.0V, as the processor takes \emph{much longer} to run the
%applications. In this case, the increase in static DRAM energy \fix{outweighs}
%the dynamic DRAM energy savings. We demonstrate that reducing \varr provides
%a DRAM energy reduction of 11.5\%, averaged across memory-intensive
%workloads, when $V_{array}$=1.1V, which causes a performance loss of only 5.8\%.

Third, \fix{reducing \varr leads to a system energy reduction only when} the
reduction in DRAM energy outweighs the increase \fixVI{in} CPU energy (due to the
longer execution time). For \varr=1.1V, the system energy reduces by an average
of 7.6\%. Therefore, we conclude that array voltage scaling is an effective
technique that improves system energy consumption, with a small performance
loss, for \fix{memory-intensive} workloads.

% MCF breakdown
%To show the source of the energy savings, we break down the DRAM
%and CPU energy consumption for \emph{mcf} in \figref{mcf_breakdown}. The results
%show that the DRAM energy reduction is much greater than the increase in CPU
%energy. For example, the CPU leakage energy increases by only 3\% when \varr
%drops 1.35V to 1.0V, due to the 5\% system performance loss.
%\figputHWL{powerbreakdown/power_breakdown_vsweep_mcf}{Energy breakdown for \emph{mcf} with array voltage scaling.}{mcf_breakdown}

%AVG 1.0V sys e savings 8.8\%
%stop reach: AVG 1.0V sys e savings 7.6\%
%Voltron - 5\% loss %8.6\% %stop reach: 7.2\%

\paratitle{\fix{Non-Memory-Intensive} Workloads} \label{ssec:comp}
\tabref{non_mem_intensive_results} summarizes the \fixIV{system performance
  loss} and energy savings of 20 \fix{non-memory-intensive} workloads as \varr
varies from 1.30V to 0.90V, over the performance and energy consumption under a
nominal \varr of 1.35V. Compared to the \fix{memory-intensive} workloads,
\fix{non-memory-intensive} workloads \fixIV{obtain} smaller system energy
savings, as the system energy is dominated by the processor. Although the
workloads are more compute-intensive, lowering \varr \emph{does} reduce their
system energy consumption, by decreasing the energy consumption of DRAM. For
example, at 1.2V, array voltage scaling achieves an overall system energy
savings of 2.5\% with a performance loss of only 1.4\%.

% Prior version that shows the DRAM energy consumption
%\tabref{non_mem_intensive_results} summarizes the performance and energy savings
%of 20 memory non-intensive workloads as \varr varies from 1.30V to 0.90V, over
%the performance and energy consumption under a nominal \varr of 1.35V. Compared
%to the memory-intensive workloads, memory non-intensive workloads show smaller
%system energy savings, as the system energy is dominated by the processor.
%Although the workloads are more compute-intensive, lowering \varr \emph{does}
%reduce their system energy consumption, mainly by decreasing the static energy
%consumption of DRAM. For example, at 1.2V, array voltage scaling achieves an
%overall system energy savings of 2.5\% with a performance loss of only 1.4\%.

% \vspace{-0.1in}
\input{sections/tables/non_mem_intensive}
% \vspace{-0.12in}

% ===  Final version ===
\subsection{Effect of Performance-Aware Voltage Control}
\label{ssec:pavc_eval}

In this section, we evaluate the effectiveness of \fix{our complete proposal for Voltron,
which incorporates} \fixIII{our} \emph{performance-aware voltage control} mechanism
\fixIII{to drive the array voltage scaling component intelligently}. The \fixIII{performance-aware voltage control}
mechanism selects the lowest voltage level that satisfies the performance loss
bound (provided by the user or system designer) based on our performance model
(see \ssecref{pavc}). We evaluate \voltron with a target performance loss of
5\%. \voltron executes the performance-aware voltage control mechanism once
every four million cycles.\footnote{\fix{We evaluate the sensitivity to the \fixIII{frequency} at
  which we execute the mechanism (i.e., the interval \fix{length} of Voltron) in
  \ssecref{interval}.}} We quantitatively
compare Voltron \fixIV{to} \textit{\memdvfs}, a dynamic DRAM frequency and voltage
scaling mechanism proposed by prior work~\cite{david-icac2011}, which we
describe in \ssecref{dvfs}. Similar to the configuration used in the prior work,
we enable \memdvfs to switch dynamically between three frequency steps: 1600,
1333, and 1066 MT/s, which employ \fix{supply voltages of} 1.35V, 1.3V, and 1.25V, respectively.

\figref{memdvfs} shows the system performance (WS) loss, DRAM power savings, and
system energy savings due to \memdvfs and \voltron, compared to a baseline DRAM
with \fix{a supply voltage of} 1.35V. We show one graph per metric, where each graph uses boxplots to show
the distribution among all workloads. \fix{In each graph, we categorize the workloads as}
%low or high memory intensity.
\fixV{either non-memory-intensive or memory-intensive}.
Each box illustrates the quartiles of the population, and the
whiskers indicate the minimum and maximum values. The red dot indicates the
mean. We make four major observations.

\input{sections/subplots/voltron_memdvfs}

First, \fix{as shown in \figref{volt_vs_mem_perf}}, \voltron consistently
selects a \varr value that satisfies the performance loss bound of 5\% across
all workloads. \voltron incurs \fix{ an average (maximum) performance loss of 2.5\% (4.4\%) and 2.9\% (4.1\%)}
%for \fixIV{low- and high-memory-intensity} workloads,
for \fixV{non-memory-intensive and memory-intensive} workloads,
respectively. This demonstrates that our performance model enables \voltron to
select a low voltage value that saves energy while bounding performance loss
based on the user's requirement. We evaluate \voltron with a range of different
performance targets in \ssecref{vary_perf_target}.

Second, \memdvfs has almost zero effect on \fixIV{memory-intensive} workloads.
This is because \memdvfs avoids scaling DRAM frequency \fix{(and hence voltage)}
when an application's memory bandwidth \fixIV{utilization} is above a fixed
threshold. Reducing the frequency can result in a large performance loss since
the \fixIV{memory-intensive} workloads require high data throughput. As
\fix{memory-intensive} applications have high memory bandwidth consumption that
easily exceeds the \fixIV{fixed} threshold \fixIV{used by \memdvfs}, \memdvfs
\emph{cannot} perform frequency and voltage scaling during most of the execution
time. These results are consistent with the results reported in
\memdvfs\cite{david-icac2011}. In contrast, \voltron reduces system energy
\fix{(shown in \figref{volt_vs_mem_syse})} by 7.0\% on average for
\fix{memory-intensive} workloads, at the cost of 2.9\% system performance loss,
which is well within the specified performance loss target of 5\% \fix{(shown in
  \figref{volt_vs_mem_perf})}.

Third, both \memdvfs and \voltron reduce the average system energy consumption
for \fix{non-memory-intensive} workloads. \memdvfs reduces system energy by
dynamically scaling the frequency and voltage of DRAM, which lowers the DRAM
power consumption \fix{(as shown in \figref{volt_vs_mem_dpow})}. By reducing the
DRAM array voltage to a lower value than \memdvfs, \voltron is able to provide a
slightly higher DRAM power and system energy reduction \fix{for
  \fix{non-memory-intensive} workloads} \fixIV{than \memdvfs}.

Fourth, although \voltron reduces the system energy with a small performance
loss, the average system energy efficiency, in terms of \emph{performance per
  watt} (not shown in the figure), still improves by 3.3\% and 7.4\% for
%high- and \fixIV{low-memory-intensity} workloads,
\fixIV{\mbox{non-memory-intensive} and memory-intensive} workloads, respectively, over
the baseline. \fix{Thus, we} demonstrate that \voltron is an effective mechanism
that improves \fixIV{system} energy efficiency not only on
\fix{non-memory-intensive} applications, but also \fixIV{(especially)} on
\fix{memory-intensive} workloads where prior work was unable to do so.

\fix{To summarize, across \fixIV{non-memory-intensive and memory-intensive}
  workloads, Voltron reduces the average system energy consumption by 3.2\% and
  7.0\% while limiting average system performance loss to only 2.5\% and 2.9\%,
  respectively.  Voltron ensures that no workload loses performance by more than
  the specified target of 5\%. We conclude that Voltron is an effective DRAM
  \fixIV{and system} energy reduction mechanism that significantly outperforms
  prior memory DVFS mechanisms.}

\fix{
\subsection{\fixIII{System Energy Breakdown}}
\label{ssec:energy_breakdown}

To demonstrate the source of energy savings from Voltron, \figref{breakdown}
compares the system energy breakdown of Voltron to the baseline\fix{, which}
operates at the nominal voltage level \fix{of 1.35V}. The breakdown shows the
average CPU and DRAM energy consumption across workloads\fix{, which} are
categorized into \fixIV{non-memory-intensive and memory-intensive workloads}.
%low and high memory intensity.
We make \fix{two observations from the figure}.

\figputHSL{powerbreakdown/power_breakdown_voltron_vs_baseline}{0.31}{breakdown}{Breakdown of system energy consumption (lower is better).}

First, in the \fixIV{non-memory-intensive} workloads, \fix{the} CPU consumes an
average of 80\% of the total system energy when \fix{the} DRAM uses the nominal
voltage level. As a result, Voltron has less potential \fix{to reduce} the
overall system energy \fix{as} it \fix{reduces \emph{only}} the DRAM energy,
which \fix{makes up only} 20\% of the \fix{total} system energy. Second, DRAM
consumes an average of 53\% of the total system energy in the
\fix{memory-intensive} workloads.  \fixIII{As a result, Voltron has a larger
  room for potential improvement for memory-intensive workloads than for}
\fix{non-memory-intensive} workloads. Across the \fix{memory-intensive}
workloads, Voltron reduces the average dynamic and static DRAM energy by 14\%
and 11\%, respectively. However, Voltron increases the CPU energy consumption by
1.7\%, because \fix{the application} incurs a small system performance
degradation (due to \fix{the} increased \fix{memory} access latency), which is
within \fix{our 5\%} performance loss target (as shown in \ssecref{pavc_eval}).
\fixIV{We conclude that Voltron is effective in reducing DRAM energy, and it is
  an effective system energy reduction mechanism, especially when DRAM is a
  major consumer of energy in the system.} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Evaluation results on Voltron's control policy
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  ====== Submission Writing ========
%\subsection{Effect of Performance-Aware Voltage Control}
%\label{ssec:pavc_eval}
%
%In this section, we evaluate the effectiveness of the full mechanisms of
%\voltron by using our performance-aware voltage control mechanism, which selects
%the lowest voltage level that satisfies the performance loss bound (provided by
%the user or system designer) based on our performance model (see
%\ssecref{pavc}). \changes{We compare \voltron to an oracle policy
%  (\emph{Oracle}) that always chooses the \emph{exact minimum} voltage that
%  satisfies the performance loss bound for each workload.} We set the maximum
%allowable performance loss to 5\%. \figref{voltron} shows the performance loss,
%DRAM energy savings, and system energy savings of \emph{\voltron} and
%\emph{Oracle}. We make two major observations.
%
%\input{sections/subplots/voltron}
%
%First, \emph{\voltron} consistently selects a \varr value that satisfies the
%performance loss bound across all workloads. On average, \emph{\voltron} and
%\emph{Oracle} result in 2.8\% and 3.4\% performance degradation, respectively.
%\emph{Oracle} incurs a higher performance loss because it is able to select a
%lower voltage level than \emph{\voltron}, due to the approximate nature of the
%performance model used by \emph{\voltron}.
%
%Second, \emph{\voltron} enables both DRAM and system energy savings by finding a
%suitable low voltage value. \emph{\voltron} reduces the average DRAM and system
%energy consumption by 13.0\% and 4.4\% (up to 26.5\% and 12.6\%), respectively.
%On the other hand, \emph{Oracle} provides additional DRAM and system energy
%reduction over \emph{\voltron} by only 1.5\% and 0.5\%, respectively. This
%demonstrates that our performance model enables \emph{\voltron} to capture most
%of the energy savings of the \emph{Oracle}.
%
%Third, \voltron enables system energy savings for both memory intensive and
%non-intensive workloads. \emph{\voltron} reduces the average system energy
%consumption of memory-intensive/non-intensive workloads by 7.4\%/3.3\%, with
%only a 3.5\%/2.6\% system performance loss. Memory-intensive workloads attains
%higher system energy savings (by 2.2x) because they have higher tolerance to
%increased memory latency, thus allowing lower array voltage while still
%satisfying the performance loss bound. We conclude that that \emph{\voltron} is
%an effective mechanism that improves both DRAM and system energy efficiency with
%minimal performance degradation by intelligently reducing the DRAM array
%voltage.


==> sec/voltron_final/tables/ecc.tex <==
\begin{table}[h]
%\reftiny
  \centering
    \setlength{\tabcolsep}{.65em}
    \begin{tabular}{ccrrrrr}
        \toprule
        \multirow{2}{3em}{\centering Vendor} & \multirow{2}{5em}{\centering Correctable Timing} & \multicolumn{5}{c}{Voltage}  \\
        \cmidrule(lr){3-7}
        & & 1.05 & 1.075 & 1.1 & 1.125 & 1.15  \\
        \midrule
        \multirow{3}{3em}{\centering A \\ \tiny 10 DIMMs \quad}
         & tRCD & - & - & 1/1 & - & - \\
         & tRP & - & - & - & - & - \\

        \cmidrule(lr){1-7}
        \multirow{3}{3em}{\centering B \\ \tiny 12 DIMMs \quad}
         & tRCD & 2/5 & 3/5 & 1/1 & 0 & 0 \\
         & tRP & 2/5 & 6/7 & 2/5 & 0/1 & - \\

        \cmidrule(lr){1-7}
        \multirow{3}{3em}{\centering C \\ \tiny 9 DIMMs \qquad}
         & tRCD & 0 & 0 & 0 & 3/4 & 3/3 \\
         & tRP & - & - & 0/1 & 0/5 & 0/5 \\
        \bottomrule
    \end{tabular}

  \caption{Performance results of memory non-intensive workloads with different
  \varr values.}
  \label{tab:non_mem_intensive_results}
\end{table}


==> sec/voltron_final/tables/motivation_freq_scaling.tex <==
\begin{table}[h]
%\reftiny
  \centering
    \setlength{\tabcolsep}{.35em}
    \begin{tabular}{ccccc}
        \toprule
        Workload & Speedup & Bandwidth & DRAM Energy & System Energy \\
        \midrule
        \emph{mcf} & \textbf{-19\%} & -20\% & -11\% & -2\% \\
        \emph{perl} & -2\% & -2\% & \textbf{-30\%} & -2\% \\
        \bottomrule
    \end{tabular}
  \caption{Workload behavior when the channel frequency reduces by half from
    1600 MT/s to 800 MT/s.}
  \label{tab:motivation}
\end{table}


==> sec/voltron_final/tables/mwork.tex <==
\definecolor{lightgray}{gray}{0.95}

\begin{table*}[h]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing}
\\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\bottomrule
\end{tabular}
%\input{tbl/module_legend}
%\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em A} (sorted by manufacturing date)}
%\label{tbl:vendor1}
\end{table*}

\ignore{
\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering \mycolorii{Vulnerability Ratio}$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule

%% MICRON
\cellcolor{white} & \module{B}{ 1}{} & 10-09 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 2}{} & 10-22 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 3}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 4}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 5}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 6}{} & 11-26 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 7}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.1  & --   \\
\cellcolor{white} & \module{B}{ 8}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 479  & --   \\
\cellcolor{white} & \module{B}{ 9}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 1.9  & --   \\
\cellcolor{white} & \module{B}{10}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 4.3  & --   \\
\cellcolor{white} & \module{B}{11}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 161  & --   \\
\cellcolor{white} & \module{B}{12}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.3  & --   \\
\cellcolor{white} & \module{B}{13}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 16.0 & --   \\
\cellcolor{white} & \module{B}{14}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 8.6  & --   \\
\cellcolor{white} & \module{B}{15}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{B}{16}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{B}{17}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{18}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{19}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{20}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{21}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 4.3  & 11.4 \\
\cellcolor{white} & \module{B}{22}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 472  & --   \\
\cellcolor{white} & \module{B}{23}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 279  & --   \\
\cellcolor{white} & \module{B}{24}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 3276 & --   \\
\cellcolor{white} & \module{B}{25}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{B}{26}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{B}{27}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{28}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 78.3 & 8.2  \\
\cellcolor{white} & \module{B}{29}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 23.4 & 5.8  \\
\multirow{-32}{5em}{\centering {\large\em B} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{B}{30}{} & 14-09 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\bottomrule
\end{tabular}

\input{tbl/module_legend}

\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em B} (sorted by manufacturing date)}
\label{tbl:vendor2}
\end{table*}


\newpage

\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering \mycolor{Vulnerability Ratio}$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule


%% SAMSUNG
\cellcolor{white} & \module{C}{ 1}{} & 08-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 2}{} & 09-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{E}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 3}{} & 10-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 4}{} & 11-16 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 5}{} & 11-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 6}{} & 11-25 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 7}{} & 11-37 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 2.6  \\
\cellcolor{white} & \module{C}{ 8}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 32.9 \\
\cellcolor{white} & \module{C}{ 9}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 42.3 \\
\cellcolor{white} & \module{C}{10}{} & 11-49 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{11}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 104  \\
\cellcolor{white} & \module{C}{12}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 117  \\
\cellcolor{white} & \module{C}{13}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 291  \\
\cellcolor{white} & \module{C}{14}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{15}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 97.0 \\
\cellcolor{white} & \module{C}{16}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 493  \\
\cellcolor{white} & \module{C}{17}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 61.8 \\
\cellcolor{white} & \module{C}{18}{} & 12-25 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.2  & 3.3  \\
\cellcolor{white} & \module{C}{19}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 473  & 3.1  \\
\cellcolor{white} & \module{C}{20}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 5.4  & 2.7  \\
\cellcolor{white} & \module{C}{21}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 3.5  & 3.0  \\
\cellcolor{white} & \module{C}{22}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 545  & 3.0  \\
\cellcolor{white} & \module{C}{23}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.7  & 3.0  \\
\cellcolor{white} & \module{C}{24}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 27.2 & 2.9  \\
\cellcolor{white} & \module{C}{25}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.3  \\
\cellcolor{white} & \module{C}{26}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 54.2 & 19.1 \\
\cellcolor{white} & \module{C}{27}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.1  \\
\cellcolor{white} & \module{C}{28}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 29.0 & 5.4  \\
\cellcolor{white} & \module{C}{29}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 120  & 6.7  \\
\cellcolor{white} & \module{C}{30}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 196  & 3.2  \\
\cellcolor{white} & \module{C}{31}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 599  & 8.5  \\
\cellcolor{white} & \module{C}{32}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 51.6 & --   \\
\cellcolor{white} & \module{C}{33}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.5  \\
\cellcolor{white} & \module{C}{34}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.6  \\
\cellcolor{white} & \module{C}{35}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.6  \\
\multirow{-38}{5em}{\centering {\large\em C} \\ {\tiny \quad \\} \centering Total of \\ \centering 36 DIMMs}
\cellcolor{white} & \module{C}{36}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.9  \\
\bottomrule
\end{tabular}

\input{tbl/module_legend}

\caption{Sample Population of 36 DDR3 DIMMs from Vendor {\em C} (sorted by manufacturing date)}
\label{tbl:vendor3}

\end{table*}
}


==> sec/voltron_final/tables/test.tex <==
%\reftiny


==> sec/voltron_final/voltron.tex <==
% !TEX root=../paper.tex

\section{Voltron: Reducing DRAM Energy Without Sacrificing Memory Throughout}
\label{sec:varray}

\changes{Based on the extensive understanding we developed on reduced-voltage
operation of real DRAM chips in \secref{dram_exp}, we propose a new mechanism
called \emph{\voltron}, which reduces DRAM energy without sacrificing memory
throughput. \voltron exploits the fundamental observation that reducing the
supply voltage to DRAM requires increasing the latency of the three DRAM
operations in order to prevent errors. Using this observation, the key idea of
Voltron is to use a performance model to determine \fix{by how much to reduce
  the DRAM supply voltage}, without introducing errors and without exceeding a
user-specified threshold for performance loss. \voltron consists of two main
components: \myitem{i} \emph{array voltage scaling}, a hardware mechanism that
leverages our \fix{experimental observations} to scale \emph{only} the voltage supplied
to the DRAM array; and \myitem{ii} \emph{performance-aware voltage control},
\fixIII{a software} mechanism\footnote{\fixIV{Note that this mechanism can also
    be implemented in hardware, or as a cooperative hardware/software
    mechanism.}} that automatically chooses the minimum DRAM array voltage that
meets a \fixIV{user-specified} performance target.}

% Notes:
% power vs. energy
% varry scaling - still say power
% ** even though we reduce the power things take longer so the energy may not be
% lower.
% everything 5.2 should be on energy.

\subsection{Array Voltage Scaling}
\label{ssec:avs}

\changes{ As we discussed in \secref{dram_power}, the DRAM supply voltage to the
peripheral circuitry determines the maximum operating frequency. If we reduce
the supply voltage directly, the frequency needs to be lowered as well.
%the DRAM supply voltage, which is distributed to both the DRAM array and the
%peripheral circuitry, determines the maximum operating frequency since DRAM
%requires a minimum peripheral circuitry voltage to ensure stable operation at a
%certain frequency. If we reduce the supply voltage directly, the frequency
%needs to be lowered as well.
As more applications become more sensitive to memory bandwidth, reducing DRAM
frequency can result in a substantial performance loss due to lower data
throughput. In particular, we find that reducing the DRAM frequency from 1600
MT/s to 1066 MT/s significantly degrades performance of our evaluated
\fix{memory-intensive} applications by 16.1\%. Therefore, the design challenge
of \voltron is to reduce \fixIII{the} DRAM supply voltage \emph{without}
\fixIII{changing the} DRAM frequency.

To address this challenge, the key idea of Voltron's first component,
\emph{array voltage scaling}, is to reduce the voltage supplied to the
\emph{DRAM array} (\varr) \emph{without changing the voltage supplied to the
  peripheral circuitry}, thereby allowing the DRAM channel to maintain a high
frequency while reducing the power consumption of the DRAM array. To prevent
errors from occurring during reduced-voltage operation, \voltron increases the
latency of the three DRAM operations (activation, restoration, and precharge) in
every DRAM bank based on our observations in \secref{dram_exp}.

%\emph{Array voltage scaling} is built on top of our observations we make in
%\secref{dram_exp}.

By reducing \varr, we effectively reduce \myitem{i} the dynamic DRAM power on
activate, precharge, and refresh \fixIV{operations}; and \myitem{ii} the portion
of the static power that comes from the DRAM array. These power components
decrease \emph{quadratically} with the square of \fix{the} array voltage
reduction in a modern DRAM chip~\cite{keeth-dram-tutorial, baker-dram}. The
trade-off is that reducing \varr requires \fixIV{increasing} the latency of the
three DRAM operations, \fixIV{for reliable operation}, \fix{thereby} leading to
some system performance degradation, which we quantify in our evaluation
(\secref{eval}). }

%\todo{We dont want to adjust peri voltage b/c recall from background, peri.
%  voltage determines the maximum frequency. If we reduce the peri voltage, we
%  have to reduce frequency, which lowers data throughput, hurting apps with high
%  bandwidth demand.
%}
%1600 to 1333=16.7
%9.8\%
%1600 to 1066=33
%20.4\%

%Notably, we show that the latency of the three fundamental DRAM array
%operations does not correlate with the channel frequency, as each operation
%is a clock-independent analog operation that mainly depends on the
%cell capacitance, bitline capacitance, and voltage~\cite{keeth-dram-tutorial}
%(\ssecref{volt_sensitivity}).

\subsection{Performance-Aware Voltage Control}
\label{ssec:pavc}

%TODO:
%  high-level view of the mechanism
%we build a model and we use counter to tune the model.
%We use the model to find that doesn't harm predicted performance loss.
%Mention piece-wise linear model.
%mention performance loss predictor.

Array voltage scaling provides system users with the ability to decrease \varr
to reduce DRAM power. Employing a lower \varr provides greater power savings,
but at the cost of longer DRAM access latency, which leads to larger performance
degradation. This trade-off varies widely across different applications, as each
application has a different tolerance to the increased memory latency. This
raises the question of how to pick a ``suitable'' array voltage level for
different applications as a system user or designer. For this work, we say that
an array voltage level is suitable if it does not degrade system performance by
more than a user-specified threshold. Our goal is to provide a simple \fixIII{technique}
that can automatically select \fix{a} suitable \varr \fix{value} for
different applications. \changes{To this end, we propose
  \emph{performance-aware voltage control}, a \fix{power-performance} management
  policy that selects a minimum \varr that satisfies a desired performance
  constraint. The key observation is that an application's performance loss (due
  to increased memory latency) scales linearly with the application's memory
  \fix{demand \fixIII{(e.g., memory intensity)}.}
  Based on this \fixIV{empirical} observation \fixIV{we make}, we build a
  \emph{performance loss predictor} that leverages a linear model to predict an
  application's performance loss based on its characteristics at runtime. Using
  the performance loss predictor, Voltron finds a \varr that \fix{can keep the}
  predicted performance within a user-specified target at runtime. }

%build a
%linear model that predicts the performance loss based on the running
%application's characteristics, and
%
%the key idea is to leverage a linear model to predict the
%performance loss based on the running application's characteristics. We
%now describe the key observation that led to our design.

\paratitle{Key Observation} We find that an application's performance loss due
to higher latency has a strong linear relationship with its memory \fix{demand
  \fixIII{(e.g., memory intensity)}}. \figref{voltron_mot} shows the
relationship between the performance loss of each application \fix{(due to
  reduced voltage)} and its memory \fix{demand} under two different
\fix{reduced-voltage} values (see \ssecref{meth} for our methodology). Each data
point represents a single application. \fixIV{\figref{mpki}} shows each
application's performance loss versus its \emph{memory intensity}, expressed
using the commonly-used metric MPKI (last-level cache misses per
kilo-instruction). \fixIV{\figref{memstall}} shows \fix{each application's
  performance loss versus its \emph{memory stall time}}, the fraction of
execution time for which memory requests stall the CPU's \fixIV{instruction
  window}  (i.e., reorder buffer). In \fixIV{\figref{mpki}}, we
see that the performance loss is a \fix{\emph{piecewise linear function}} based
on the MPKI. The observation that an application's \emph{sensitivity to memory
  latency} is correlated with MPKI has also been \fixV{made} and utilized by prior
\fixIV{works~\cite{kim-hpca2010, kim-micro2010, mutlu-isca2008, zheng-icpp2008,
    mutlu-micro2007, muralidhara-micro2011, das-hpca2013, das-micro2009,
    usui-taco2016, zhao-micro2014, das-isca2010}.}

%\vspace{-0.1in}
\input{sections/subplots/voltron_motivation}
%\vspace{-0.1in}


When an application is \fix{\emph{not} memory-intensive} (i.e., \fixIV{has an} $MPKI < 15$), its performance
loss grows linearly with MPKI, becoming \emph{more sensitive} to memory latency.
\fix{ Latency-sensitive applications spend most of their time \fixIII{performing computation at the CPU cores} and
  issue memory requests infrequently. As a result, increasing the number of
  memory requests causes more stall cycles in the CPU. }
%in a wasted cycle that could have been spent on computation.
%This is because
%latency-sensitive applications spend most of their time at the CPU and every
%additional cycle stalling for memory results in a wasted cycle that could have
%been spent on computation.

On the other hand, the performance of \fix{memory-intensive} applications (i.e.,
\fixIV{those with} $MPKI \ge 15$) is \emph{less sensitive} to memory latency as
the MPKI grows. This is because \fix{memory-intensive} applications experience
frequent cache misses and spend a large portion of their time waiting on pending
memory requests. As a result, their rate of progress is significantly affected
by the memory bandwidth, \fix{and therefore they are more} \emph{sensitive to
  memory throughput} instead of latency. \fix{With more \fixIII{outstanding}
  memory requests (i.e., higher MPKI), the memory \fixIII{system} is more likely
  to service them in parallel, leading to more \emph{memory-level
    parallelism}\fixIII{~\cite{kim-micro2010,mutlu-isca2008,glew-asploswac98,
      mutlu-hpca2003, mutlu-ieeemicro2006, lee-micro2009}}. Therefore, improved
  memory-level parallelism enables applications to tolerate \fixIII{higher
    latencies} more easily.}


%Even if a single memory request is quickly serviced, subsequent
%  memory requests from the same memory-intensive application will quickly stall
%  the program execution.

\fixIV{\figref{memstall}} shows that an application's performance loss increases
with its \fixIV{instruction window (reorder buffer)} \emph{stall time
  \fixIV{fraction}} due to memory requests for both \fix{memory-intensive and
  non-memory-intensive} applications. \fix{A stalled \fixIV{instruction window}
  prevents the CPU from fetching or dispatching new
  instructions~\cite{mutlu-hpca2003}, thereby degrading the running
  application's performance.} This observation has also been \fixIII{made} and
utilized by prior
\fixV{works~\cite{ghose-isca2013,mutlu-ieeemicro2006,mutlu-isca2005,mutlu-hpca2003}}.



\paratitle{Performance Loss Predictor} Based on the observed linear
relationships \fixIV{between performance loss vs. MPKI and memory stall time
  fraction}, we use \emph{ordinary least squares (OLS)} regression to develop
a piecewise linear model for each application \fix{that can serve} as the performance loss
predictor for Voltron. Equation~\ref{eq:plm} shows the model, which takes the
following inputs: memory latency ($Latency=tRAS+tRP$), the application's MPKI, and
its memory stall time \fixIV{fraction}.

%%%%% LINEAR MODEL %%%%%
\vspace{-0.15in}
\begin{align}
    \mathrm{PredictedLoss}_{i} =
    \begin{cases}
        \label{eq:plm}
        \!\begin{aligned}
        &\alpha_{1} + \beta_{1}  \mathrm{Latency}_{i} + \beta_{2}
        \mathrm{App.MPKI}_{i} \\&+ \beta_{3}  \mathrm{App.StallTimeFraction}_{i} \\[1.5ex]
        \end{aligned} &\text{if } MPKI < 15 \\
        \!\begin{aligned}
        &\alpha_{2} + \beta_{4}  \mathrm{Latency}_{i} + \beta_{5}
        \mathrm{App.MPKI}_{i} \\&+ \beta_{6}  \mathrm{App.StallTimeFraction}_{i}
        \end{aligned} &\text{otherwise}
    \end{cases}
\end{align}
\vspace{-0.1in}
\begin{table}[h]
    \renewcommand{\arraystretch}{0.9}
    \centering
    \setlength{\tabcolsep}{.45em}
    \begin{tabular}{llll|llll}
        \toprule
        $\alpha_{1}$ & $\beta_{1}$ & $\beta_{2}$ & $\beta_{3}$  & $\alpha_{2}$ &
        $\beta_{4}$ & $\beta_{5}$ & $\beta_{6}$ \\
        \midrule
        -30.09 & 0.59 & 0.01 & 19.24 & -50.04 & 1.05 & -0.01 & 15.27 \\
        \bottomrule
    \end{tabular}
\end{table}
%\vspace{-0.1in}
%%%%% END LINEAR MODEL %%%%%

$\mathrm{PredictedLoss}_{i}$ is the predicted performance loss for the
application. The subscript $i$ refers to each data sample,
%which consists of a particular application's MPKI and stall time as measured
%under the nominal supply voltage, whereas the memory latency is a value
%associated with a specific voltage level.
\fixIV{which describes a particular application's characteristics (MPKI and
  memory stall time fraction) and the memory latency associated with the
  selected voltage level.} \fixIV{To generate the data samples, we run a total
  of 27 workloads across 8 different voltage levels that range from 1.35V to
  \fixVI{0.90V}, at a 50mV step (see \ssecref{meth} for our methodology). In total, we
  generate 216 data samples for finding the coefficients (i.e., $\alpha$ and
  $\beta$ values) in our model. To avoid overfitting the model, we use
  \fixIII{the \emph{scikit-learn} machine learning toolkit}~\cite{scikit} to
  perform cross-validation, which randomly splits the data samples into a
  training set (151 samples) and a test set (65 samples)}. To assess the fit of
the model, we use a common metric, root-mean-square error (RMSE), which is 2.8
and 2.5 for the low-MPKI and high-MPKI pieces of the model, respectively.
Furthermore, we calculate the R\textsuperscript{2} value to be 0.75 and 0.90 for
the low-MPKI and high-MPKI models, respectively. \fixV{Therefore, the RMSE and
R\textsuperscript{2} metrics
  indicate that our model provides high accuracy for predicting the performance
  loss of applications under different \varr values.}

\paratitle{Array Voltage Selection} Using the performance loss predictor,
\voltron selects the minimum value of \varr that satisfies the given user target
for performance loss. \fix{Algorithm~\ref{voltron} depicts the array voltage
  selection component of Voltron.} The voltage selection \fixIII{algorithm is
  executed} at periodic intervals throughout the runtime of an application.
During each interval, the application's memory \fix{demand} is profiled. At the
end of an interval, \voltron uses the profile to iteratively compare the
\fix{performance loss} target to the predicted performance loss incurred by each
voltage level, starting from a minimum value of 0.90V. Then, \voltron selects
the minimum \varr that \fixIV{does not exceed} the performance loss target and
\fixIII{uses} this selected \varr\fixIII{\ as the DRAM supply voltage} in the
subsequent interval. In our evaluation, we provide \voltron with a total of 10
voltage levels (every 0.05V step from 0.90V to 1.35V) for selection.

\fix{
\input{sections/algos/volt_select}
}

%We exclude voltage levels below 1.00V,
%as they provide diminished or negative energy benefits due to excessively long
%memory latency to maintain reliable operations without errors.

\subsection{Implementation}

\voltron's two components require modest modifications \fix{to} different parts of the
system. In order to support array voltage scaling, \voltron requires minor
changes to the power delivery network of DIMMs, as commercially-available DIMMs
currently \fixIII{use} a single supply voltage for both the DRAM array and \fixIII{the} peripheral
circuitry. Note that this supply voltage goes through \emph{separate} power
pins: $V_{DD}$ and $V_{DDQ}$ for the DRAM array and peripheral circuitry,
respectively, on a modern DRAM chip~\cite{micronDDR3L_2Gb}. Therefore, to enable
independent voltage adjustment, we propose to partition the power delivery
network on the DIMM into two domains: one domain to supply only the DRAM array
($V_{DD}$) and the other domain to supply only the peripheral circuitry
($V_{DDQ}$). %\todo{what's the overhead? 1-2 sentences.}

Performance-aware voltage control requires \myitem{i} performance monitoring
hardware that records the MPKI and memory stall time of each application; and
\myitem{ii} a control algorithm block, which predicts the performance loss at
different \varr values and accordingly selects the smallest acceptable \varr.
\voltron utilizes the performance counters that exist in most modern CPUs to
perform performance monitoring, thus requiring no additional hardware overhead.
\voltron reads these counter values and feeds them into the \fix{array voltage
  selection algorithm, which is} implemented in the system software layer.
\fix{Although reading the performance monitors has a small amount of software
  overhead, we believe the overhead is negligible because we do so only at the
  end of each interval \fixV{(i.e., every four million cycles in most of our
    evaluations; see sensitivity studies in \ssecref{interval})}.}

Voltron periodically executes this performance-aware voltage control
\fix{mechanism} during the runtime of the target application. During each time
interval, Voltron monitors the application's behavior through hardware counters.
At the end of an interval, the \fixIII{system software} \fix{executes the array
  voltage selection algorithm} to select the predicted \varr and
\fixIV{accordingly adjust} the timing parameters stored in the memory controller
for activation, restoration, and precharge. \fix{Note that there could be other
  (e.g., completely hardware-based) implementations of Voltron. We leave a
  detailed explanation of different implementations to future work.}

%Note that existing DIMMs do not support \emph{dynamic} voltage scaling, but
%requires a system reboot for the DIMMs to operate at a new voltage level.
%Therefore, in order to scaling voltage (whether it's \vdd or \varr), DIMMs would
%require a new voltage regulator design. However, scaling \varr has one advantage
%over \vdd scaling: scaling \varr avoids synchronization at the DLL, thereby
%shortening the transition time.
%
%Notes:
%Our current implementation has the profiled information of the applications
%during the representative phases. Discuss how to take care of phase changes.
%
%Then discuss hardware counters and varray voltage domain in dimm. Also can talk
%about letting the vendor to support this as part of tuning the vdd which can
%also help tune the clock frequency.
%
%We perform a simple selection based on the program's behavior during the
%representative phases. To address phase changes in programs, one can extend the
%existing model to apply it for every phase by monitoring and collecting these
%simple stats every epoch. This is out of the scope of our current work.


==> sty/macros_latvar.tex <==
% =============================================
%
% Lots of useful macros
%
% =============================================

\usepackage{ifthen}
\usepackage{calc}
\usepackage{pifont}
\usepackage{color}
\usepackage{xcolor}
\usepackage{fancyhdr}
\usepackage{tikz}

% Spacing b/w words
\newdimen\origiwspc%
\origiwspc=\fontdimen2\font% original inter word space

\newcommand{\squishlist} {
	\begin{list}{$\bullet$} {
		\setlength{\itemsep}{-2pt}
		\setlength{\parsep}{2pt}
		\setlength{\topsep}{0pt}
		\setlength{\partopsep}{0pt}
		\setlength{\leftmargin}{1.0em}
		\setlength{\labelwidth}{1em}
		\setlength{\labelsep}{0.5em}
	}
}
\newcommand{\squishend} {
	\end{list}
}

% =============================================
% Misc.
% =============================================

\newcounter{hours}
\newcounter{minutes}
\newcommand{\printtime}{%
  \setcounter{hours}{\time/60}%
  \setcounter{minutes}{\time-\value{hours}*60}%
  \thehours:\theminutes}
% Set timeofmake to 'true' to print the time the file was compiled
\newboolean{timeofmake}
\setboolean{timeofmake}{false}

\clubpenalty=10000
\widowpenalty=10000

% Compress itemize and enumerate environments.
\RequirePackage{enumerate}
\RequirePackage{enumitem}
\setlist{leftmargin=*, topsep=0pt, partopsep=0pt}
\addtolength{\itemsep}{-0.1in}

% Highlight
\def\HiLi{\leavevmode\rlap{\hbox to \hsize{\color{yellow!50}\leaders\hrule height .8\baselineskip depth .5ex\hfill}}}

% =============================================
% Comment macros
% =============================================

\newcommand{\ignore}[1]{}
\newcommand{\todo}[1]{{\color{red}TODO: \textbf{#1}}\xspace}
%\newcommand{\new}[1]{{\color{blue}#1}\xspace}
%\newcommand{\newt}[1]{{\color{red}#1}\xspace}
%\newcommand{\newthree}[1]{{\color{blue}#1}\xspace}
\newcommand{\new}[0]{}
\newcommand{\newt}[0]{}
\newcommand{\newthree}[0]{}

\newcommand{\dhl}[1]{{\color{blue} \textbf{Donghyuk: #1}}\xspace}
\newcommand{\kevin}[1]{{\color{brown} \textbf{Kevin: #1}}\xspace}
\newcommand{\sg}[1]{{\color{orange} \textbf{Saugata: #1}}\xspace}

% =============================================
% Insert # points
% =============================================

% (i), (ii), etc
\newcommand{\romnum}[1]{{\em (#1)}\xspace}

% =============================================
% Acronyms for DRAM commands and timings
% =============================================

% DIMM label
\newcommand{\dimm}[2]{$\texttt{D}^{#1}_{#2}$\xspace}

\newcommand{\patt}[1]{\texttt{#1}\xspace}

% Vendor
\newcommand{\vd}[1]{{{#1}}\xspace}

% begin observation
\newcounter{observation}
%\newcommand{\obs}[1]{\emph{\textbf{Observation~\theobservation:
%#1}}\xspace\stepcounter{observation}}

\newcommand{\obs}[1]{
    \refstepcounter{observation}%
    \textbf{Observation \theobservation:}~\textit{#1}}

\newenvironment{observation}[0]% environment name
{% begin code
    \par
    \refstepcounter{observation}%
    \textbf{Observation \theobservation:}
    \begin{itshape}%
    %\begin{bfseries}%
    }%
    {% end code
    %\end{bfseries}%
    \end{itshape}%
}
% end

% Mechanism
\newcommand{\mech}[0]{\mbox{FLY-DRAM}\xspace}
\newcommand{\mechlong}[0]{{Flexible-LatencY DRAM}\xspace}

% pattern
\newcommand{\pattzero}[0]{\texttt{{0x00}}\xspace}
\newcommand{\pattff}[0]{\texttt{0xff}\xspace}
\newcommand{\pattaa}[0]{\texttt{0xaa}\xspace}
\newcommand{\pattcc}[0]{\texttt{0xcc}\xspace}

% CMD
%\newcommand{\act}[0]{\texttt{{ACTIVATE}}\xspace}
%\newcommand{\acts}[0]{\texttt{{ACTIVATEs}}\xspace}
%\newcommand{\crd}[0]{\texttt{{READ}}\xspace}
%\newcommand{\cwr}[0]{\texttt{{WRITE}}\xspace}
%\newcommand{\cpre}[0]{\texttt{{PRECHARGE}}\xspace}

\newcommand{\act}[0]{\textsc{{activate}}\xspace}
\newcommand{\acts}[0]{\textsc{{activates}}\xspace}
\newcommand{\crd}[0]{\textsc{{read}}\xspace}
\newcommand{\cwr}[0]{\textsc{{write}}\xspace}
\newcommand{\cpre}[0]{\textsc{{precharge}}\xspace}

% Timing
\newcommand{\refab}[0]{{\texttt{$REF_{ab}$}}\xspace}
\newcommand{\refpb}[0]{{\texttt{$REF_{pb}$}}\xspace}
\newcommand{\trefi}[0]{{\texttt{$tREFI_{ab}$}}\xspace}
\newcommand{\trefipb}[0]{{\texttt{$tREFI_{pb}$}}\xspace}
\newcommand{\trfc}[0]{{\texttt{$tRFC_{ab}$}}\xspace}
\newcommand{\trfcpb}[0]{{\texttt{$tRFC_{pb}$}}\xspace}
\newcommand{\trc}[0]{{\texttt{tRC}}\xspace}

%\newcommand{\tras}[0]{{\texttt{tRAS}}\xspace}
%\newcommand{\trase}[0]{\texttt{tRAS}=}
\newcommand{\tras}[0]{{{\small t}\textsc{ras}}\xspace}
\newcommand{\trase}[0]{{{\small t}\textsc{ras}}=}

%\newcommand{\trp}[0]{{\texttt{tRP}}\xspace}
%\newcommand{\trpe}[0]{\texttt{tRP}=}
\newcommand{\trp}[0]{{{\small t}\textsc{rp}}\xspace}
\newcommand{\trpe}[0]{{{\small t}\textsc{rp}}=}

\newcommand{\trrd}[0]{{\texttt{tRRD}}\xspace}
\newcommand{\tfaw}[0]{{\texttt{tFAW}}\xspace}

%\newcommand{\trcd}[0]{{\texttt{\texttt{tRCD}}}\xspace}
%\newcommand{\trcde}[0]{\texttt{tRCD}=}
\newcommand{\trcd}[0]{{{\small t}\textsc{rcd}}\xspace}
\newcommand{\trcde}[0]{{{\small t}\textsc{rcd}}=}

%\newcommand{\tcl}[0]{{\texttt{tCL}}\xspace}
%\newcommand{\tcle}[0]{\texttt{tCL}=}
\newcommand{\tcl}[0]{{{\small t}\textsc{cl}}\xspace}
\newcommand{\tcle}[0]{{{\small t}\textsc{cl}}=}

%\newcommand{\tcwl}[0]{{\texttt{tCWL}}\xspace}
\newcommand{\tcwl}[0]{{{\small t}\textsc{cwl}}\xspace}
\newcommand{\tcwle}[0]{{{\small t}\textsc{cwl}}=}

\newcommand{\tccd}[0]{{\texttt{tCCD}}\xspace}
\newcommand{\trtw}[0]{{\texttt{tRTW}}\xspace}
\newcommand{\twr}[0]{{\texttt{tWR}}\xspace}
%\newcommand{\tbl}[0]{{{\small t}\textsc{bl}}\xspace}
%\newcommand{\tble}[0]{{{\small t}\textsc{bl}}=}

%\newcommand{\tbl}[0]{{\emph{BL}}\xspace}
%\newcommand{\tble}[0]{{\emph{BL}}=}
\newcommand{\tbl}[0]{{\textsc{bl}}\xspace}
\newcommand{\tble}[0]{{\textsc{bl}}=}

\newcommand{\putsec}[2]{\vspace{-0.05in}\section{#2}\label{sec:#1}\vspace{-0.075in}}
\newcommand{\putssec}[2]{\vspace{-0.05in}\subsection{#2}\label{ssec:#1}\vspace{-0.075in}}
\newcommand{\putsssec}[2]{\vspace{0.05in}\subsubsection{#2}\label{sssec:#1}\vspace{0.075in}}
\newcommand{\putsssecX}[1]{\vspace{0.0in}\subsubsection*{#1}\vspace{0.0in}}

\newcommand{\halfvdd}[0]{{$V_{DD}/2$}\xspace}
\newcommand{\halfdelta}[0]{{$V_{DD}/2+\Delta$}\xspace}
\newcommand{\vdd}[0]{{$V_{DD}$}\xspace}
\newcommand{\zerov}[0]{{$0$V}\xspace}

% Black-background circled text
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle,draw,inner sep=0.8pt,fill=black,text=white] (char)
{\textbf{#1}};}}

% =============================================
% Macros for referring to figs/secs/tabs etc
% =============================================
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\eq}[1]{Table~\ref{tab:#1}}
\newcommand{\refsec}[1]{\S\ref{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\ssecref}[1]{Section~\ref{ssec:#1}}
\newcommand{\sssecref}[1]{Section~\ref{sssec:#1}}


% =============================================
% Macros for inserting a figure
% =============================================
\newcommand{\figput}[4][1.0\linewidth]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#3, clip, width=#1]{plots/#2}
\end{center}
\caption{#4 \label{fig:#2}}
\end{minipage}
\end{figure}
}

\newcommand{\figputW}[2]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[clip,width=\linewidth]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputWS}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputH}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth, height=#2]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}


\newcommand{\figputTW}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#2}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHW}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#2}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGHW}[2]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGTW}[2]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHSTrim}[4]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#4,clip,scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHS}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputHSL}[4]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#4}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGHS}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}
\newcommand{\figputGTS}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGTWS}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/gnuplots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputTWS}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputTS}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputT}[2]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[clip, width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.1in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputTT}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#2, clip, width=1.0\linewidth]{plots/#1}
\end{center}
%\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputPlaceHolder}[2]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=0.8, width=1.0\linewidth]{plots/PlaceHolder}
\end{center}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}



==> sty/macros_ref.tex <==
\usepackage{ifthen}
\usepackage{calc}
\usepackage{pifont}
\usepackage{color}
\usepackage{fancyhdr}
\usepackage{tikz}

\newcounter{hours}
\newcounter{minutes}
\newcommand{\printtime}{%
  \setcounter{hours}{\time/60}%
  \setcounter{minutes}{\time-\value{hours}*60}%
  \thehours:\theminutes}

%%%%%%%%%%
% Alias
%%%%%%%%%%
% Set timeofmake to 'true' to print the time the file was compiled
\newboolean{timeofmake}
\setboolean{timeofmake}{false}

\newcommand{\ignore}[1]{}
\newcommand{\todo}[1]{{\color{red} \textbf{#1}}\xspace}
\newcommand{\dhl}[1]{{\color{blue} \textbf{Donghyuk: #1}}\xspace}
\newcommand{\kevin}[1]{{\color{brown} \textbf{Kevin: #1}}\xspace}

\newcommand{\intersub}[0]{{Subarray Access Refresh Parallelization}\xspace}
\newcommand{\Intersub}[0]{{Subarray Access Refresh Parallelization}\xspace}
\newcommand{\is}[0]{{\text{SARP}}\xspace}
\newcommand{\sarp}[0]{{\text{SARP}}\xspace}
\newcommand{\isab}[0]{{$\text{SARP}_{\text{ab}}$}\xspace}
\newcommand{\ispb}[0]{{$\text{SARP}_{\text{pb}}$}\xspace}
%\newcommand{\warp}[0]{{WRP}\xspace}
\newcommand{\warplongCap}[0]{{\mbox{Write-refresh} Parallelization}\xspace}
\newcommand{\warplong}[0]{{\mbox{write-refresh} parallelization}\xspace}
\newcommand{\Warplong}[0]{{\mbox{Write-refresh} parallelization}\xspace}
\newcommand{\darp}[0]{{DARP}\xspace}
\newcommand{\darplong}[0]{{Dynamic Access Refresh Parallelization}\xspace}
\newcommand{\Ooolong}[0]{{\mbox{Out-of-order} per-bank refresh}\xspace}
\newcommand{\ooolong}[0]{{\mbox{out-of-order} per-bank refresh}\xspace}
\newcommand{\ooolongCap}[0]{{\mbox{Out-of-order} Per-bank Refresh}\xspace}
\newcommand{\ib}[0]{{\darp}\xspace}
\newcommand{\emphintersub}[0]{{\emph{\intersub}}\xspace}
%\newcommand{\combo}[0]{{DARP+\ispb}\xspace}
\newcommand{\combo}[0]{{DSARP}\xspace}

\newcommand{\act}[0]{\texttt{\small{ACTIVATE}}\xspace}
\newcommand{\acts}[0]{\texttt{\small{ACTIVATEs}}\xspace}
\newcommand{\refab}[0]{{\small\emph{$REF_{ab}$}}\xspace}
\newcommand{\refpb}[0]{{\small\emph{$REF_{pb}$}}\xspace}
\newcommand{\trefi}[0]{{\small\emph{$tREFI_{ab}$}}\xspace}
\newcommand{\trefipb}[0]{{\small\emph{$tREFI_{pb}$}}\xspace}
\newcommand{\trfc}[0]{{\small\emph{$tRFC_{ab}$}}\xspace}
\newcommand{\trfcpb}[0]{{\small\emph{$tRFC_{pb}$}}\xspace}
\newcommand{\trc}[0]{{\small\emph{tRC}}\xspace}
\newcommand{\tras}[0]{{\small\emph{tRAS}}\xspace}
\newcommand{\trp}[0]{{\small\emph{tRP}}\xspace}
\newcommand{\trrd}[0]{{\small\emph{tRRD}}\xspace}
\newcommand{\tfaw}[0]{{\small\emph{tFAW}}\xspace}
\newcommand{\fgr}[0]{{\small\emph{FGR}}\xspace}

% For captions
\newcommand{\caprefab}[0]{\small{\textbf{\textit{REF\textsubscript{ab}}}}\xspace}
\newcommand{\caprefpb}[0]{\small{\textbf{\textit{REF\textsubscript{pb}}}}\xspace}
\newcommand{\captrfc}[0]{\small{\textbf{\textit{tRFC\textsubscript{ab}}}}\xspace}
\newcommand{\captrfcpb}[0]{\small{\textbf{\textit{tRFC\textsubscript{pb}}}}\xspace}
\newcommand{\captrefi}[0]{\small{\textbf{\textit{tREFI\textsubscript{ab}}}}\xspace}

\newcommand{\putsec}[2]{\vspace{-0.05in}\section{#2}\label{sec:#1}\vspace{-0.075in}}
\newcommand{\putssec}[2]{\vspace{-0.05in}\subsection{#2}\label{ssec:#1}\vspace{-0.075in}}
\newcommand{\putsssec}[2]{\vspace{0.05in}\subsubsection{#2}\label{sssec:#1}\vspace{0.075in}}
\newcommand{\putsssecX}[1]{\vspace{0.0in}\subsubsection*{#1}\vspace{0.0in}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.8pt,fill=black,text=white] (char) {#1};}}

\newcommand{\figput}[4][1.0\linewidth]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#3, clip, width=#1]{plots/#2}
\end{center}
\caption{#4 \label{fig:#2}}
\end{minipage}
\end{figure}
}

%\newcommand{\figputW}[4][1.0\linewidth]{
%\begin{figure*}[t]
%\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
%\begin{center}
%\includegraphics[trim=#3, clip, width=#1]{plots/#2}
%\end{center}
%\vspace{-0.2in}
%\caption{#4 \label{fig:#2}}
%\end{minipage}
%\end{figure*}
%}

\newcommand{\figputW}[2]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\begin{center}
\includegraphics[clip,width=\linewidth]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure*}
}

\newcommand{\figputH}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth, height=#2]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}
\newcommand{\figputHW}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}
\newcommand{\figputHS}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGHS}[3]{
\begin{figure}[h]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{gnuplots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputGTS}[3]{
\begin{figure*}[t]
\begin{minipage}{\linewidth}
%\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{gnuplots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure*}
}


\newcommand{\figputTS}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[scale=#2]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputT}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#2, clip, width=1.0\linewidth]{plots/#1}
%\includegraphics[trim=#2, clip, scale=0.75]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputTT}[3]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=#2, clip, width=1.0\linewidth]{plots/#1}
\end{center}
\vspace{-0.15in}
\caption{#3 \label{fig:#1}}
\end{minipage}
\end{figure}
}

\newcommand{\figputPlaceHolder}[2]{
\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize %also for forcing a baselinestretch update
\begin{center}
\includegraphics[trim=0in 5.5in 5.8in 0in, clip, width=1.0\linewidth]{plots/PlaceHolder.pdf}
\end{center}
\caption{#2 \label{fig:#1}}
\end{minipage}
\end{figure}
}

%\renewcommand{\figurename}{\renewcommand{\baselinestretch}{1.0}\vspace{-0.0in}\footnotesize\sf\bfseries Figure}
%\renewcommand{\tablename}{\renewcommand{\baselinestretch}{1.0}\vspace{-0.0in}\footnotesize\sf\bfseries Table}

\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\ssecref}[1]{Section~\ref{ssec:#1}}
\newcommand{\sssecref}[1]{Section~\ref{sssec:#1}}


